Efficient and Effective Similar Subtrajectory Search with Deep Reinforcement Learning

Similar trajectory search is a fundamental problem and has been well studied over the past two decades. However, the similar subtrajectory search (SimSub) problem, aiming to return a portion of a trajectory (i.e., a subtrajectory) which is the most similar to a query trajectory, has been mostly disregarded despite that it could capture trajectory similarity in a finer-grained way and many applications take subtrajectories as basic units for analysis. In this paper, we study the SimSub problem and develop a suite of algorithms including both exact and approximate ones. Among those approximate algorithms, two that are based on deep reinforcement learning stand out and outperform those non-learning based algorithms in terms of effectiveness and efficiency. We conduct experiments on real-world trajectory datasets, which verify the effectiveness and efficiency of the proposed algorithms.

==> bss.tex <==
\subsection{Backward Suffix Search (BSS)}
\label{ha:bss}
We observe that the high time cost of GA is mainly due to the suffix trajectory enumeration as shown in Figure~\ref{example:ga}. In particular, every time we get a new suffix trajectory via splitting, its representation needs to be computed from scratch. Motivated by this, we propose Backward Suffix Search (BBS), aiming at saving such computational cost. Before we describe the solution, we first give an intuition.
\begin{intuition}
\label{intu}
Given two trajectories $C$ and $Q$, we encode $C$ and $Q$ from left to right by $t2vec$ and get dissimilarity value $\Psi_{forward}$.
Similarly, we encode $C$ and $Q$ from right to left and get another dissimilarity value $\Psi_{backward}$. Intuitively, $\Psi_{forward}$ should be equal to $\Psi_{backward}$ because there is no changes in their relative positions.
\end{intuition}

To compute each suffix trajectory dissimilarity value $\Psi_{S}$ in GA, we have to encode the whole suffix trajectory in each time step. If the above intuition is correct, we can first get the representation vector $h_{\overleftarrow{Q}}$ for the reverse query trajectory $\overleftarrow{Q}$, and preprocess each backward hidden vector $h'$ for $\overleftarrow{C}$ by $t2vec$. In each time step, we compute the $\Psi_{S}$ by Euclidean distance between $h_{\overleftarrow{Q}}$ and $h'$.
%More details are presented in Algorithm~\ref{bss}. 
\textcolor[rgb]{1.00,0.00,0.00}{Note that if the returned subtrajectory $C_{\Lambda}$ is a suffix trajectory, which means that the similarity $\Psi$ is obtained by encoding trajectories in reverse, so we need to adjust it to a exact value by forward encoding according to the interval $\Lambda$, and we will use the value to evaluate algorithms in experiments.}

%\begin{algorithm}[t]
%	\caption{Backward Suffix Search}
%	\footnotesize{
%		\label{bss}
%		\begin{algorithmic}[1]
%			\Require
%			Candidate trajectory $C$ and query trajectory $Q$;
%			\Ensure
%			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
%            \State get representation vector $h_{Q}$ and $h_{\overleftarrow{Q}}$ for $Q$ and $\overleftarrow{Q}$;
%            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma,\Delta \leftarrow \emptyset$, $sp \leftarrow 1$ and $h_{0}, h'_{0} \leftarrow None$;
%            \For{each time step $1 \leq t \leq |C|$}
%                \State $h'_{t} = t2vec(h'_{t-1}, x_{|c|+1-t})$;
%            \EndFor
%			\For{each time step $1 \leq t \leq |C|$}
%                \State $\Gamma \leftarrow [sp, t]$, $\Delta \leftarrow [t+1, |C|]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$;
%                \State $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$, $\Psi_{S} \leftarrow d(h_{\overleftarrow{Q}}, h'_{|C|-t})$;
%                \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
%                    \If {$\Psi_{P} < \Psi_{S}$}
%                        \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                    \Else
%                        \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
%                    \EndIf
%                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$;
%                \EndIf
%			\EndFor
%            \State adjust $\Psi$ to a true dissimilarity value if $C_{\Lambda}$ is a suffix trajectory.
%	\end{algorithmic}}
%\end{algorithm}

\begin{lemma}
\label{tc:bss}
The total time complexity of BSS is $O(n)$.
\end{lemma}

\begin{proof}
\textcolor[rgb]{1.00,0.00,0.00}{Recall that the proofing of Lemma~\ref{lemma:ga}, BSS needs to preprocess each backward hidden vector $h'$ for $\overleftarrow{C}$, which is $O(n)$. After that, we only need to compute Euclidean distance between $h_{\overleftarrow{Q}}$ and corresponding $h'$, whose complexity is $O(1)$. The adjustment operation takes $O(n)$ time, as it needs to encode the suffix trajectory by $t2vec$. Hence, the overall time cost of BSS is $O(n)$.}
\end{proof}


==> dps.tex <==
\subsection{Delayed Prefix Search (DPS)}
\label{ha:dps}
We observe that PFS is involved in frequent splitting due to the lack of suffix information. In our Example~\ref{example_idea_pfs}, the splitting happens at $t=1$, $t=2$ and $t=4$ for a trajectory with only 4 points. Here, a straightforward idea is that when we find a subtrajectory, we let it wait for a few time steps $K$ and then split it out. In that case, we may find a better result. We illustrate the main idea in Example~\ref{example_idea_dps}.% and more details are presented in Algorithm~\ref{dps}.
\begin{example}
\label{example_idea_dps}
Consider a pair of candidate and query trajectory $C$, $Q$ in Figure~\ref{example:pfs}, where $t$ is the current time step and the target delayed time steps $K$ is set to 2 in this example.
\begin{itemize}[leftmargin=8pt]
  \item $t=1$, we initialize $sp$ as the current $t$, the current $delay$ as 0, the initial dissimilarity value $\Psi$ as infinity, the initial intervals $\Lambda, \Gamma$ as empty sets, and the first hidden state as none. We consider the prefix trajectory $C_{\Gamma=[1,1]}$. It is smaller than the initial dissimilarity value $\Psi$, but the current $delay$ has not reached the $K$. We skip and go to the next step.
  \item $t=2$, it gets a better dissimilarity value, but $delay$ has not reached the $K$ yet. We skip again.
  \item $t=3$, the $delay$ reaches the $K$ and gets a better result, so we split it at this time and maintain the prefix trajectory $C_{\Gamma=[1,3]}$. Then, $sp$ is updated.
  \item $t=4$, we delete the edge between 3 and 4 because a splitting happened in last time. We do not maintain $C_{\Gamma=[4,4]}$ because it is not better than current $C_{\Lambda=[1,3]}$. Hence, the final returned result is the subtrajectory with interval $\Lambda = [1,3]$.
\end{itemize}
\end{example}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/example_dps}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{An example illustrating the DPS.}\label{example:dps}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}

%\begin{algorithm}[t]
%	\caption{Delayed Prefix Search}
%	\footnotesize{
%		\label{dps}
%		\begin{algorithmic}[1]
%			\Require
%			Candidate trajectory $C$, query trajectory $Q$ and delayed steps $K$;
%			\Ensure
%			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
%            \State get representation vector $h_{Q}$ for query trajectory $Q$;
%            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma \leftarrow \emptyset$, $sp \leftarrow 1$, $h_{0} \leftarrow None$ and $delay \leftarrow 0$;
%			\For{each time step $1 \leq t \leq |C|$}
%                \State $\Gamma \leftarrow [sp, t]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$, $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$;
%                \If {$\Psi_{P} < \Psi$}
%                    \If{$delay = K$}
%                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$, $delay \leftarrow 0$;
%                    \Else
%                        \State $delay \leftarrow delay + 1$;
%                    \EndIf
%                \EndIf
%			\EndFor
%	\end{algorithmic}}
%\end{algorithm}

\begin{lemma}
The total time complexity of DPS is $O(n)$.
\end{lemma}
\begin{proof}
The delayed splitting does not cause additional calculations, so the proof is same as the PFS.
\end{proof}


==> efficiency.tex <==
%\subsection{Efficiency Evaluation}
%

\smallskip
\noindent\textbf{Scalability.} We can also evaluate the scalability of all the algorithms based on the results reported in Figure~\ref{fig:efficiencyRLS}(a)-(r). As can be seen, all the algorithms scale nearly linearly with the size of points in the database. We also observe that PSS, POS, POS-D, and RLS scales better than the other algorithms, such as ExactS, and the disparity between them with Exact becomes larger as the size of the dataset increases. For example, \textcolor[rgb]{1.00,0.00,0.00}{RLS is 10.4 times faster than ExactS. (zheng: the result in DTW and Frechet is around 10.4, in 2vec is around 7.6 times for all data size)
when the data size is 0.4 million, RLS is 10.4 times faster than ExactS; When the data size is 2 million, RLS is...
{\bf gao pls fill}}
%evaluate the scalability of all methods on Porto and Harbin datasets. As Figure~\ref{fig:efficiencyRLS}(a)-(r) suggested, the nearly linear scalability is obvious, and the
%performance gap between the exact algorithms and approximation algorithms tended to be bigger when the data size was increasing.

%\noindent\textbf{Comparison with datasets.} We observe similar performance on the two datasets Porto and Harbin. In addition, we know the average length of Harbin dataset (around 120) is bigger than Porto (around 60), and thus the corresponding time is also costly. For example, in terms of the results without index, when we increased the data size from 0.4 to 2.0 on Porto, Exact took from 3019 seconds to 13531 seconds for t2vec in Figure~\ref{fig:efficiencyRLS}(a), while it took from 3853 seconds to 18691 seconds on Harbin in Figure~\ref{fig:efficiencyRLS}(b).

%\noindent\textbf{Comparison with similarity measures.} DTW and Frechet are both point-matching based similarity measures and share a similar formulation, and therefore a similar performance and time cost are consistently under the different datasets and indexes. Regarding the t2vec, it is not very fast for the online scenario, because it needs to call deep learning model step by step on the incremental computing and resulting in some extra cost. For example in Figure~\ref{fig:efficiencyRLS}(a), (c) and (e), Exact with t2vec (3019 seconds to 13531 seconds) achieves only around $2-3\times$ speedup over DTW (5740 seconds to 27876 seconds) and Frechet (7024 seconds to 34383 seconds).

\smallskip \noindent\textbf{The effect of query length.} To evaluate the effect of query length on the accuracy of the proposed approximate algorithms, we group the query trajectories according to their lengths into four groups $G1=[30,45)$, $G2=[45,60)$, $G3=[60,75)$ and $G4=[75,90)$ and report the result of each group. The results on Porto and Harbin datasets with respect to t2vec,  DTW and Frechet are shown in Figure~\ref{fig:groupingRLS}.
%
%In terms of different similarity measures, we can see that DTW (g)-(l) and Frechet (m)-(r) are consistently similar under the three evaluation metrics AR, MR and RR because they are both point-matching based distance, and t2vec also shows consistent performance for Porto and Harbin.
%
We observe that the effectiveness of PSS, POS, POS-D, and RLS remains stable when the query length grows. However, the accuracy of SizeS fluctuates significantly with the change of the query length. This is because the length of the most similar subtrajectory may not have similar length as the query trajectory, and thus it may miss  better results since its search space is limited by the parameter $\xi$.
%

Figure~\ref{time:querylength} shows the effect of query length on the running time. We can see that for t2vec the running time of all the algorithms are almost not affected by query length. This is because we only need to represent the query trajectory into a vector once, which takes $O(m)$ time, and this has little impact on the running time. We observe that the running of all the algorithms increases linearly or super-linearly with the query length for DTW and Frechet, which is consistent with the time complexity result in Table~\ref{tab:algorithm-complexities}.

{\bf gao pls check.. i do not see the new figures}
\begin{figure}
\hspace*{-.5cm}
\centering
\begin{tabular}{c c c}
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/porto_t2vec_without}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/porto_dtw_without}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/porto_frechet_without}
  \end{minipage}
  \\
  \scriptsize (a) Porto (t2vec)
  &
  \scriptsize (b) Porto (DTW)
  &
  \scriptsize (c) Porto (Frechet)
 \\
  \end{tabular}
\caption{Efficiency of varying query lengths.}
\label{time:querylength}
\vspace*{-2mm}
\end{figure}


\smallskip
\noindent\textbf{Working with indexes.} Our proposed algorithms are able to work with indexes to further improve the efficiency of subtrajectory similarity search.
%We further study the effect of indexes for subtrajectory similarity search.
Following two recent studies~\cite{yao2019computing, wang2018torch} on trajectory similarity search, we employ the same indexing techniques for subtrajectory similarity search: Bounding Box R-tree Index and Grid-based Inverted Index. Note that we do not employ those indexing and prunning methods that are specially designed for a specific trajectory similarity measure as they cannot generalize to other similarity measures, or the scenario of subtrajectory similarlty search.
%
% bounded computations~\cite{rakthanmanon2012searching, keogh2005exact} are another acceleration method, which is achieved by estimating the lower bound for pruning; however, it cannot be guaranteed for our subtrajectory search and thus we do not use it in this experiment.
%
 Compared with the results without indexes in Figure~\ref{fig:efficiencyRLS}(a)-(f), the results using the R-tree index shown in Figure~\ref{fig:efficiencyRLS}(g)-(l) achieves around 10--20\% reduction in running time. The results based on the Inverted Index are shown in Figure~\ref{fig:efficiencyRLS}(m)-(r), and its speedup over the results without indexes is more significant, which is around 30 times.

 % because a huge number of maximum bounding rectangles (MBR) have an interaction relationship, and a simple grid index in Figure~\ref{fig:efficiencyRLS}(m)-(r) can be considered as a more useful index structure in such scenarios and it achieves around $30\times$ speedup.

\label{effi_evaluation}
\begin{figure*}
\hspace*{-.5cm}
\centering
\begin{tabular}{c c c c c c}
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_t2v_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_t2v_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_dtw_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_dtw_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_fre_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_fre_h}
  \end{minipage}
  \\
  \scriptsize (a) Porto (t2vec)
  &
  \scriptsize (b) Harbin (t2vec)
  &
  \scriptsize (c) Porto (DTW)
  &
  \scriptsize (d) Harbin (DTW)
  &
  \scriptsize (e) Porto (Frechet)
  &
  \scriptsize (f) Harbin (Frechet)
  \\

  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_t2v_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_t2v_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_dtw_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_dtw_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_fre_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_fre_h}
  \end{minipage}
  \\
  \scriptsize (g) Porto (t2vec)
  &
  \scriptsize (h) Harbin (t2vec)
  &
  \scriptsize (i) Porto (DTW)
  &
  \scriptsize (j) Harbin (DTW)
  &
  \scriptsize (k) Porto (Frechet)
  &
  \scriptsize (l) Harbin (Frechet)
  \\
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_t2v_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_t2v_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_dtw_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_dtw_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_fre_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_fre_h}
  \end{minipage}
  \\
  \scriptsize (m) Porto (t2vec)
  &
  \scriptsize (n) Harbin (t2vec)
  &
  \scriptsize (o) Porto (DTW)
  &
  \scriptsize (p) Harbin (DTW)
  &
  \scriptsize (q) Porto (Frechet)
  &
  \scriptsize (r) Harbin (Frechet)
  \end{tabular}
\caption{Results of efficiency evaluation without index (a)-(f), with R-tree index (g)-(l) and Inverted index (m)-(r).}
\label{fig:efficiencyRLS}
\vspace*{-2mm}
\end{figure*}


==> exact.tex <==
\section{THE EXACT ALGORITHM}
\label{section:exact}
Before introducing the exact algorithm, we give the following definitions and lemmas first.

\begin{definition}[Prefix Trajectory]
A trajectory $T_P = <s_1,s_2,..,s_{|T_P|}>$ is a prefix of a trajectory $T = <p_1,p_2,...,p_{|T|}>$, denoted by $T_P\preceq T$, if and only if $|T_P|\leq|T|$ and $\forall 1 \leq i \leq |T_P|, s_i = p_i$.
\end{definition}
For example, $T_P = <p_1,p_2>$ is a prefix of $T_1 = <p_1,p_2,p_3>$, but it is not a prefix of trajectory $T_2 = <p_1,p_3>$.

\begin{definition}[Suffix Trajectory]
A trajectory $T_S = <s_1,s_2,..,s_{|T_S|}>$ is a suffix of a trajectory $T = <p_1,p_2,...,p_{|T|}>$, denoted by $T_S\preceq T$, if and only if $|T_S|\leq|T|$ and $\forall 1 \leq i \leq |T_S|, s_i = p_{|T|-|T_S|+i}$.
\end{definition}
For example, $T_S = <p_2,p_3>$ is a suffix of $T_1 = <p_1,p_2,p_3>$, but it is not a suffix of trajectory $T_2 = <p_1,p_3>$.

\begin{lemma}
\label{lemma:subt}
Given a candidate trajectory $C$, any subtrajectory is a prefix trajectory of a suffix trajectory in $C$.
\end{lemma}
\begin{proof}
It can be easily proofed by the definition of subtrajectory. We denote $C_{\Lambda=[i,j]}$ is a subtrajectory that starts from index $i$ to index $j$, where $1 \leq i \leq j \leq |C|$. Any $C_{\Lambda=[i,j]}$ is a prefix trajectory of $C_{\Lambda=[i,|C|]}$ and $C_{\Lambda=[i,|C|]}$ is a suffix trajectory in $C$.
\end{proof}

\begin{lemma}
\label{lemma:t2vec}
The representation of prefix trajectories in a given trajectory can be computed in $O(n)$ time by $t2vec$, where $n$ is the length of the candidate trajectory~\footnote{In the rest of the paper, we will consistently use $n$ to refer to the length of the candidate trajectory.}.
\end{lemma}
\begin{proof}
Recall that in Section~\ref{pre:t2vec}, we explain as follows: (1) it takes $O(n)$ to convert a location sequence to its corresponding token sequence by the pretrained embedding layer, and each map operation from a location $p$ to its token vector $x$ is $O(1)$; (2) it takes roughly $O(n)$ time to scan the token sequence and fed the vectors $x$ to the GRU units. In each time step, we can get each prefix trajectory representation $h$. Hence, the overall time complexity is $O(n)$.
\end{proof}

The Lemma~\ref{lemma:subt} and Lemma~\ref{lemma:t2vec} suggest that in order to search an exact subtrajectory, we can enumerate each suffix trajectory in $C$, and then enumerate each prefix trajectory of the suffix trajectory. During the search process, we maintain a subtrajectory interval with the minimum dissimilarity value.

\begin{algorithm}[t]
	\caption{Exact Algorithm}
	\footnotesize{
		\label{exact}
		\begin{algorithmic}[1]
			\Require
			Candidate trajectory $C$ and query trajectory $Q$;
			\Ensure
			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
            \State get representation vector $h_{Q}$ for query trajectory $Q$;
            \State initialize $\Psi \leftarrow \infty$ and $\Lambda \leftarrow \emptyset$;
			\For{each time step $1 \leq t \leq |C|$}
                \State $h_{t-1} \leftarrow None$;
                    \For{each time step $t \leq t' \leq |C|$}
                        \State $h_{t'} \leftarrow t2vec(h_{t'-1}, x_{t'})$;
                        \If {$d(h_{Q}, h_{t'}) < \Psi$}
                            \State $\Psi \leftarrow d(h_{Q}, h_{t'})$, $\Lambda \leftarrow [t, t']$;
                        \EndIf
                    \EndFor
			\EndFor
	\end{algorithmic}}
\end{algorithm}

We present the details of the exact algorithm in Algorithm~\ref{exact}. It first gets the token sequence for the candidate trajectory $C$, which is used to enumerate each subtrajectory, and gets the representation $h_Q$ for query trajectory $Q$ (lines 1-2). Then, we initialize the optimal dissimilarity value $\Psi$ and the corresponding interval $\Lambda$ (line 3). Next, in the first for-loop, we enumerate each suffix trajectory of $C$ (lines 4-16), and enumerate each prefix trajectory of the suffix trajectory in the second for-loop (lines 6-11). Let $t2vec(\cdot,\cdot)$ denote the incremental computation by t2vec, the input is the last time hidden vector $h_{t-1}$ and current token vector $x_{t}$ (line 7). Note that it needs to initialize the first time hidden vector as $None$ (line 5). Finally, we need to maintain the best subtrajectory interval and the dissimilarity value during this process (lines 8-10), where $d(\cdot,\cdot)$ denotes the Euclidean distance between two vectors.

\begin{lemma}
The total time cost of the exact algorithm is $O(n^2)$.
\end{lemma}
\begin{proof}
It takes $O(n)$ time to generate the token sequence and the representation vector for the query trajectory. The first for-loop needs to be executed for $n$ times, and according to the Lemma~\ref{lemma:t2vec}, we know the time complexity of the second for-loop is $O(n)$. Note that in the second for-loop, the Euclidean distance computation is a constant which is obvious. Hence, the overall time cost is $O(n^2)$.
\end{proof}


==> fss.tex <==
\subsection{Double Model Search (DMS)}
\label{ha:fss}
Nevertheless, the Intuition~\ref{intu} might not be true in most cases. This is because $t2vec$ is an RNN-based similarity measure, which means that for the same trajectory, the representation vectors are not equal when we encode the trajectory forward and backward. A straightforward solution to solve this issue is to modify the model structure; however, we use the following two interesting lemmas to show that changing the model structure can guarantee the Intuition~\ref{intu} but it will lose the efficiency at the same time.

\begin{lemma}
\label{lemma:inte1}
A bidirectional RNN-based t2vec (bi-$t2vec$) can achieve $\Psi_{backward} = \Psi_{forward}$.
\end{lemma}
\begin{proof}
A bidirectional RNN~\cite{schuster1997bidirectional} contains two modules - a forward RNN and a backward RNN. Given two trajectories $C$ and $Q$, we denote $h_{f}^{C}$ is the final hidden state of the forward RNN for $C$, and $h_{b}^{C}$ is the final hidden state of the backward RNN for $C$. We concatenate the two hidden states $\big[h_{f}^{C}, h_{b}^{C}\big]^{\mathrm{T}}$ to represent trajectory $C$. Similarity, we have the trajectory $Q$ representation $\big[h_{f}^{Q}, h_{b}^{Q}\big]^{\mathrm{T}}$. Further, we have
\begin{equation}
  \Psi_{forward} =    \left\|\left[\begin{array}{c}
                        h_{f}^{C} \\
                        h_{b}^{C} \\
                      \end{array}\right] -
                             \left[\begin{array}{c}
                        h_{f}^{Q} \\
                        h_{b}^{Q} \\
                      \end{array}\right]
                      \right\|_{2}.
\end{equation}
For the reserve trajectories $\overleftarrow{C}$ and $\overleftarrow{Q}$, we know their representations are only the position exchange of hidden states, that is
$\big[h_{f}^{\overleftarrow{C}}, h_{b}^{\overleftarrow{C}}\big]^{\mathrm{T}} = \big[h_{b}^{C}, h_{f}^{C}\big]^{\mathrm{T}}$,
$\big[h_{f}^{\overleftarrow{Q}}, h_{b}^{\overleftarrow{Q}}\big]^{\mathrm{T}} = \big[h_{b}^{Q}, h_{f}^{Q}\big]^{\mathrm{T}}$. According to commutative law in Euclidean distance computation, we have
\begin{equation}
\begin{aligned}
  \Psi_{backward} & =    \left\|\left[\begin{array}{c}
                        h_{f}^{\overleftarrow{C}} \\
                        h_{b}^{\overleftarrow{C}} \\
                      \end{array}\right] - \left[\begin{array}{c}
                        h_{f}^{\overleftarrow{Q}} \\
                        h_{b}^{\overleftarrow{Q}} \\
                      \end{array}\right]\right\|_{2} = \left\|\left[\begin{array}{c}
                        h_{b}^{C} \\
                        h_{f}^{C} \\
                      \end{array}\right] -
                             \left[\begin{array}{c}
                        h_{b}^{Q} \\
                        h_{f}^{Q} \\
                      \end{array}\right]
                      \right\|_{2}\\
  & =                 \left\|\left[\begin{array}{c}
                        h_{f}^{C} \\
                        h_{b}^{C} \\
                      \end{array}\right] -
                             \left[\begin{array}{c}
                        h_{f}^{Q} \\
                        h_{b}^{Q} \\
                      \end{array}\right]
                      \right\|_{2} = \Psi_{forward}.
\end{aligned}
\end{equation}
Hence, Lemma~\ref{lemma:inte1} holds.
\end{proof}

\begin{lemma}
\label{lemma:inte2}
In each time step, the update computation by bi-$t2vec$ is $O(n)$.
\end{lemma}

\begin{proof}
Recall that in $t2vec$, we can get $h_{t}$ by inputting $h_{t-1}$ and $x_{t}$, the time cost is $O(1)$.
In bi-$t2vec$, the update time cost of forward hidden state $h_{f}$ is the same as $t2vec$ $O(1)$. However, for the backward hidden state $h_{b}$, the time complexity will increase to $O(n)$ because the starting point is changed, RNN needs to read the whole trajectory again to get current $h_{b}$.
\end{proof}
From the above lemmas, we observe that modifying the model structure is also difficult to decrease time complexity. Thus, we try to decouple the bidirectional model, and pretrain the backward RNN $\widehat{t2vec}$ to capture the reverse candidate and query trajectories as input. The output $\Psi_{backward}$ can be considered as a predicted value of $\Psi_{forward}$. We call this algorithm Double Model Search (DMS), the main idea is to approximate $\Psi_{forward}$ with less time cost. 
%More details are presented in Algorithm~\ref{fss}. 
Note that it also needs to adjust $\Psi$ if $C_{\Lambda}$ is obtained by a suffix trajectory.
%\begin{algorithm}[t]
%	\caption{Double Model Search}
%	\footnotesize{
%		\label{fss}
%		\begin{algorithmic}[1]
%			\Require
%			Candidate trajectory $C$, query trajectory $Q$;
%			\Ensure
%			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
%            \State get representation vector $h_{Q}$ for $Q$ by $t2vec$ and $h_{\overleftarrow{Q}}$ for $\overleftarrow{Q}$ by $\widehat{t2vec}$;
%            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma,\Delta \leftarrow \emptyset$, $sp \leftarrow 1$ and $h_{0}, h'_{0} \leftarrow None$;
%            \For{each time step $1 \leq t \leq |C|$}
%                \State $h'_{t} = \widehat{t2vec}(h'_{t-1}, x_{|c|+1-t})$;
%            \EndFor
%			\For{each time step $1 \leq t \leq |C|$}
%                \State $\Gamma \leftarrow [sp, t]$, $\Delta \leftarrow [t+1, |C|]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$;
%                \State $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$, $\Psi_{S} \leftarrow d(h_{\overleftarrow{Q}}, h'_{|C|-t})$;
%                \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
%                    \If {$\Psi_{P} < \Psi_{S}$}
%                        \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                    \Else
%                        \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
%                    \EndIf
%                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$;
%                \EndIf
%			\EndFor
%            \State adjust $\Psi$ to a true dissimilarity value if $C_{\Lambda}$ is a suffix trajectory.
%	\end{algorithmic}}
%\end{algorithm}

\begin{lemma}
The total time complexity of DMS is $O(n)$.
\end{lemma}
\begin{proof}
\textcolor[rgb]{1.00,0.00,0.00}{Based on Lemma~\ref{tc:bss}, it only uses another pretrained model $\widehat{t2vec}$ to receive reverse trajectories, so the proof is same as the BSS.}
\end{proof}


==> ga.tex <==
\section{HEURISTIC ALGORITHM}
\label{section:heuristic}
The quadratic time complexity makes the exact algorithm very time-consuming, and then we propose some heuristic algorithms to approximately get the similarity, which largely improve the efficiency. Section~\ref{ha:idea} presents the high-level idea of our proposed heuristic algorithms. Section~\ref{ha:ga} -~\ref{ha:dps} elaborates on some detailed designs.

\subsection{Trajectory Splitting}
\label{ha:idea}
The major limitation of the exact algorithm is its high computational cost, which makes it impractical for longer trajectories. To alleviate this issue, we model the computation of subtrajectory similarity as a trajectory splitting problem. The high-level idea is if we can scan the given trajectory one time and accurately split the best subtrajectory without enumerating each suffix trajectory as shown in the exact algorithm, then we can achieve more efficient search. However, a new issue is how can we achieve the exact splitting? In the rest of this section, we introduce the heuristic methods for trajectory splitting.

\subsection{Greedy Algorithm (GA)}
\label{ha:ga}
A straightforward solution to the trajectory splitting is the greedy algorithm. When we enumerate the points of a given trajectory $C$ from 1 to |C|, in each time step, we need to decide whether to split at this point or not. If a trajectory is decided to be split, it will generate a prefix trajectory and a suffix trajectory, whose intervals are represented by $\Gamma$ and $\Delta$. We define the range of $\Gamma$ and $\Delta$ as follows.
\begin{equation}
\label{interval}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\Gamma = [sp, t], \Delta = [t+1, |C|],
\end{aligned}
\end{equation}
where $sp$ denotes the index of the splitting point and it continues to update by splitting operation. $t$ is the current time step. Note that in our definition, the two intervals are non-overlapping. This is because our trajectory similarity via $t2vec$ depends on the token vector of each sampling point. The greedy algorithm always maintain the current best trajectory between $C_{\Gamma}$ and $C_{\Delta}$, so we need to perform a splitting if there is a better result occurs at this time. We illustrate the working process in Example~\ref{workingex:ga}.

\begin{example}
\label{workingex:ga}
Consider a pair of candidate and query trajectory $C$, $Q$ in Figure~\ref{example:ga}, where $t$ is the current time step.%~\footnote{We use dashed lines with arrows to label the prefix interval $\Gamma$ and suffix interval $\Delta$ for ease of reference. The solid lines with arrows indicate there is a splitting operation at this time step, and we label the maintaining interval $\Lambda$ with red color during this process.}.
\begin{itemize}[leftmargin=8pt]
  \item $t=1$, we initialize $sp$ as the current $t$, the initial dissimilarity value $\Psi$ as infinity, the initial intervals $\Lambda, \Gamma, \Delta$ as empty sets, and the first hidden state as none. We get two candidate subtrajectories $C_{\Gamma=[1,1]}$ and $C_{\Delta=[2,4]}$ according to Equation~\ref{interval}. we maintain the suffix $C_{\Delta=[2,4]}$ because it is more similar to $Q$ than $C_{\Gamma=[1,1]}$, and then we update $sp$ as the next time step.
  \item $t=2$, we delete the edge between 1 and 2 because a splitting operation happened in $t=1$. We do not need to maintain $C_{\Gamma=[2,2]}$ or $C_{\Delta=[3,4]}$ because neither of them is better than $C_{\Lambda=[2,4]}$.
  \item $t=3$, we get two subtrajectories $C_{\Gamma=[2,3]}$ and $C_{\Delta=[4,4]}$, we decide to maintain the prefix $C_{\Gamma=[2,3]}$ because it is more similar to $Q$ compared with $C_{\Lambda=[2,4]}$, and thus a splitting operation happened. Note that the current $sp=2$ and we update it as the next time step again.
  \item $t=4$, we delete the edge between 3 and 4 because a splitting operation happened in the last step, and the maintaining subtrajectory does not change. Note that in the final step, the suffix trajectory is none. The final result is the subtrajectory with interval $\Lambda = [2,3]$.
\end{itemize}
\end{example}
We present the corresponding idea in Algorithm~\ref{ga}.

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/example_ga}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{An example illustrating the GA. We use dashed lines with arrows to label the prefix interval $\Gamma$ and suffix interval $\Delta$ for ease of reference. The solid lines with arrows indicate there is a splitting operation at this time step, and we label the maintaining interval $\Lambda$ with red color during this process.}\label{example:ga}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}

\begin{algorithm}[t]
	\caption{Greedy Algorithm}
	\footnotesize{
		\label{ga}
		\begin{algorithmic}[1]
			\Require
			Candidate trajectory $C$ and query trajectory $Q$;
			\Ensure
			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
            \State get representation vector $h_{Q}$ for query trajectory $Q$;
            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma,\Delta \leftarrow \emptyset$, $sp \leftarrow 1$ and $h_{0} \leftarrow None$;
			\For{each time step $1 \leq t \leq |C|$}
                \State $\Gamma \leftarrow [sp, t]$, $\Delta \leftarrow [t+1, |C|]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$;
                \State get representation vector $h_{C_{\Delta}}$ for suffix trajectory $C_{\Delta}$;
                \State $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$, $\Psi_{S} \leftarrow d(h_{Q}, h_{C_{\Delta}})$;
                \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
                    \If {$\Psi_{P} < \Psi_{S}$}
                        \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
                    \Else
                        \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
                    \EndIf
                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$;
                \EndIf
			\EndFor
	\end{algorithmic}}
\end{algorithm}

\begin{lemma}
\label{lemma:ga}
The total time complexity of GA is $O(n^2)$.
\end{lemma}
\begin{proof}
In Algorithm~\ref{ga}, the for-loop needs to be executed for $n$ times (lines 4-16). In each time step, it needs to get representation vector $h_{C_{\Delta}}$ for suffix trajectory $C_{\Delta}$ (line 6), which is $O(n)$ because it needs to encode the whole suffix via t2vec. Note that for the prefix trajectory $C_{\Gamma}$, the update of $t2vec$ is $O(1)$ in each time step. Hence, the overall time cost is $O(n^2)$.
\end{proof}

Although we can see the computational cost of GA is also quadratic, it provides a good framework for trajectory splitting. In order to handle the issue, we further propose the following four algorithms based on GA.


==> instantiation.tex <==
\section{Similarity Measure}

\subsection{DTW and Frechet}
DTW~\cite{yi1998efficient} and Frechet~\cite{alt1995computing} are two of the most widely adopted trajectory similarity measures in temporal sequence analyses. Thus, we first use DTW and Frechet as examples to discuss the costs of $\Phi$, $\Phi_{ini}$ and $\Phi_{inc}$.

Given a data trajectory $T = <p_1, p_2,...,p_n>$ and a query trajectory $Q = <q_1, q_2,...,q_m>$, DTW is computed as below
\begin{equation}
\label{dtw_sm}
D_{n,m}=\left\{
\begin{aligned}
& \sum\nolimits_{i=1}^{n}d(p_i,q_1)&\text{if } m = 1\\
& \sum\nolimits_{j=1}^{m}d(p_1,q_j)&\text{if } n = 1\\
& d(p_n,q_m) + \\
& \min(D_{n-1,m-1}, D_{n-1,m},D_{n,m-1})&\text{otherwise}
\end{aligned}
\right.
\end{equation}
where $D_{n,m}$ denotes DTW distance between the prefix trajectory of $T$ with length $n$ and the prefix trajectory of $Q$ with length $m$, and $d(p_n,q_m)$ is a point-to-point distance (typically Euclidean distance with $O(1)$ time complexity) between $p_n$ and $q_m$. The time complexity of $\Phi$ can be easily observed from the Equation~\ref{dtw_sm} because it needs to compute all the pairwise point-matching distances, that is $O((n \cdot m) \cdot 1) = O(n \cdot m)$. Based on the general time complexity of $\Phi = O(n \cdot m)$, the $\Phi_{ini}$ can be considered as the data trajectory only has one point that is $n=1$, and thus $\Phi_{ini} = O(1 \cdot m) = O(m)$. For the incremental computation $\Phi_{inc}$, we can save the previous time step value $D_{t-1,m}$. If we want to update $D_{t,m}$ from $D_{t-1,m}$, firstly, we need to get $D_{t,1}$, which follows $D_{t,1}=D_{t-1,1}+d(p_t,q_1)$ according to the Equation~\ref{dtw_sm}. Then, we need to update $D_{t,i}$ for each time step $i$ from 2 to $m$ that is $D_{t,i}=d(p_{t},q_{i})+
min\big(D_{t-1,i-1},D_{t-1,i},D_{t,i-1}\big), 2\leq i\leq m$. In each time step, the computation is $O(1)$ and thus the total time complexity is completely related to the query length $m$ that is $O(1 + m - 1) = O(m)$.

Similarly, we have the same conclusion for the Frechet distance based on the Equation~\ref{fre_sm}.
\begin{equation}
\label{fre_sm}
F_{n,m}=\left\{
\begin{aligned}
&\max\nolimits_{i=1}^{n}d(p_i,q_1)&\text{if }m = 1\\
&\max\nolimits_{j=1}^{m}d(p_1,q_j)&\text{if }n = 1\\
&\max(d(p_n,q_m),\\
& \min(F_{n-1,m-1},F_{n-1,m},F_{n,m-1}))&\text{otherwise}
\end{aligned}
\right.
\end{equation}
where $F_{n,m}$ denotes the Frechet distance.

\subsection{t2vec}
t2vec~\cite{li2018deep} is a state-of-the-art trajectory similarity measure based on deep representation learning. It adapts the sequence encoder-decoder framework based on RNN~\cite{cho2014learning} to build learning model, and it takes the final hidden vector of the encoder~\cite{rumelhart1988learning} to represent a trajectory. Finally, t2vec computes the trajectory similarity between the Euclidean distance of hidden vectors.

Given a data trajectory with length $n$ and a query trajectory with length $m$, it takes $O(n)$ and $O(m)$ to get their hidden vectors and $O(1)$ to compute the Euclidean distance (Details are discussed in~\cite{li2018deep}.). And thus $\Phi = O(n + m + 1) = O(n + m)$. Note that t2vec is different from point-matching based similarity such DTW and Frechet, it can preprocess all of the hidden vectors of trajectories in database offline. Thus, $\Phi_{ini}$ is $O(1)$ because it only needs to input one point in the data trajectory to the model, the model computation based on RNN is $O(1)$, and the hidden vector of query is preprocessed offline. Similarly, the incremental computation $\Phi_{inc}$ is also $O(1)$ because we can save the previous hidden vector, and it takes $O(1)$ to update the current hidden vector from the model.




==> other.tex <==
\section{OTHER SIMILARITY MEASURES}
\label{section:other}
DTW~\cite{yi1998efficient} and Frechet~\cite{alt1995computing} are two of the most widely adopted trajectory similarity measures in temporal sequence analyses. Thus, in this section, we use DTW and Frechet as examples to show how to support other distance functions in our reinforcement learning framework.

\subsection{DTW Distance}
\begin{definition}[DTW Distance]
\label{dtw:definition}
Given a candidate trajectory $C = <p_1, p_2,...,p_n>$ and a query trajectory $Q = <q_1, q_2,...,q_m>$, DTW is computed as below
\begin{equation}
D_{n,m}=\left\{
\begin{aligned}
& \sum\nolimits_{i=1}^{n}d(p_i,q_1)&\text{if } m = 1\\
& \sum\nolimits_{j=1}^{m}d(p_1,q_j)&\text{if } n = 1\\
& d(p_n,q_m) + \\
& \min(D_{n-1,m-1}, D_{n-1,m},D_{n,m-1})&\text{otherwise}
\end{aligned}
\right.
\end{equation}
where $D_{n,m}$ denotes DTW distance between the prefix trajectory of $C$ with length $n$ and the prefix trajectory of $Q$ with length $m$, and $d(p_n,q_m)$ is a point-to-point distance (typically Euclidean distance) between $p_n$ and $q_m$.
\end{definition}
To support DTW in our reinforcement learning framework, the core is to update the trajectory dissimilarity value from the previous time step $D_{t-1,m}$ to the current value $D_{t,m}$. The update process is illustrated in Figure~\ref{fig:dtw}. We use the matrix $Mat$ to record DTW distances between each pairwise prefix trajectory similarity. If we want to update $D_{t,m}$ from $D_{t-1,m}$, firstly, we need to get $D_{t,1}$, which follows the equation $D_{t,1}=D_{t-1,1}+d(p_t,q_1)$ according to the Definition~\ref{dtw:definition}. Then, we need to update $D_{t,i}$ for each time step $i$ from 2 to $m$ that is $D_{t,i}=d(p_{t},q_{i})+
min\big(D_{t-1,i-1},D_{t-1,i},D_{t,i-1}\big), 2\leq i\leq m$. Let vector $\mathcal{V}_{t}$ denote the $t$-row of DTW matrix $Mat$, and thus we have the update equation as follows.
\begin{equation}\label{dtwupdate}
  \mathcal{V}_{t} = dtw(\mathcal{V}_{t-1}, p_{t}, Q), D_{t,m} = \mathcal{V}_{t,m},
\end{equation}
where $dtw(\cdot,\cdot,\cdot)$ is a update function as explained above, the input includes the given last time vector $\mathcal{V}_{t-1}$, the sampling point $p_t$ in the candidate trajectory $C$ and query trajectory $Q$, and the final element of $\mathcal{V}_{t}$ is our target dissimilarity value $D_{t,m}$. We analyze the time complexity of DTW update using Lemma~\ref{dtw_time}.
\begin{lemma}
\label{dtw_time}
The time complexity of DTW update is $O(m)$.
\end{lemma}
\begin{proof}
In Figure~\ref{fig:dtw}, it needs to update $D_{t,1}$ from $D_{t-1,1}$ and then update $D_{t,i}$ for $2 \leq i \leq m$ from its neighbors. In each time step, the computation is $O(1)$ and thus the total time complexity is $O(m)$, where $m$ is the length of query trajectory.
\end{proof}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/dtw}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{\small{Illustrating the DTW distance update.}}\label{fig:dtw}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}
Next, we show the online part of DTW subtrajectory search in Algorithm~\ref{algo:dtw}, which has a similar framework with $t2vec$. Note that the input $Q^*$ has been trained offline. In addition, DTW is a point-matching based method, so our Intuition~\ref{intu} can be guaranteed in this similarly measure (We proof it in Lemma~\ref{dtw_sim_nochange}.), and we can directly input reverse trajectories in order to achieve fast computation for suffix similarity $\Psi_S$. Further, we denote state $s = (\Psi, \Psi_{P}, \Psi_{S})$ because the $\Psi_S$ is an exact value now for DTW similarity.

\begin{lemma}
\label{dtw_sim_nochange}
The Intuition~\ref{intu} is correct for DTW distance.
\end{lemma}
\begin{proof}
Given two trajectories $C$ and $Q$
\begin{equation*}
  C = <p_1,...,p_i,...,p_n>, Q = <q_1,...,q_j,...,q_m>.
\end{equation*}
DTW distance is to construct a warp path $W$
\begin{equation*}
  W = w_1,w_2,...,w_K, \text{ } \max(n,m) \leq K < n+m,
\end{equation*}
where $K$ is the length of the warp path, and the $k^{th}$ element of the warp path is $w_k=(i,j)$, $i$ is an index from trajectory $C$ and $j$ is an index from trajectory $Q$. In addition, the starting and ending points of this path are fixed that is $w_1 = (1, 1)$ and $w_K = (n, m)$.
The objective of DTW distance is to find an optimal warp path (or point matching) which has the minimal cumulative distances.
\begin{equation}
  D_{n,m} = \sum\nolimits_{k=1}^{K}d(p_i,q_j), \text{ and } w_k=(i,j),
\end{equation}
where $D_{n,m}$ is the DTW distance of trajectory $C$ with length $n$ and $Q$ with length $m$, $d$ denotes Euclidean distance of two points. We observe the similarity $D_{n,m}$ is independent of the order of accumulation when the optimal warp path is given, that is the similarity is unchanged if we read $C$ and $Q$ in reverse.
\end{proof}

\textcolor[rgb]{1.00,0.00,0.00}{In algorithm~\ref{algo:dtw}, we first need to do the preprocess for suffix similarity and the corresponding DTW values are record in computation matrix $Mat$ as shown in Figure~\ref{fig:dtw} (line 1). Before the for-loop of iterating the time steps (lines 3-18), we need to initialize the index of splitting point $sp$, update vector $\mathcal{V}$, dissimilarity value $\Psi$ and its maintaining interval $\Lambda$ first (lines 2). After that, we select an action guided by $Q^*$ (line 4), if $a = 1$, we cut the trajectory at this time step (lines 5-7). Next, we compute the prefix similarity $\Psi_P$ and suffix similarity $\Psi_S$ and get their intervals (lines 8-9), and concatenate $(\Psi, \Psi_P, \Psi_S)$
as the current state $s$, which is used to input to $Q^*$ (line 10). Finally, we need to maintain the current best subtrajectory from prefix or suffix trajectory (lines 11-17).}

\begin{algorithm}[t]
	\caption{Online Subtrajectory Search for DTW}
	\footnotesize{
		\label{algo:dtw}
		\begin{algorithmic}[1]
			\Require
			Candidate trajectory $C$, query trajectory $Q$ and learned $Q^*$;
			\Ensure
			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
            \State get DTW computation matrix $Mat$ for reverse trajectory $C$ and $Q$;
            \State initialize $sp \leftarrow 1$, $\mathcal{V}_0 \leftarrow None$, $\Lambda \leftarrow [1,n]$, $\Psi \leftarrow Mat_{n,m}$;
            \For{each time step $2 \leq t \leq n$}
            \State select $a = max_{a}Q^*(s,a;\theta)$ using $Q^*$;
            \If{$a = 1$}
            \State $sp \leftarrow t$, $\mathcal{V}_{t-1} \leftarrow None$;
            \EndIf
            \State $\Gamma \leftarrow [sp, t]$, $\Delta \leftarrow [t+1, |C|]$, $\mathcal{V}_t \leftarrow dtw(\mathcal{V}_{t-1}, p_t, Q)$;
            \State $\Psi_P \leftarrow \mathcal{V}_{t,m}$, $\Psi_S \leftarrow Mat_{n-t,m}$;
            \State $s \leftarrow concat(\Psi, \Psi_{P}, \Psi_{S})$;
            \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
                \If {$\Psi_{P} < \Psi_{S}$}
                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
                \Else
                    \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
                \EndIf
            \EndIf
            \EndFor
	\end{algorithmic}}
\end{algorithm}

%\begin{algorithm}[t]
%	\caption{Maintain}
%	\footnotesize{
%		\label{rlst_2}
%		\begin{algorithmic}[1]
%			\Require
%			$\Psi, \Psi_{P}, \Psi_{S}, \Lambda, \Gamma, \Delta$;
%			\Ensure
%			Updated $\Lambda$, $\Psi$;
%            \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
%                \If {$\Psi_{P} < \Psi_{S}$}
%                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                \Else
%                    \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
%                \EndIf
%            \EndIf
%	\end{algorithmic}}
%\end{algorithm}
\begin{lemma}
The time complexity of DTW based subtrajectory similarity computation is $O(nm)$.
\end{lemma}
\begin{proof}
As shown In Algorithm~\ref{algo:dtw}, (1) it takes $O(nm)$ to conduct preprocessing for suffix similarity (line 1). (2) In each time step, the time cost of action selection by $Q^*$ is a constant as explained before (line 6). (3) The time cost of DTW distance update (line 11) is $O(m)$ as shown in Lemma~\ref{dtw_time}. Hence, the overall time complexity is $O(nm)$.
\end{proof}

\subsection{Frechet Distance}
\begin{definition}[Frechet Distance]
Given a candidate trajectory $C = <p_1, p_2,...,p_n>$ and a query trajectory $Q = <q_1, q_2,...,q_m>$, Frechet is computed as below
\begin{equation}
F_{n,m}=\left\{
\begin{aligned}
&\max\nolimits_{i=1}^{n}d(p_i,q_1)&\text{if }m = 1\\
&\max\nolimits_{j=1}^{m}d(p_1,q_j)&\text{if }n = 1\\
&\max(d(p_n,q_m),\\
& \min(F_{n-1,m-1},F_{n-1,m},F_{n,m-1}))&\text{otherwise}
\end{aligned}
\right.
\end{equation}
$F_{n,m}$ is Frechet distance between the prefix trajectory of $C$ with length $n$ and the prefix trajectory of $Q$ with length $m$, and $d(p_n,q_m)$ denotes the Euclidean distance of point $p_n$ and $q_m$.
\end{definition}
We observe the definition of Frechet distance has a similar form with DTW, and thus we have the Frechet update equation as follows.
\begin{equation}\label{dtwupdate}
  \mathcal{V}_{t} = frechet(\mathcal{V}_{t-1}, p_{t}, Q), F_{t,m} = \mathcal{V}_{t,m},
\end{equation}
Similarly, the Lemma~\ref{dtw_sim_nochange} is fulfilled by Frechet distance, and we can replace $dtw(\cdot,\cdot,\cdot)$ as $frechet(\cdot,\cdot,\cdot)$ simply in the framework of Algorithm~\ref{algo:dtw}.


==> parameter.tex <==
%\subsection{Parameter Study}\label{para_study}
\noindent\textbf{The effect of parameters.} This experiment is to evaluate the effect of the soft margin $\xi$ for SizeS. Intuitively, a big $\xi$ value indicates a larger search space, which approaches the search space of the ExactS algorithm as $\xi$ increases. Therefore, SizeS will check more candidate subtrajectories and its running time of SizeS will increase.  Figure~\ref{para_fls} shows the effectiveness results in terms of AR, MR and RR and the running time on 10,000 trajectory pairs of Porto dataset. In Figure~\ref{para_fls}, we increase the value of $\xi$ until the result of SizeS is better than that of RLS in terms of AR, MR and RR.
%, and at the same time, we show the RLS and Exact results for ease of reference.
As expected, as $\xi$ grows the effectiveness of SizeS (as shown in Figure~\ref{para_fls}(a)-(c) for t2vec, (e)-(g) for DTW and (i)-(k) for Frechet) becomes better (approaches and exceeds RLS gradually); However, its running time  increases and approaches that of the exact algorithm while RLS runs much master (as shown in Figure~\ref{para_fls}(d) for t2vec, (h) for DTW and (l) for Frechet).

%Additionally, we can observe that the time change of DTW and Frechet is more significantly than t2vec as $\xi$ increases. This is because the incremental computation for DTW and Frechet is linear, which is higher than the constant update of t2vec as shown in Lemma~\ref{dtw_time}.


%\begin{figure}
%\centering
%\begin{tabular}{c c c}
%  \begin{minipage}{4cm}%5.5
%	\includegraphics[width=4cm]{figures/par_ar}
%  \end{minipage}
%  &
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{figures/par_mr}
%  \end{minipage}
%  \\
%  \scriptsize{(a) Approximation Ratio}
%  &
%  \scriptsize{(b) Mean Rank}
%  \\
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{figures/par_rr}
%  \end{minipage}
%  &
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{figures/par_time}
%  \end{minipage}
%  \\
%  \scriptsize{(c) Relative Rank}
%  &
%  \scriptsize{(d) Time Cost}
%  \end{tabular}
%  \setlength{\belowcaptionskip}{1pt}
%\caption{The influence of soft margin $\xi$ in FLS.}
%\label{para_fls}
%\vspace*{-2mm}
%\end{figure}
\begin{figure*}
\hspace*{-.3cm}
\centering
\begin{tabular}{c c c c}
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/t2v_ar}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/t2v_mr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/t2v_rr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/t2v_time}
  \end{minipage}
  \\
  \small (a) Approximation Ratio (t2vec)
  &
  \small (b) Mean Rank (t2vec)
  &
  \small (c) Relative Rank (t2vec)
  &
  \small (d) Time Cost (t2vec)
  \\
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/dtw_ar}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/dtw_mr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/dtw_rr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/dtw_time}
  \end{minipage}
  \\
  \small (e) Approximation Ratio (DTW)
  &
  \small (f) Mean Rank (DTW)
  &
  \small (g) Relative Rank (DTW)
  &
  \small (h) Time Cost (DTW)
  \\
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/fre_ar}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/fre_mr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/fre_rr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/fre_time}
  \end{minipage}
  \\
  \small (i) Approximation Ratio (Frechet)
  &
  \small (j) Mean Rank (Frechet)
  &
  \small (k) Relative Rank (Frechet)
  &
  \small (l) Time Cost (Frechet)
\end{tabular}
\caption{The influence of soft margin $\xi$ of FLS for t2vec, DTW and Frechet.}
\label{para_fls}
\vspace*{-2mm}
\end{figure*}

%\subsection{Problem Comparison}
\smallskip
\noindent\textbf{Comparison with trajectory similarity computation.}
The traditional Trajectory Similarity Computation (TSC) can be considered as a subproblem of Subtrajectory Similarity Computation (SSC) because the whole trajectory is actually only one of subtrajectories in the target trajectory.
%
This experiment is to evaluate the accuracy if we use the result of TSC to approximate the result of SSC.
  Similar to earlier experiments, we use the exact algorithm as the ground truth, and compare the average results of TSC and SSC  using 10,000 trajectory pairs from Porto and Harbin datasets, respectively. We use RLS for SSC.  As shown in Table~\ref{tscssc}, in terms of effectiveness, we can see that SSC performs much better than TSC: The mean rank and relative rank of TSC are around 10 times larger than those of SSC for t2vec and 20 times for DTW and Frechet.
  %
  This result shows that TSC is not a good approximation for SSC, although TSC runs faster.


%Regarding the efficiency, the time cost of SSC with RLS ia slightly larger than TSC. This is as expected and we explain as follows: (1) for point-matching based measures DTW and Frechet, we need to read trajectories from right to left to get suffix similarities, which is equivalent to a one time TSC; (2) we compute prefix similarities incrementally and it is also equivalent to a one time TSC; (3) we need to call the learning model to obtain a split decision at each time step; (4) note that in t2vec, we do not need to compute the suffix similarities as input, and thus t2vec (around $3\times$ TSC) is faster than DTW and Frechet (around $5\times$ TSC).

\begin{table*}
\hspace*{-.3cm}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Similarity Measure} & \multicolumn{4}{c|}{t2vec} & \multicolumn{4}{c|}{DTW} & \multicolumn{4}{c|}{Frechet} \\ \hline
Dataset                    & Problem    & AR  & MR  & RR  & Time (s) & AR  & MR & RR & Time (s) & AR   & MR  & RR  & Time (s)  \\ \hline
\multirow{2}{*}{Porto}     & TSC        &1.313     &156.153     &23.3\%     &285          &2.100     &752.831    &70.7\%    &181          &1.883      &559.462     &56.5\%     &192           \\ \cline{2-14}
                           & SSC        &1.098     &18.323     &3.0\%     &623          &1.028     &41.138    &3.5\%    &850          &1.034      &34.162     &3.6\%     &739           \\ \hline
\multirow{2}{*}{Harbin}    & TSC        &1.293     &678.311     &46.9\%     &317          &2.326     &1218.908    &72.2\%    & 283          &1.891      &854.042     &53.9\%     &152        \\ \cline{2-14}
                           & SSC        &1.025     &14.945     &1.3\%     &1024          &1.081     &75.324    &4.1\%    & 1346         &1.045      &64.729     &4.4\%     &887       \\ \hline
\end{tabular}
\caption{Comparison with Trajectory Similarity Computation and Subtrajectory Similarity Computation.}
\vspace*{-2mm}
\label{tscssc}
\end{table*}



==> pfs.tex <==
\subsection{Prefix First Search (PFS)}
\label{ha:pfs}
In Lemma~\ref{lemma:subt}, we know any subtrajectory must correspond to a prefix of a suffix trajectory. Actually, the $\Psi_{S}$ of a suffix trajectory only provides some additional dissimilarity values during the search process, which means that we can ignore the $\Psi_{S}$ and only maintain $\Psi_{P}$ if the given trajectory can be exactly split. Based on this intuition, we design a new algorithm, called Prefix First Search (PFS). We illustrate the main idea using Example~\ref{example_idea_pfs}.

\begin{example}
\label{example_idea_pfs}
Consider a pair of candidate and query trajectory $C$, $Q$ in Figure~\ref{example:pfs}, where $t$ is the current time step.
\begin{itemize}[leftmargin=8pt]
  \item $t=1$, we initialize $sp$ as the current $t$, the initial dissimilarity value $\Psi$ as infinity, the initial intervals $\Lambda, \Gamma$ as empty sets, and the first hidden state as none. Compared with BSS and FSS, we only consider the prefix trajectory $C_{\Gamma=[1,1]}$. we split it because it is smaller than initial dissimilarity value $\Psi$, and then we update $sp$ as the next time step and have $C_{\Lambda=[1,1]}$.
  \item $t=2$, we delete the edge between 1 and 2 because a splitting operation happened in last time. We consider the prefix trajectory $C_{\Gamma=[2,2]}$ (Note that the interval update still follows the Equation~\ref{interval}), and decide to maintain it because it is smaller than current dissimilarity value. And then a splitting happens and $sp$ will be updated to next time step.
  \item $t=3$, we consider the prefix trajectory $C_{\Gamma=[3,3]}$, and do not split it because it is not smaller than current dissimilarity value~\footnote{The dissimilarity value computed by $t2vec$. Here, we only show an example to illustrate the current dissimilarity value is not smaller.}. Note that the current $sp$ is still 2 and not be updated at this time.
  \item $t=4$, we get a new prefix trajectory $C_{\Gamma=[3,4]}$, and maintain it because it is more similar than last $C_{\Lambda=[2,2]}$. A splitting happens at this time and $sp$ will be updated. Hence, the final returned result is the subtrajectory with interval $\Lambda = [3,4]$.
\end{itemize}
\end{example}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/example_pfs}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{An example illustrating the PFS.}\label{example:pfs}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}

%\begin{algorithm}[t]
%	\caption{Prefix First Search}
%	\footnotesize{
%		\label{pfs}
%		\begin{algorithmic}[1]
%			\Require
%			Candidate trajectory $C$ and query trajectory $Q$;
%			\Ensure
%			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
%            \State get representation vector $h_{Q}$ for query trajectory $Q$;
%            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma \leftarrow \emptyset$, $sp \leftarrow 1$ and $h_{0} \leftarrow None$;
%			\For{each time step $1 \leq t \leq |C|$}
%                \State $\Gamma \leftarrow [sp, t]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$, $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$;
%                \If {$\Psi_{P} < \Psi$}
%                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$;
%                \EndIf
%			\EndFor
%	\end{algorithmic}}
%\end{algorithm}
% We present the algorithm details in Algorithm~\ref{pfs}.
\begin{lemma}
The total time complexity of PFS is $O(n)$.
\end{lemma}
\begin{proof}
\textcolor[rgb]{1.00,0.00,0.00}{The time cost of preprocessing is $O(n)$. In each time step, the update of $t2vec$ and Euclidean distance computation are $O(1)$. Hence, the overall time cost of PFS is $O(n)$.}
\end{proof}


==> preliminary.tex <==
\subsection{Preliminary}
\label{pre:t2vec}
$t2vec$~\cite{li2018deep} is a state-of-the-art trajectory similarity measure based on deep representation learning. It adapts the sequence encoder-decoder framework to build learning model, as depicted in Figure~\ref{t2vec}.
It first considers locations $p$ as discrete tokens, and then maps each $p$ to a corresponding vector $x$ by a pretrained embedding layer, which is a simple forward neural network~\cite{bengio2003neural}. And $x$ can be considered as the representation of the current location $p$.

There are two main modules in the $t2vec$ - an encoder and a decoder. The encoder encodes the sequence $x$ into a fixed-dimensional vector $h$ by a kind of popular recurrent neural networks - GRU. Similarly, each $h$ in the encoder can be considered as the representation of each current prefix subtrajectory. For example in Figure~\ref{t2vec}, $h_1, h_2$ and $h_3$ are the representations of prefix $<p_1>, <p_1, p_2>$ and $<p_1, p_2, p_3>$. In $t2vec$, the representations of last encoder states can be used to compute trajectory similarity by the Euclidean distance between the vectors.

The decoder decodes out predicted location sequence $p^{pred}$ conditioned on the final output by the encoder. Also, $t2vec$ applies specific denoising mechanism and customized loss function, which makes it outperforms many popular similarity measures such as DTW~\cite{yi1998efficient}.

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/t2vec}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{\small{t2vec: representation learning-based trajectory similarity measure. The model reads
  the sequence $x$ and outputs the sequence of predicted location $p^{pred}$, where EOS is a special token indicating the end of a trajectory. Each $x$ is the representation of each $p$, and each hidden vector $h$ is the representation of each corresponding prefix subtrajectory in $<p_{1}, p_{2},...>$.}}\label{t2vec}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}


==> proof.tex <==
\section{Theoretical Analysis}
For any given data trajectory $T$ with the length $n$, we denote $\Psi(\cdot) = \frac{rank_{T}(T_{\Lambda})}{\#subt_{T}}$ to measure the closeness of approximate approaches to the optimal result, where $\#subt_{T} = \frac{n(n+1)}{2}$ denotes the total number of candidate subtrajectories in $T$, and $rank_{T}(T_{\Lambda})$ denotes the rank of the returned subtrajectory $T_{\Lambda}$ by one of approximate approaches. Here, we default to rank all the subtrajectories in ascending order of their dissimilarity values with query, and thus a smaller $\Psi$ means that the result is closer to the optimal.

\begin{theorem}
$\Psi$(SizeS) has an upper bound $\frac{n^2-(4\xi+1)n+(4\xi+2)m-4\xi}{n^2+n}$.
\end{theorem}
\begin{proof}

Recall that in SizeS, we need to enumerate all subtrajectories with sizes within the range $[m-\xi, m+\xi]$, where $m$ is the length of query trajectory and $\xi \in [0, n-m]$ is a pre-defined parameter. During the search process, we will traverse $\Delta = (n-m+1)(2\xi+1)$ subtrajectories by SizeS and maintain the best one between them. We can assume that these subtrajectories are the worst of all $\#subt_{T}$ subtrajectories in $T$, because we cannot know one subtrajectory will definitely be better than another, that depends on the trajectory measurements (e.g. t2vec is a learning-based similarity.), and thus $\Delta$ is bounded by $\xi$ as $n-m+1 \leq \Delta \leq 2(n-m)^2+3(n-m)+1$, and we can further get an upper bound:
\begin{equation}
\begin{aligned}
\Psi(SizeS) & \leq \frac{\#subt_{T}-(n-m+1)+1}{\#subt_{T}}= \frac{n^2-n+2m}{n^2+n},
\end{aligned}
\end{equation}
and a lower bound:
\begin{equation}
\begin{aligned}
\Psi(SizeS) & \geq \frac{\#subt_{T}-(2(n-m)^2+3(n-m)+1)+1}{\#subt_{T}}\\
&= \frac{-3n^2-4m^2+8mn-5n+6m}{n^2+n}.
\end{aligned}
\end{equation}

\end{proof}

\begin{theorem}
The upper bound of $\Psi$(PSS) and $\Psi$(RLS) is $\frac{n^2-3n+2}{n^2+n}$.
\end{theorem}
\begin{proof}
Recall that in the splitting-based algorithms PSS or RLS, it needs to make a decision (split or not) at each time step, and we can always get two different subtrajectories (prefix and suffix), and thus we will traverse $2n$ subtrajectories during the search and maintain the best. Similarly, we can get an upper bound for PSS and RLS:
\begin{equation}
\begin{aligned}
\Psi(PSS), \Psi(RLS) \leq \frac{\#subt_{T}-2n+1}{\#subt_{T}} = \frac{n^2-3n+2}{n^2+n}.
\end{aligned}
\end{equation}
\end{proof}

\begin{theorem}
The upper bound of $\Psi$(POS) is $\frac{n^2-n+2}{n^2+n}$.
\end{theorem}
\begin{proof}
In POS, we only consider the prefix subtrajectories during the search, and the upper bound of $\Psi(POS)$ is $\frac{\#subt_{T}-n+1}{\#subt_{T}} = \frac{n^2-n+2}{n^2+n}$.
\end{proof}

\begin{theorem}
$\Psi$(POS-D) has an upper bound $\frac{n^2-n+2}{n^2+n}$, and a lower bound $\frac{n^2-(4K+1)n+2}{n^2+n}$.
\end{theorem}
\begin{proof}
POS-D is an improved version of POS, it waits for $K (K > 0)$ positions when a more similar prefix is found and then split at one of these positions, and scan $T$ again from the split. Thus, Let $ \Delta = n+\overline{K}\#split$ denote the number of subtrajectories traversed by POS-D, where $\overline{K}$ denotes the uncovered mean number of subtrajectories during the delay, which is bounded by $0 \leq \overline{K} \leq 2K$, and $\#delay$ means the number of delay, that is $0\leq \#delay \leq n$. Thus $n \leq \Delta \leq (2K+1)n$. Further. we have:
\begin{equation}
\begin{aligned}
\frac{\#subt_{T}-(2K+1)n+1}{\#subt_{T}} &\leq \Psi(POS-D) \leq \frac{\#subt_{T}-n+1}{\#subt_{T}}\\
\frac{n^2-(4K+1)n+2}{n^2+n} & \leq \Psi(POS-D) \leq \frac{n^2-n+2}{n^2+n}
\end{aligned}
\end{equation}
\end{proof}

The summary of theoretical analysis on achievable guarantees of approximate algorithms is presented in Table~\ref{tab:algorithm-theoretical}.
\begin{table}[t!]
	%	\hspace*{-.3cm}
	\caption{Theoretical analysis of approximate algorithms}
	\begin{tabular}{|l||c|c|c|c|}
		\hline
		Algorithms		&	lower bound &	upper bound							\\\hline
		SizeS			&	$\frac{-3n^2-4m^2+8mn-5n+6m}{n^2+n}$ &   $\frac{n^2-n+2m}{n^2+n}$  \\\hline
		PSS	            &   N/A &	$\frac{n^2-3n+2}{n^2+n}$		\\\hline
        POS	            &   N/A &   $\frac{n^2-n+2}{n^2+n}$  	\\\hline
        POS-D	        &   $\frac{n^2-(4K+1)n+2}{n^2+n}$ &	$\frac{n^2-n+2}{n^2+n}$   \\\hline
		RLS			    &   N/A &	$\frac{n^2-3n+2}{n^2+n}$  \\\hline
	\end{tabular}
	%	\vspace*{-2mm}
	\label{tab:algorithm-theoretical}
\end{table}


==> related.tex <==
\section{RELATED WORK}
\label{related}
\textbf{Measuring Trajectory Similarity}.
Measuring the similarity between trajectories is a fundamental problem and has been studied extensively. Some classical solutions focus on indexing trajectories and performing similarity computation by the alignment of matching sample points. For example, DTW~\cite{yi1998efficient} is the first attempt at solving the local time shift issue for computing trajectory similarity. Frechet distance~\cite{alt1995computing} is a classical similarity measure that treats each trajectory as a spatial curve and takes into account the location and order of the sampling points. Further, ERP~\cite{chen2004marriage} and EDR~\cite{chen2005robust} are proposed to improve the ability to capture the spatial semantics in trajectories. However, these point-matching methods are inherently sensitive to noise and involved in quadratic time complexity, which exists commonly in trajectory-related problems. In recent years, some learning-based algorithms were proposed to speed up the similarity computation. Li et al.~\cite{li2018deep} propose to learn representations of trajectories in the form of vectors and then measure the similarity between two trajectories as the Euclidean distance between their corresponding vectors. Based on the deep representation learning, Wang et al.~\cite{wang2019effective} propose multiple trajectory similarity used in sports retrieval. Yao et al.~\cite{yao2019computing} employ deep metric learning to accelerate trajectory similarity computation. Nevertheless, all of the above-mentioned studies focus on measuring the whole trajectory similarity, which cannot be directly applied to measuring subtrajectory similarity. In particular, the efficiency of conventional similarity measures is challenged by a much larger candidate set, as a trajectory with length $n$ consists of $O(n^2)$ possible subtrajectories if we only simply enumerate each one.

\noindent
\textbf{Subtrajectory Similarity Related Problems}.
Measuring subtrajectory similarity is also a fundamental functionality in many tasks such as clustering~\cite{agarwal2018subtrajectory,lee2007trajectory,buchin2011detecting} and similarity join~\cite{tampakis2019distributed}. In~\cite{lee2007trajectory}, a general partition and group framework for subtrajectory clustering is proposed by Lee et al. Further, Buchin et al.~\cite{buchin2011detecting} show that the hardness of subtrajectory clustering based on Freechet distance, and Agarwal et al.~\cite{agarwal2018subtrajectory} apply the trajectory simplification technique to approximate discrete Frechet to reduce the time cost of clustering. Very recently, Tampakis et al.~\cite{tampakis2019distributed,tampakis2019scalable} proposed a distributed solution for subtrajectory join and clustering by utilizing the MapReduce programming model. Although these algorithms are related to subtrajectory similarity computation, they only focus on some specific problem settings and specific similarity measures such as Frechet distance. Additionally, in~\cite{van2007definition}, computation of subtrajectory similarity is proposed by considering the shape-dependent and time-dependent of trajectories. To improve the insufficiency of the existing point-matching trajectory measures, Xie et al.~\cite{xie2014eds} proposed a new segment-based distance EDS for subtrajectory similarity search. Although subtrajectory similarity computation is an important problem, it still lacks an efficient and general solution so far. For example, EDS is only a specially designed similarity measure and it also involves the $O(n^3)$ time complexity because of traversing all possible subtrajectories.

\noindent
\textbf{Index-based Trajectory Search}. Fast trajectory similarity search for large-scale database has attracted plenty of research interest as well. Classical trajectory works spend more effort on indexing DTW distance~\cite{yi1998efficient,keogh2005exact}. Subsequently, many studies proposed other advanced index structures for their respective similarity measures such as LCSS~\cite{vlachos2002discovering}, ERP~\cite{chen2004marriage} and EDR~\cite{chen2005robust}. In recent years, Ranu et al.~\cite{ranu2015indexing} formulate a robust distance function called EDwP and develop a new index TrajTree by borrowing the idea of TB-tree index~\cite{pfoser2000novel} and SETI~\cite{chakka2003indexing}. In addition, Yao et al.~\cite{yao2019computing} employ two spatial-based indexes (R-tree and Grid Inverted) for their trajectory similarity search based on metric learning.

\noindent
\textbf{Subsequence (Substring) Matching}. There is another related but different problem of subtrajectory similarity computation, called subsequence matching, which aims to obtain a subsequence that has the same length as the query in a given candidate sequence. In general, the candidate sequence is relatively long, containing for example millions or even trillions~\cite{rakthanmanon2012searching,rakthanmanon2013addressing} of elements. Several existing works ~\cite{gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked,moon2001duality,faloutsos1994fast} have proposed efficient pruning algorithms to obtain the matching. Compared with solutions of trajectory or subtrajectory similarity problems, there is no constraint for the length of query and candidate trajectories. In other words, the length of the target subtrajectory is not fixed. In addition, most of the subsequence studies proposed lower bounding pruning or early abandoning techniques based on some specific distance such as DTW~\cite{gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked} and Euclidean distance~\cite{faloutsos1994fast,moon2001duality}; however, our solution is general and distance independent. Similar to subsequence matching, substring matching wants to find exact occurrences of a short query string within a long candidate string, classical solutions such as KMP algorithm. To generalize from strings to continuous time series, chen et al.~\cite{chen2005robust} proposed EDR to handle strict equality of strings, it takes the real values
into account and relaxes equality to be within a certain tolerance. Further, they proposed a metric based similarity measure ERP~\cite{chen2004marriage} based on a similar idea of EDR.

\noindent
\textbf{Reinforcement Learning}. The goal of reinforcement learning is to guide agents on how to take actions to maximize a cumulative reward~\cite{sutton2018reinforcement} in an environment with unknown parameters, and the environment is generally modeled as a Markov decision process (MDP)~\cite{puterman2014markov}. In recent years, RL models are often utilized to solve some database related problems. For example, Zhang et al.~\cite{zhang2019end} use RL model for automatic DBMS tuning. Trummer et al.~\cite{trummer2018skinnerdb} use RL to learn optimal join orders in the SkinnerDB system. Wang et al.~\cite{wang2019adaptive} design an effective RL-based algorithm to the bipartite graph matching.
In this paper, we study subtrajectory similarity computation based on a popular reinforcement learning method - Deep Q Network (DQN), which is widely used to solve some problems with large state space such as Atari~\cite{mnih2013playing}. To the best of our knowledge, this is the first learning-based solution that supports measuring subtrajectory similarity.


==> response.tex <==

\newpage

\noindent
{\large
\textbf{Response to Review Report of Paper Titled with ``Efficient and Effective Similar Subtrajectory Search with Deep Reinforcement Learning'' (VLDB20 Paper ID = 1006)}}
%\label{sec:response}

\smallskip\noindent Dear PVLDB Meta-reviewer and Reviewers,

\smallskip
First, we would like to thank the reviewers for their constructive and inspiring comments. We have gone through these comments carefully and revised our draft accordingly.  Below we summarize the major changes that we have made in the revised paper.

%\section{Major Changes}
%\label{sec:majorChanges}

%We have the following major changes (marked in red of the current submission).
%\smallskip\noindent\textbf{Summary of Major Changes:}

\begin{enumerate}
  \item We have included some discussions on the approximation qualities of all approximate algorithms proposed in this paper. They could be found in the individual sections where the algorithms are proposed (Section~\ref{sec:non-learning} and Section~\ref{section:RLS}). Due to the page limit, we put their corresponding proofs in the appendix of the technical report version~\cite{TR}.
  \item We have included an example problem (shown in Figure~\ref{fig:input}) and use it for illustrating two representative algorithms PSS and RLS-Skip in Table~\ref{table:pss} and Table~\ref{table:rls_skip}, respectively.
  \item We have included two competitor algorithms, namely UCR and Random-S. UCR is adapted from the literature of time series as inspired by Reviewer 1's Comment 1 and Random-S is suggested by Reviewer 3. The descriptions of these algorithms could be found in Section~\ref{exper_setup} and the results of the comparisons between them and our RLS-Skip algorithm could be found in Figure~\ref{fig:UCR} and Figure~\ref{fig:random-s} of the revised paper. Overall, none of them are as competitive as RLS-Skip, e.g., UCR is dominated by RLS-Skip and works for DTW only, and Random-S provides trade-offs between efficiency and effectiveness not as good as those by RLS-Skip and is dominated by RLS-Skip in some cases.
  \item We have included a third trajectory dataset that is based on traces of humans, as suggested by Reviewer 1. The description of this dataset could be found in Section~\ref{exper_setup} and the results on this dataset are presented together with those on the two old datasets (due to the page limit, some results are presented in the technical report version). In general, the results on this newly-added dataset provide similar clues as those on the two old datasets.

  \item We have removed some experimental results from the revised paper, including the efficiency results on Harbin (some sub-figures of Figure 3 in the old version), the effectiveness results of varying query lengths in terms of AR and MR on Porto and in terms of AR, MR and RR on Harbin (some sub-figures of Figure 4 in the old version), and the effect of soft margin $\xi$ for SizeS in terms of AR and MR (some sub-figures in Figure 6 in the old version) and presented them in the technical report version~\cite{TR}. The reason is that they deliver similar clues as the results that remain in the revised paper and there is a page limit.
\end{enumerate}

These major changes are highlighted in blue in the revised paper.
Appended please find our detailed responses to both the reviewers' and meta-reviewer's comments.
Thank you for your time reading them.

\smallskip\noindent Yours sincerely\\
\smallskip\noindent Zheng, Cheng, Gao, and Yiding

%----------------
%\newpage
\section{Response to Reviewer 1's Report}
\label{subsec:reviewerOneReport}

\begin{comment1}
``R1W1. Although the framework is general, trajectory similarity metrics share some commons. For some of them, the ExactS approach can be optimized in the same way. So its performance can be better. But the paper does not talk about this potential of ExactS.''
\label{comment1:Optimization-ExactS}
\end{comment1}

\noindent\textbf{Response.}
Thank you for raising this very good point. First, we note that for some similarity measurements such as t2vec, it is hard to optimize ExactS further since ExactS has it time complexity of $O(n^2)$ for t2vec and it needs to traverse $O(n^2)$ subtrajectories.
For some other similarity measurements such as DTW and Frechet, since they were originally proposed for time series data and have been extensively studied for this data type, we searched the literature of time series more thoroughly, as inspired by this comment. We  found the UCR method~\cite{mueen2016extracting,rakthanmanon2012searching,rakthanmanon2013addressing}, which is a highly-cited tool for similar time series search and could be possibly adapted to our problem (though it works for DTW only).
%
A brief description of UCR is provided in the part of ``Compared Methods'' of Section~\ref{exper_setup}. We copy it here for easy reference.
%
\emph{``UCR was originally developed for searching subsequences of a time series, which are the most similar to a query time series and the similarity is based on the DTW distance. UCR enumerates all subsequences that are of the same length of the query time series and employs a rich set of techniques for pruning many of the subsequences.
%Spring is designed for the problem of finding a subsequence of a data time series, which is the most similar to a query time series.
%Spring corresponds to the dynamic programming process for computing the DTW or Frechet distance between the data time series and the query time series, where the latter is padded with a fictitious point that could be aligned with any point of the data time series with distance equal to 0.
We adapt UCR for our similar subtrajectory search problem (details of adaptions are provided in the appendix of the technical report version~\cite{TR}).''}
%
%We note that UCR only works for DTW, but not for Frechet or t2vec and Spring works for both DTW and Frechet, but not for t2vec.

We present the results of the comparison between UCR and RLS-Skip in Figure~\ref{fig:UCR}.
% and Figure~\ref{fig:spring}.
%
A detailed description of these results could be found in the part ``(9) Comparison with UCR'' of Section~\ref{effectiveness}. Here, we make a few notes: (1) UCR does not return exact solutions since it only considers those subtrajectories of the same size of the query trajectory;
%(2) UCR always run slower than RLS-Skip; (3) UCR returns worse solutions than RLS-Skip in most of the cases;
and
(2) UCR is dominated by RLS-Skip in terms of efficiency and effectiveness.
%(3) Spring can return exact solutions, in which cases, it runs faster than ExactS but much slower than RLS-Skip; and
%(4) In some cases, RLS-Skip dominates Spring in terms of both efficiency and effectiveness and in other cases, they provide different trade-offs, but not vice versa.

\begin{comment1}
``R1W2. The paper uses the taxi trajectory datasets in the experiments. But the taxi trip dataset has some uncommon characteristics that trajectories always follow the road network. So the trajectory is not as general as some other moving objects such as human beings. It would be better if some other datasets can be used besides the taxi trajectory dataset.''
\label{comment1:OtherDatasets}
\end{comment1}


\noindent\textbf{Response.} Thank you for your comment. In the revised paper, we include a third dataset called Sports, which involves trajectories of human beings, i.e., soccer players (Section~\ref{exper_setup}). We copy the description of the dataset here for easy reference. \emph{``The third dataset, denoted by Sports, involves around 0.2 million soccer player and ball trajectories collected from STATS Sports~\footnote{https://www.stats.com/artificial-intelligence (STATS, copyright 2019)} with a uniform sampling rate of 10 times per second and a mean length around 170.''}
%
We have conducted the sames experiments on this dataset as we did on the two old datasets. In general, the results on this newly-added dataset provide similar clues as those on the two old datasets.


\begin{comment1}
``R1D1. All splitting based and learning based algorithms have a trade-off between efficiency and effectiveness. The problem is that it does not discuss the maximum percentage of accuracy loss by various approximate algorithms. An algorithm without any guarantee on error bound is not reliable.''
\label{comment1:ApproximationRatio}
\end{comment1}

\noindent\textbf{Response.}
Thank you for your comment. In the revised paper, we include some discussion on the approximation quality for each of the approximate algorithms proposed in this paper. Unfortunately, neither the heuristic-based algorithms nor learning-based algorithms can provide a certain guarantee on the quality of the approximate solution. The proofs, which correspond to problem instances, could be found in the appendix in the technical report version~\cite{TR}. We note that while these results are negative in theory, these approximate algorithms, especially those learning-based ones such as RLS and RLS-Skip, work quite well in practice (e.g., all splitting-based algorithms have the approximation ratio smaller than 1.3 and RLS has the approximation ratio smaller than 1.1 for all similarity measurements and on all datasets (Figure~\ref{effect_result})). In addition, the problem instances that we constructed for proving the negative results in fact rarely happen in practice,
which are confirmed by the effectiveness results on real datasets.

In addition, we would like to note that machine learning has recently been used to develop algorithms for solving database problems and algorithm problems, which has been published in major DB conferences and algorithm conferences. Unfortunately, these algorithms usually have no guarantees, although they perform well empirically. For example, reinforcement learning can be successful used to solve combinatorial problems like TSP, Clique, Vertex Cover, etc., as well as database problems, such as knob tunning, view selection, join order selection, etc.  We appreciate the beauty of elegant algorithms with performance guarantees. However, we think heuristic algorithms with good empirical results also make good contributions.


\begin{comment1}
``R1D2. Approximate algorithms have a soft margin parameter which controls the trade-off between efficiency and effectiveness. This soft margin is the allowed gap between the query trajectory size and a subtrajectory size. The paper does not discuss the maximum allowed value of this soft margin in order to have sufficient reduction in search time while maintaining a good accuracy.''
\label{comment:soft-margin}
\end{comment1}

\noindent\textbf{Response.}
Thank you for your comment. The soft margin is a parameter of the SizeS algorithm. We studied the effects of this parameter on the effectiveness and efficiency of SizeS. The results are shown in Figure 6 in the old version (which now becomes Figure~\ref{para_fls} in the revised version). From the results, we notice that (1) when the soft margin is around 36, SizeS would become competitive in terms of effectiveness (i.e., its solution has similar RR as that of RLs-Skip); and (2) when the soft margin increases, the running time of SizeS increases, and for all settings of soft margin, SizeS runs slower than RLS-Skip (e.g., even when the soft margin is equal to 0, meaning only the subtrajectories of the same size as the query trajectory are considered, SizeS runs slower than RLS-Skip). In conclusion, when SizeS gives competitive effectiveness (e.g., when the soft margin is set to be 36), its running time becomes close to that of the exact algorithm ExactS (i.e., around 650ms v.s. 800ms), and when SizeS gives competitive efficiency (e.g., when the soft margin is set to be 0), its RR is above 50\%, which is far from being satisfactory.


\begin{comment1}
``R1D3. Although it is easily understandable why RLS-Skip takes less time compared to RLS algorithm, the paper does not discuss why RLS-Skip is better than splitting based algorithms in terms of accuracy and search time.''
\label{comment:explanation-RLS-Skip}
\end{comment1}

\noindent\textbf{Response.}
Thank you for your comment. In terms of accuracy, we include in Section~\ref{subsec:rls} a possible explanation on why RLS is better than non-learning splitting based algorithms. We copy it here for easy reference. \emph{``and the reason is possibly that RLS is based on a learned policy,
which makes decision more intelligent than simple heuristics that are human-crafted.''} Since RLS-Skip is a generalized version of RLS, this explanation applies to RLS-Skip as well. In terms of efficiency, the explanation was provided in the part of ``(2) Efficiency results'' of Section~\ref{effectiveness} in the old version. We copy it here for easy reference. \emph{``RLS-Skip runs the fastest since on those points that have been skipped, the cost of maintaining the states and making decisions is saved. In contrast, none of the other algorithms skip points.''}



\begin{comment1}
``R1D4. The paper also has grammatical error. For example, the first contribution discussed in Page-2, Column-1 has grammatical error. The sentence is The SimSub problem relies a trajectory similarity measurement.''
\label{comment:Typo}
\end{comment1}

\noindent\textbf{Response.} Thank you for your comment. We have fixed this grammatical error. We have also proof-read the draft and fixed all grammatical errors we found.


\section{Response to Reviewer 2's Report}
\label{subsec:reviewerTwoReport}


\begin{comment2}
``R2W1 and R2D1. The motivation could be improved. The motivation in page 1 is weak. It would be interesting to see some applications on top of spatiotemporal trajectories like those taxi traces used in the experiments.''
\label{comment2:Reviewer2-Motivation}
\end{comment2}


\noindent\textbf{Response.} Thank you for your comment. In the revised paper, we include an application of detour route detection (in Section~\ref{intro}), which is based on taxi traces. We copy the description here for easy reference. \emph{``Another potential application is detour route detection. 	It first collects those routes that have been reported by passengers to be detour routes and then searches for those subtrajectories of taxis' routes, which are similar to a detour route. The found subtrajectories are probably detour routes as well.''}
In addition, we note that technically it is possible to use the similarity between a part of a data trajectory $T$ and a query trajectory $T_q$ as a new type of similarity measurement between $T$ as a whole and $T_q$.
%Therefore, any applications of ``similar trajectory search'' could be those of ``similar subtrajectory search'' in this sense.
Therefore, ``similar subtrajectory search'' could be potentially used in those applications of ``similar trajectory search'', which are well-recognized and commonly-encountered in real life.


\begin{comment2}
``R2W2 and R2D2. The presentation of the algorithms is plain without illustrative examples. Sections 4 and 5 would benefit from a running example that explains how each algorithm works.''
	\label{comment2:Examples}
\end{comment2}


\noindent\textbf{Response.} Thank you for the suggestion. In the revised paper, we include an example problem (shown in Figure~\ref{fig:input}) and use it for illustrating two representative algorithms PSS and RLS-Skip in Table~\ref{table:pss} and Table~\ref{table:rls_skip}, respectively. Due to page limit, we do not illustrate the ExactS and SizeS algorithms (since they are easy enough), the POS and POS-D algorithms (since they are similar to PSS), or the RLS algorithm (since it is a special version of RLS-Skip).



\begin{comment2}
``R2W3 and R2D3. There is not analysis on the approximation ratios for the approximate algorithms. The paper would be more solid if it conducts analysis on the approximation ratios for those approximate algorithms.''
	\label{comment2:Approximation-Ratio}
\end{comment2}


\noindent\textbf{Response.} Thank you for your comment.
%Please refer to our response to Reviewer 1's Comment 3.
This comment is also mentioned by Reviewer 1 (Reviewer 1's Comment 3). Therefore, please refer to our response to Reviewer 1's Comment 3.


\begin{comment2}
``R2D4. The experiments for Figure 4: It's also interesting to see how the proposed algorithms handle very long query trajectories, e.g., with the same length as the data trajectories or even longer.''
	\label{comment2:LongQueryTrajectories}
\end{comment2}


\noindent\textbf{Response.} Thank you for your comment. This aspect has, in fact, been explored in the experiments of ``(5) The effect of query trajectory length'' in Section~\ref{effectiveness} of the old paper. We revised the experimental set-up for this part a bit in the revised paper to maker it clearer. We copy it here for easy reference.
\emph{``We prepare four groups of query trajectories from a dataset, namely $G1$, $G2$, $G3$, and $G4$, each with 10,000 trajectories, such that the lengths of the trajectories in a group are as follows: $G1=[30,45)$, $G2=[45,60)$, $G3=[60,75)$ and $G4=[75,90)$. Then, for each query trajectory, we prepare a data trajectory from the dataset. Note that for a query trajectory and a corresponding data trajectory, the latter may be longer than or shorter than the former. For each group, we report the average results.''}
%
We make a few notes here:
(1) based on how the query trajectories and data trajectories are prepared for this part of experiments, it could happen that the query trajectory has the length larger or equal to that of the data trajectory;
(2) from group $G1$ to $G4$, the lengths of query trajectories are increasing while the expected length of the data trajectories is unchanged, and thus the results from group $G1$ to $G4$ show a trend of how the algorithms would perform when the length of query trajectories increases; and
(3) based on the results, which are are shown in Figure~\ref{RR:querylength}, we notice that in terms of the effectiveness, the length of query trajectories does not have much effect except for SizeS, and in terms of efficiency, the length of query trajectories has some effect for DTW and Frechet but less for t2vec (since when using t2vec, all trajectories are mapped to vectors and then processed).

\begin{comment2}
``R2D5. The following paper should be cited and discussed in the trajectory similarity measurement part in Section	2. - KSQ: Top-k Similarity Query on Uncertain Trajectories. TKDE 25(9): 2049-2062 (2013)''
	\label{comment2:OneCitation}
\end{comment2}


\noindent\textbf{Response.} Thank you for referring this related study. We have cited this study in Section~\ref{related} of the revised paper. We copy it here for easy reference. \emph{``In addition, Ma et al.~\cite{ma2012ksq} propose a similarity measurement called p-distance for uncertain trajectories and study the problem of searching for top-k similar trajectories to a given query trajectory based on p-distance.''} In addition, we would like to note that this study targets uncertain trajectories and regards each trajectory as a whole for consideration, which are both different from our work.

\balance
\section{Response to Reviewer 3's Report}
\label{subsec:reviewerThreeReport}

\begin{comment3}
``R3W1. The proposed heuristic solutions (in Sections 4.2 and 4.3) and learning-based solutions (in Section 5) do not provide any theoretical guarantee on the rank of result. In Table 3, the mean rank of RLS-Skip is far from 1.''
\label{comment3:TheoreticalGuarantee}
\end{comment3}


\noindent\textbf{Response.}
Thank you for your comment.
This comment is also mentioned by Reviewer 1 (Reviewer 1's Comment 3). Therefore, please refer to our response to Reviewer 1's Comment 3.
%
We also note that in Table 3, the mean ranks, which are are far from 1 (e.g., from 40 to 100), should be acceptable if put in the context that there are a few thousands of subtrajetories, e.g., the corresponding relative ranks are not large (e.g., from 3.5\% to 8.9\%).

\begin{comment3}
``R3W2: The experimental study has not considered the following sampling algorithm as competitor method: "sample X random subtrajectories from the given trajectory, then compute the similarity of those subtrajectories to the query trajectory $T_q$". I speculate that this method can achieve an expected mean rank of 1\% by sampling only 100 random subtrajectories (regardless of the total number $O(n^2)$ of subtrajectories). As for comparison, in Table 3, the relative rank of RLS-Skip ranges from 3.5\% to 8.9\%.''
\label{comment3:Competitor}
\end{comment3}

\noindent\textbf{Response.} Thank you for raising this very good point. We call this method Random-S. With 100 sampled subtrajectories, the probability that Random-S returns a subtrajectory with RR at most 1\% (resp. 5\%) is equal to $(1-(1-1\%)^{100}) = 0.634$ (resp. $(1-(1-5\%)^{100}) = 0.994$), which look quite promising. Therefore, we consider Random-S as a competitor method in the revised paper and compare it against RLS-Skip. The results are shown in Figure~\ref{fig:random-s}. Indeed, when the sample size is around 100, the RR of Random-S approaches 1\% (Figure~\ref{fig:random-s} (a)), but meantime, its running time gets close to that of the exact algorithm ExactS (Figure~\ref{fig:random-s} (b)). In addition, for Random-S, the subtrajectories that are considered could be quite different, and thus it is not possible to compute their similarities \emph{incrementally} as it does for ExactS. As a result, even for a relatively small sample size, e.g., 100, the running time of Random-S is almost that of ExactS and significantly larger than that of RLS-Skip (25 times higher). Whereas when the sample size is small, e.g., below 20, Random-S has its effectiveness significantly degraded, which is clearly worse than that of RLS-Skip (Figure~\ref{fig:random-s}(a)), and meantime it still runs slower than RLS-Skip (Figure~\ref{fig:random-s}(b)).
%In conclusion, RLS-Skip dominates Random-S for some settings of sample size in terms of both efficiency and effectiveness and provides different trade-offs between them for other settings, but not vice versa.


\begin{comment3}
``R3W3. It is not easy to follow Sections 5.3 and 5.4. It'd be better if the authors could include some figures or examples to illustrate the techniques used in those subsections.''
\label{comment3:Examples}
\end{comment3}

\noindent\textbf{Response.} Thank you for the comment. In the revised paper, we include an example for illustrating RLS-Skip, where the input is shown in Figure~\ref{fig:input} and the process of RLS-Skip is illustrated in Table~\ref{table:rls_skip}. We do not illustrate the RLS algorithm since it is a special version of RLS-Skip and the space is limited.

\begin{comment3}
``R3D1. In Equation 2, there is an extra ')' in the "otherwise" case. In Table 2, a ')' is missing in the Big-O notation of the abstract similarity measurement of ExactS.''
\label{comment3:Typo}
\end{comment3}

\noindent\textbf{Response.} Thank you for the comments. We have fixed these typos in the revised paper.


\begin{comment3}
``R3D2. The experimental setup (Section 6.1) did not mention the parameter setting of SizeS.''
\label{comment3:ParameterSetting}
\end{comment3}

\noindent\textbf{Response.} Thank you for the comment. In the old version, the parameter setting of SizeS is mentioned when SizeS is specified in the part of ``Computed Methods'' in Section~\ref{exper_setup}. We copy it here for reference. \emph{``For SizeS, we use the setting $\xi = 5$ (with the results of its effect shown later on).''} In this revised paper, we have moved this description in the part of ``Parameter Setting'' in Section~\ref{exper_setup} since it looks natural to put there.

\begin{comment3}
``R3D3. Please report the learning time of RLS and RLS-skip in the experimental section. How much is the learning time compared to the "time without index" in Figure 3? How much is the learning time compared to the index construction time?''
\label{comment3:LearningTime}
\end{comment3}

\noindent\textbf{Response.} Thank you for the comment.
%
In the revised paper, we have presented the results of learning time of RLS and RLS-Skip in the part of ``(11) Training time'' in Section~\ref{effectiveness}. We copy the description here for easy reference. \emph{``The training times of the RLS and RLS-Skip models on different datasets are shown in Table~\ref{learntime}. It normally takes a couple of hours to train a reinforcement learning model for RLS and RLS-Skip. It takes less time to train RLS-Skip than RLS since we use the same number of trajectory pairs and epochs for training both algorithms and RLS-Skip runs faster.''}
For comparison with the time of query processing and index construction,
we consider the experiment of running queries over a database of 2 million points collected from the Porto dataset, whose results are shown in Figure~\ref{fig:efficiencyRLS}. It takes 4.4 hours to train RLS-Skip offline. Once it has been trained, it could be used for many queries online, e.g., for a query of finding top-50 similar subtrajectories from the database, the time is about 522s if no index structures are used and 23.08s if the Inverted index is used. Besides, on this database, the time of building the Inverted list is small, e.g., around 5.16s. The message is that the training time is still manageable, e.g., a couple of hours usually. In addition, the training is a one-time process, and after training, it can be used to serve the query processing of many queries.

\section{Response to Meta-Reviewer's Report}
%\subsection{Meta-Reviewer Comments and Response}

\begin{revision}
	``An analysis on the approximation ratios for those approximate algorithms needs to be provided.''
\end{revision}

\noindent\textbf{Response.}
Thank you for your comment.
We have finished this revision item.
Please refer to our response to Reviewer 1's Comment 3.

\begin{revision}
	``The presentation needs to be further improved significantly, including running examples, figures, etc.''
\end{revision}

\noindent\textbf{Response.}
Thank you for your comment.
We have finished this revision item.
Please refer to our response to Reviewer 2's Comment 2 and Reviewer 3's Comment 3.

\begin{revision}
	``More competitors need to be included in the comparison to justify the novelty.''
\end{revision}

\noindent\textbf{Response.}
Thank you for your comment.
We have finished this revision item.
Please refer to our responses to Reviewer 1's Comment 1 and Reviewer 3's Comment 2.

\begin{revision}
	``Additional trajectory datasets need to be tested.''
\end{revision}

\noindent\textbf{Response.}
Thank you for your comment.
We have finished this revision item.
Please refer to our responses to Reviewer 1's Comment 2.



==> rl.tex <==
\section{RL-BASED SEARCH (RLS)}
\label{section:RLS}
Inspired by all the heuristic algorithms mentioned above, we further propose a data-driven method to guide trajectory splitting based on deep reinforcement learning, called RL-based Search (RLS).
\subsection{Trajectory Splitting in MDP Modeling}
From a high-level perspective, we first explain why we use the reinforcement learning.
The trajectory splitting process can be considered as a Markov decision process (MDP)~\cite{puterman2014markov} with unknown parameters. Recall that in each time step, we need to interact with the environment (i.e., the whole trajectory $C$) to make a decision (i.e., split or not), and then get a immediate reward (i.e., the dissimilarity value $\Psi$). In order to find an optimal strategy to split trajectories, we apply Reinforcement Learning (RL)~\cite{sutton2018reinforcement}, because it has been proven to be able to optimize the sequential decision-making problem in MDPs effectively. Next, we give the formal definitions for MDP in our problem.
\subsection{Definitions for MDP Modeling}
Given a candidate trajectory $C$ (environment), we define a Markov decision process in our problem is a 4-tuple $M = (\mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R})$.
\begin{definition}[State]
$\mathcal{S}$ is a state space for every state $s \in \mathcal{S}$.
\end{definition}
Recall that in heuristic algorithms, we have three candidate dissimilarity values in each time step, $\Psi$ denotes the dissimilarity value that we maintain currently. $\Psi_{P}$ denotes the prefix trajectory dissimilarity value, and $\Psi_{S}$ denotes the suffix trajectory dissimilarity value. We concatenate $\Psi$ and $\Psi_{P}$ to represent the current state $s = (\Psi, \Psi_{P})$. Here, we do not concatenate $\Psi_{S}$ because as discussed before, it is only a approximate value via encoding the trajectories in reverse, and thus may misguide the model's real decision.

\begin{definition}[Action]
$\mathcal{A} = \{0, 1\}$ is a action space for every action $a \in \mathcal{A}$.
\end{definition}
Action 0 means to make no splits and go to the next time step, and action 1 means to split at the current time step.

\begin{definition}[Transition Distribution]
$\mathcal{T}:(\mathcal{S} \times \mathcal{A} \times \mathcal{S'}) \rightarrow [0,1]$ is a transition distribution, which models the probability that action $a$ in state $s$ at time $t$ will lead to state $s'$ at next time $t+1$.
\end{definition}
We illustrate an example of state transition in Figure~\ref{state}. Note that the interval update still follows the Equation~\ref{interval} proposed in heuristic algorithms.
\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/state}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{\small{An example illustrating state transition $\mathcal{S} \times \mathcal{A} \times \mathcal{S'}$ for trajectory $T = <p_1, p_2, p_3>$.}}\label{state}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}

\begin{definition}[Reward]
$\mathcal{R}:(\mathcal{S} \times \mathcal{A}) \rightarrow \mathbb{R}^{+}$ is a reward function, the immediate reward $r$ is received after we conduct an action $a$ at state $s$.
\end{definition}
We define the reward $r$ in our problem as the difference between two adjacent dissimilarity values $\Psi$, that is $r_t = \Psi_{t-1} - \Psi_{t}$. We proof our definition is sound and RL can be used to solve the search problem using Lemma~\ref{lemma:opt}.
\begin{lemma}
\label{lemma:opt}
Finding the optimal subtrajectory is equivalent to maximizing the cumulative rewards at the initial state.
\end{lemma}

\begin{proof}
The goal of reinforcement learning is to find the optimal policy $\pi^*$ which can maximize expected cumulative reward.
\begin{equation}
\begin{aligned}
\label{eproof:given}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\pi^* = \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t= 0}^{|C|-1}\gamma^{t} r_{t+1}|\pi \bigg],
\end{aligned}
\end{equation}
where $\gamma$ is a discount rate and $\gamma \in [0,1)$. By our definition,
\begin{equation}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
r_{t+1} = \Psi_{t} - \Psi_{t+1} \geq 0.
\end{aligned}
\end{equation}
Thus, we have
\begin{equation}
\begin{aligned}
\label{eproof:rl}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\pi^* = \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t= 0}^{|C|-1}\gamma^{t} r_{t+1}|\pi \bigg] \Leftrightarrow \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}r_{t+1}|\pi \bigg].
%& = \max\limits_{\pi} \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}(\Psi_{t} - \Psi_{t+1})|\pi \bigg]
%= \max\limits_{\pi}(\Psi_{0} - \Psi_{|C|}) \Leftrightarrow \min\limits_{\pi}\Psi_{|C|}.
\end{aligned}
\end{equation}
We proof the Equation~\ref{eproof:rl} by contradiction. Suppose $\pi^*$ is not an optimal policy which can maximize the expected cumulative reward without discount rate $\gamma$. Thus, there exists a policy $\pi^0$ such that
\begin{equation}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}r_{t+1}|\pi^* \bigg] < \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}r_{t+1}|\pi^0 \bigg],
\end{aligned}
\end{equation}
and $\pi^* \neq \pi^0$. We know the reward $r_{t+1} \geq 0$ and $0 \leq \gamma^{t} \leq 1$ for $t \in \big[0, |C|-1\big]$. Further, we have
\begin{equation}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}\gamma^{t} r_{t+1}|\pi^* \bigg] < \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}\gamma^{t} r_{t+1}|\pi^0 \bigg],
\end{aligned}
\end{equation}
which contradicts our given Equation~\ref{eproof:given}, and thus Equation~\ref{eproof:rl} holds. Furthermore, we have
\begin{equation}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\pi^* & \Leftrightarrow \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}r_{t+1}|\pi \bigg]
= \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}(\Psi_{t} - \Psi_{t+1})|\pi \bigg]\\
& = \argmax\limits_{\pi}(\Psi_{0} - \Psi_{|C|}) \Leftrightarrow \argmin\limits_{\pi}\Psi_{|C|} \Leftrightarrow \arg\limits_{\pi}opt.
\end{aligned}
\end{equation}
$\Psi_{0}$ is a fixed initial value when given a pair of candidate
trajectory $C$ and query trajectory $Q$, and $\Psi_{|C|}$ is the final returned similarity. We know the $\min\Psi_{|C|}$ is equivalent to the optimal solution $opt$ because the optimal subtrajectory is a subtrajectory with the minimal dissimilarity value in all of the candidate subtrajectories. Hence, Lemma~\ref{lemma:opt} holds.
\end{proof}

\subsection{Deep Q Network (DQN)}
In this section, we give a brief preliminary of our reinforcement learning framework - Deep Q Network (DQN)~\cite{mnih2013playing}. DQN is a popular value-based RL method, whose core is the Q-value calculation defined as $Q^*(s, a)$, and furthermore, the iterative loss function is defined as follows.
\begin{equation}
\label{eq:rlobj}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
& Q^*(s_{t}, a_{t}) \leftarrow Q^*(s_{t}, a_{t}) + \\
& \alpha[r_{t+1}+\gamma\max \limits_{a} \underbrace{Q^*(s_{t+1}, a)}_{Target-NN} - \underbrace{Q^*(s_{t}, a_{t})}_{Current-NN}],
\end{aligned}
\end{equation}
where $\alpha$ is a learning rate, $s_t$ is the current state, $a_t$ is a chosen action, which depends on the current Q-value, $r_{t+1}$ is an obtained reward after taking action $a_t$, and $s_{t+1}$ is the next state. There are two main modules in DQN: $Current-NN$ and $Target-NN$, $Current-NN$ is used to calculate $Q^*(s_{t}, a_{t})$ and it interacts with the environment (the candidate trajectory $C$) to get transitions $(s_t,a_t,r_t,s_{t+1})$, which is stored in the replay memory $\mathcal{M}$, and $\mathcal{M}$ can be considered as a collection, we randomly sample transitions from $\mathcal{M}$ in the training process.
$Target-NN$ is used to calculate the next Q-value $Q^*(s_{t+1}, a_{t})$. Note that the parameters (weights) in the $Current-NN$ and $Target-NN$ will be updated during the training process. We illustrate the detailed DQN working process in Figure~\ref{rlmodel}.

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/rlmodel_v4}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{\small{RLS model.}}\label{rlmodel}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}
\subsection{Algorithm Sketch}
\textcolor[rgb]{1.00,0.00,0.00}{In this section, we present the two main parts of RL-based Search (RLS): offline training (Algorithm~\ref{rlst_1}) and online search (Algorithm~\ref{rlst_3}). In Algorithm~\ref{rlst_1}, We first initialize the function $Q^*$ ($Current-NN$ and $Target-NN$) with some random weights and the size of the replay memory $\mathcal{M}$ (line 1). In the outer loop of iterating the episodes (lines 2-21), we first random a trajectory pair $C$ and $Q$ from trajectory database $\mathcal{D}$ (line 3), and then we need to get token sequences used to prefix trajectory similarity computation (line 4), representation vectors for query $Q$ (line 5). Note that here do not encode backward $h'$ for suffix trajectory similarity computation because we do not use $\Psi_{S}$ to define states as explained before.
Before the inner loop of iterating the time steps (lines 6-21), we need to initialize the trajectory dissimilarity values $\Psi, \Psi_{P}$, and concatenate them to get state $s$ (lines 6-7). In the training process (lines 8-20), we first get a greedy action at the current state with $\epsilon-$greedy strategy, which is a common approach in DQN, the main idea of this strategy is to select an action with an uniform
probability proportion $\epsilon$, and a typical parameter value for $\epsilon$ is generally set to 0.1 (line 9). If $a=1$, which means that we need to cut the trajectory (lines 10-12). And then we get a new state $s'$ (lines 13-14), maintain the current best $\Psi$ in order to calculate reward $r$ (line 15). Finally, we store the transition of this step $(s,a,r,s')$ in $\mathcal{M}$ and sample a minibatch for optimizing $Q^*$ according to Equation \ref{eq:rlobj} (lines 16-18). Note that the current $s$ is updated to the next $s'$ (line 19).}

\begin{algorithm}[t]
	\caption{RL-based Search: Offline Training}
	\footnotesize{
		\label{rlst_1}
		\begin{algorithmic}[1]
			\Require
			Trajectory database $\mathcal{D}$ and learning rate $\alpha$;
			\Ensure
			Learned action-value function $Q^*$;
            \State initialize $Q^*$ with random weights and replay memory $\mathcal{M}$;
            \For{$episode = 1, 2, 3,...$}
            \State sample candidate trajectory $C$ and query trajectory $Q$ from $\mathcal{D}$;
            \State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
            \State get representation vector $h_{Q}$ for $Q$;
            \State initialize $h_{0} \leftarrow None$, $h_{1} \leftarrow t2vec(h_{0}, x_{1})$;
            \State $\Psi_{P} \leftarrow d(h_{Q}, h_{1}), \Psi \leftarrow \Psi_{P}, s \leftarrow concat(\Psi, \Psi_{P})$;
            \For{each time step $2 \leq t \leq |C|$ in each $episode$}
            \State select $a = max_{a}Q^*(s,a;\theta)$ with $\epsilon-$greedy strategy;
            \If{$a = 1$}
            \State $h_{t-1} \leftarrow None$;
            \EndIf
            \State $h_{t} \leftarrow t2vec(h_{t-1}, x_{t}), \Psi_{P} \leftarrow d(h_{Q}, h_{t})$;
            %\State , $\Psi_{S} \leftarrow d(h_{\overleftarrow{Q}}, h'_{|C|-t})$;
            \State $s' \leftarrow concat(\Psi, \Psi_{P})$;%, \Psi_{S}
            \State $tmp \leftarrow \Psi$, $\Psi \leftarrow min(\Psi, \Psi_{P})$, $r \leftarrow tmp - \Psi$;%, \Psi_{S}
            \State store transition $(s,a,r,s')$ in $\mathcal{M}$;
            \State Sample random minibatch of transitions from $\mathcal{M}$;
            \State optimize $Q^*$ by gradient descent in Equation \ref{eq:rlobj};
            \State $s \leftarrow s'$;
            \EndFor
            \EndFor
	\end{algorithmic}}
\end{algorithm}
\textcolor[rgb]{1.00,0.00,0.00}{
The output of the offline training is the $Q^*$ of the $Current-NN$~\footnote{Note that the weights of $Target-NN$ is updated by $Current-NN$ during the training process as shown in Figure~\ref{rlmodel}, so finally, they have the same model structure and shared weights.}. In the online part, we first need to do the same preprocess as shown in offline (lines 1-2). Before the for-loop of iterating the time steps (lines 5-15), we need to initialize the index of splitting point $sp$, dissimilarity value $\Psi_{P}, \Psi$, and maintaining interval $\Lambda$ first (lines 3-4). After that, we select an action guided by $Q^*$ (line 6), if $a=1$, we cut the trajectory at this time step (lines 7-9). Next, we compute the $\Psi_{P}$ according to its interval $\Gamma$ (lines 10), and concatenate these two values as the state $s$, which is used to input to $Q^*$ (line 11). Finally, we update the target $\Lambda$ and $\Psi$ if there is a better result (line 12-14).} Overall, the online part shares a similar framework with the heuristic algorithms; however, the splitting strategy is determined by a data-driven model RLS.

%\begin{algorithm}[t]
%	\caption{RL-based Search: Update}
%	\footnotesize{
%		\label{rlst_2}
%		\begin{algorithmic}[1]
%			\Require
%			$\Psi, \Psi_{P}, \Psi_{S}, \Lambda, \Gamma, \Delta$;
%			\Ensure
%			Updated $\Lambda$, $\Psi$;
%            \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
%                \If {$\Psi_{P} < \Psi_{S}$}
%                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                \Else
%                    \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
%                \EndIf
%            \EndIf
%	\end{algorithmic}}
%\end{algorithm}

\begin{algorithm}[t]
	\caption{RL-based Search: Online Search}
	\footnotesize{
		\label{rlst_3}
		\begin{algorithmic}[1]
			\Require
			Candidate trajectory $C$, query trajectory $Q$ and learned $Q^*$;
			\Ensure
			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
            \State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
            \State get representation vector $h_{Q}$ for $Q$;
            %\State set $h'_{0} \leftarrow None$ and get each backward hidden state $h'_{t}$ for $\overleftarrow{C}$;
            \State initialize $sp \leftarrow t$, $h_{0} \leftarrow None$, $h_{1} \leftarrow t2vec(h_{0}, x_{1})$;
            \State $\Psi_{P} \leftarrow d(h_{Q}, h_{1}), \Psi \leftarrow \Psi_{P}, s \leftarrow concat(\Psi, \Psi_{P}), \Lambda \leftarrow [1,1]$;
            \For{each time step $2 \leq t \leq |C|$}
            \State select $a = max_{a}Q^*(s,a;\theta)$ using $Q^*$;
            \If{$a = 1$}
            \State $sp \leftarrow t$, $h_{t-1} \leftarrow None$;
            \EndIf
            \State $\Gamma \leftarrow [sp, t]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$, $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$;
            \State $s \leftarrow concat(\Psi, \Psi_{P})$;
            \If{$\Psi_{P} < \Psi$}
            \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
            \EndIf
            \EndFor
	\end{algorithmic}}
\end{algorithm}

\begin{lemma}
The total time complexity of RLS is $O(n)$.
\end{lemma}
\begin{proof}
In Algorithm~\ref{rlst_3}, we explain the time complexity as follows: (1) it takes $O(n)$ to finish preprocessing (lines 1-2). (2) In each time step, the time cost of action selection by $Q^*$ is a constant (line 8) because the state $s$ is only a 2-dimensional vector and the neural network of $Q^*$ is only a simple forward neural network with 2-layers in our experimental evaluation. (3) The time cost of Euclidean distance computation, update and concatenation is a constant, which is obvious by observing the pseudocodes. Hence, the overall time complexity of RLS is $O(n)$.
\end{proof}


==> setup.tex <==
\section{EXPERIMENTS}
\label{experiment}

\subsection{Experimental Setup}
\label{exper_setup}
\textbf{Dataset.} Our experiments are conducted on two real-world taxi trajectory datasets. The first dataset is collected from the city of Porto~\footnote{https://www.kaggle.com/c/pkdd-15-predict-taxi-service-trajectory-i/data}, Portugal around 18 months with a sampling interval of 15 seconds. %and each location sampled at 15 second intervals.
After filtering the trajectories with fewer than 30 sampling points, we obtain 1.2 million trajectories with a mean length around 60. The second dataset consists of trajectories collected from 13,000 taxis over 8 months in Harbin, China with non-uniform sampling rates. After removing the trajectories with fewer than 30 points, we get over 1 million trajectories with a mean length around 120.

\noindent\textbf{Parameter Setting.} For training t2vec model, we follow the original paper~\cite{li2018deep} for  parameter setting. We use a forward neural network with 2-layers to record Q-values in our RLS model. In the training process, the size of replay memory $\mathcal{M}$ is set at 2000. We train our model on 25k random trajectory pairs, using Adam stochastic gradient descent with an initial learning rate of 0.01. The minimal $\epsilon$ is set at 0.1 with decay 0.99 for $\epsilon$-greedy strategy, and the reward discount rate $\gamma$ is set at 0.95.

\noindent\textbf{Compared Methods.} We compare RL-based Search (RLS) and the proposed non-learning based algorithms (Section~\ref{sec:non-learning}), namely ExactS, SizeS, PSS, POS, and POS-D.
%Note that for DTW and Frechet distance we  modify GA by reading suffix trajectories from right to left, and thus do not need the BSS method. {\bf Gao not clear.. BCC is the same as GA for DTW?}
%
%In addition, inspired by the algorithms for approximate matching for substring and subsequence~\cite{kim2013efficient,zhang2010bed,gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked,moon2001duality,faloutsos1994fast}, we further propose a baseline, called Fixed-Length Search (FLS) with soft margin $\xi$. Specifically, we search the subtrajectories with lengths from $|Q|-\xi$ to $|Q|+\xi$ in the candidate trajectory $C$, where $|Q|$ denotes the length of query trajectory and $\xi\in[0,|Q|)$. In case the fixed search lengths exceed the length of candidate trajectory $C$, we further limit the search bound from $min(|Q|-\xi,|C|)$ to $min(|Q|+\xi,|C|)$. Note that the result will get better as $\xi$ gets larger although the time cost will increase, and in extreme cases it may return the same result as the exact algorithm.
%
The default value of $\xi$ in PSS is set at 5 and we will report the effect of the parameter $\xi$ in our experiments.
For POS-D, we vary the delay positions $K$  from 4 to 7, and the results are similar. We set $K$ at 5 in our experiments. For RLS, when t2vec is adopted, we ignored the $\Theta_{suf}$ component of a state based on empirical findings.

\noindent\textbf{Evaluation Metrics.} We use three metrics to evaluate the effectiveness of the approximate algorithms using the results of the exact algorithm as the ground truth. (1) Approximate Ratio (AR). AR for the subtrajectory similarity computation is defined as $\frac{\Psi_{app}}{\Psi_{opt}}$, where $\Psi_{app}$ is the dissimilarity value returned by one of the approximate algorithms (e.g., SizeS, PSS, POS, POS-D, and RLS), and $\Psi_{opt}$ is the dissimilarity value of the exact algorithm.
%AR measures the performance of an online algorithm by the distance between the optimal solution, and thus
A smaller AR value indicates a better algorithm.
(2) Mean Rank (MR). %MR is a rank-based metric. Consider a trajectory pair $(C, Q)$,
We sort all the subtrajectories of the given candidate trajectory $C$ in ascending order of their dissimilarity values with query $Q$. %obtained by the exact algorithm, and
We denote by $rank_{C}(C_{\Lambda})$  the rank of the returned subtrajectory $C_{\Lambda}$ for a query trajectory $Q$ by an algorithm. We report the mean number of $rank_{C}(C_{\Lambda})$ as MR.
(3) Relative Rank (RR). %For the candidate trajectories $C$ with different lengths,
As the number of subtrajectories of a candidate trajectory $C$ varies a lot, we normalize the rank by the number of subtrajectories, i.e., $\frac{rank_{C}(C_{\Lambda})}{\#subt_{C}}$, where $\#subt_{C} = \frac{|C|(|C|+1)}{2}$. We call the matric by Relative Rank (RR).
Smaller MR or RR value indicates a better algorithm.

%is also different. Here, we denote the RR as the mean number of $\frac{rank_{C}(C_{\Lambda})}{\#subt_{C}}$, where $\#subt_{C}$ is the total number of subtrajectories of $C$, if the length of $C$ is $n$,  $\#subt_{C} = \frac{n(n+1)}{2}$.


\noindent\textbf{Evaluation Platform.} All the methods are implemented in Python 3.6. The implementation of RLS is based on Keras 2.2.0. The experiments are conducted on a server with 32-cores of Intel(R) Xeon(R) Gold 6150 CPU @ 2.70GHz 768.00GB RAM and one Nvidia Tesla V100-SXM2 GPU.


==> theory.tex <==

\newpage
{\color{red}
\section{Quality Analysis of the SizeS Algorithm}
\label{sec:sizes-proof}
There usually exists a space, within which the objects move. Therefore, we assume the points of trajectories are all located in a $d_{max} \times d_{max}$ rectangle, where $d_{max}$ is a large number that captures the extent of the space. We use a coordinate system whose origin is at the middle of this rectangle.
%

\smallskip\noindent\textbf{Case 1: DTW.}
Consider a problem input with a query trajectory with $m$ points $T_q = <p_1', p_2', ..., p_m'>$ and a data trajectory with $n = m^2$ points $T = <p_{1,1}, p_{1,2}, ..., p_{1,m}, p_{2,1}, p_{2,2}, ..., p_{2,m}, ..., p_{m,1}, p_{m,2}, p_{m,m}>$. We assume that $m$ is an even number and $l = m / 2$. In addition, we let $d = d_{max} / m$.
The locations of the points in these trajectories are provided as follows.
\begin{itemize}
	\item $p_i' = ( - ( l - i + 1/2) \cdot d, 0)$ for $i = 1, 2, ..., l$;
	\item $p_i' = ( (i - l - 1/2) \cdot d, 0)$ for $i = l+1, l+2, ..., m$;
	\item $p_{i,j}$'s ($1\le j \le m$) are evenly located at the circle with its center at $p_i'$ and its radius equal to $\epsilon$, where $\epsilon$ is a very small real number for $i = 1, 2, ..., m$;
\end{itemize}

Consider the optimal solution. Its DTW distance, denoted by $D_o$, is at most the distance between $T$ and $T_q$, which is equal to $m^2\cdot \epsilon$ (points $p_{i,j}$ for $1\le j\le m$ are aligned with point $p_i'$ for $1\le i\le m$). That is, we have $D_o \le m^2 \cdot \epsilon$.

Consider the approximate solution returned by SizeS.  Suppose that $\xi = 0$. That is, we only consider subtrajectories with the length exactly equal to $m$. We further know that each such sub-trajectory consists of points, either all located at a circle with the center at one of the point of $T_q$ or some located at a circle with the center at a point $p_i'$ and others located at a circle with the center at a point $p_{i+1}'$ ($1\le i < m$). It could be verified that among these subtrajectories, the one with some located at the circle with the center at $p_l'$ and others at $p_{l+1}'$ has the smallest DTW distance from $T_q$ and would be returned. We denote its DTW distance to $T_q$ by $D_a$. It could be verified that $D_a > 2\times (\Sigma_{i=1}^{l-1} ((l-i)\cdot d - \epsilon) + \epsilon)$, where the lower bound of the Euclidean distance from a point of $T_q$ to its aligned point of the returned subtrajectory is (1) $((l-i)\cdot d - \epsilon)$ for $1\le i\le l-1$ and (2) $\epsilon$ for $i = l$; and (3) that of the point symmetric to $p_i'$ (w.r.t. the origin) for $l+1\le i\le m$ due to the symmetry. Therefore, we have
\begin{align*}
\frac{D_a}{D_o} 
& \ge \frac{2\times (\Sigma_{i=1}^{l-1} ((l-i)\cdot d - \epsilon) + \epsilon)}{m^2 \cdot \epsilon}\\
& = \frac{m^2/4\cdot d - m/2\cdot d - m\cdot \epsilon + 4\cdot\epsilon}{m^2\cdot \epsilon} \\
&= \frac{1/4\cdot d - 1/(2m)\cdot d - \epsilon/m + 4/m^2\cdot \epsilon}{\epsilon}
\end{align*}
which approaches infinity when m approaches infinity and $\epsilon$ approaches 0.
In summary, the solution returned by SizeS could be arbitrarily worse than the optimal one when DTW distance is used.

\smallskip\noindent\textbf{Case 2: Frechet and t2vec.}
Consider the case when Frechet distance is used. The optimal solution and the approximate solution returned would be the sames as the case when DTW distance is used, but the distances would be different. $D_o$ would be equal to $\epsilon$ and $D_a$ would be at least $((l-1)\cdot d - \epsilon)$. Therefore, we have
$$
\frac{D_a}{D_o} \ge \frac{(l-1)\cdot d - \epsilon}{\epsilon}
$$
which approaches infinity when $\epsilon$ approaches 0.

Consider the case when t2vec is used. Since it is a learning-based distance - in theory, it may reduce to any possible distance metric such as DTW and Frechet. Thus, the analysis for DTW or Frechet could be carried over for t2vec.

\if 0
We provide a theoretical guarantee on the rank for SizeS algorithm. SizeS enumerates all subtrajectories with the sizes within the range $[m-\xi, m+\xi]$, where $m$ is the length of query trajectory and $\xi$ is a controllable parameter. During the search process, we know SizeS will traverse $(n-m+1)(2\xi+1)$ subtrajectories and return the best one among them. We can safely assume the worst case is the subtrajectories tried by SizeS are the worst (i.e., smallest similarity) in all $\frac{n(n+1)}{2}$ subtrajectories in $T$. Thus, the rank is bounded by $\frac{n(n+1)}{2}-(n-m+1)(2\xi+1)+1$. The tightness of the bound is controllable by the parameter $\xi$.
\fi


\section{Quality Analysis of Spliting-based Algorithms}
\label{sec:splitting-proof}

\smallskip\noindent\textbf{Case 1: PSS with DTW.}
Consider a problem input with a data trajectory with $n+3$ points $T=<p_1', p_2', p_1, p_2, ..., p_n, p_3'>$ ($n$ is a positive integer) and a query trajectory $T_q = <p'>$. Let $d = d_{max}/2$. The locations of the points in these trajectories are provided as follows.
\begin{itemize}
	\item $p_1' = (-d/2, 0)$, $p_2' = (-d, 0)$;
	\item $p_i = (0, 0)$ for $i = 1, 2, ..., n$;
	\item $p_3' = (d, 0)$;
	\item $p' = (0, \epsilon)$, where $\epsilon$ is a very small non-negative real number;
\end{itemize}

Consider the optimal solution. It could be any subtrajectory $<p_i>$ ($1\le i \le n$) and the corresponding DTW distance is equal to $\epsilon$, which we denote by $D_o$.

Consider the approximate solution returned by PSS. It is the subtrajectory $<p_1'>$, which is explained as follows. When it scans the first point $p_1'$, it would split the trajectory at $p_1'$ and update the best-known subtrajectory to be $<p_1'>$ with the DTW distance equal to $\sqrt{d^2/4 + \epsilon^2}$. It then continues to scan the following points $p_2', p_1, ..., p_n, p_3'$ and would not perform any split operations at these points due to the fact that $p_2'$ and $p_3'$ are farther away from $p'$ than $p_1'$. As a result, $<p_1'>$ would be returned as a solution. We denote the DTW distance of this solution by $D_a$, i.e., $D_a = \sqrt{d^2/4 + \epsilon^2}$.

Consider the approximation ratio (AR). We have 
$$
\frac{D_a}{D_o} = \frac{\sqrt{d^2/4 + \epsilon^2}}{\epsilon} > \frac{d/2}{\epsilon}
$$
which approaches infinity when $\epsilon$ approaches zero.

Consider the mean rank (MR). We know that the rank of the approximate solution $<p_1'>$ is at least $\frac{n(n+1)}{2}+1$ since any subtrajectory of $<p_1, p_2, ..., p_n>$ has a smaller DTW distance than $<p_1'>$ (assuming $\epsilon = 0$). Therefore, the mean rank would approach infinity when $n$ approaches infinity.

Consider the relative rank (RR). Based on the analysis of mean rank, we know that the relative rank of the approximate solution $<p_1'>$ is at least $\frac{\frac{n(n+1)}{2}+1}{\frac{(n+3)(n+4)}{2}}$, which approaches 1 when $n$ approaches infinity.

In conclusion, the solution returned by PSS could be arbitrarily worse than the optimal one in terms of AR, MR, and RR, when the DTW distance is used.

\smallskip\noindent\textbf{Case 2: Other Algorithms and Similarity Measurements}
Consider the other algorithms, i.e., POS and POS-D. It could be verified that they would run exactly in the same way as PSS on the problem input provided in the Case 1. Therefore, the conclusion would be carried over. Consider the other measurements, namely, Frechet and t2vec. For Frechet, it could be verified that the optimal solution and the approximate solution returned by the algorithms are the same as those in the Case 1 and their Frechet distances and DTW distances to $T_q$ are equal since both solutions and $T_q$ involve one single point. As a result, the conclusion for DTW distance could be carried over for Frechet distance. For t2vec, since it is a learning-based distance - in theory, it may reduce to any possible distance metric such as DTW and Frechet. Thus, the analysis for DTW in the Case 1 could be carried over for t2vec.

}

\if 0
\section*{B. Arbitrary worse for splitting-based algorithms (PSS, POS and POS-D)}
\label{splitting-proof}
We prove the splitting-based algorithms are arbitrary worse by constructing the following cases for the approximation ratio and rank, respectively.
\subsection*{B.1 Approximation ratio analysis}
We consider two adjacent positions in a trajectory are bounded by a distance $d_{bound}$ and construct the case as follows:
\begin{equation*}
  \begin{aligned}
    &T=<p_1,p_2,\underbrace{...}_{k \text{ points}},p_*,\underbrace{...}_{k \text{ points}},p_n>, \text{and } T_q=<p_*>,
  \end{aligned}
\end{equation*}
where we instantiate the similarity with trajectory distance (e.g., DTW or Frechet by default) denoted by $D(\cdot,\cdot)$ and $dist(\cdot,\cdot)$ denotes the distance between the points (typically the Euclidean distance). Let $D(<p_1>, T_q) = d_1$, $dist(p_2, p_*) = d_2$ and $dist(p_n, p_*) = d_3$, we construct $d_1 < d_2$ and $d_1 < d_3$ and then we prove it is arbitrary worse for approximation ratio under the construction.

Run the splitting-based algorithms (PSS, POS and POS-D), we find a splitting is happened on $p_1$ due to the initial condition of these algorithms. Then, we choose to maintain the subtrajectory $<p_1>$ with the distance $d_1$ because it is smaller. We continue to scan the trajectory $T$, and we find no splitting will happen because we cannot find a smaller distance than $d_1$ from prefix $<p_2,...,p_i>$ and suffix $<p_i,...,p_n>$ for $2\leq i \leq n$ due to the boundary condition (recall the distance definition) of DTW or Frechet. Finally, these algorithms output subtrajectory $<p_1>$ with distance $d_1$ as results. Under the construction $d_1<d_2$, we can let the three points $p_1$, $p_2$ and $p_*$ form a triangle. Then, we have
\begin{equation*}
  \begin{aligned}
    &dist(p_1,p_*)+dist(p_1,p_2)>dist(p_2, p_*)\\
    &d_1>d_2-dist(p_1,p_2)>d_2-d_{bound}\\
  \end{aligned}
\end{equation*}
We know there is $k$ points between $p_2$ and $p_*$. we may assume $d_2=(k+1)*d_{bound}$, i.e., these points are collinear with the adjacent distance $d_{bound}$. Then, we further have
\begin{equation*}
  \begin{aligned}
    &d_1>(k+1)*d_{bound}-d_{bound}=k*d_{bound}\\
  \end{aligned}
\end{equation*}
We know $d_1$ increases as $k$ increases; however, the distance for the optimal solution is 0 because $T_q=<p_*>$ is a portion of $T$. Thus, the difference between the optimal distance and the approximate distance approaches arbitrary worse.

\subsection*{B.2 Rank analysis}
\label{splitting-proof-rank}
We construct the following case for rank analysis.
\begin{equation*}
  \begin{aligned}
    &T=<p_1,p_2,\underbrace{p_*,...,p_*}_{k \text{ points}},p_n>, \text{and } T_q=<p_*>.
  \end{aligned}
\end{equation*}
Here, we assume an object stays at position $p_*$ and GPS collects $k$ same points $p_*$ in the trajectory $T$. Similarly, we let $D(<p_1>, T_q) = d_1$, $dist(p_2, p_*) = d_2$ and $dist(p_n, p_*) = d_3$ and construct $d_1 < d_2$, $d_1 < d_3$. Based on the above analysis, we know splitting-based algorithms return the subtrajectory $<p_1>$ with the distance $d_1$, and there are $\frac{k(k+1)}{2}$ subtrajectories formed by the $k$ points with trajectory distance 0. Thus, the rank for these splitting-based algorithms is larger than $\frac{k(k+1)}{2}$ at least, and it increases as $k$ increases. The rank is also arbitrary worse.

\section*{C. Arbitrary worse for learning-based algorithms (RLS, RLS-Skip)}
We proof learning-based algorithms (RLS, RLS-Skip) is also arbitrary worse based on approximation ratio and rank analysis, respectively.
\subsection*{C.1 Approximation ratio analysis}
We construct the following case:
\begin{equation*}
  \begin{aligned}
    T=<p_1,\underbrace{...}_{k \text{ points}},p_*,\underbrace{...}_{k \text{ points}},p_n>, \text{and } T_q=<p_*>,
  \end{aligned}
\end{equation*}
We use the same notations as defined in the proof above. Let $dist(p_1, p_*) = d_1$ and $dist(p_n, p_*) = d_2$. We know learning-based algorithms can output arbitrary actions because it is a data-driven method. We consider the case of all actions are 0, which means no splitting will be happened during the MDP, and it will try $2*n$ subtrajectories that is prefix $<p_1, ... , p_i>$ and suffix $<p_i, ... , p_n>$ for $1 \leq i\leq n$. Similarly, we instantiate the trajectory similarity by DTW or Frechet distance, and we discuss the following two situations:
\begin{enumerate}
  \item If the returned subtrajectory from prefix $<p_1,..., p_i>$, we know $D(<p_1,..., p_i>, T_q) \geq dist(p_1, p_*)=d_1$ by DTW or Frechet definition. We know there are $k$ points between $p_1$ and $p_*$. We may assume $d_1 = (k + 1)*d_{bound}$ by constructing these points collinear with the adjacent distance $d_{bound}$. Then, $d_1$ will increase as $k$ increases; however, the distance outputted by the optimal solution is 0. Thus, the proof holds based on prefix analysis.
  \item Similarly, if the returned subtrajectory from suffix $<p_i,...,p_n>$, we know $D(<p_i,..., p_n>, T_q) \geq dist(p_n, p_*)=d_2$, and we can let the points between $p_*$ and $p_n$ collinear with the adjacent distance $d_{bound}$. Then, $d_2 = (k + 1)*d_{bound}$, and the distance difference between the optimal and the approximate is also arbitrary worse as $k$ increases.
\end{enumerate}
\subsection*{C.2 Rank analysis}
Similar to rank analysis above. We construct the following case and let all actions are 0 outputted by learning-based algorithms.
\begin{equation*}
  \begin{aligned}
    &T=<p_1,\underbrace{p_*,...,p_*}_{k \text{ points}},p_n>, \text{and } T_q=<p_*>.
  \end{aligned}
\end{equation*}
We know there are $\frac{k(k+1)}{2}$ subtrajectories formed by the $k$ same points $p_*$ with the trajectory distance 0. However, the returned distance of learning-based algorithms is either larger than $d_1$ or $d_2$ outputted by prefix or suffix, respectively. Thus, the rank of learning-based algorithms is larger than $\frac{k(k+1)}{2}$ at least, and it increases as $k$ increases. The proof for arbitrary worse based on rank holds.
\fi

==> v13 - technical/abstract.tex <==



Similar trajectory search is a fundamental problem and has been well studied over the past two decades. However, the similar subtrajectory search (SimSub) problem, aiming to return a portion of a trajectory (i.e., a subtrajectory), which is the most similar to a query trajectory, has been mostly disregarded despite that it could capture trajectory similarity in a finer-grained way and many applications take subtrajectories as basic units for analysis. In this paper, we study the SimSub problem and develop a suite of algorithms including both exact and approximate ones.
Among those approximate algorithms, two that are based on deep reinforcement learning stand out and outperform those non-learning based algorithms in terms of effectiveness and efficiency.
We conduct experiments on real-world trajectory datasets, which verify the effectiveness and efficiency of the proposed algorithms.
%Moreover, the proposed algorithms are elastic to cooperate with existing indexing techniques.}
%Moreover, it is efficient and elastic to cooperate with existing indexing methods.


==> v13 - technical/bss.tex <==
\subsection{Backward Suffix Search (BSS)}
\label{ha:bss}
We observe that the high time cost of GA is mainly due to the suffix trajectory enumeration as shown in Figure~\ref{example:ga}. In particular, every time we get a new suffix trajectory via splitting, its representation needs to be computed from scratch. Motivated by this, we propose Backward Suffix Search (BBS), aiming at saving such computational cost. Before we describe the solution, we first give an intuition.
\begin{intuition}
\label{intu}
Given two trajectories $C$ and $Q$, we encode $C$ and $Q$ from left to right by $t2vec$ and get dissimilarity value $\Psi_{forward}$.
Similarly, we encode $C$ and $Q$ from right to left and get another dissimilarity value $\Psi_{backward}$. Intuitively, $\Psi_{forward}$ should be equal to $\Psi_{backward}$ because there is no changes in their relative positions.
\end{intuition}

To compute each suffix trajectory dissimilarity value $\Psi_{S}$ in GA, we have to encode the whole suffix trajectory in each time step. If the above intuition is correct, we can first get the representation vector $h_{\overleftarrow{Q}}$ for the reverse query trajectory $\overleftarrow{Q}$, and preprocess each backward hidden vector $h'$ for $\overleftarrow{C}$ by $t2vec$. In each time step, we compute the $\Psi_{S}$ by Euclidean distance between $h_{\overleftarrow{Q}}$ and $h'$.
%More details are presented in Algorithm~\ref{bss}. 
\textcolor[rgb]{1.00,0.00,0.00}{Note that if the returned subtrajectory $C_{\Lambda}$ is a suffix trajectory, which means that the similarity $\Psi$ is obtained by encoding trajectories in reverse, so we need to adjust it to a exact value by forward encoding according to the interval $\Lambda$, and we will use the value to evaluate algorithms in experiments.}

%\begin{algorithm}[t]
%	\caption{Backward Suffix Search}
%	\footnotesize{
%		\label{bss}
%		\begin{algorithmic}[1]
%			\Require
%			Candidate trajectory $C$ and query trajectory $Q$;
%			\Ensure
%			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
%            \State get representation vector $h_{Q}$ and $h_{\overleftarrow{Q}}$ for $Q$ and $\overleftarrow{Q}$;
%            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma,\Delta \leftarrow \emptyset$, $sp \leftarrow 1$ and $h_{0}, h'_{0} \leftarrow None$;
%            \For{each time step $1 \leq t \leq |C|$}
%                \State $h'_{t} = t2vec(h'_{t-1}, x_{|c|+1-t})$;
%            \EndFor
%			\For{each time step $1 \leq t \leq |C|$}
%                \State $\Gamma \leftarrow [sp, t]$, $\Delta \leftarrow [t+1, |C|]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$;
%                \State $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$, $\Psi_{S} \leftarrow d(h_{\overleftarrow{Q}}, h'_{|C|-t})$;
%                \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
%                    \If {$\Psi_{P} < \Psi_{S}$}
%                        \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                    \Else
%                        \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
%                    \EndIf
%                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$;
%                \EndIf
%			\EndFor
%            \State adjust $\Psi$ to a true dissimilarity value if $C_{\Lambda}$ is a suffix trajectory.
%	\end{algorithmic}}
%\end{algorithm}

\begin{lemma}
\label{tc:bss}
The total time complexity of BSS is $O(n)$.
\end{lemma}

\begin{proof}
\textcolor[rgb]{1.00,0.00,0.00}{Recall that the proofing of Lemma~\ref{lemma:ga}, BSS needs to preprocess each backward hidden vector $h'$ for $\overleftarrow{C}$, which is $O(n)$. After that, we only need to compute Euclidean distance between $h_{\overleftarrow{Q}}$ and corresponding $h'$, whose complexity is $O(1)$. The adjustment operation takes $O(n)$ time, as it needs to encode the suffix trajectory by $t2vec$. Hence, the overall time cost of BSS is $O(n)$.}
\end{proof}


==> v13 - technical/conclusion.tex <==
\section{CONCLUSION}
\label{conclusion}
%Compared with trajectory similarity computation, subtrajectory similarity computation is a more general problem and can be widely used in many applications. However, it suffers from a higher computation cost.
In this paper, we study the similar subtrajectory search (SimSub) problem and develop a suite of algorithms including an exact algorithm, an approximate algorithm providing a controllable trade-off between efficiency and effectiveness, and a few splitting-based algorithms, among which some are based on pre-defined heuristics and some are based on deep reinforcement learning called RLS and RLS-Skip.
We conducted extensive experiments on real datasets, which verified that among the approximate algorithms, learning based algorithms achieve the best effectiveness and efficiency.
%, which is extended by a popular reinforcement learning framework - Deep Q Network (DQN). RLS is generic to support any existing trajectory measures and achieves the same level time complexity as trajectory similarity computation. Also, we evaluate experiments on two real-world trajectory datasets and find RLS achieves better effectiveness and efficiency performance than baselines.
%
%One possible direction for future research is to develop other indexing techniques to further accelerate the similar subtrajectory search on large-scale datasets.
%One possible direction for future research is to develop learning-based methods for other subtrajectory related problems such as subtrajectory join.
%In this paper, we demonstrate the techniques for three similarity measurements on trajectory data, namely DTW, Frechet and t2vec.
In the future, we plan to explore some more similarity measurements for the SimSub problem, e.g., the constrained DTW distance and other similarity measurements reviewed in Section~\ref{related}.


\smallskip
\noindent\textbf{Acknowledgments.} This research is supported by the Nanyang Technological University Start-UP Grant from the College of Engineering under Grant M4082302 and by the Ministry of Education, Singapore, under its Academic Research Fund Tier 1 (RG20/19 (S)).
Gao Cong acknowledges the support by Singtel Cognitive and Artificial Intelligence Lab for Enterprises (SCALE@NTU), which is a collaboration between Singapore Telecommunications Limited (Singtel) and Nanyang Technological University
(NTU) that is funded by the Singapore Government through the Industry Alignment Fund - Industry Collaboration Projects Grant, and a Tier-1 project RG114/19.
The authors would like to thank Eamonn Keogh for pointing out some references to the time series literature and also the anonymous reviewers for their constructive comments.


==> v13 - technical/dps.tex <==
\subsection{Delayed Prefix Search (DPS)}
\label{ha:dps}
We observe that PFS is involved in frequent splitting due to the lack of suffix information. In our Example~\ref{example_idea_pfs}, the splitting happens at $t=1$, $t=2$ and $t=4$ for a trajectory with only 4 points. Here, a straightforward idea is that when we find a subtrajectory, we let it wait for a few time steps $K$ and then split it out. In that case, we may find a better result. We illustrate the main idea in Example~\ref{example_idea_dps}.% and more details are presented in Algorithm~\ref{dps}.
\begin{example}
\label{example_idea_dps}
Consider a pair of candidate and query trajectory $C$, $Q$ in Figure~\ref{example:pfs}, where $t$ is the current time step and the target delayed time steps $K$ is set to 2 in this example.
\begin{itemize}[leftmargin=8pt]
  \item $t=1$, we initialize $sp$ as the current $t$, the current $delay$ as 0, the initial dissimilarity value $\Psi$ as infinity, the initial intervals $\Lambda, \Gamma$ as empty sets, and the first hidden state as none. We consider the prefix trajectory $C_{\Gamma=[1,1]}$. It is smaller than the initial dissimilarity value $\Psi$, but the current $delay$ has not reached the $K$. We skip and go to the next step.
  \item $t=2$, it gets a better dissimilarity value, but $delay$ has not reached the $K$ yet. We skip again.
  \item $t=3$, the $delay$ reaches the $K$ and gets a better result, so we split it at this time and maintain the prefix trajectory $C_{\Gamma=[1,3]}$. Then, $sp$ is updated.
  \item $t=4$, we delete the edge between 3 and 4 because a splitting happened in last time. We do not maintain $C_{\Gamma=[4,4]}$ because it is not better than current $C_{\Lambda=[1,3]}$. Hence, the final returned result is the subtrajectory with interval $\Lambda = [1,3]$.
\end{itemize}
\end{example}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/example_dps}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{An example illustrating the DPS.}\label{example:dps}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}

%\begin{algorithm}[t]
%	\caption{Delayed Prefix Search}
%	\footnotesize{
%		\label{dps}
%		\begin{algorithmic}[1]
%			\Require
%			Candidate trajectory $C$, query trajectory $Q$ and delayed steps $K$;
%			\Ensure
%			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
%            \State get representation vector $h_{Q}$ for query trajectory $Q$;
%            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma \leftarrow \emptyset$, $sp \leftarrow 1$, $h_{0} \leftarrow None$ and $delay \leftarrow 0$;
%			\For{each time step $1 \leq t \leq |C|$}
%                \State $\Gamma \leftarrow [sp, t]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$, $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$;
%                \If {$\Psi_{P} < \Psi$}
%                    \If{$delay = K$}
%                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$, $delay \leftarrow 0$;
%                    \Else
%                        \State $delay \leftarrow delay + 1$;
%                    \EndIf
%                \EndIf
%			\EndFor
%	\end{algorithmic}}
%\end{algorithm}

\begin{lemma}
The total time complexity of DPS is $O(n)$.
\end{lemma}
\begin{proof}
The delayed splitting does not cause additional calculations, so the proof is same as the PFS.
\end{proof}


==> v13 - technical/effectiveness.tex <==
\section{EXPERIMENTS}
\label{experiment}

We present the experimental set-up in Section~\ref{exper_setup} and then the experimental results in Section~\ref{effectiveness}.

\subsection{Experimental Setup}
\label{exper_setup}

\smallskip
\noindent\textbf{Dataset.} Our experiments are conducted on three real-world trajectory datasets. The first dataset, denoted by Porto, is collected from the city of Porto~\footnote{https://www.kaggle.com/c/pkdd-15-predict-taxi-service-trajectory-i/data}, Portugal, which consists around 1.7 million taxi trajectories over 18 months with a sampling interval of 15 seconds and a mean length around 60. %and each location sampled at 15 second intervals.
%After filtering the trajectories with fewer than 30 sampling points, we obtain 1.2 million trajectories with a mean length around 60.
The second dataset, denoted by Harbin, involves around 1.2 million taxi trajectories collected from 13,000 taxis over 8 months in Harbin, China with non-uniform sampling rates and a mean length around 120.
%After removing the trajectories with fewer than 30 points, we get over 1 million trajectories with a mean length around 120.
The third dataset, denoted by Sports, involves around 0.2 million soccer player and ball trajectories collected from STATS Sports~\footnote{https://www.stats.com/artificial-intelligence (STATS, copyright 2019)} with a uniform sampling rate of 10 times per second and a mean length around 170.

\smallskip
\noindent\textbf{Parameter Setting.} For training t2vec model, we follow the original paper~\cite{li2018deep} by excluding those trajectories that are short and use their parameter settings.
%
For SizeS, we use the setting $\xi = 5$ (with the results of its effect shown later on).
%The default value of $\xi$ in PSS is set at 5 and we will report the effect of the parameter $\xi$ in our experiments.
For POS-D, we vary the parameter $D$ from 4 to 7, and since the results are similar, we use the setting $D = 5$.
%
For the neural networks involved in the RL-based algorithms, i.e., RLS and RLS-Skip, we use a feedforward neural network with 2 layers. In the first layer, we use the ReLu function with 20 neurons, and in the second layer, we use the sigmoid function with $2+k$ neurons as the output corresponding to different actions, where for RLS we use $k=0$ and for RLS-Skip, we use $k = 3$ by default.
%Note that when $k=0$, that is RLS; otherwise, that is RLS-Skip. We vary $k$ from 1 to 5 for RLS-Skip, the default $k$ is 3 and we will report the effect of the hyperparameter in experiments.}
In the training process, the size of replay memory $\mathcal{M}$ is set at 2000. We train our model on 25k random trajectory pairs, using Adam stochastic gradient descent with an initial learning rate of 0.001. The minimal $\epsilon$ is set at 0.05 with decay 0.99 for the $\epsilon$-greedy strategy, and the reward discount rate $\gamma$ is set at 0.95.

\smallskip
\noindent\textbf{Compared Methods.} We compare RL-based Search (RLS), RL-based Search with skipping (RLS-Skip) and the proposed non-learning based algorithms (Section~\ref{sec:non-learning}), namely ExactS, SizeS, PSS, POS, and POS-D.
%
For RLS and RLS-Skip, when t2vec is adopted, we ignore the $\Theta_{suf}$ component of a state based on empirical findings.


%
In addition, we consider three competitor methods, namely UCR~\cite{mueen2016extracting,rakthanmanon2012searching,rakthanmanon2013addressing}, Spring~\cite{sakurai2007stream},
and Random-S.
UCR was originally developed for searching subsequences of a time series, which are the most similar to a query time series and the similarity is based on the DTW distance. UCR enumerates all subsequences that are of the same length of the query time series and employs a rich set of techniques for pruning many of the subsequences.
%Spring is designed for the problem of finding a subsequence of a data time series, which is the most similar to a query time series.
%Spring corresponds to the dynamic programming process for computing the DTW or Frechet distance between the data time series and the query time series, where the latter is padded with a fictitious point that could be aligned with any point of the data time series with distance equal to 0.
We adapt UCR for our similar subtrajectory search problem (details of adaptions are provided in the appendix of the technical report version~\cite{TR}).
We note that UCR only works for DTW, but not for Frechet or t2vec.
% and Spring works for both DTW and Frechet, but not for t2vec.
Spring is an existing algorithm for searching a subsequence of a time series, which is the most similar to a query time series. It is designed for DTW.
Random-S randomly samples a certain number of subtrajectories of data trajectory and among them, returns the one with the highest similarity to the query trajectory. Since these methods are either not general for all similarity measurements (e.g., UCR) or involve some parameter that is difficult to set (e.g., Random-S with a parameter of sample size), we compare these two competitor methods with our RLS-Skip algorithm only in terms of effectiveness and efficiency.
%

%Note that for DTW and Frechet distance we  modify GA by reading suffix trajectories from right to left, and thus do not need the BSS method. {\bf Gao not clear.. BCC is the same as GA for DTW?}
%
%In addition, inspired by the algorithms for approximate matching for substring and subsequence~\cite{kim2013efficient,zhang2010bed,gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked,moon2001duality,faloutsos1994fast}, we further propose a baseline, called Fixed-Length Search (FLS) with soft margin $\xi$. Specifically, we search the subtrajectories with lengths from $|Q|-\xi$ to $|Q|+\xi$ in the candidate trajectory $C$, where $|Q|$ denotes the length of query trajectory and $\xi\in[0,|Q|)$. In case the fixed search lengths exceed the length of candidate trajectory $C$, we further limit the search bound from $min(|Q|-\xi,|C|)$ to $min(|Q|+\xi,|C|)$. Note that the result will get better as $\xi$ gets larger although the time cost will increase, and in extreme cases it may return the same result as the exact algorithm.
%
\begin{figure}[t]
	\centering
	\begin{tabular}{c c c}
		\centering
		\begin{minipage}{2.6cm}%5.5
			\includegraphics[width=2.8cm]{effect_t2v_ar_v2}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.8cm]{effect_t2v_mr_v2}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.8cm]{effect_t2v_rr_v2}
		\end{minipage}
		\\
		\scriptsize{(a) AR (t2vec)}
		&
		\scriptsize{(b) MR (t2vec)}
		&
		\scriptsize{(c) RR (t2vec)}
		\\
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.8cm]{effect_dtw_ar_v2}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.8cm]{effect_dtw_mr_v2}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.8cm]{effect_dtw_rr_v2}
		\end{minipage}
		\\
		\scriptsize{(d) AR (DTW)}
		&
		\scriptsize{(e) MR (DTW)}
		&
		\scriptsize{(f) RR (DTW)}
		\\
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.8cm]{effect_fre_ar_v2}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.8cm]{effect_fre_mr_v2}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.8cm]{effect_fre_rr_v2}
		\end{minipage}
		\\
		\scriptsize{(g) AR (Frechet)}
		&
		\scriptsize{(h) MR (Frechet)}
		&
		\scriptsize{(i) RR (Frechet)}
	\end{tabular}
	%\setlength{\belowcaptionskip}{1pt}
	%\vspace{-2mm}
	\caption{Effectiveness for t2vec (a)-(c), DTW (d)-(f) and Frechet (g)-(i).}
	\label{effect_result}
	%\vspace{-2mm}
\end{figure}
\begin{figure}[t]
	%	\hspace*{-.5cm}
	\centering
	\begin{tabular}{c c c}
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{without_t2v_p}
		\end{minipage}
		%		&
		%		\begin{minipage}{2.6cm}
		%			\includegraphics[width=2.85cm]{without_t2v_h}
		%		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{without_dtw_p}
		\end{minipage}
		%		&
		%		\begin{minipage}{2.6cm}
		%			\includegraphics[width=2.85cm]{without_dtw_h}
		%		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{without_fre_p}
		\end{minipage}
		%		&
		%		\begin{minipage}{2.6cm}
		%			\includegraphics[width=2.85cm]{without_fre_h}
		%		\end{minipage}
		\\
		\scriptsize (a) Porto (t2vec)
		%		&
		%		\scriptsize (b) Harbin (t2vec)
		&
		\scriptsize (b) Porto (DTW)
		%		&
		%		\scriptsize (d) Harbin (DTW)
		&
		\scriptsize (c) Porto (Frechet)
		%		&
		%		\scriptsize (f) Harbin (Frechet)
		\\
		
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{rtree_t2v_p}
		\end{minipage}
		%		&
		%		\begin{minipage}{2.6cm}
		%			\includegraphics[width=2.85cm]{rtree_t2v_h}
		%		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{rtree_dtw_p}
		\end{minipage}
		%		&
		%		\begin{minipage}{2.6cm}
		%			\includegraphics[width=2.85cm]{rtree_dtw_h}
		%		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{rtree_fre_p}
		\end{minipage}
		%		&
		%		\begin{minipage}{2.6cm}
		%			\includegraphics[width=2.85cm]{rtree_fre_h}
		%		\end{minipage}
		\\
		\scriptsize (d) Porto (t2vec)
		%		&
		%		\scriptsize (h) Harbin (t2vec)
		&
		\scriptsize (e) Porto (DTW)
		%		&
		%		\scriptsize (j) Harbin (DTW)
		&
		\scriptsize (f) Porto (Frechet)
		%		&
		%		\scriptsize (l) Harbin (Frechet)
		
		%		&
		%		\scriptsize (r) Harbin (Frechet)
	\end{tabular}
	%\vspace{-2mm}
	\caption{Efficiency without index (a)-(c) and with R-tree index (d)-(f) on Porto.}
	\label{fig:efficiencyRLS}
	%	\vspace{-2mm}
\end{figure}

\smallskip
\noindent\textbf{Evaluation Metrics.} We use three metrics to evaluate the effectiveness of an approximate algorithm. (1) Approximate Ratio (AR): It is defined as %$\frac{\Psi_{app}}{\Psi_{opt}}$, where $\Psi_{app}$ is
the ratio between the dissimilarity of the solution wrt a query trajectory, which is returned by an approximate algorithm, and that of the solution returned by an exact algorithm.
%AR measures the performance of an online algorithm by the distance between the optimal solution, and thus
A smaller AR indicates a better algorithm.
(2) Mean Rank (MR): %MR is a rank-based metric. Consider a trajectory pair $(C, Q)$,
We sort all the subtrajectories of a data trajectory in ascending order of their dissimilarities wrt a query trajectory. %obtained by the exact algorithm, and
MR is defined as the rank of the solution returned by an approximate algorithm.
%, denoted by $rank_{T}(T_{\Lambda})$.
%We report the mean number of $rank_{T}(T_{\Lambda})$ as MR.
(3) Relative Rank (RR): %For the candidate trajectories $C$ with different lengths,
RR is a normalized version of MR by the total number subtrajectories of a data trajectory.
%As the number of subtrajectories of a data trajectory $T$ varies a lot, we normalize the rank by the number of subtrajectories, i.e., $\frac{rank_{T}(T_{\Lambda})}{\#subt_{T}}$, where $\#subt_{T} = \frac{|T|(|T|+1)}{2}$. We call the metric Relative Rank (RR).
A smaller MR or RR indicates a better algorithm.

%is also different. Here, we denote the RR as the mean number of $\frac{rank_{C}(C_{\Lambda})}{\#subt_{C}}$, where $\#subt_{C}$ is the total number of subtrajectories of $C$, if the length of $C$ is $n$,  $\#subt_{C} = \frac{n(n+1)}{2}$.

\smallskip
\noindent\textbf{Evaluation Platform.} All the methods are implemented in Python 3.6. The implementation of RLS is based on Keras 2.2.0. The experiments are conducted on a server with 32-cores of Intel(R) Xeon(R) Gold 6150 CPU @ 2.70GHz 768.00GB RAM and one Nvidia Tesla V100-SXM2 GPU.

\subsection{Experimental Results}
\label{effectiveness}

\noindent\textbf{(1) Effectiveness results.}
%We evaluate the effectiveness of the proposed approximate algorithms, including SizeS, PSS, POS,  POS-D, RLS and RLS-Skip, in terms of three evaluation metrics. Specifically,
We randomly sample 10,000 trajectory pairs from a dataset, and for each pair we use one trajectory as the query trajectory to search the most similar subtrajectory from the other one.
%
%Next, we report the results of different methods under three evaluation metrics (AR, MR and RR) on
Figure~\ref{effect_result} shows the results.
% of different algorithms on two datesets, using three trajectory similarity measurements, namely, t2vec, DTW and Frechet.
%
The results clearly show that
%the proposed learning-based algorithms including
RLS and RLS-Skip consistently outperform all other non-learning based approximate algorithms in terms of all three metrics on both datasets and under all three trajectory similarity measurements.
%
For example, RLS outperforms POS-D, the best non-learning algorithm when using t2vec, by 70\% (resp. 83\%) in terms of RR on Porto (resp. Harbin); RLS outperforms PSS, the best non-learning based algorithm when using DTW, by 25\% (resp. 20\%) in terms of MR on Porto (resp. Harbin); RLS outperforms PSS, the best non-learning based algorithm when using Frechet, by 25\% (resp. 20\%) in terms of MR on Porto (resp. Harbin).
%
%compare GA and others.
Among PSS, POS, and POS-D, PSS performs the best for DTW and Frechet; However, for t2vec, PSS provides similar accuracy as POS and POS-D on Porto, but performs much worse on Harbin.
%
The reason is that for DTW and Frechet, PSS computes exact similarity values for suffix subtrajectories, while for t2vec, it computes only approximate ones. Therefore, PSS has a relatively worse accuracy when used for t2vec.
%
%The reason that for t2vec, PSS performs relatively better on Porto than on Harbin could be that the mean length of trajectories of Porto (around 60) is smaller than that of Harbin (around 120), and thus PSS is likely to make more incorrect splitting decisions on Harbin based on the approximate similarity values estimated for the suffix trajectories.
%, but when we evaluate the final results on the ground truth, its results will get worse,
%
%This is because the mean length of trajectories of Porto (around 60) is smaller than Harbin (around 120), and BSS will be more likely to incorrectly maintain an approximate suffix trajectory during the search process, but when we evaluate the final results on the ground truth, its results will get worse,
%
%compare PFS and DPS
%As expected, POS-D performs slightly better than POS in terms of accuracy since it essentially checks more subtrajectories for choosing points for splitting.
% {\bf Gao this result is strange... DPS should be better. why worse.. this cannot be explained. }
 %Note that for DPS, we tune the parameter of delayed steps and report the best results in this experiment, and we do not report the detailed parameter study of this part due to the space limitation.
%
% and observe similar results of them on the two datasets because DTW and Frechet are both point-matching based similarity measurements and thus they have a high consistency between results.
%In addition, we observe DMS is inferior to BSS because there are two models for DMS method during the search, and it is difficult to guarantee their similarity distributions.
%
We also observe that SizeS is not competitive compared with other approximate algorithms.
% as it simply increases the search space to check more subtrajectories.
%
In addition, RLS-Skip has its effectiveness a bit worse than RLS, but still better than those non-learning based algorithms due to the fact that it is based on a learned policy for decision making.
%RLS-Skip as a variant of RLS for efficiently pruning candidate subtrajectories during the search, it loses some effectiveness slightly because it uses approximate states to guide the model decisions.
%

%GA and FLS (with $\xi=5$) are two competitive methods for RLS on t2vec measurement; however, they are involved in a high time cost, and we will evaluate their efficiency in Section~\ref{effi_evaluation} and parameter study for $\xi$ in Section~\ref{para_study}.

%As expected, RLS consistently outperforms the compared methods for different similarity measurements under different evaluation metrics.





\smallskip
\noindent\textbf{(2) Efficiency results.}
We prepare different databases of data trajectories by including different amounts of trajectories from a dataset and vary the total number of points in a databases.
For each database, we randomly sample 10 query trajectories from the dataset, run for each query trajectory a query for finding the top-50 similar subtrajectories, and then collect the average running time over 10 queries.
The results of running time on the Porto dataset are shown in Figure~\ref{fig:efficiencyRLS}, and those on the other datasets could be found in the technical report~\cite{TR}.
% To better evaluate the efficiency of the proposed algorithms, we perform subtrajectory similarity search on a set of 50 data trajectories, rather than on one trajectory. For a query, we return the most similar subtrajectory that is contained in each of the 50 data trajectories
% and collect the average running time.
%
%This set of experiments is to report the efficiency results for subtrajectory similarity search~\footnote{Without loss of generality, we define each candidate trajectory can only return one of the most similar subtrajectory in the KNN search.} with top-$k=50$.
%
%The average running time of different algorithms is shown in
%The results are shown in
%Figure~\ref{fig:efficiencyRLS}, where we vary the number of points in the trajectory database.
%Note that the complexity of all methods is directly related to the number of points in the data trajectory.
%
RLS-Skip runs the fastest
since on those points that have been skipped,
the cost of maintaining the states and making decisions is saved.
In contrast, none of the other algorithms skip points.
%
ExactS has the longest running time, e.g., ExactS is usually around 7-15 times slower than PSS, POS, POS-D, RLS and 20-30 times slower than RLS-Skip.
%, which have the same time complexity.
%
%PSS, POS, POS-D, RLS and RLS-Skip have similar running time for DTW and Frechet. This is expected as they have the same time complexity.
%We also observe that
RLS is slightly slower than PSS, POS, POS-D.
This is because RLS makes the splitting decision via a learning model while the other three use a simple similarity comparison.
%{\color{red} In terms of RLS-Skip, this is expected it performs the fastest among all methods. This is because RLS-Skip can efficient skip (or prune) some points, and computations only spend on some of points in a data trajectory.}
%
%\textcolor[rgb]{1.00,0.00,0.00}{The running time of SizeS is close to that of ExactS for t2vec, and it is much faster than ExactS for DTW and Frechet. This is because the incremental computation for t2vec is $O(1)$; however, it is $O(m)$ for DTW and Frechet, and thus the time gap will more obvious when the number of points increase.
%{\bf Gao how to explain this result?}}
%
%We compare the time efficiency of RLS with heuristic algorithms (GA, PFS, DPS, BSS, DMS), Exact and FLS. For t2vec, Exact and GA perform extremely slow because the overall time cost of those is square to the number of the points over a database. Moreover, GA is slightly larger than Exact. This is because compared with Exact, GA needs to additionally calculate the prefix similarities in addition to encoding each suffix trajectories. FLS has an approximate quadratic computational complexity, and therefore it is slightly lower than Exact. RLS, PFS, DPS, BSS and DMS have similar running time because they are all linear methods; however, we can observe RLS is a little higher than the others because the split decision at each time step is determined by the learning model rather than a simple similarity comparison used in heuristic algorithms. With regard to DTW and Frechet, GA is further speeded up because of the proof of Lemma~\ref{dtw_sim_nochange}, and thus it has the same quadratic time complexity with RLS, PFS and DPS. Similarly, Exact still performs extremely slow because of the super-cubic time complexity for the point-matching based measurement, and FLS is between the Exact and heuristic algorithms.
%
%We also observe that each algorithm takes longer to run on Harbin than on Porto, especially for DTW and Frechet. This is possibly because the average trajectory length of Harbin is around 120 and that of Porto is around 60.

%, and the time complexity of . For example, in terms of the results without index, when we increased the data size from 0.4 to 2.0 on Porto, Exact took from 3019 seconds to 13531 seconds for t2vec in Figure~\ref{fig:efficiencyRLS}(a), while it took from 3853 seconds to 18691 seconds on Harbin in Figure~\ref{fig:efficiencyRLS}(b).


%\subsection{Other Experimental Results}
%\subsection{Efficiency Evaluation}
%

\smallskip
\noindent\textbf{(3) Scalability.} We investigate the scalability of all the algorithms based on the results reported in Figure~\ref{fig:efficiencyRLS}.
%As can be seen, all the algorithms scale nearly linearly with the number of points in the database.
%We also observe that PSS, POS, POS-D, RLS and RLS-Skip scales better than the other algorithms, such as ExactS, and the disparity between them with ExactS becomes larger as the size of the dataset increases.
All those splitting-based algorithms including PSS, POS, POS-D, RLS and RLS-Skip scale well. 
%In particular, RLS-Skip runs for less than 100s on all datasets for all similarity measurements with the Inverted Index.

%For example, RLS is around 10 times faster than ExactS for DTW and Frechet.
%(zheng: the result in DTW and Frechet is around 10.4, in 2vec is around 7.6 times for all data size)
%when the data size is 0.4 million, RLS is 10.4 times faster than ExactS; When the data size is 2 million, RLS is...

%evaluate the scalability of all methods on Porto and Harbin datasets. As Figure~\ref{fig:efficiencyRLS}(a)-(r) suggested, the nearly linear scalability is obvious, and the
%performance gap between the exact algorithms and approximation algorithms tended to be bigger when the data size was increasing.

%\noindent\textbf{Comparison with datasets.} We observe similar performance on the two datasets Porto and Harbin. In addition, we know the average length of Harbin dataset (around 120) is bigger than Porto (around 60), and thus the corresponding time is also costly. For example, in terms of the results without index, when we increased the data size from 0.4 to 2.0 on Porto, Exact took from 3019 seconds to 13531 seconds for t2vec in Figure~\ref{fig:efficiencyRLS}(a), while it took from 3853 seconds to 18691 seconds on Harbin in Figure~\ref{fig:efficiencyRLS}(b).

%\noindent\textbf{Comparison with similarity measurements.} DTW and Frechet are both point-matching based similarity measurements and share a similar formulation, and therefore a similar performance and time cost are consistently under the different datasets and indexes. Regarding the t2vec, it is not very fast for the online scenario, because it needs to call deep learning model step by step on the incremental computing and resulting in some extra cost. For example in Figure~\ref{fig:efficiencyRLS}(a), (c) and (e), Exact with t2vec (3019 seconds to 13531 seconds) achieves only around $2-3\times$ speedup over DTW (5740 seconds to 27876 seconds) and Frechet (7024 seconds to 34383 seconds).

\smallskip
\noindent\textbf{(4) Working with indexes.}
%Our proposed algorithms are able to work with indexes to further improve the efficiency of subtrajectory similarity search.
%We further study the effect of indexes for subtrajectory similarity search.
Following two recent studies~\cite{yao2019computing, wang2018torch} on trajectory similarity search, we employ the Bounding Box R-tree Index for boosting the efficiency. 
%two indexes: Bounding Box R-tree Index and Grid-based Inverted Index. 
%
%The first one builds a R tree, indexing
It indexes the MBRs of data trajectories and prunes all those data trajectories whose MBRs do not interact with the MBR of a given query trajectory.
%The second one partitions the space into cells, maintains for each cell the ids of the trajectories traveling through the cell, and then restrict the search on the trajectories whose ids are among those maintained by the cells traveled through by a given query trajectory.
%
%We use 100m by 100m cells for Porto and Harbin and 1m by 1m cells for Sports.
%
We note that in theory, exact solutions might be filtered out by the index (e.g., the most similar subtrajectory may be part of a trajectory, whose MBR does not interact with that of a query one), but in practice, this rarely happen. For example, as found in our experiments on the Porto dataset, when DTW and Frechet are used, the results returned when using the index and those when using no indexes are exactly the same, i.e., no results are missed out. When t2vec is used, at most 20\% results are missed.  Furthermore, for cases of finding approximate solutions, as most of the proposed algorithms do, missing some potential solutions for better efficiency is acceptable.
%
%We do not employ those indexes and pruning methods that are specially designed for a specific trajectory similarity measurement as they cannot be applied to other similarity measurements and/or subtrajectory similarity search.
%
Compared with the results without indexes in Figure~\ref{fig:efficiencyRLS}(a)-(c), the results using the R-tree index as shown in Figure~\ref{fig:efficiencyRLS}(d)-(f) are lower by around 20--30\%.
% and the results based on the Inverted Index as shown in Figure~\ref{fig:efficiencyRLS}(g)-(i) are further lower.


%Compared with the results without indexes in Figure~\ref{fig:efficiencyRLS}(a)-(f), the results using the R-tree index shown in Figure~\ref{fig:efficiencyRLS}(g)-(l) show around 10--20\% reduction in running time. The results based on the Inverted Index are shown in Figure~\ref{fig:efficiencyRLS}(m)-(r), and according to these results, the speedups are around 30 times.

\begin{figure}[!t]
	%	\hspace*{-.5cm}
	\centering
	\begin{tabular}{c c c}
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{t2v_rr_p}
			%\includegraphics[width=2.85cm]{porto_t2vec_without}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{dtw_rr_p}
			%\includegraphics[width=2.85cm]{porto_dtw_without}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			\includegraphics[width=2.85cm]{fre_rr_p}
			%\includegraphics[width=2.85cm]{porto_frechet_without}
		\end{minipage}
		\\
		\scriptsize (a) Porto (t2vec)
		&
		\scriptsize (b) Porto (DTW)
		&
		\scriptsize (c) Porto (Frechet)
		% \\
		%   \begin{minipage}{2.6cm}
		%	\includegraphics[width=2.85cm]{n_porto_t2vec_without}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{2.6cm}
		%	\includegraphics[width=2.85cm]{n_porto_dtw_without}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{2.6cm}
		%	\includegraphics[width=2.85cm]{n_porto_fre_without}
		%  \end{minipage}
		%  \\
		%  \scriptsize (d) Porto (t2vec)
		%  &
		%  \scriptsize (e) Porto (DTW)
		%  &
		%  \scriptsize (f) Porto (Frechet)
	\end{tabular}
	%\vspace{-2mm}
	\caption{Effectiveness with varying query lengths.}
	\label{RR:querylength}
	%	\vspace{-2mm}
\end{figure}

\begin{figure}[!t]
	%	\hspace*{-.5cm}
	\centering
	\begin{tabular}{c c c}
		\begin{minipage}{2.6cm}
			%\includegraphics[width=2.85cm]{t2v_rr_p}
			\includegraphics[width=2.85cm]{porto_t2vec_without}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			%\includegraphics[width=2.85cm]{dtw_rr_p}
			\includegraphics[width=2.85cm]{porto_dtw_without}
		\end{minipage}
		&
		\begin{minipage}{2.6cm}
			%\includegraphics[width=2.85cm]{fre_rr_p}
			\includegraphics[width=2.85cm]{porto_frechet_without}
		\end{minipage}
		\\
		\scriptsize (a) Porto (t2vec)
		&
		\scriptsize (b) Porto (DTW)
		&
		\scriptsize (c) Porto (Frechet)
		% \\
		%   \begin{minipage}{2.6cm}
		%	\includegraphics[width=2.85cm]{n_porto_t2vec_without}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{2.6cm}
		%	\includegraphics[width=2.85cm]{n_porto_dtw_without}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{2.6cm}
		%	\includegraphics[width=2.85cm]{n_porto_fre_without}
		%  \end{minipage}
		%  \\
		%  \scriptsize (d) Porto (t2vec)
		%  &
		%  \scriptsize (e) Porto (DTW)
		%  &
		%  \scriptsize (f) Porto (Frechet)
	\end{tabular}
	%\vspace{-2mm}
	\caption{Efficiency with varying query lengths.}
	\label{time:querylength}
	%\vspace{-2mm}
\end{figure}

\smallskip \noindent\textbf{(5) The effect of query trajectory length.}
%To evaluate the effect of query length on the effectiveness of the proposed approximate algorithms,
We prepare four groups of query trajectories from a dataset, namely $G1$, $G2$, $G3$, and $G4$, each with 10,000 trajectories, such that the lengths of the trajectories in a group are as follows: $G1=[30,45)$, $G2=[45,60)$, $G3=[60,75)$ and $G4=[75,90)$. Then, for each query trajectory, we prepare a data trajectory from the dataset. Note that for a query trajectory and a corresponding data trajectory, the latter may be longer than or shorter than the former.
%
For each group, we report the average results.
%
The results of RR on Porto are shown in Figure~\ref{RR:querylength}.
%
%In terms of different similarity measurements, we can see that DTW (g)-(l) and Frechet (m)-(r) are consistently similar under the three evaluation metrics AR, MR and RR because they are both point-matching based distance, and t2vec also shows consistent performance for Porto and Harbin.
%
We observe that the RRs of all algorithms except for SizeS remain stable when the query length grows.
%However, the accuracy of SizeS
For SizeS, the RRs fluctuate with the change of the query length. This is because the length of the most similar subtrajectory may not have similar length as the query trajectory, and thus it may miss high-quality results when the search space is constrained by the parameter $\xi$.
%
%Figure~\ref{time:querylength}(a)-(c) shows the effect of query length on the running time.
The results of running time on Porto are shown in Figure~\ref{time:querylength}.
We notice that for t2vec, the running times of all the algorithms are almost not affected by the query length. This is because for t2vec, the time complexity of computing a similarity is constant once the vector of the query trajectory is learned. For DTW, Frechet, the time complexity of computing a similarity increase with the query length, as shown in Table~\ref{tab:algorithm-complexities}.
%{\color{blue}Furthermore, we fix the query trajectory and vary the length of data trajectory, and the results are illustrated in Figure~\ref{time:querylength} (d)-(f). As expected, the running times of all the algorithms are consistently with the Table~\ref{tab:algorithm-complexities} as well.}
%
% bounded computations~\cite{rakthanmanon2012searching, keogh2005exact} are another acceleration method, which is achieved by estimating the lower bound for pruning; however, it cannot be guaranteed for our subtrajectory search and thus we do not use it in this experiment.
%
\if 0
Compared with the results without indexes in Figure~\ref{fig:efficiencyRLS}(a)-(f), the results using the R-tree index shown in Figure~\ref{fig:efficiencyRLS}(g)-(l) show around 10--20\% reduction in running time. The results based on the Inverted Index are shown in Figure~\ref{fig:efficiencyRLS}(m)-(r), and according to these results, the speedups are around 30 times.
\fi
 % because a huge number of maximum bounding rectangles (MBR) have an interaction relationship, and a simple grid index in Figure~\ref{fig:efficiencyRLS}(m)-(r) can be considered as a more useful index structure in such scenarios and it achieves around $30\times$ speedup.

%\begin{figure}
%\centering
%\begin{tabular}{c c c}
%  \begin{minipage}{4cm}%5.5
%	\includegraphics[width=4cm]{par_ar}
%  \end{minipage}
%  &
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{par_mr}
%  \end{minipage}
%  \\
%  \scriptsize{(a) Approximation Ratio}
%  &
%  \scriptsize{(b) Mean Rank}
%  \\
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{par_rr}
%  \end{minipage}
%  &
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{par_time}
%  \end{minipage}
%  \\
%  \scriptsize{(c) Relative Rank}
%  &
%  \scriptsize{(d) Time Cost}
%  \end{tabular}
%  \setlength{\belowcaptionskip}{1pt}
%\caption{The influence of soft margin $\xi$ in FLS.}
%\label{para_fls}
%\vspace*{-2mm}
%\end{figure}

%\subsection{Problem Comparison}
%Regarding the efficiency, the time cost of SSC with RLS ia slightly larger than TSC. This is as expected and we explain as follows: (1) for point-matching based measurements DTW and Frechet, we need to read trajectories from right to left to get suffix similarities, which is equivalent to a one time TSC; (2) we compute prefix similarities incrementally and it is also equivalent to a one time TSC; (3) we need to call the learning model to obtain a split decision at each time step; (4) note that in t2vec, we do not need to compute the suffix similarities as input, and thus t2vec (around $3\times$ TSC) is faster than DTW and Frechet (around $5\times$ TSC).
 %\subsection{Parameter Study}\label{para_study}
\begin{table}[!t]
	\centering
	\scriptsize
%	\hspace*{-.3cm}
	\caption{The effect of skipping steps $k$ for RLS-Skip.}
	\begin{tabular}{|c|c|c|c|c|c|c|c|}
		\hline
		Metrics & $k=0$ &$k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$\\ \hline
		AR  &1.028 &1.039 &1.042 &1.044  &1.055 &1.069 \\
		MR  &41.138 &56.633 &58.077 &64.741 &70.281 &94.356 \\
		RR  &3.5\% &5.4\% &5.6\% &5.8\% &6.3\% &8.9\% \\
		Time (ms)    &55.2 &39.8 &38.5 &35.8 &31.8 &22.9 \\ \hline
		Skip Pts &0\% &3.1\% &13.1\% &17.7\% &29.5\% &47.6\% \\ \hline
	\end{tabular}
	%\vspace{-2mm}
	\label{para_steps}
\end{table}
\begin{table*}[t!]
	\centering
	\scriptsize
%	\hspace*{-.3cm}
	\caption{Comparison with Trajectory Similarity Computation and Subtrajectory Similarity Computation.}
	\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
		\hline
		\multicolumn{2}{|c|}{Similarity} & \multicolumn{4}{c|}{t2vec} & \multicolumn{4}{c|}{DTW} & \multicolumn{4}{c|}{Frechet} \\ \hline
		Dataset                    & Problem    & AR  & MR  & RR  & Time (ms) & AR  & MR & RR & Time (ms) & AR   & MR  & RR  & Time (ms)  \\ \hline
		\multirow{2}{*}{Porto}     & SimTra        &1.313     &156.153     &23.3\%     &28.5          &2.100     &752.831    &70.7\%    &18.1          &1.883      &559.462     &56.5\%     &19.2           \\ \cline{2-14}
		& SimSub        &1.098     &18.323     &3.0\%     &39.6          &1.028     &41.138    &3.5\%    &55.2          &1.034      &34.162     &3.6\%     &69.6           \\ \hline
		\multirow{2}{*}{Harbin}    & SimTra        &1.293     &678.311     &46.9\%     &31.7          &2.326     &1218.908    &72.2\%    & 27.1          &1.891      &854.042     &53.9\%     &28.6        \\ \cline{2-14}
		& SimSub        &1.025     &14.945     &1.3\%     &62.6          &1.081     &75.324    &4.1\%    & 114.4         &1.045      &64.729     &4.4\%     &130.6       \\ \hline
		\multirow{2}{*}{Sports}    & SimTra        &1.221     &345.488    &43.4\%     &46.1          &1.659    &4291.666   &59.8\%   &107.5         &1.403      &3272.743     &48.2\%    &133.3        \\ \cline{2-14}
		& SimSub        &1.045     &28.761     &3.8\%     &210.3          &1.005    &126.334   &2.1\%   &254.7         &1.002      &95.280     &1.7\%    &302.3       \\ \hline
	\end{tabular}
	%\vspace*{-2mm}
	\label{tscssc}
\end{table*}

\smallskip
\noindent\textbf{(6) The effect of skipping steps $k$.}
%This part is to evaluate the influence of the skipping steps $k$ for RLS-Skip.
According to the results, a general trend is that with larger settings of $k$, RLS-Skip has its effectiveness drop but its efficiency grow because RLS-Skip tends to skip more points.
We present in Table~\ref{para_steps} the results on Porto for DTW only due to the page limit. We also report the portion of skipped points in the Porto dataset with 10,000 trajectories. Note that when $k$ is set to 0, RLS-Skip degrades to RLS. For other experiments, we choose $k=3$ as a reasonable trade-off between effectiveness and efficiency.
%Additionally, we can observe that the time change of DTW and Frechet is more significantly than t2vec as $\xi$ increases. This is because the incremental computation for DTW and Frechet is linear, which is higher than the constant update of t2vec as shown in Lemma~\ref{dtw_time}.

\smallskip
\noindent\textbf{(7) The effect of parameter $\xi$.} 
%This experiment is to evaluate the effect of the soft margin $\xi$ for SizeS. 
%Intuitively, a big $\xi$ value indicates a larger search space, which approaches the search space of the ExactS algorithm as $\xi$ increases. Therefore, SizeS will check more candidate subtrajectories and its running time  will increase.
Figure~\ref{para_fls} shows SizeS's RR and running time averaged on 10,000 trajectory pairs from the Porto dataset. 
%In Figure~\ref{para_fls}, we increase the value of $\xi$ until the result of SizeS is better than that of RLS and RLS-Skip in terms of AR, MR and RR.
%, and at the same time, we show the RLS and Exact results for ease of reference.
As expected, as $\xi$ grows, the RR of SizeS becomes better, but running time increases and approaches to that of ExactS.

\begin{figure}[t]
	\hspace{-0.4cm}
	\centering
	\begin{tabular}{c c}
		%  \begin{minipage}{4cm}
		%  \includegraphics[width=4.15cm]{t2v_ar}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{4cm}
		%    \includegraphics[width=4.15cm]{t2v_mr}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{4cm}
		%  \includegraphics[width=4.15cm]{t2v_rr}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{4cm}
		%    \includegraphics[width=4.15cm]{t2v_time}
		%  \end{minipage}
		%  \\
		%  \small (a) Approximation Ratio (t2vec)
		%  &
		%  \small (b) Mean Rank (t2vec)
		%  &
		%  \small (c) Relative Rank (t2vec)
		%  &
		%  \small (d) Time Cost (t2vec)
		%  \\
		%		\begin{minipage}{4cm}
		%			\includegraphics[width=4.15cm]{dtw_ar}
		%		\end{minipage}
		%		&
		%		\begin{minipage}{4cm}
		%			\includegraphics[width=4.15cm]{dtw_mr}
		%		\end{minipage}
		%		&
		\begin{minipage}{4cm}
			\includegraphics[width=4.15cm]{dtw_rr}
		\end{minipage}
		&
		\begin{minipage}{4cm}
			\includegraphics[width=4.15cm]{dtw_time}
		\end{minipage}
		\\
		%		\small (a) Approximation Ratio (DTW)
		%		&
		%		\small (b) Mean Rank (DTW)
		%		&
		\small (a) Relative Rank (DTW)
		&
		\small (b) Time Cost (DTW)
		%  \\
		%  \begin{minipage}{4cm}
		%  \includegraphics[width=4.15cm]{fre_ar}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{4cm}
		%    \includegraphics[width=4.15cm]{fre_mr}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{4cm}
		%  \includegraphics[width=4.15cm]{fre_rr}
		%  \end{minipage}
		%  &
		%  \begin{minipage}{4cm}
		%    \includegraphics[width=4.15cm]{fre_time}
		%  \end{minipage}
		%  \\
		%  \small (i) Approximation Ratio (Frechet)
		%  &
		%  \small (j) Mean Rank (Frechet)
		%  &
		%  \small (k) Relative Rank (Frechet)
		%  &
		%  \small (l) Time Cost (Frechet)
	\end{tabular}
	%\vspace{-2mm}
	\caption{The effect of soft margin $\xi$ for SizeS.}
	%\vspace{-4mm}
	\label{para_fls}
	%	\vspace{-0.5mm}
\end{figure}




\smallskip
\noindent\textbf{(8) Comparison with similar trajectory search (SimTra).}
The solution of the similar trajectory search (SimTra) could be regarded as an approximate solution of the SimSub problem because a data trajectory by itself is a subtrajectory.
%
%This experiment is to evaluate the accuracy if we use the result of SimTra to approximate the result of SimSub.
%Similar to earlier experiments,
%We use the result of ExactS algorithm as the ground truth, and
%compare the average results of SimTra and SimSub using 10,000 trajectory pairs.
%We use RLS for SimSub.
We compare this approximate solution by SimTra and that by the RLS algorithm.
We report the average results over 10,000 trajectory pairs.
The results are shown in Table~\ref{tscssc}.
%In terms of effectiveness, SimSub performs much better than SimTra:
The MR and RR of SimTra are around 10 times larger than those of SimSub for t2vec and 20 times for DTW and Frechet,
which shows that SimTra is not a good approximation for SimSub, though SimTra runs faster than SimSub.

\smallskip
\noindent\textbf{(9) Comparison with algorithms for specific measurements (UCR and Spring).}
In UCR and Spring, a point $q_i$ from the query trajectory can be aligned with only those points $p_j$ from the data trajectory $T$ with $j\in [i-R\cdot |T|, i+R\cdot |T|]$. 
We vary the parameter $R$ in this experiment.
When $R = 1$, it reduces to the unconstrained DTW that is used in this paper.
%
Essentially, $R$ controls how accurately the DTW distance is computed: the higher $R$ is, the more accurate (but also more costly) the computation is.
%
We note that even when $R=1$,
UCR does not return exact solutions since it considers subtrajectories of the same size of the query one only.
%
For this part of experiment,
we drop the component $\Theta_{suf}$ when defining the MDP of RLS-Skip for better efficiency and call the resulting algorithm \emph{RLS-Skip+}.
%
The results are shown in Figure~\ref{fig:UCR}, where we vary the parameter $R$ from 0 to 1. 
We notice that (1) RLS-Skip+ dominates UCR in terms of both efficiency and effectiveness;
(2) the RR of UCR changes slightly from 60.1\% (when $R=0$) to 59.7\% (when $R=1$),
which shows that the performance of UCR is insensitive to the parameter $R$;
(3) under settings of $0.2\le R\le 0.3$, RLS-Skip+ dominates Spring in terms of both effectiveness and efficiency; and (4) under other settings, RLS-Skip+ and Spring provide different trade-offs between effectiveness and efficiency.
% One possible reason is that the warping path is generally close the diagonal, and thus the performance of UCR is insensitive to the parameter $R$.
\if 0
(1) UCR has its RR always worse than that of RLS-Skip; (2) UCR has its running time larger than that of RLS-Skip when $R=1$, i.e., when the unconstrained DTW is used, and also when $R$ are not very small, e.g., $R\ge 0.2$; and (3) UCR runs faster than RLS-Skip only when $R$ is small (while these settings are considered for time series, we are not aware of studies adopting these settings for trajectory data).
\fi


\if 0
{\color{blue}
\smallskip
\noindent\textbf{(10) Comparison with Spring.}
Same as UCR, Spring involves the same parameter $R$. The results are shown in Figure~\ref{fig:spring}, where we vary $R$ from 0 to 1. We notice that (1) under settings of $0.2\le R\le 0.3$, Spring is dominated by RLS-Skip in terms of both effectiveness and efficiency; and (2) under other settings, Spring provides different trade-offs between effectiveness and efficiency, compared with RLS-Skip, and under no settings would Spring dominate RLS-Skip.
}
\fi

\begin{figure}[t]
	%	\hspace{-0.4cm}
	\centering
	\begin{tabular}{c c c c}
		%		\begin{minipage}{4cm}
		%			\includegraphics[width=4.15cm]{sampling_ap_dtw}
		%		\end{minipage}
		%		&
		%		\begin{minipage}{4cm}
		%			\includegraphics[width=4.15cm]{sampling_mr_dtw}
		%		\end{minipage}
		%		&
		\begin{minipage}{4cm}
			\includegraphics[width=4.15cm]{spring_ucr_rr_dtw_p}
		\end{minipage}
		&
		\begin{minipage}{4cm}
			\includegraphics[width=4.15cm]{spring_ucr_time_dtw_p}
		\end{minipage}
		\\
		%		\small (a) Approximation Ratio (DTW)
		%		&
		%		\small (b) Mean Rank (DTW)
		%		&
		\small (a) Relative Rank (DTW)
		&
		\small (b) Time Cost (DTW)
	\end{tabular}
	%\vspace{-2mm}
	\caption{Comparison with UCR and Spring.}
	%\vspace{-2mm}
	\label{fig:UCR}
\end{figure}




\smallskip
\noindent\textbf{(10) Comparison with Random-S.}
The results are shown in Figure~\ref{fig:random-s}, where we vary the sample size from 10 to 100 and for each sample size, we run the algorithm 100 times and collect the average and standard deviations of the metrics of RR and running time. We notice that for a relatively small sample size, e.g., 100, the running time of Random-S is almost that of ExactS and significantly larger than that of RLS-Skip (25 times higher). This is because for Random-S, the subtrajectories that are considered could be quite different, and thus it is not possible to compute their similarities \emph{incrementally} as it does for ExactS. Whereas when the sample size is small, e.g., below 20, Random-S has its effectiveness significantly degraded, which is clearly worse than that of RLS-Skip.
%In conclusion, RLS-Skip dominates Random-S for some settings of sample size in terms of both efficiency and effectiveness and provides different trade-offs between them for other settings, but not vice versa.

\if 0
\begin{figure}[h]
%	\hspace{-9mm}
	\centering
	{\color{blue}
		\begin{tabular}{c c c c}
			%		\begin{minipage}{4cm}
			%			\includegraphics[width=4.15cm]{sampling_ap_dtw}
			%		\end{minipage}
			%		&
			%		\begin{minipage}{4cm}
			%			\includegraphics[width=4.15cm]{sampling_mr_dtw}
			%		\end{minipage}
			%		&
			\begin{minipage}{4cm}
				\includegraphics[width=4.15cm]{spring_rr_dtw_p}
			\end{minipage}
			&
			\begin{minipage}{4cm}
				\includegraphics[width=4.15cm]{spring_time_dtw_p}
			\end{minipage}
			\\
			%		\small (a) Approximation Ratio (DTW)
			%		&
			%		\small (b) Mean Rank (DTW)
			%		&
			\small (a) Relative Rank (DTW)
			&
			\small (b) Time Cost (DTW)
		\end{tabular}
		%\vspace{-2mm}
		\caption{Comparison with Spring.}
		%\vspace{-2mm}
		\label{fig:spring}
	}
\end{figure}
\fi
\begin{figure}[t]
	\hspace{-4mm}
	\centering
	\begin{tabular}{c c c c}
%		\begin{minipage}{4cm}
%			\includegraphics[width=4.15cm]{sampling_ap_dtw}
%		\end{minipage}
%		&
%		\begin{minipage}{4cm}
%			\includegraphics[width=4.15cm]{sampling_mr_dtw}
%		\end{minipage}
%		&
		\begin{minipage}{4cm}
			\includegraphics[width=4.15cm]{sampling_rr_dtw}
		\end{minipage}
		&
		\begin{minipage}{4cm}
			\includegraphics[width=4.15cm]{sampling_time_dtw}
		\end{minipage}
		\\
%		\small (a) Approximation Ratio (DTW)
%		&
%		\small (b) Mean Rank (DTW)
%		&
		\small (a) Relative Rank (DTW)
		&
		\small (b) Time Cost (DTW)
	\end{tabular}
	%\vspace{-2mm}
	\caption{Comparison with Random-S.}
	%\vspace{-2mm}
	\label{fig:random-s}
\end{figure}


\smallskip
\noindent\textbf{(11) Training time.}
The training times of the RLS and RLS-Skip models on different datasets are shown in Table~\ref{learntime}. It normally takes a couple of hours to train a reinforcement learning model for RLS and RLS-Skip. It takes less time to train RLS-Skip than RLS since we use the same number of trajectory pairs and epochs for training both algorithms and RLS-Skip runs faster.


%\hspace*{-12mm}
\begin{table}[t]
\label{learntime}
	\centering
	\scriptsize
	\captionof{table}{Training time (hours).}
	\hspace{-2mm}
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		\parbox{1cm}{Similarity} & \multicolumn{2}{c|}{t2vec} & \multicolumn{2}{c|}{DTW} & \multicolumn{2}{c|}{Frechet} \\ \hline
		Algorithms             & RLS       & RLS-Skip       & RLS      & RLS-Skip      & RLS      & RLS-Skip      \\ \hline
		Porto                  &7.2           &4.4                &10.1          &4.8               &10.6          &5.5               \\ \hline
		Harbin                 &9.7           &5.4                &13.9          &5.7               &14.2          &8.3               \\ \hline
		Sports                 &12.5           &7.6                &83.3          &46.6               &104.1          &52.4               \\ \hline
	\end{tabular}
    \label{learntime}
	%\vspace{-2mm}
\end{table}

%\begin{table}
%\centering
%\scriptsize
%\vspace{-2mm}
%\caption{The influence of skipping steps $k$.}
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%\multicolumn{7}{|c|}{Similarity measurement: t2vec} \\ \hline
%Metrics & $k=0$ & $k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$\\ \hline
%AR  &1.098               &1.124 &1.159 &\textbf{1.112} &1.201 &1.217\\
%MR  &18.322            &28.499 &44.265 &\textbf{23.853} &68.145 &78.650\\
%RR  &3.0\% &5.1\% &7.8\% &\textbf{4.2\%} &11.6\% &12.2\%\\
%Time (s)    &396             &287 &256 &307 &210 &\textbf{196}\\ \hline
%Skipped Pts &0\% &21.8\% &40.4\% &16.3\% &45.8\% &\textbf{63.6\%}\\ \hline\hline
%\multicolumn{7}{|c|}{Similarity measurement: DTW} \\ \hline
%Metrics & $k=0$ &$k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$\\ \hline
%AR  &1.028 &\textbf{1.039} &1.042 &1.044  &1.055 &1.069\\
%MR  &41.138 &\textbf{56.633} &58.077 &64.741 &70.281 &94.356\\
%RR  &3.5\% &\textbf{5.4\%} &5.6\% &5.8\% &6.3\% &8.9\%\\
%Time (s)    &552 &398 &385 &358 &318 &\textbf{229}\\ \hline
%Skipped Pts &0\% &3.1\% &13.1\% &17.7\% &29.5\% &\textbf{47.6\%}\\ \hline\hline
%\multicolumn{7}{|c|}{Similarity measurement: Frechet} \\ \hline
%Metrics & $k=0$ & $k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$\\ \hline
%AR  &1.034 &1.094 &1.095 &\textbf{1.040} &1.096 &1.108\\
%MR  &34.162 &64.897 &74.449 &\textbf{35.029} &77.999 &84.310\\
%RR  &3.6\% &5.9\% &6.8\% &\textbf{3.7\%} &7.4\% &8.1\%\\
%Time (s)    &696  &262 &226 &326 &215 &\textbf{181}\\ \hline
%Skipped Pts &0\% &25.3\% &40.4\% &9.5\% &58.1\% &\textbf{75.1\%}\\ \hline
%\end{tabular}
%%\vspace{-6mm}
%\label{para_steps}
%\end{table}

%\begin{table}
%\centering
%\scriptsize
%\vspace{-2mm}
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%Metrics & $k=0$ &$k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$\\ \hline
%AR  &1.028 &\textbf{1.039} &1.042 &1.044  &1.055 &1.069\\
%MR  &41.138 &\textbf{56.633} &58.077 &64.741 &70.281 &94.356\\
%RR  &3.5\% &\textbf{5.4\%} &5.6\% &5.8\% &6.3\% &8.9\%\\
%Time (s)    &552 &398 &385 &358 &318 &\textbf{229}\\ \hline
%Skipped points &0\% &3.1\% &13.1\% &17.7\% &29.5\% &\textbf{47.6\%}\\ \hline
%\end{tabular}
%\caption{The influence of skipping steps $k$ (DTW).}
%%\vspace{-6mm}
%\label{para_steps_dtw}
%\end{table}

%\begin{table}
%\centering
%\scriptsize
%\vspace{-2mm}
%\begin{tabular}{|c|c|c|c|c|c|c|}
%\hline
%Metrics & $k=0$ & $k=1$ & $k=2$ & $k=3$ & $k=4$ & $k=5$\\ \hline
%AR  &1.034 &1.094 &1.095 &\textbf{1.040} &1.096 &1.108\\
%MR  &34.162 &64.897 &74.449 &\textbf{35.029} &77.999 &84.310\\
%RR  &3.6\% &5.9\% &6.8\% &\textbf{3.7\%} &7.4\% &8.1\%\\
%Time (s)    &696  &262 &226 &326 &215 &\textbf{181}\\ \hline
%Skipped points &0\% &25.3\% &40.4\% &9.5\% &58.1\% &\textbf{75.1\%}\\ \hline
%\end{tabular}
%\caption{The influence of skipping steps $k$ (Frechet).}
%%\vspace{-6mm}
%\label{para_steps_fre}
%\end{table}






==> v13 - technical/efficiency.tex <==
%\subsection{Efficiency Evaluation}
%

\smallskip
\noindent\textbf{Scalability.} We can also evaluate the scalability of all the algorithms based on the results reported in Figure~\ref{fig:efficiencyRLS}(a)-(r). As can be seen, all the algorithms scale nearly linearly with the size of points in the database. We also observe that PSS, POS, POS-D, and RLS scales better than the other algorithms, such as ExactS, and the disparity between them with Exact becomes larger as the size of the dataset increases. For example, \textcolor[rgb]{1.00,0.00,0.00}{RLS is 10.4 times faster than ExactS. (zheng: the result in DTW and Frechet is around 10.4, in 2vec is around 7.6 times for all data size)
when the data size is 0.4 million, RLS is 10.4 times faster than ExactS; When the data size is 2 million, RLS is...
{\bf gao pls fill}}
%evaluate the scalability of all methods on Porto and Harbin datasets. As Figure~\ref{fig:efficiencyRLS}(a)-(r) suggested, the nearly linear scalability is obvious, and the
%performance gap between the exact algorithms and approximation algorithms tended to be bigger when the data size was increasing.

%\noindent\textbf{Comparison with datasets.} We observe similar performance on the two datasets Porto and Harbin. In addition, we know the average length of Harbin dataset (around 120) is bigger than Porto (around 60), and thus the corresponding time is also costly. For example, in terms of the results without index, when we increased the data size from 0.4 to 2.0 on Porto, Exact took from 3019 seconds to 13531 seconds for t2vec in Figure~\ref{fig:efficiencyRLS}(a), while it took from 3853 seconds to 18691 seconds on Harbin in Figure~\ref{fig:efficiencyRLS}(b).

%\noindent\textbf{Comparison with similarity measures.} DTW and Frechet are both point-matching based similarity measures and share a similar formulation, and therefore a similar performance and time cost are consistently under the different datasets and indexes. Regarding the t2vec, it is not very fast for the online scenario, because it needs to call deep learning model step by step on the incremental computing and resulting in some extra cost. For example in Figure~\ref{fig:efficiencyRLS}(a), (c) and (e), Exact with t2vec (3019 seconds to 13531 seconds) achieves only around $2-3\times$ speedup over DTW (5740 seconds to 27876 seconds) and Frechet (7024 seconds to 34383 seconds).

\smallskip \noindent\textbf{The effect of query length.} To evaluate the effect of query length on the accuracy of the proposed approximate algorithms, we group the query trajectories according to their lengths into four groups $G1=[30,45)$, $G2=[45,60)$, $G3=[60,75)$ and $G4=[75,90)$ and report the result of each group. The results on Porto and Harbin datasets with respect to t2vec,  DTW and Frechet are shown in Figure~\ref{fig:groupingRLS}.
%
%In terms of different similarity measures, we can see that DTW (g)-(l) and Frechet (m)-(r) are consistently similar under the three evaluation metrics AR, MR and RR because they are both point-matching based distance, and t2vec also shows consistent performance for Porto and Harbin.
%
We observe that the effectiveness of PSS, POS, POS-D, and RLS remains stable when the query length grows. However, the accuracy of SizeS fluctuates significantly with the change of the query length. This is because the length of the most similar subtrajectory may not have similar length as the query trajectory, and thus it may miss  better results since its search space is limited by the parameter $\xi$.
%

Figure~\ref{time:querylength} shows the effect of query length on the running time. We can see that for t2vec the running time of all the algorithms are almost not affected by query length. This is because we only need to represent the query trajectory into a vector once, which takes $O(m)$ time, and this has little impact on the running time. We observe that the running of all the algorithms increases linearly or super-linearly with the query length for DTW and Frechet, which is consistent with the time complexity result in Table~\ref{tab:algorithm-complexities}.

{\bf gao pls check.. i do not see the new figures}
\begin{figure}
\hspace*{-.5cm}
\centering
\begin{tabular}{c c c}
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/porto_t2vec_without}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/porto_dtw_without}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/porto_frechet_without}
  \end{minipage}
  \\
  \scriptsize (a) Porto (t2vec)
  &
  \scriptsize (b) Porto (DTW)
  &
  \scriptsize (c) Porto (Frechet)
 \\
  \end{tabular}
\caption{Efficiency of varying query lengths.}
\label{time:querylength}
\vspace*{-2mm}
\end{figure}


\smallskip
\noindent\textbf{Working with indexes.} Our proposed algorithms are able to work with indexes to further improve the efficiency of subtrajectory similarity search.
%We further study the effect of indexes for subtrajectory similarity search.
Following two recent studies~\cite{yao2019computing, wang2018torch} on trajectory similarity search, we employ the same indexing techniques for subtrajectory similarity search: Bounding Box R-tree Index and Grid-based Inverted Index. Note that we do not employ those indexing and prunning methods that are specially designed for a specific trajectory similarity measure as they cannot generalize to other similarity measures, or the scenario of subtrajectory similarlty search.
%
% bounded computations~\cite{rakthanmanon2012searching, keogh2005exact} are another acceleration method, which is achieved by estimating the lower bound for pruning; however, it cannot be guaranteed for our subtrajectory search and thus we do not use it in this experiment.
%
 Compared with the results without indexes in Figure~\ref{fig:efficiencyRLS}(a)-(f), the results using the R-tree index shown in Figure~\ref{fig:efficiencyRLS}(g)-(l) achieves around 10--20\% reduction in running time. The results based on the Inverted Index are shown in Figure~\ref{fig:efficiencyRLS}(m)-(r), and its speedup over the results without indexes is more significant, which is around 30 times.

 % because a huge number of maximum bounding rectangles (MBR) have an interaction relationship, and a simple grid index in Figure~\ref{fig:efficiencyRLS}(m)-(r) can be considered as a more useful index structure in such scenarios and it achieves around $30\times$ speedup.

\label{effi_evaluation}
\begin{figure*}
\hspace*{-.5cm}
\centering
\begin{tabular}{c c c c c c}
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_t2v_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_t2v_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_dtw_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_dtw_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_fre_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/without_fre_h}
  \end{minipage}
  \\
  \scriptsize (a) Porto (t2vec)
  &
  \scriptsize (b) Harbin (t2vec)
  &
  \scriptsize (c) Porto (DTW)
  &
  \scriptsize (d) Harbin (DTW)
  &
  \scriptsize (e) Porto (Frechet)
  &
  \scriptsize (f) Harbin (Frechet)
  \\

  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_t2v_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_t2v_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_dtw_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_dtw_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_fre_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/rtree_fre_h}
  \end{minipage}
  \\
  \scriptsize (g) Porto (t2vec)
  &
  \scriptsize (h) Harbin (t2vec)
  &
  \scriptsize (i) Porto (DTW)
  &
  \scriptsize (j) Harbin (DTW)
  &
  \scriptsize (k) Porto (Frechet)
  &
  \scriptsize (l) Harbin (Frechet)
  \\
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_t2v_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_t2v_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_dtw_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_dtw_h}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_fre_p}
  \end{minipage}
  &
  \begin{minipage}{2.75cm}
	\includegraphics[width=2.85cm]{figures/inverted_fre_h}
  \end{minipage}
  \\
  \scriptsize (m) Porto (t2vec)
  &
  \scriptsize (n) Harbin (t2vec)
  &
  \scriptsize (o) Porto (DTW)
  &
  \scriptsize (p) Harbin (DTW)
  &
  \scriptsize (q) Porto (Frechet)
  &
  \scriptsize (r) Harbin (Frechet)
  \end{tabular}
\caption{Results of efficiency evaluation without index (a)-(f), with R-tree index (g)-(l) and Inverted index (m)-(r).}
\label{fig:efficiencyRLS}
\vspace*{-2mm}
\end{figure*}


==> v13 - technical/exact.tex <==
\section{THE EXACT ALGORITHM}
\label{section:exact}
Before introducing the exact algorithm, we give the following definitions and lemmas first.

\begin{definition}[Prefix Trajectory]
A trajectory $T_P = <s_1,s_2,..,s_{|T_P|}>$ is a prefix of a trajectory $T = <p_1,p_2,...,p_{|T|}>$, denoted by $T_P\preceq T$, if and only if $|T_P|\leq|T|$ and $\forall 1 \leq i \leq |T_P|, s_i = p_i$.
\end{definition}
For example, $T_P = <p_1,p_2>$ is a prefix of $T_1 = <p_1,p_2,p_3>$, but it is not a prefix of trajectory $T_2 = <p_1,p_3>$.

\begin{definition}[Suffix Trajectory]
A trajectory $T_S = <s_1,s_2,..,s_{|T_S|}>$ is a suffix of a trajectory $T = <p_1,p_2,...,p_{|T|}>$, denoted by $T_S\preceq T$, if and only if $|T_S|\leq|T|$ and $\forall 1 \leq i \leq |T_S|, s_i = p_{|T|-|T_S|+i}$.
\end{definition}
For example, $T_S = <p_2,p_3>$ is a suffix of $T_1 = <p_1,p_2,p_3>$, but it is not a suffix of trajectory $T_2 = <p_1,p_3>$.

\begin{lemma}
\label{lemma:subt}
Given a candidate trajectory $C$, any subtrajectory is a prefix trajectory of a suffix trajectory in $C$.
\end{lemma}
\begin{proof}
It can be easily proofed by the definition of subtrajectory. We denote $C_{\Lambda=[i,j]}$ is a subtrajectory that starts from index $i$ to index $j$, where $1 \leq i \leq j \leq |C|$. Any $C_{\Lambda=[i,j]}$ is a prefix trajectory of $C_{\Lambda=[i,|C|]}$ and $C_{\Lambda=[i,|C|]}$ is a suffix trajectory in $C$.
\end{proof}

\begin{lemma}
\label{lemma:t2vec}
The representation of prefix trajectories in a given trajectory can be computed in $O(n)$ time by $t2vec$, where $n$ is the length of the candidate trajectory~\footnote{In the rest of the paper, we will consistently use $n$ to refer to the length of the candidate trajectory.}.
\end{lemma}
\begin{proof}
Recall that in Section~\ref{pre:t2vec}, we explain as follows: (1) it takes $O(n)$ to convert a location sequence to its corresponding token sequence by the pretrained embedding layer, and each map operation from a location $p$ to its token vector $x$ is $O(1)$; (2) it takes roughly $O(n)$ time to scan the token sequence and fed the vectors $x$ to the GRU units. In each time step, we can get each prefix trajectory representation $h$. Hence, the overall time complexity is $O(n)$.
\end{proof}

The Lemma~\ref{lemma:subt} and Lemma~\ref{lemma:t2vec} suggest that in order to search an exact subtrajectory, we can enumerate each suffix trajectory in $C$, and then enumerate each prefix trajectory of the suffix trajectory. During the search process, we maintain a subtrajectory interval with the minimum dissimilarity value.

\begin{algorithm}[t]
	\caption{Exact Algorithm}
	\footnotesize{
		\label{exact}
		\begin{algorithmic}[1]
			\Require
			Candidate trajectory $C$ and query trajectory $Q$;
			\Ensure
			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
            \State get representation vector $h_{Q}$ for query trajectory $Q$;
            \State initialize $\Psi \leftarrow \infty$ and $\Lambda \leftarrow \emptyset$;
			\For{each time step $1 \leq t \leq |C|$}
                \State $h_{t-1} \leftarrow None$;
                    \For{each time step $t \leq t' \leq |C|$}
                        \State $h_{t'} \leftarrow t2vec(h_{t'-1}, x_{t'})$;
                        \If {$d(h_{Q}, h_{t'}) < \Psi$}
                            \State $\Psi \leftarrow d(h_{Q}, h_{t'})$, $\Lambda \leftarrow [t, t']$;
                        \EndIf
                    \EndFor
			\EndFor
	\end{algorithmic}}
\end{algorithm}

We present the details of the exact algorithm in Algorithm~\ref{exact}. It first gets the token sequence for the candidate trajectory $C$, which is used to enumerate each subtrajectory, and gets the representation $h_Q$ for query trajectory $Q$ (lines 1-2). Then, we initialize the optimal dissimilarity value $\Psi$ and the corresponding interval $\Lambda$ (line 3). Next, in the first for-loop, we enumerate each suffix trajectory of $C$ (lines 4-16), and enumerate each prefix trajectory of the suffix trajectory in the second for-loop (lines 6-11). Let $t2vec(\cdot,\cdot)$ denote the incremental computation by t2vec, the input is the last time hidden vector $h_{t-1}$ and current token vector $x_{t}$ (line 7). Note that it needs to initialize the first time hidden vector as $None$ (line 5). Finally, we need to maintain the best subtrajectory interval and the dissimilarity value during this process (lines 8-10), where $d(\cdot,\cdot)$ denotes the Euclidean distance between two vectors.

\begin{lemma}
The total time cost of the exact algorithm is $O(n^2)$.
\end{lemma}
\begin{proof}
It takes $O(n)$ time to generate the token sequence and the representation vector for the query trajectory. The first for-loop needs to be executed for $n$ times, and according to the Lemma~\ref{lemma:t2vec}, we know the time complexity of the second for-loop is $O(n)$. Note that in the second for-loop, the Euclidean distance computation is a constant which is obvious. Hence, the overall time cost is $O(n^2)$.
\end{proof}


==> v13 - technical/fss.tex <==
\subsection{Double Model Search (DMS)}
\label{ha:fss}
Nevertheless, the Intuition~\ref{intu} might not be true in most cases. This is because $t2vec$ is an RNN-based similarity measure, which means that for the same trajectory, the representation vectors are not equal when we encode the trajectory forward and backward. A straightforward solution to solve this issue is to modify the model structure; however, we use the following two interesting lemmas to show that changing the model structure can guarantee the Intuition~\ref{intu} but it will lose the efficiency at the same time.

\begin{lemma}
\label{lemma:inte1}
A bidirectional RNN-based t2vec (bi-$t2vec$) can achieve $\Psi_{backward} = \Psi_{forward}$.
\end{lemma}
\begin{proof}
A bidirectional RNN~\cite{schuster1997bidirectional} contains two modules - a forward RNN and a backward RNN. Given two trajectories $C$ and $Q$, we denote $h_{f}^{C}$ is the final hidden state of the forward RNN for $C$, and $h_{b}^{C}$ is the final hidden state of the backward RNN for $C$. We concatenate the two hidden states $\big[h_{f}^{C}, h_{b}^{C}\big]^{\mathrm{T}}$ to represent trajectory $C$. Similarity, we have the trajectory $Q$ representation $\big[h_{f}^{Q}, h_{b}^{Q}\big]^{\mathrm{T}}$. Further, we have
\begin{equation}
  \Psi_{forward} =    \left\|\left[\begin{array}{c}
                        h_{f}^{C} \\
                        h_{b}^{C} \\
                      \end{array}\right] -
                             \left[\begin{array}{c}
                        h_{f}^{Q} \\
                        h_{b}^{Q} \\
                      \end{array}\right]
                      \right\|_{2}.
\end{equation}
For the reserve trajectories $\overleftarrow{C}$ and $\overleftarrow{Q}$, we know their representations are only the position exchange of hidden states, that is
$\big[h_{f}^{\overleftarrow{C}}, h_{b}^{\overleftarrow{C}}\big]^{\mathrm{T}} = \big[h_{b}^{C}, h_{f}^{C}\big]^{\mathrm{T}}$,
$\big[h_{f}^{\overleftarrow{Q}}, h_{b}^{\overleftarrow{Q}}\big]^{\mathrm{T}} = \big[h_{b}^{Q}, h_{f}^{Q}\big]^{\mathrm{T}}$. According to commutative law in Euclidean distance computation, we have
\begin{equation}
\begin{aligned}
  \Psi_{backward} & =    \left\|\left[\begin{array}{c}
                        h_{f}^{\overleftarrow{C}} \\
                        h_{b}^{\overleftarrow{C}} \\
                      \end{array}\right] - \left[\begin{array}{c}
                        h_{f}^{\overleftarrow{Q}} \\
                        h_{b}^{\overleftarrow{Q}} \\
                      \end{array}\right]\right\|_{2} = \left\|\left[\begin{array}{c}
                        h_{b}^{C} \\
                        h_{f}^{C} \\
                      \end{array}\right] -
                             \left[\begin{array}{c}
                        h_{b}^{Q} \\
                        h_{f}^{Q} \\
                      \end{array}\right]
                      \right\|_{2}\\
  & =                 \left\|\left[\begin{array}{c}
                        h_{f}^{C} \\
                        h_{b}^{C} \\
                      \end{array}\right] -
                             \left[\begin{array}{c}
                        h_{f}^{Q} \\
                        h_{b}^{Q} \\
                      \end{array}\right]
                      \right\|_{2} = \Psi_{forward}.
\end{aligned}
\end{equation}
Hence, Lemma~\ref{lemma:inte1} holds.
\end{proof}

\begin{lemma}
\label{lemma:inte2}
In each time step, the update computation by bi-$t2vec$ is $O(n)$.
\end{lemma}

\begin{proof}
Recall that in $t2vec$, we can get $h_{t}$ by inputting $h_{t-1}$ and $x_{t}$, the time cost is $O(1)$.
In bi-$t2vec$, the update time cost of forward hidden state $h_{f}$ is the same as $t2vec$ $O(1)$. However, for the backward hidden state $h_{b}$, the time complexity will increase to $O(n)$ because the starting point is changed, RNN needs to read the whole trajectory again to get current $h_{b}$.
\end{proof}
From the above lemmas, we observe that modifying the model structure is also difficult to decrease time complexity. Thus, we try to decouple the bidirectional model, and pretrain the backward RNN $\widehat{t2vec}$ to capture the reverse candidate and query trajectories as input. The output $\Psi_{backward}$ can be considered as a predicted value of $\Psi_{forward}$. We call this algorithm Double Model Search (DMS), the main idea is to approximate $\Psi_{forward}$ with less time cost. 
%More details are presented in Algorithm~\ref{fss}. 
Note that it also needs to adjust $\Psi$ if $C_{\Lambda}$ is obtained by a suffix trajectory.
%\begin{algorithm}[t]
%	\caption{Double Model Search}
%	\footnotesize{
%		\label{fss}
%		\begin{algorithmic}[1]
%			\Require
%			Candidate trajectory $C$, query trajectory $Q$;
%			\Ensure
%			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
%            \State get representation vector $h_{Q}$ for $Q$ by $t2vec$ and $h_{\overleftarrow{Q}}$ for $\overleftarrow{Q}$ by $\widehat{t2vec}$;
%            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma,\Delta \leftarrow \emptyset$, $sp \leftarrow 1$ and $h_{0}, h'_{0} \leftarrow None$;
%            \For{each time step $1 \leq t \leq |C|$}
%                \State $h'_{t} = \widehat{t2vec}(h'_{t-1}, x_{|c|+1-t})$;
%            \EndFor
%			\For{each time step $1 \leq t \leq |C|$}
%                \State $\Gamma \leftarrow [sp, t]$, $\Delta \leftarrow [t+1, |C|]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$;
%                \State $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$, $\Psi_{S} \leftarrow d(h_{\overleftarrow{Q}}, h'_{|C|-t})$;
%                \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
%                    \If {$\Psi_{P} < \Psi_{S}$}
%                        \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                    \Else
%                        \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
%                    \EndIf
%                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$;
%                \EndIf
%			\EndFor
%            \State adjust $\Psi$ to a true dissimilarity value if $C_{\Lambda}$ is a suffix trajectory.
%	\end{algorithmic}}
%\end{algorithm}

\begin{lemma}
The total time complexity of DMS is $O(n)$.
\end{lemma}
\begin{proof}
\textcolor[rgb]{1.00,0.00,0.00}{Based on Lemma~\ref{tc:bss}, it only uses another pretrained model $\widehat{t2vec}$ to receive reverse trajectories, so the proof is same as the BSS.}
\end{proof}


==> v13 - technical/ga.tex <==
\section{HEURISTIC ALGORITHM}
\label{section:heuristic}
The quadratic time complexity makes the exact algorithm very time-consuming, and then we propose some heuristic algorithms to approximately get the similarity, which largely improve the efficiency. Section~\ref{ha:idea} presents the high-level idea of our proposed heuristic algorithms. Section~\ref{ha:ga} -~\ref{ha:dps} elaborates on some detailed designs.

\subsection{Trajectory Splitting}
\label{ha:idea}
The major limitation of the exact algorithm is its high computational cost, which makes it impractical for longer trajectories. To alleviate this issue, we model the computation of subtrajectory similarity as a trajectory splitting problem. The high-level idea is if we can scan the given trajectory one time and accurately split the best subtrajectory without enumerating each suffix trajectory as shown in the exact algorithm, then we can achieve more efficient search. However, a new issue is how can we achieve the exact splitting? In the rest of this section, we introduce the heuristic methods for trajectory splitting.

\subsection{Greedy Algorithm (GA)}
\label{ha:ga}
A straightforward solution to the trajectory splitting is the greedy algorithm. When we enumerate the points of a given trajectory $C$ from 1 to |C|, in each time step, we need to decide whether to split at this point or not. If a trajectory is decided to be split, it will generate a prefix trajectory and a suffix trajectory, whose intervals are represented by $\Gamma$ and $\Delta$. We define the range of $\Gamma$ and $\Delta$ as follows.
\begin{equation}
\label{interval}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\Gamma = [sp, t], \Delta = [t+1, |C|],
\end{aligned}
\end{equation}
where $sp$ denotes the index of the splitting point and it continues to update by splitting operation. $t$ is the current time step. Note that in our definition, the two intervals are non-overlapping. This is because our trajectory similarity via $t2vec$ depends on the token vector of each sampling point. The greedy algorithm always maintain the current best trajectory between $C_{\Gamma}$ and $C_{\Delta}$, so we need to perform a splitting if there is a better result occurs at this time. We illustrate the working process in Example~\ref{workingex:ga}.

\begin{example}
\label{workingex:ga}
Consider a pair of candidate and query trajectory $C$, $Q$ in Figure~\ref{example:ga}, where $t$ is the current time step.%~\footnote{We use dashed lines with arrows to label the prefix interval $\Gamma$ and suffix interval $\Delta$ for ease of reference. The solid lines with arrows indicate there is a splitting operation at this time step, and we label the maintaining interval $\Lambda$ with red color during this process.}.
\begin{itemize}[leftmargin=8pt]
  \item $t=1$, we initialize $sp$ as the current $t$, the initial dissimilarity value $\Psi$ as infinity, the initial intervals $\Lambda, \Gamma, \Delta$ as empty sets, and the first hidden state as none. We get two candidate subtrajectories $C_{\Gamma=[1,1]}$ and $C_{\Delta=[2,4]}$ according to Equation~\ref{interval}. we maintain the suffix $C_{\Delta=[2,4]}$ because it is more similar to $Q$ than $C_{\Gamma=[1,1]}$, and then we update $sp$ as the next time step.
  \item $t=2$, we delete the edge between 1 and 2 because a splitting operation happened in $t=1$. We do not need to maintain $C_{\Gamma=[2,2]}$ or $C_{\Delta=[3,4]}$ because neither of them is better than $C_{\Lambda=[2,4]}$.
  \item $t=3$, we get two subtrajectories $C_{\Gamma=[2,3]}$ and $C_{\Delta=[4,4]}$, we decide to maintain the prefix $C_{\Gamma=[2,3]}$ because it is more similar to $Q$ compared with $C_{\Lambda=[2,4]}$, and thus a splitting operation happened. Note that the current $sp=2$ and we update it as the next time step again.
  \item $t=4$, we delete the edge between 3 and 4 because a splitting operation happened in the last step, and the maintaining subtrajectory does not change. Note that in the final step, the suffix trajectory is none. The final result is the subtrajectory with interval $\Lambda = [2,3]$.
\end{itemize}
\end{example}
We present the corresponding idea in Algorithm~\ref{ga}.

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/example_ga}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{An example illustrating the GA. We use dashed lines with arrows to label the prefix interval $\Gamma$ and suffix interval $\Delta$ for ease of reference. The solid lines with arrows indicate there is a splitting operation at this time step, and we label the maintaining interval $\Lambda$ with red color during this process.}\label{example:ga}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}

\begin{algorithm}[t]
	\caption{Greedy Algorithm}
	\footnotesize{
		\label{ga}
		\begin{algorithmic}[1]
			\Require
			Candidate trajectory $C$ and query trajectory $Q$;
			\Ensure
			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
            \State get representation vector $h_{Q}$ for query trajectory $Q$;
            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma,\Delta \leftarrow \emptyset$, $sp \leftarrow 1$ and $h_{0} \leftarrow None$;
			\For{each time step $1 \leq t \leq |C|$}
                \State $\Gamma \leftarrow [sp, t]$, $\Delta \leftarrow [t+1, |C|]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$;
                \State get representation vector $h_{C_{\Delta}}$ for suffix trajectory $C_{\Delta}$;
                \State $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$, $\Psi_{S} \leftarrow d(h_{Q}, h_{C_{\Delta}})$;
                \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
                    \If {$\Psi_{P} < \Psi_{S}$}
                        \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
                    \Else
                        \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
                    \EndIf
                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$;
                \EndIf
			\EndFor
	\end{algorithmic}}
\end{algorithm}

\begin{lemma}
\label{lemma:ga}
The total time complexity of GA is $O(n^2)$.
\end{lemma}
\begin{proof}
In Algorithm~\ref{ga}, the for-loop needs to be executed for $n$ times (lines 4-16). In each time step, it needs to get representation vector $h_{C_{\Delta}}$ for suffix trajectory $C_{\Delta}$ (line 6), which is $O(n)$ because it needs to encode the whole suffix via t2vec. Note that for the prefix trajectory $C_{\Gamma}$, the update of $t2vec$ is $O(1)$ in each time step. Hence, the overall time cost is $O(n^2)$.
\end{proof}

Although we can see the computational cost of GA is also quadratic, it provides a good framework for trajectory splitting. In order to handle the issue, we further propose the following four algorithms based on GA.


==> v13 - technical/instantiation.tex <==
\section{Similarity Measure}

\subsection{DTW and Frechet}
DTW~\cite{yi1998efficient} and Frechet~\cite{alt1995computing} are two of the most widely adopted trajectory similarity measures in temporal sequence analyses. Thus, we first use DTW and Frechet as examples to discuss the costs of $\Phi$, $\Phi_{ini}$ and $\Phi_{inc}$.

Given a data trajectory $T = <p_1, p_2,...,p_n>$ and a query trajectory $Q = <q_1, q_2,...,q_m>$, DTW is computed as below
\begin{equation}
\label{dtw_sm}
D_{n,m}=\left\{
\begin{aligned}
& \sum\nolimits_{i=1}^{n}d(p_i,q_1)&\text{if } m = 1\\
& \sum\nolimits_{j=1}^{m}d(p_1,q_j)&\text{if } n = 1\\
& d(p_n,q_m) + \\
& \min(D_{n-1,m-1}, D_{n-1,m},D_{n,m-1})&\text{otherwise}
\end{aligned}
\right.
\end{equation}
where $D_{n,m}$ denotes DTW distance between the prefix trajectory of $T$ with length $n$ and the prefix trajectory of $Q$ with length $m$, and $d(p_n,q_m)$ is a point-to-point distance (typically Euclidean distance with $O(1)$ time complexity) between $p_n$ and $q_m$. The time complexity of $\Phi$ can be easily observed from the Equation~\ref{dtw_sm} because it needs to compute all the pairwise point-matching distances, that is $O((n \cdot m) \cdot 1) = O(n \cdot m)$. Based on the general time complexity of $\Phi = O(n \cdot m)$, the $\Phi_{ini}$ can be considered as the data trajectory only has one point that is $n=1$, and thus $\Phi_{ini} = O(1 \cdot m) = O(m)$. For the incremental computation $\Phi_{inc}$, we can save the previous time step value $D_{t-1,m}$. If we want to update $D_{t,m}$ from $D_{t-1,m}$, firstly, we need to get $D_{t,1}$, which follows $D_{t,1}=D_{t-1,1}+d(p_t,q_1)$ according to the Equation~\ref{dtw_sm}. Then, we need to update $D_{t,i}$ for each time step $i$ from 2 to $m$ that is $D_{t,i}=d(p_{t},q_{i})+
min\big(D_{t-1,i-1},D_{t-1,i},D_{t,i-1}\big), 2\leq i\leq m$. In each time step, the computation is $O(1)$ and thus the total time complexity is completely related to the query length $m$ that is $O(1 + m - 1) = O(m)$.

Similarly, we have the same conclusion for the Frechet distance based on the Equation~\ref{fre_sm}.
\begin{equation}
\label{fre_sm}
F_{n,m}=\left\{
\begin{aligned}
&\max\nolimits_{i=1}^{n}d(p_i,q_1)&\text{if }m = 1\\
&\max\nolimits_{j=1}^{m}d(p_1,q_j)&\text{if }n = 1\\
&\max(d(p_n,q_m),\\
& \min(F_{n-1,m-1},F_{n-1,m},F_{n,m-1}))&\text{otherwise}
\end{aligned}
\right.
\end{equation}
where $F_{n,m}$ denotes the Frechet distance.

\subsection{t2vec}
t2vec~\cite{li2018deep} is a state-of-the-art trajectory similarity measure based on deep representation learning. It adapts the sequence encoder-decoder framework based on RNN~\cite{cho2014learning} to build learning model, and it takes the final hidden vector of the encoder~\cite{rumelhart1988learning} to represent a trajectory. Finally, t2vec computes the trajectory similarity between the Euclidean distance of hidden vectors.

Given a data trajectory with length $n$ and a query trajectory with length $m$, it takes $O(n)$ and $O(m)$ to get their hidden vectors and $O(1)$ to compute the Euclidean distance (Details are discussed in~\cite{li2018deep}.). And thus $\Phi = O(n + m + 1) = O(n + m)$. Note that t2vec is different from point-matching based similarity such DTW and Frechet, it can preprocess all of the hidden vectors of trajectories in database offline. Thus, $\Phi_{ini}$ is $O(1)$ because it only needs to input one point in the data trajectory to the model, the model computation based on RNN is $O(1)$, and the hidden vector of query is preprocessed offline. Similarly, the incremental computation $\Phi_{inc}$ is also $O(1)$ because we can save the previous hidden vector, and it takes $O(1)$ to update the current hidden vector from the model.




==> v13 - technical/introduction.tex <==
\section{INTRODUCTION}
\label{intro}

%Trajectory data and applications;
Trajectory data, which corresponds to a type of data for capturing the traces of moving objects, is ubiquitous. It has been used for various types of analysis such as clustering~\cite{agarwal2018subtrajectory,lee2007trajectory,buchin2011detecting} and similarity search~\cite{chen2004marriage,chen2005robust,xie2014eds,ranu2015indexing,li2018deep,yi1998efficient}. The majority of existing studies take \emph{a trajectory as a whole} for analysis~\cite{chen2004marriage,chen2005robust,xie2014eds,ranu2015indexing,li2018deep,yi1998efficient}. Motivated by the phenomenon that two trajectories could be dissimilar to each other if each is considered a whole but similar if only some portion of each is considered, there have been a few studies, which take \emph{a portion of a trajectory} as a basic entity for analysis~\cite{agarwal2018subtrajectory,lee2007trajectory,buchin2011detecting,tampakis2019distributed,tampakis2019scalable}. Some examples include subtrajectory clustering~\cite{agarwal2018subtrajectory,lee2007trajectory,buchin2011detecting} and subtrajectory join~\cite{tampakis2019distributed,tampakis2019scalable}. For example, the subtrajectory clustering method in~\cite{lee2007trajectory} first partitions raw trajectories into different subtrajectories using some principle and then groups those subtrajectories that are similar to one another into clusters.


In this paper, we study a query with its goal to search for a portion of a trajectory from a database storing many trajectories called \emph{data trajectories}, which is the most similar to a given trajectory called \emph{query trajectory}. In this query, a portion of a trajectory, called \emph{subtrajectory}, is considered as a basic entity and a query trajectory is taken as a whole for analysis.
Therefore, it captures trajectory similarity in a finer-grained way than conventional similar trajectory search.
%
For instance, consider a data trajectory and a query trajectory.
When considered as a whole, the data trajectory is not similar to the query trajectory based on some trajectory similarity measurement,
but some portion of it is very similar to the query trajectory.
%
With the conventional similar trajectory search query,
this data trajectory would be ruled out,
though a portion of it is very similar to the query trajectory, which is interesting.
%


Moreover, in quite a few real-life applications, subtrajectories are naturally considered as basic units for analysis,
e.g., subtrajectory search~\cite{sha2016chalkboarding}, subtrajectory join~\cite{tampakis2019distributed}, subtrajectory clustering~\cite{buchin2011detecting}, etc.
%
One application is the subtrajectory search query on sports play data.
In sports such as soccer and basketball, a common practice nowadays is to track the movements of players and/or the ball using some special-purpose camera and/or GPS devices~\cite{wang2019effective}.
The resulting trajectory data is used to capture the semantics of the plays and for different types of data analyses.
%, among which, such as play/player retrieval~\cite{}, team performance analysis~\cite{}, tactics discovery~\cite{}, etc.
One typical task on such sports play data is to search for a portion/segment of play from a database of plays, with its trajectories of players and/or its trajectory of the ball similar to those and/or that of a given query play~\cite{sha2016chalkboarding}. This task is essentially one of searching for similar subtrajectories.
%
Another potential application is detour route detection.
%In some cities, people especially tourists experience the detour route problem often - taxi drivers would deliberately take an unnecessary detour route when going from a source location to a destination location, yet detecting detour routes is challenging. 
%The aforementioned query could be potentially applied for detecting detour routes 
It first collect those routes that have been reported by passengers to be detour routes and then searches for those subtrajectories of taxis' routes, which are similar to a detour route.
The found subtrajectories are probably detour routes as well. 
%In this case, taxis' routes correspond to data trajectories and a detour route that is known corresponds to a query trajectory.

\if 0
In this paper, we study a query with its goal to search for a portion of a trajectory from a database storing many trajectories called \emph{data trajectories}, which is the most similar to a given trajectory called \emph{query trajectory}. In this query, a portion of a trajectory, called \emph{subtrajectory}, is considered as a basic entity and a query trajectory is taken as a whole for analysis. While there are many existing studies on the similar trajectory search problem with each trajectory considered a whole, there are quite few studies on this query,
despite that it has many real-life applications as illustrated as follows.
%\begin{itemize}
%	\item \textbf{Car pooling.}

%The first application is \emph{carpooling}. Suppose that we have a customer who has his/her planned commute route (which could be captured by a trajectory) and would like to find a car for pooling among many cars each of which has a planned route. In this application, a possible solution is to find the car whose planned route contains a portion that is the most similar to the  customer's route. This could be captured by the above query where the planned routes of the cars correspond to data trajectories and the customer's planned route corresponds to a query trajectory.
%	\item \textbf{Detour detection.}

The first application is \emph{detour route detection}. In some cities, people especially tourists experience the detour route problem often - taxi drivers would deliberately take an unnecessary detour route when going from a source location to a destination  location, yet detecting detour routes is challenging. The aforementioned query could be potentially applied for detecting detour routes by first collecting those routes that have been reported by passengers to be detour routes and then searching for those subtrajectories of taxis' routes that are similar to a detour route - the found subtrajectories are probably detour routes as well. In this case, taxis' routes correspond to data trajectories and a detour route that is known corresponds to a query trajectory.

The second application is the \emph{sports play retrieval}. Nowadays, a common practice is that in a sports games such as soccer and basketball plays, the movements of players and/or the ball are tracked using some special-purpose camera and/or GPS devices. The resulting trajectory data is used to capture the semantics of the plays and for different types of data analyses.
%, among which, such as play/player retrieval~\cite{}, team performance analysis~\cite{}, tactics discovery~\cite{}, etc.
One typical task on such sports play data is to search for a portion/segment of play from a database of plays, with its trajectories of players and/or its trajectory of the ball similar to those and/or that of a given query play~\cite{sha2016chalkboarding}. This task is essentially one of searching for similar subtrajectories.
\fi

%{\color{blue}
\if 0
The second application is \emph{similar play retrieval}. Sports play (e.g., a soccer game) is usually captured by trajectories, which record the movements of players by multiple sequences of time-stamped locations. A common query on play retrieval is based on the role of a player~\cite{sha2016chalkboarding}, i.e., it first matches a trajectory pair of two players who share the same role in a game, and then compute its similarity; however, a play would generally involves huge amount sampled locations in a game~\cite{wang2019effective}, and a typical task is to find players' movements within a short period (subtrajectories), which are similar to some query movements (a query trajectory) given by users, rather than take the play as a whole.
\fi
%}
%\end{itemize}
%\smallskip\noindent\textbf{Car pooling.}

%\smallskip\noindent\textbf{Detour detection.} In some cities, people especially tourists experience the detour route problem often - taxi drivers would deliberately take an unnecessary detour when going from a source location to a destination  location, yet detecting detour routes is challenging. The SubSim problem could be potentially applied for detecting detour routes by first collecting those routes that have been reported by passengers to be detour routes and then searching for those subtrajectories of taxis' routes that are similar to a detour route - the found subtrajectories are probably detour routes as well. In this case, taxis' routes correspond to data trajectories and a detour route that is known corresponds to a query trajectory.

%\smallskip\noindent\textbf{Sports game retrieval.} Nowadays, it becomes that in a sports game such as soccer and basketball, the players and the ball are tracked dozens of times per second using some the real-many team-based sports games are monitoring

\if 0
The query as discussed above relies on a trajectory similarity measurement to measure to which extent two trajectories are similar to each other. In the literature, several ``dissimilarity measurements'' have been proposed for trajectories including: DTW~\cite{yi1998efficient}, Frechet~\cite{alt1995computing}, LCSS~\cite{vlachos2002discovering}, ERP~\cite{chen2004marriage}, EDR~\cite{chen2005robust}, EDS~\cite{xie2014eds}, EDwP~\cite{ranu2015indexing}, and t2vec~\cite{li2018deep}. Different measurements have different merits and suit different application scenarios. In this paper, we assume an abstract similarity measurement, which could be instantiated with any of these existing measurements \emph{by applying some inverse operation} such as taking the ratio between 1 and a distance (a dissimilarity).
\fi

A key problem that is involved in answering the query mentioned above is to find a subtrajectory of a data trajectory, which is the most similar to a given query trajectory. We call this problem the \emph{similar subtrajectory search} (SimSub) problem. 
%
While there are many existing studies on the similar trajectory search problem with each trajectory considered a whole, there are very few studies on the SimSub problem.
%
Let $T$ be a data trajectory involving $n$ points and $T_q$ be a query trajectory involving $m$ points. %Note that there are $\frac{n(n+1)}{2}$ possible subtrajectories of $T$. 
%
We design an exact algorithm, which enumerates all possible subtrajectories of $T$, computes the similarity between each subtrajectory and the query trajectory, and returns the one with the greatest similarity. 
We further adopt an \emph{incremental} strategy for computing the similarities that are involved in the exact algorithm, which helps to improve the time complexity by $O(n)$.
%
%We note some existing algorithms~\cite{sakurai2007stream}, which are originally designed for searching for similar subsequences of a data time series, can be used for the SimSub problem and have better time complexities than the exact algorithm, but they work for some specific similarity measurements such as DTW and Frechet only but not for others such as those learning-based ones including t2vec.
%
\if 0
A straightforward implementation of this method would incur $O(n^3)$ time for some measurements such as t2vec (for which the cost of similarity computation is $O(n)$) and even $O(n^3m)$ time for some other measurements such as DTW and Frechet (for which the cost of similarity computation is $O(nm)$), and this is prohibitively expensive for large-scale applications. 
We improve the implementation via an \emph{incremental} strategy for computing similarities and achieve $O(n^2)$ for some measurements such as t2vec~\cite{li2018deep} and $O(n^2m)$ for some other measurements such as DTW~\cite{yi1998efficient} and Frechet~\cite{alt1995computing}. 
\fi
%
We also follow some existing studies on subsequence matching~\cite{kim2013efficient,zhang2010bed} and design an algorithm, which considers only those subtrajectories with their sizes similar to that of the query trajectory and controlled by a user parameter. This would provide a controllable trade-off between efficiency and effectiveness.


To push the efficiency further up, we propose several algorithms, which share the idea of splitting a data trajectory into some subtrajectories to be candidate solutions to the problem and differ in using different methods for splitting the data trajectory. Specifically, the process is to scan the points of a data trajectory one by one sequentially and for each one, it decides whether to split the data trajectory at the point. Some of them use pre-defined heuristics, e.g., a greedy one. Others model the process as a \emph{markov decision process} (MDP)~\cite{puterman2014markov} and use deep reinforcement learning to learn an optimal policy for the MDP, which is then used for splitting the data trajectory. 
These splitting-based algorithms have time complexities much lower than the exact algorithm in general, e.g., for measurements such as t2vec, each splitting-based algorithm runs in $O(n)$ time while the exact algorithm runs in $O(nm)$ time.

The major contributions of this paper are as follows.
\begin{itemize}
	\item We propose the SimSub problem, and this to the best of our knowledge, corresponds to the first systematic study on searching subtrajectories that are similar to a query trajectory.
	%This problem considers portions of a data trajectory as entities and a query trajectory as a whole for analysis, which is different from existing studies which consider all trajectories either each as a whole or their portions as entities.
	The SimSub problem relies on a trajectory similarity measurement, and in this paper, we assume an abstract one, which could be instantiated with any existing measurement.
	% such as DTW~\cite{yi1998efficient} and Frechet~\cite{alt1995computing}.
	
	\item We develop a suite of algorithms for the SimSub problem: (1) one exact algorithm, (2) one approximate algorithm, which provides a controllable trade-off between efficiency and effectiveness, and (3) several splitting-based algorithms including both heuristics-based ones and deep reinforcement learning based ones. These algorithms should cover a wide spectrum of application scenarios in terms of efficiency and effectiveness requirements.
	
	\item Third, we conducted extensive experiments, which verified that splitting-based algorithms in general have good efficiency and among them, the algorithms based on deep reinforcement learning achieve the best effectiveness and efficiency.
\end{itemize}

\noindent
\textbf{Organization}. We review the related work in Section~\ref{related} and provide the problem definition and
some preliminaries in Section~\ref{problem_and_preliminary}.
Section~\ref{sec:non-learning} presents all non-learning based algorithms and
Section~\ref{section:RLS} presents the deep reinforcement learning based algorithms.
%Section~\ref{section:other} introduces other similarity measures for RLS.
We report our experimental results in Section~\ref{experiment} and conclude this paper and discuss some future work in Section~\ref{conclusion}.

%Solutions;
%Contributions;
%Organizations;

\if 0
With the popularity of location-tracking devices, trajectory data has witnessed unprecedented growth in the last decade. A trajectory is typically embedded both spatial and temporal information to record the moving of an object, and measuring the similarity between trajectories is widely regarded as a fundamental problem in various applications such as mining movement patterns of animals~\cite{li2011movemine}, discovering popular routes~\cite{chen2011discovering} and detecting environmental disasters such as tornado~\cite{passe2006exploring}.

Trajectory Similarity Computation (TSC) is a process of finding those trajectories from the database, each of which as a whole is similar to the given query trajectory. Actually, in most cases, a trajectory is not similar to the query trajectory at the whole level; however, it might contain a portion (subtrajectory) that is similar to the query, which is called Subtrajectory Similarity Computation (SSC). SSC is more general and useful than TSC in many application scenarios and we present three examples:
\begin{itemize}[leftmargin=8pt]
  \item Weather Prognosis: As studied in~\cite{passe2006exploring,powell2001accuracy}, accurate environmental disaster forecasts such as hurricane landing can effectively avoid property damage, and in that case, meteorologists usually pay more attention to the trajectories in some special areas such as coastlines rather than the overall trajectory. The SSC algorithms can therefore benefit these application scenarios.
  \item Animal Movements: Measuring the distance between the road and animals has been identified as a significant predictor of animal distributions~\cite{wisdom2004spatial,li2011movemine}, and thus zoologists are trying to discover the similar subtrajectories of animal movements near the road.
  \item Anomalous Trajectory Detection: As discussed in~\cite{zhang2011ibat}, in order to detect whether driving fraud behavior happened by some greedy taxi drivers who overcharge passengers by taking an unnecessary route, it needs to compute the similarity with normal taxi trajectories; however, it is hardly to be similar to the query if we compute the similarity as a whole, because the anomalous trajectories are usually long while the normal ride is relatively short.
\end{itemize}

Although SSC is such an important problem, to the best of our knowledge, it still lacks enough research focus now. The core challenge of SSC is the efficiency. An intuitive idea is that enumerates each possible subtrajectory of a given trajectory and then computes the distance between the query trajectory by using one of the existing similarity measures such as Dynamic Time Warping (DTW) distance~\cite{yi1998efficient} or Frechet distance~\cite{alt1995computing}, which, however, is huge computation cost in practice because
a trajectory with $n$ sampling points consists of $O(n^2)$ possible subtrajectories, and that would impose a big challenge on the efficiency.

The second challenge is the effectiveness. In order to balance the efficiency, one may think of some approximate algorithms that only traverse partial subtrajectories such as the subtrajectories that have similar lengths with the query; however, the simple solution is unreasonable and will lose some effectiveness definitely. In our experiment, we will illustrate the effectiveness of the solution.

The third one is the genericness. Previous studies such as EDS~\cite{xie2014eds} that are specific to one similarity measure for subtrajectory computation. Actually, the existing measures are good enough. For example, t2vec~\cite{li2018deep} is a state-of-the-art trajectory similarity measure, it can effectively handle the trajectory uncertainty (against sampling errors or noise errors) in TSC problem. Based on that, a generic framework that can support effective and efficient SSC is needed.

In this paper, we use the t2vec as a default similarity measure to study SSC problem. We first develop an exact algorithm, which takes $O(n^2)$ time to answer a query trajectory, where $n$ denotes the length of the candidate trajectory. This is very costly, and is impractical for large trajectory databases, so we turn to model the SSC problem as a kind of trajectory splitting problem, which aims to accurately split the best subtrajectory from the whole, and thus a greedy algorithm is proposed. However, the greedy algorithm is also involved in a quadratic time complexity. To overcome the efficiency, we further propose a series of heuristic algorithms that take only linear time. However, these algorithms cannot achieve better accuracy with a small approximation ratio with the exact algorithm. To tackle the issue of effectiveness and inspired by the algorithms mentioned above, we further propose a data-driven method RLS based on deep reinforcement learning, which can effectively support our trajectory splitting with a theoretical proofing. Finally, we further extend our RLS to a generic framework that can support any popular measures such as DTW. Overall, the RLS model has the following attractive characteristics:
\begin{itemize}[leftmargin=8pt]
  \vspace{-2mm}\item Efficient: RLS achieves the same level time complexity as TSC algorithms for a more complex problem SSC. For example, RLS takes $O(n)$ time for SSC based on t2vec measure and takes $O(n^2)$ time for SSC based on DTW measure.
  \vspace{-2mm}\item Effective: RLS has superb approximation performance in practice. On two real trajectory datasets Porto and Harbin, it achieves an approximation ratio less than $1.1$ compared with the exact algorithm, and ranks Top 5\% for t2vec, DTW and Frechet.
  \vspace{-2mm}\item Generic: RLS is generic enough to support widely used similarity measures rather than previous works~\cite{xie2014eds} that are specific to one measure for subtrajectories, and thus RLS can be applied to search for better results in existing trajectory problems.
 \vspace{-2mm} \item Elastic: RLS computes the subtrajectory similarity without losing spatial information, which makes it elastic to cooperate with existing indexing and pruning strategies~\cite{wang2018torch,yao2019computing}. In our experiments, we will illustrate the results of index-based subtrajectory search with RLS.
\end{itemize}

In summary, our main contribution includes: (1) We propose to model SSC problem as a trajectory splitting problem, which can effectively alleviate time cost caused by enumerating subtrajectories. (2) We propose a greedy framework based on the idea of trajectory splitting, and design a series of heuristic algorithms to further improve time efficiency. (3) We propose a deep learning model, RLS, which is a data-driven method and achieves an effective trajectory splitting strategy. To the best of our knowledge, this is the first deep learning based solution. (4) We extend RLS to support most of the widely adopted trajectory similarity measures. To the best of our knowledge, it is also the first method that supports generic SSC problem, which makes it widely applicable to various downstream trajectory tasks. (5) We conduct extensive experiments on two real-world taxi trajectory datasets, which show that RLS method consistently outperforms the baselines in terms of effectiveness and efficiency.
\fi



==> v13 - technical/non-learning.tex <==

\section{Non-Learning based Algorithms}
\label{sec:non-learning}

In this part, we introduce three types of algorithms, namely an exact algorithm ExactS, an approximate algorithm SizeS, and splitting-based algorithms including PSS, POS and POS-D. The ExactS algorithm is based on an exhaustive search with some careful implementation and has the highest complexity, the SizeS algorithm is inspired by existing studies on subsequence matching~\cite{kim2013efficient,zhang2010bed} and provides a tunable parameter for controlling the trade-off between efficiency and effectiveness, and the splitting-based algorithms are based on the idea of splitting the data trajectory for constructing subtrajectories as candidates of the solution and run the fastest. A summary of the time complexities of these algorithms is presented in Table~\ref{tab:algorithm-complexities}.

\begin{table*}[t!]
\centering
	%\hspace*{-.8cm}
	\caption{Time complexities of algorithms ($n_1 << n$)}
	\begin{tabular}{|l||c|c|c|c|}
		\hline
		Algorithms		&	abstract similarity	measurement							&	t2vec 					&	DTW								&	Frechet							\\\hline
		ExactS			&	$O(n\cdot ( \Phi_{ini} + n \cdot \Phi_{inc}))$			& 	$O(n^2)$		&	$O(n^2\cdot m)$					&	$O(n^2\cdot m)$					\\\hline
		SizeS			& 	$O(n\cdot( \Phi_{ini} + (m + \xi) \cdot \Phi_{inc}))$	& 	$O((\xi + m)\cdot n)$	&	$O((\xi + m)\cdot n\cdot m)$	&	$O((\xi + m)\cdot n\cdot m)$	\\\hline
		PSS, POS, POS-D	&	$O(n_1\cdot \Phi_{ini} + n\cdot \Phi_{inc})$			& 	$O(n)$					&	$O(n \cdot m)$					&	$O(n \cdot m)$					\\\hline\hline
		\parbox{2.5cm}{RLS, RLS-Skip (learning-based)}				&	$O(n_1\cdot \Phi_{ini} + n\cdot \Phi_{inc})$			& 	$O(n)$					&	$O(n \cdot m)$					&	$O(n \cdot m)$					\\\hline
%		POS			&	$O(n_1\cdot \Phi_{ini} + n\cdot \Phi_{inc})$			&	$O(n \cdot m)$			&	$O(n \cdot m)$			& 	$O(n)$		\\\hline
%		POS-D		&	$O(n_1\cdot \Phi_{ini} + n\cdot \Phi_{inc})$			&	$O(n \cdot m)$			&	$O(n \cdot m)$			& 	$O(n)$		\\\hline
	\end{tabular}	
	%\vspace*{-2mm}
	\label{tab:algorithm-complexities}
\end{table*}

%\smallskip\noindent\textbf{Exact Algorithm: SizeS.}
\subsection{The ExactS Algorithm}
\if 0
A straightforward algorithm for the SimSub problem on $T$ and $T_q$ is to enumerate all possible subtrajectories $T[i, j]$ ($1\le i\le j\le n$) of the data trajectory $T$ and compute the similarity between each $T[i, j]$ and $T_q$, i.e., $\Theta(T[i, j], T_q)$, and then return the one with the greatest similarity. 
We call this algorithm \emph{ExactS}. 
A straightforward implementation of ExactS would incur a time cost of $O(n^2\cdot \Phi)$ since $T$ has $\frac{n\cdot (n+1)}{2} = O(n^2)$ subtrajectories and the cost of computing the similarity between each subtrajectory and $T_q$ is $\Phi$ in general.
%In conclusion, ExactS would have a time complexity of $O(n^2) \cdot \Phi = O(n^2\cdot \Phi)$.
For example, when DTW or Frechet is used, the time complexity is $O(n^2\cdot nm) = O(n^3m)$ and when t2vec is used, it is $O(n^2 \cdot (n+m))$.
%That is, would incur high time complexity, i.e., at least $O(n^3)$, no matter which similarity measurement is used.
\fi
%A slightly better implementation and the corresponding time complexity;

Let $T$ be a data trajectory and $T_q$ be a query trajectory.
The ExactS algorithm enumerates all possible subtrajectories $T[i, j]$ ($1\le i\le j\le n$) of the data trajectory $T$ and computes the similarity between each $T[i, j]$ and $T_q$, i.e., $\Theta(T[i, j], T_q)$, and then returns the one with the greatest similarity. 
For better efficiency,
ExactS computes the similarities between the subtrajectories and $T_q$ \emph{incrementally} as much as possible as follows. 
It involves $n$ iterations, and in the $i^{th}$ iteration, it computes the similarity between each subtrajectory starting from the $i^{th}$ point and the query trajectory in an ascending order of the ending points, i.e., it computes $\Theta(T[i, i], T_q)$ (from scratch) first and then computes $\Theta(T[i, i+1], T_q)$, ..., $\Theta(T[i, n], T_q)$ sequentially and incrementally. During the process, it maintains the subtrajectory that is the most similar to the query one, among those that have been traversed so far. As could be verified, it would traverse all possible subtrajectories after $n$ iterations. The ExactS algorithm with this implementation is presented in Algorithm~\ref{alg:ExactS}.

Consider the time complexity of ExactS. Since there are $n$ iterations and in each iteration, the time complexity of computing $\Theta(T[i, i], T_q)$ is $\Phi_{ini}$ and the time complexity of computing $\Theta(T[i, i+1], T_q)$, ..., and $\Theta(T[i, n], T_q)$ is $O(n\cdot \Phi_{inc})$, we know that the overall time complexity is $O(n\cdot ( \Phi_{ini} + n \cdot \Phi_{inc}))$. 
%For example, when DTW or Frechet is used, it is $O(n\cdot (m + n \cdot m)) = O(n^2m)$ and when t2vec is used, it is $O(n\cdot (1 + n \cdot 1)) = O(n^2)$. 
%Compared with the straightforward implementation, this implementation based on incremental computations is faster by a factor of $O(n)$ roughly. 
%Besides, it is hard to improve the implementation of ExactS in general, e.g., when t2vec is used, ExactS has its time complexity of $O(n^2)$ for traversing $O(n^2)$ subtrajectories.

We note that for some specific similarity measurement, there may exist algorithms that have better time complexity than ExactS. For example, the Spring algorithm~\cite{sakurai2007stream}, which finds the most similar subsequence of a data time series to a query one, is applicable to the SimSub problem and has the time complexity of $O(nm)$. The major idea of Spring is a dynamic programming process for computing the DTW distance between the data time series and the query one, where the latter is padded with a fictitious point that could be aligned with any point of the data time series with distance equal to 0 (so as to cover all possible suffixes of the data time series). Nevertheless, Spring is designed for the specific similarity DTW while ExactS works for an abstract one that could be instantiated to be any similarity.
%\begin{algorithm}[t!]
%	\caption{ExactS}
%		\footnotesize{
%	%		\label{exact}
%	\begin{algorithmic}[1]
%		\Require
%		A data trajectory $T$ and a query trajectory $T_q$;
%		\Ensure
%		A subtrajectory of $T$ that is the most similar to $T_q$;
%		%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $\Phi$;
%		%			\State get representation vector $h_{Q}$ for query trajectory $Q$;
%		%			\State initialize $\Psi \leftarrow \infty$ and $\Lambda \leftarrow \emptyset$;
%		\State $T_{best} \leftarrow \emptyset$; $\Theta_{best} \leftarrow 0$;
%		\ForAll{$1 \leq i \leq |T|$}
%		\State compute $\Theta(T[i, i], T_q)$;
%		%				\State $h_{t-1} \leftarrow None$;
%		\If{$\Theta(T[i, i], T_q) > \Theta_{best}$}
%		\State $T_{best} \leftarrow T[i, i]$; $\Theta_{best} \leftarrow \Theta(T[i, i], T_q)$;
%		\EndIf
%		\ForAll{$i+1 \le j\le |T|$}
%		%					\State $h_{t'} \leftarrow t2vec(h_{t'-1}, x_{t'})$;
%		\State compute $\Theta(T[i, j], T_q)$ based on $\Theta(T[i, j-1], T_q)$;
%		\If{$\Theta(T[i, j], T_q) > \Theta_{best}$}
%		\State $T_{best} \leftarrow T[i, j]$; $\Theta_{best} \leftarrow \Theta(T[i, j], T_q)$;
%		\EndIf
%		\EndFor
%		\EndFor
%		\State \textbf{return} $T_{best}$;
%	\end{algorithmic}
%	}
%	\label{alg:ExactS}
%\end{algorithm}
\begin{algorithm}[t!]
        \caption{ExactS}\label{alg:ExactS}
		\footnotesize{
		\KwIn{
		A data trajectory $T$ and query trajectory $T_q$;}
		\KwOut{
		A subtrajectory of $T$ that is the most similar to $T_q$;}
		%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $\Phi$;
		%			\State get representation vector $h_{Q}$ for query trajectory $Q$;
		%			\State initialize $\Psi \leftarrow \infty$ and $\Lambda \leftarrow \emptyset$;
		$T_{best} \leftarrow \emptyset$; $\Theta_{best} \leftarrow 0$;\\
		\ForAll{$1 \leq i \leq |T|$}{
		compute $\Theta(T[i, i], T_q)$;\\
		%				\State $h_{t-1} \leftarrow None$;
		\If{$\Theta(T[i, i], T_q) > \Theta_{best}$}{
		$T_{best} \leftarrow T[i, i]$; $\Theta_{best} \leftarrow \Theta(T[i, i], T_q)$;
		}
		\ForAll{$i+1 \le j\le |T|$}{
		%					\State $h_{t'} \leftarrow t2vec(h_{t'-1}, x_{t'})$;
		compute $\Theta(T[i, j], T_q)$ based on $\Theta(T[i, j-1], T_q)$;\\
		\If{$\Theta(T[i, j], T_q) > \Theta_{best}$}{
		$T_{best} \leftarrow T[i, j]$; $\Theta_{best} \leftarrow \Theta(T[i, j], T_q)$;
		}
		}
		}
		\textbf{return} $T_{best}$;
	}
\end{algorithm}


%Still, at least quadratic;
%\smallskip\noindent\textbf{Approximate Algorithm: SizeS.}
\subsection{The SizeS Algorithm}
%While the ExactS algorithm could be implemented with incremental computations as above, it has time complexity still at least $O(n^2)$, which makes it limited to small and moderate datasets only. This is essentially due to the fact that 
ExactS explores all possible $\frac{n(n+1)}{2}$ subtrajectories, many of which might be quite dissimilar from the query trajectory and could be ignored. For example, by following some existing studies on subsequence matching~\cite{kim2013efficient,zhang2010bed}, we could restrict our attention to only those subtrajectories, which have similar sizes as the query one for better efficiency. Specifically, we enumerate all subtrajectories that have their sizes within the range $[m - \xi, m + \xi]$, where $\xi\in [0, n-m]$ is a pre-defined parameter that controls the trade-off between the efficiency and effectiveness of the algorithm. Again, we adopt the strategy of incremental computation for the similarities between those subtrajectories starting from the same point and the query trajectory.
%, i.e., $\Theta(T[i, i+(m-\xi-1)], T_q)$, $\Theta(T[i, i+(m-\xi)], T_q)$, ..., $\Theta(T[i, i+(m+\xi-1)], T_q)$ for some $i \in [1, n]$ (note that for some $i$'s such as $i = n$, there exist no subtrajectories starting from the $i^{th}$ point and having their sizes in $[m-\xi, m+\xi]$ and in these cases, no subtrajectories are considered).
We call this algorithm \emph{SizeS} and analyze its time complexity as follows. The time complexity of computing the similarities between all subtrajectories starting from a specific point and having their sizes within the range $[m - \xi, m+\xi]$ is $O(\Phi_{ini} + (m-\xi-1)\cdot \Phi_{inc} + 2\xi \cdot \Phi_{inc})$, where $\Phi_{ini} + (m-\xi-1)\cdot \Phi_{inc}$ is cost of computing $\Theta(T[i, i+m-\xi-1], T_q)$ and $2\xi \cdot \Phi_{inc}$ is the cost of computing $\Theta(T[i, j], T_q)$ for $j\in [i+m-\xi, i+m+\xi-1]$. It could be further reduced to $O(\Phi_{ini} + (m+\xi)\cdot \Phi_{inc})$. Therefore, the overall time complexity of SizeS is $O(n\cdot( \Phi_{ini} + (m + \xi) \cdot \Phi_{inc}))$. For example, when DTW or Frechet is used, it is $O(n\cdot (m + (m + \xi)\cdot m)) = O((\xi + m)\cdot n\cdot m)$ and when t2vec is used, it is $O(n\cdot (1 + (\xi + m)\cdot 1)) = O((\xi + m)\cdot n)$.

In summary, SizeS achieves a better efficiency than ExactS at the cost of its effectiveness. Besides, SizeS still needs to explore $O(\xi \cdot n)$ subtrajectories, which restricts its application on small and moderate datasets only.
Unfortunately, SizeS may return a solution, which is arbitrarily worse than the best one. We illustrate this in the technical report version~\cite{TR} due to the page limit.

%which could be too expensive for those applications where the efficiency is critical.
\if 0
SizeS achieves a better efficiency than ExactS at the cost of its effectiveness. Nevertheless, SizeS may still be not adequate in some cases. First, SizeS has its effectiveness rely on an implicit assumption that two sequences that are similar to each other have their sizes (or lengths) similar. While this assumption usually holds for some types of sequence data such as strings, it is not always the case for trajectory data. For example, in cases where the trajectories are collected using different sampling rates, two trajectories that are similar to each other may have their sizes deviate significantly from each other, i.e., the one with a higher sampling rate has many more points than the one with a lower sampling rate. In these cases, setting $\xi$ too low would miss many subtrajectories that are similar to the query one while setting $\xi$ too high would incur a high time complexity. Second, SizeS still needs to explore $O(\xi \cdot n)$ subtrajectories, which could be too expensive for those applications where the efficiency is critical.
\fi

%Rule-based algorithms; Linear algorithm Non-learning based algorithms; Reinforcement-learning based algorithms;
\subsection{Splitting-based Algorithms}

\begin{figure*}[htb]
	\centering
%\vspace{-8mm}
\begin{tabular}{cc}
	\centering
  \begin{minipage}{4cm}
    \centering
    \includegraphics[width=4cm]{pss_exp_v2}
    %\vspace{-6mm}
  \caption{A problem input.}
  %\vspace{-4mm}
  \label{fig:input}
  \end{minipage}
  &
  \begin{minipage}{13cm}
  	%\vspace{-6mm}
    \centering
  	\scriptsize
    \captionof{table}{Illustration of PSS with the DTW distance.}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Initial   & \multicolumn{6}{c|}{$h = 1$, $T_{best} = \emptyset$ and $\Theta_{best} = 0$}                      \\ \hline
Point & Prefix                       & Suffix                           & Split & $h$ & $\Theta_{best}$ & $T_{best}$ \\ \hline
$p_1$         & $\Theta(T[1, 1], T_q)=0.124$ & $\Theta(T[1, 5]^R, T_q^R)=0.150$ & Yes       &	2	& 0.150           & $T[1,5]$   \\ \hline
$p_2$         & $\Theta(T[2, 2], T_q)=0.236$ & $\Theta(T[2, 5]^R, T_q^R)=0.227$ & Yes       &	3	& 0.236           & $T[2,2]$   \\ \hline
$p_3$         & $\Theta(T[3, 3], T_q)=0.183$ & $\Theta(T[3, 5]^R, T_q^R)=0.215$ & No        &	3	& 0.236           & $T[2,2]$   \\ \hline
$p_4$         & $\Theta(T[3, 4], T_q)=0.236$ & $\Theta(T[4, 5]^R, T_q^R)=0.215$ & No        &	3	& 0.236           & $T[2,2]$   \\ \hline
$p_5$         & $\Theta(T[3, 5], T_q)=0.215$ & $\Theta(T[5, 5]^R, T_q^R)=0.152$ & No        &	3	& 0.236           & $T[2,2]$   \\ \hline
Output    & \multicolumn{6}{c|}{$T_{best} = T[2,2]$ with $\Theta_{best}=0.236$}                                        \\ \hline
  \end{tabular}
  \label{table:pss}
  \end{minipage}
  %\vspace{-4mm}
%\label{example_pss}
%\caption{Illustration of PSS with the DTW distance.}
\end{tabular}
%\vspace{-4mm}
\end{figure*}

The ExactS algorithm is costly since it explores $O(n^2)$ subtrajectories. The SizeS algorithm runs faster than ExactS since it explores about $O(\xi \cdot n)$ subtrajectories ($\xi << n$). Thus, an intuitive idea to push the efficiency further up is to explore fewer subtrajectories. In the following, we design a series of three approximate algorithms, which all share the idea of splitting a data trajectory into several subtrajectories and returning the one that is the most similar to the query trajectory. These algorithms differ from each other in using different heuristics for deciding where to split the data trajectory. With this splitting strategy, the number of subtrajectories that would be explored is bounded by $n$ and in practice, much smaller than $n$. We describe these algorithms as follows.

\smallskip\noindent\textbf{(1) Prefix-Suffix Search (PSS).} The PSS algorithm is a greedy one,
which maintains a variable $T_{best}$ storing the subtrajectory that is the most similar to the query trajectory found so far. Specifically, it scans the points of the data trajectory $T$ in the order of $p_1, p_2, ..., p_n$.
When it scans $p_i$, it computes the similarities between the two subtrajectories that would be formed if it splits $T$ at $p_i$, i.e., $T[h, i]$ and $T[i, n]$, and the query trajectory $T_q$, where $p_h$ is the point following the one, at which the last split was done if any and $p_h$ is the first point $p_1$ otherwise.
%
In particular, we replace the part of computing the similarity between the suffix $T[i, n]$ and the query trajectory with that between their reversed versions, denoted by $T[i, n]^R$ and $T_q^R$, respectively.
%
This is because (1) $\Theta(T[i, n]^R, T_q^R)$ could be computed incrementally based on $\Theta(T[i+1, n]^R, T_q^R)$ and
(2) $\Theta(T[i, n]^R, T_q^R)$ and $\Theta(T[i, n], T_q)$ are equal for some similarity measurements such as DTW and Frechet and positively correlated for others such as t2vec as we found via experiments.
%
If any of these two similarities are larger than the best-known similarity, it performs a split operation at $p_i$ and updates $T_{best}$ accordingly; otherwise, it continues to scan the next point $p_{i+1}$.
%
%Since $T[h, i]$ corresponds to a prefix of the trajectory that is to be split and $T[i, n]$ a suffix, we call this algorithm ``Prefix and Suffix Search'' ().
%If so, it performs a split operation at $p_i$ and updates $T_{best}$ to the subtrajectory which is more similar to the query trajectory among the two formed subtrajectories; and if not, it continues to scan the next point $p_{i+1}$.
At the end, it returns $T_{best}$. The procedure of PSS is presented in Algorithm~\ref{alg:PSS}.
%where we replace the part of computing the similarity between a suffix $T[i, n]$ and the query trajectory with that between their reversed versions, denoted by $T[i, n]^R$ and $T_q^R$, respectively, for efficiency consideration (explanations are provided with the time complexity analysis provided next).


To illustrate, consider an example shown in Figure~\ref{fig:input}, where $T$ is a data trajectory with 5 points $p_{1:5}$ and $T_q$ is a query trajectory with 3 points $q_{1:3}$. Suppose that we measure the similarity between two trajectories using the ratio of 1 over the DTW distance between them. Consider the process of the PSS algorithm, which is depicted in Table~\ref{table:pss}. When it scans $p_1$, it considers two subtrajectories, namely $T[1,1]$ and $T[1,5]$, which have the similarities, i.e., $0.124$ and $0.150$, both larger than the best-known so far, i.e., 0. Therefore, it performs a split operation at $p_1$ and updates $h$, $\Theta_{best}$ and $T_{best}$ accordingly, as shown in the $3^{rd}$ row of the table. It continues to scan $p_2$ and considers two subtrajectories $T[2,2]$ and $T[2,5]$. Since their similairities are larger than the best-known one, it performs a split at $p_2$ and updates $h$, $\Theta_{best}$ and $T_{best}$. It then scans $p_3$, $p_4$, and $p_5$ and does not perform a split at any of them. Therefore, $h$, $\Theta_{best}$ and $T_{best}$ are kept unchanged. Finally, it returns $T_{best}$, i.e., $T[2,2]$, which has the similarity of $0.236$. Note that $T[2,4]$ has the largest similarity to $T_q$, which is $1/3 = 0.333$.


We analyze the time complexity of PSS as follows. When it scans a specific point $p_i$, the time costs include that of computing $\Theta(T[h, i], T_q)$ and also that of computing $\Theta(T[i, n]^R, T_q^R)$.
Consider the former part.
If $i = h$, it is $\Phi_{ini}$.
If $i \ge h + 1$, it is $\Phi_{inc}$
since $\Theta(T[h, i], T_q)$ could be computed based on $\Theta(T[h, i-1], T_q)$ incrementally.
%If $i = h+1$, it is $(\Phi_{ini} + \Phi_{inc})$, where $\Phi_{ini}$ is the cost of computing $\Theta(T[h, h], T_q)$ and $\Phi_{inc}$ is the cost of computing $\Theta(T[h, h+1], T_q)$ based on $\Theta(T[h, h], T_q)$. If $i > h + 1$, it is $\Phi_{inc}$ since $\Theta(T[h, i], T_q)$ could be computed based on $\Theta(T[h, i-1], T_q)$ incrementally.
%The former is $(\Phi_{ini} + \Phi_{inc})$ if $i = h + 1$ in which case $\Phi_{ini}$ is the cost of computing $\Theta(T[h, h], T_q)$ and $\Phi_{inc}$ is the cost of computing $\Theta(T[h, h+1], T_q)$ based on $\Theta(T[h, h], T_q)$ and $\Phi_{inc}$ if $i > h + 1$ in which case $\Theta(T[h, i-1], T_q)$ has been computed already when it scans $p_{i-1}$.
Consider the latter part. It is simply $O(\Phi_{inc})$.
\if 0
It is $O(\Phi)$ with a straightforward implementation,
resulting a $O(n\cdot \Phi)$ time complexity of PSS.
%
To retain the efficiency of PSS,
we replace $\Theta(T[i, n], T_q)$ with $\Theta(T[i, n]^R, T_q^R)$
since (1) $\Theta(T[i, n]^R, T_q^R)$ could be computed incrementally based on $\Theta(T[i+1, n]^R, T_q^R)$ and
(2) $\Theta(T[i, n]^R, T_q^R)$ and $\Theta(T[i, n], T_q)$ are equal for some similarity measurements such as DTW and Frechet
and positively correlated for others such as t2vec as we found via experiments.
%
With this replacement applied, the latter time cost would be $O(\Phi_{inc})$.
\fi
%With this, the latter time cost would be $O(\Phi_{inc})$.
In conclusion, the time complexity of PSS is $O(n_1 \cdot (\Phi_{ini} + \Phi_{inc}) + (n-n_1) \cdot \Phi_{inc}) = O(n_1\cdot \Phi_{ini} + n\cdot \Phi_{inc})$, where $n_1$ is the number of points where splits are done.
For example, when DTW or Frechet is used, the time complexity of PSS is $O(n_1 \cdot m + n\cdot m) = O(n \cdot m)$ and when t2vec is used, it is $O(n_1 \cdot 1 + n \cdot 1) = O(n)$.

%\begin{algorithm}[t!]
%	\caption{Prefix-Suffix Search (PSS)}
%		\footnotesize{
%	\begin{algorithmic}[1]
%		\Require
%		A data trajectory $T$ and a query trajectory $T_q$;
%		\Ensure
%		A subtrajectory of $T$ that is similar to $T_q$;
%		%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $\Phi$;
%		%			\State get representation vector $h_{Q}$ for query trajectory $Q$;
%		%			\State initialize $\Psi \leftarrow \infty$ and $\Lambda \leftarrow \emptyset$;
%		\State $T_{best} \leftarrow \emptyset$; $\Theta_{best} \leftarrow 0$;
%		\State compute $\Theta(T[n,n]^R, T_q^R)$;
%		\State compute $\Theta(T[n-1,n]^R, T_q^R)$, $\Theta(T[n-2,n]^R, T_q^R)$, ..., $\Theta(T[1,n]^R, T_q^R)$ incrementally;
%		\State $h\leftarrow 1$;
%%T		\State compute $\Theta(T[h,h], Q)$;
%		\ForAll{$1 \leq i \leq |T|$}
%		\State compute $\Theta(T[h, i], T_q)$ incrementally if possible; %based on $\Theta(T[h, i-1], Q)$;
%		%				\State $h_{t-1} \leftarrow None$;
%		\If{$\max\{\Theta(T[h, i], T_q), \Theta(T[i, n]^R, T_q^R)\} > \Theta_{best}$}
%		\State $\Theta_{best} \leftarrow \max\{\Theta(T[h, i], T_q), \Theta(T[i, n]^R, T_q^R)\}$;
%		\If{$\Theta(T[h, i], T_q) > \Theta(T[i, n]^R, T_q^R)$}
%		\State $T_{best} \leftarrow T[h, i]$;
%		\Else
%		\State $T_{best} \leftarrow T[i, n]$;
%		\EndIf
%		\State $h\leftarrow i+1$;
%%		\State compute $\Theta(T[h,h], Q)$;
%		\EndIf
%		\EndFor
%		\State \textbf{return} $T_{best}$;
%	\end{algorithmic}
%	}
%	\label{alg:PSS}
%\end{algorithm}

\begin{algorithm}[t!]
	\caption{Prefix-Suffix Search (PSS)}\label{alg:PSS}
		\footnotesize{
        \KwIn{
		A data trajectory $T$ and query trajectory $T_q$;}
		\KwOut{
		A subtrajectory of $T$ that is similar to $T_q$;}
		%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $\Phi$;
		%			\State get representation vector $h_{Q}$ for query trajectory $Q$;
		%			\State initialize $\Psi \leftarrow \infty$ and $\Lambda \leftarrow \emptyset$;
		$T_{best} \leftarrow \emptyset$; $\Theta_{best} \leftarrow 0$;\\
		compute $\Theta(T[n,n]^R, T_q^R)$;\\
		compute $\Theta(T[n-1,n]^R, T_q^R)$, $\Theta(T[n-2,n]^R, T_q^R)$, ..., $\Theta(T[1,n]^R, T_q^R)$ incrementally;\\
		$h\leftarrow 1$;\\
%T		\State compute $\Theta(T[h,h], Q)$;
		\ForAll{$1 \leq i \leq |T|$}{
		compute $\Theta(T[h, i], T_q)$ incrementally if possible;\\ %based on $\Theta(T[h, i-1], Q)$;
		%				\State $h_{t-1} \leftarrow None$;
		\If{$\max\{\Theta(T[h, i], T_q), \Theta(T[i, n]^R, T_q^R)\} > \Theta_{best}$}{
		$\Theta_{best} \leftarrow \max\{\Theta(T[h, i], T_q), \Theta(T[i, n]^R, T_q^R)\}$;\\
		\eIf{$\Theta(T[h, i], T_q) > \Theta(T[i, n]^R, T_q^R)$}
        {
		$T_{best} \leftarrow T[h, i]$;
        }
		{
		$T_{best} \leftarrow T[i, n]$;
		}
		$h\leftarrow i+1$;\\
%		\State compute $\Theta(T[h,h], Q)$;
		}
		}
		\textbf{return} $T_{best}$;
	}
\end{algorithm}

\smallskip\noindent\textbf{(2) Prefix-Only Search (POS).}
In PSS, when it scans a point $p_i$, it considers two subtrajectories, namely $T[h, i]$ and $T[i, n]$.
An alternative is to consider the prefix $T[h, i]$ only - one argument is that the suffix $T[i, n]$ might be destroyed when further splits are conducted.
A consequent benefit is that the time cost of computing $\Theta(T[i, n], T_q)$ would be saved. We call this algorithm the POS algorithm.
As could be verified, POS has the same time complexity as PSS though the former runs faster in practice.


\smallskip\noindent\textbf{(3) Prefix-Only Search with Delay (POS-D).}
POS performs a split operation whenever a prefix, which is better than the best subtrajectory known so far, is found. This looks a bit rush and may prevent a better subtrajectory to be formed by extending it with a few more points. Thus, we design a variant of POS, called \emph{Prefix-Only Search with Delay} (POS-D). Whenever a prefix is found to be more similar to the query trajectory than the best subtrajectory known so far, POS-D continues to scan $D$ more points and splits at one of these $D+1$ points, which has the corresponding prefix the most similar to the query trajectory. It could be verified that with this delay mechanism, the time complexity of the algorithm does not change though in practice, it would be slightly higher.


While these splitting-based algorithms including PSS, POS and POS-D, return reasonably good solutions in practice, they may return solutions that are arbitrarily worse than the best one in theory. We illustrate this in the technical report version~\cite{TR} due to the page limit.



==> v13 - technical/other.tex <==
\section{OTHER SIMILARITY MEASURES}
\label{section:other}
DTW~\cite{yi1998efficient} and Frechet~\cite{alt1995computing} are two of the most widely adopted trajectory similarity measures in temporal sequence analyses. Thus, in this section, we use DTW and Frechet as examples to show how to support other distance functions in our reinforcement learning framework.

\subsection{DTW Distance}
\begin{definition}[DTW Distance]
\label{dtw:definition}
Given a candidate trajectory $C = <p_1, p_2,...,p_n>$ and a query trajectory $Q = <q_1, q_2,...,q_m>$, DTW is computed as below
\begin{equation}
D_{n,m}=\left\{
\begin{aligned}
& \sum\nolimits_{i=1}^{n}d(p_i,q_1)&\text{if } m = 1\\
& \sum\nolimits_{j=1}^{m}d(p_1,q_j)&\text{if } n = 1\\
& d(p_n,q_m) + \\
& \min(D_{n-1,m-1}, D_{n-1,m},D_{n,m-1})&\text{otherwise}
\end{aligned}
\right.
\end{equation}
where $D_{n,m}$ denotes DTW distance between the prefix trajectory of $C$ with length $n$ and the prefix trajectory of $Q$ with length $m$, and $d(p_n,q_m)$ is a point-to-point distance (typically Euclidean distance) between $p_n$ and $q_m$.
\end{definition}
To support DTW in our reinforcement learning framework, the core is to update the trajectory dissimilarity value from the previous time step $D_{t-1,m}$ to the current value $D_{t,m}$. The update process is illustrated in Figure~\ref{fig:dtw}. We use the matrix $Mat$ to record DTW distances between each pairwise prefix trajectory similarity. If we want to update $D_{t,m}$ from $D_{t-1,m}$, firstly, we need to get $D_{t,1}$, which follows the equation $D_{t,1}=D_{t-1,1}+d(p_t,q_1)$ according to the Definition~\ref{dtw:definition}. Then, we need to update $D_{t,i}$ for each time step $i$ from 2 to $m$ that is $D_{t,i}=d(p_{t},q_{i})+
min\big(D_{t-1,i-1},D_{t-1,i},D_{t,i-1}\big), 2\leq i\leq m$. Let vector $\mathcal{V}_{t}$ denote the $t$-row of DTW matrix $Mat$, and thus we have the update equation as follows.
\begin{equation}\label{dtwupdate}
  \mathcal{V}_{t} = dtw(\mathcal{V}_{t-1}, p_{t}, Q), D_{t,m} = \mathcal{V}_{t,m},
\end{equation}
where $dtw(\cdot,\cdot,\cdot)$ is a update function as explained above, the input includes the given last time vector $\mathcal{V}_{t-1}$, the sampling point $p_t$ in the candidate trajectory $C$ and query trajectory $Q$, and the final element of $\mathcal{V}_{t}$ is our target dissimilarity value $D_{t,m}$. We analyze the time complexity of DTW update using Lemma~\ref{dtw_time}.
\begin{lemma}
\label{dtw_time}
The time complexity of DTW update is $O(m)$.
\end{lemma}
\begin{proof}
In Figure~\ref{fig:dtw}, it needs to update $D_{t,1}$ from $D_{t-1,1}$ and then update $D_{t,i}$ for $2 \leq i \leq m$ from its neighbors. In each time step, the computation is $O(1)$ and thus the total time complexity is $O(m)$, where $m$ is the length of query trajectory.
\end{proof}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/dtw}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{\small{Illustrating the DTW distance update.}}\label{fig:dtw}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}
Next, we show the online part of DTW subtrajectory search in Algorithm~\ref{algo:dtw}, which has a similar framework with $t2vec$. Note that the input $Q^*$ has been trained offline. In addition, DTW is a point-matching based method, so our Intuition~\ref{intu} can be guaranteed in this similarly measure (We proof it in Lemma~\ref{dtw_sim_nochange}.), and we can directly input reverse trajectories in order to achieve fast computation for suffix similarity $\Psi_S$. Further, we denote state $s = (\Psi, \Psi_{P}, \Psi_{S})$ because the $\Psi_S$ is an exact value now for DTW similarity.

\begin{lemma}
\label{dtw_sim_nochange}
The Intuition~\ref{intu} is correct for DTW distance.
\end{lemma}
\begin{proof}
Given two trajectories $C$ and $Q$
\begin{equation*}
  C = <p_1,...,p_i,...,p_n>, Q = <q_1,...,q_j,...,q_m>.
\end{equation*}
DTW distance is to construct a warp path $W$
\begin{equation*}
  W = w_1,w_2,...,w_K, \text{ } \max(n,m) \leq K < n+m,
\end{equation*}
where $K$ is the length of the warp path, and the $k^{th}$ element of the warp path is $w_k=(i,j)$, $i$ is an index from trajectory $C$ and $j$ is an index from trajectory $Q$. In addition, the starting and ending points of this path are fixed that is $w_1 = (1, 1)$ and $w_K = (n, m)$.
The objective of DTW distance is to find an optimal warp path (or point matching) which has the minimal cumulative distances.
\begin{equation}
  D_{n,m} = \sum\nolimits_{k=1}^{K}d(p_i,q_j), \text{ and } w_k=(i,j),
\end{equation}
where $D_{n,m}$ is the DTW distance of trajectory $C$ with length $n$ and $Q$ with length $m$, $d$ denotes Euclidean distance of two points. We observe the similarity $D_{n,m}$ is independent of the order of accumulation when the optimal warp path is given, that is the similarity is unchanged if we read $C$ and $Q$ in reverse.
\end{proof}

\textcolor[rgb]{1.00,0.00,0.00}{In algorithm~\ref{algo:dtw}, we first need to do the preprocess for suffix similarity and the corresponding DTW values are record in computation matrix $Mat$ as shown in Figure~\ref{fig:dtw} (line 1). Before the for-loop of iterating the time steps (lines 3-18), we need to initialize the index of splitting point $sp$, update vector $\mathcal{V}$, dissimilarity value $\Psi$ and its maintaining interval $\Lambda$ first (lines 2). After that, we select an action guided by $Q^*$ (line 4), if $a = 1$, we cut the trajectory at this time step (lines 5-7). Next, we compute the prefix similarity $\Psi_P$ and suffix similarity $\Psi_S$ and get their intervals (lines 8-9), and concatenate $(\Psi, \Psi_P, \Psi_S)$
as the current state $s$, which is used to input to $Q^*$ (line 10). Finally, we need to maintain the current best subtrajectory from prefix or suffix trajectory (lines 11-17).}

\begin{algorithm}[t]
	\caption{Online Subtrajectory Search for DTW}
	\footnotesize{
		\label{algo:dtw}
		\begin{algorithmic}[1]
			\Require
			Candidate trajectory $C$, query trajectory $Q$ and learned $Q^*$;
			\Ensure
			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
            \State get DTW computation matrix $Mat$ for reverse trajectory $C$ and $Q$;
            \State initialize $sp \leftarrow 1$, $\mathcal{V}_0 \leftarrow None$, $\Lambda \leftarrow [1,n]$, $\Psi \leftarrow Mat_{n,m}$;
            \For{each time step $2 \leq t \leq n$}
            \State select $a = max_{a}Q^*(s,a;\theta)$ using $Q^*$;
            \If{$a = 1$}
            \State $sp \leftarrow t$, $\mathcal{V}_{t-1} \leftarrow None$;
            \EndIf
            \State $\Gamma \leftarrow [sp, t]$, $\Delta \leftarrow [t+1, |C|]$, $\mathcal{V}_t \leftarrow dtw(\mathcal{V}_{t-1}, p_t, Q)$;
            \State $\Psi_P \leftarrow \mathcal{V}_{t,m}$, $\Psi_S \leftarrow Mat_{n-t,m}$;
            \State $s \leftarrow concat(\Psi, \Psi_{P}, \Psi_{S})$;
            \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
                \If {$\Psi_{P} < \Psi_{S}$}
                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
                \Else
                    \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
                \EndIf
            \EndIf
            \EndFor
	\end{algorithmic}}
\end{algorithm}

%\begin{algorithm}[t]
%	\caption{Maintain}
%	\footnotesize{
%		\label{rlst_2}
%		\begin{algorithmic}[1]
%			\Require
%			$\Psi, \Psi_{P}, \Psi_{S}, \Lambda, \Gamma, \Delta$;
%			\Ensure
%			Updated $\Lambda$, $\Psi$;
%            \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
%                \If {$\Psi_{P} < \Psi_{S}$}
%                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                \Else
%                    \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
%                \EndIf
%            \EndIf
%	\end{algorithmic}}
%\end{algorithm}
\begin{lemma}
The time complexity of DTW based subtrajectory similarity computation is $O(nm)$.
\end{lemma}
\begin{proof}
As shown In Algorithm~\ref{algo:dtw}, (1) it takes $O(nm)$ to conduct preprocessing for suffix similarity (line 1). (2) In each time step, the time cost of action selection by $Q^*$ is a constant as explained before (line 6). (3) The time cost of DTW distance update (line 11) is $O(m)$ as shown in Lemma~\ref{dtw_time}. Hence, the overall time complexity is $O(nm)$.
\end{proof}

\subsection{Frechet Distance}
\begin{definition}[Frechet Distance]
Given a candidate trajectory $C = <p_1, p_2,...,p_n>$ and a query trajectory $Q = <q_1, q_2,...,q_m>$, Frechet is computed as below
\begin{equation}
F_{n,m}=\left\{
\begin{aligned}
&\max\nolimits_{i=1}^{n}d(p_i,q_1)&\text{if }m = 1\\
&\max\nolimits_{j=1}^{m}d(p_1,q_j)&\text{if }n = 1\\
&\max(d(p_n,q_m),\\
& \min(F_{n-1,m-1},F_{n-1,m},F_{n,m-1}))&\text{otherwise}
\end{aligned}
\right.
\end{equation}
$F_{n,m}$ is Frechet distance between the prefix trajectory of $C$ with length $n$ and the prefix trajectory of $Q$ with length $m$, and $d(p_n,q_m)$ denotes the Euclidean distance of point $p_n$ and $q_m$.
\end{definition}
We observe the definition of Frechet distance has a similar form with DTW, and thus we have the Frechet update equation as follows.
\begin{equation}\label{dtwupdate}
  \mathcal{V}_{t} = frechet(\mathcal{V}_{t-1}, p_{t}, Q), F_{t,m} = \mathcal{V}_{t,m},
\end{equation}
Similarly, the Lemma~\ref{dtw_sim_nochange} is fulfilled by Frechet distance, and we can replace $dtw(\cdot,\cdot,\cdot)$ as $frechet(\cdot,\cdot,\cdot)$ simply in the framework of Algorithm~\ref{algo:dtw}.


==> v13 - technical/parameter.tex <==
%\subsection{Parameter Study}\label{para_study}
\noindent\textbf{The effect of parameters.} This experiment is to evaluate the effect of the soft margin $\xi$ for SizeS. Intuitively, a big $\xi$ value indicates a larger search space, which approaches the search space of the ExactS algorithm as $\xi$ increases. Therefore, SizeS will check more candidate subtrajectories and its running time of SizeS will increase.  Figure~\ref{para_fls} shows the effectiveness results in terms of AR, MR and RR and the running time on 10,000 trajectory pairs of Porto dataset. In Figure~\ref{para_fls}, we increase the value of $\xi$ until the result of SizeS is better than that of RLS in terms of AR, MR and RR.
%, and at the same time, we show the RLS and Exact results for ease of reference.
As expected, as $\xi$ grows the effectiveness of SizeS (as shown in Figure~\ref{para_fls}(a)-(c) for t2vec, (e)-(g) for DTW and (i)-(k) for Frechet) becomes better (approaches and exceeds RLS gradually); However, its running time  increases and approaches that of the exact algorithm while RLS runs much master (as shown in Figure~\ref{para_fls}(d) for t2vec, (h) for DTW and (l) for Frechet).

%Additionally, we can observe that the time change of DTW and Frechet is more significantly than t2vec as $\xi$ increases. This is because the incremental computation for DTW and Frechet is linear, which is higher than the constant update of t2vec as shown in Lemma~\ref{dtw_time}.


%\begin{figure}
%\centering
%\begin{tabular}{c c c}
%  \begin{minipage}{4cm}%5.5
%	\includegraphics[width=4cm]{figures/par_ar}
%  \end{minipage}
%  &
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{figures/par_mr}
%  \end{minipage}
%  \\
%  \scriptsize{(a) Approximation Ratio}
%  &
%  \scriptsize{(b) Mean Rank}
%  \\
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{figures/par_rr}
%  \end{minipage}
%  &
%  \begin{minipage}{4cm}
%	\includegraphics[width=4cm]{figures/par_time}
%  \end{minipage}
%  \\
%  \scriptsize{(c) Relative Rank}
%  &
%  \scriptsize{(d) Time Cost}
%  \end{tabular}
%  \setlength{\belowcaptionskip}{1pt}
%\caption{The influence of soft margin $\xi$ in FLS.}
%\label{para_fls}
%\vspace*{-2mm}
%\end{figure}
\begin{figure*}
\hspace*{-.3cm}
\centering
\begin{tabular}{c c c c}
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/t2v_ar}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/t2v_mr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/t2v_rr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/t2v_time}
  \end{minipage}
  \\
  \small (a) Approximation Ratio (t2vec)
  &
  \small (b) Mean Rank (t2vec)
  &
  \small (c) Relative Rank (t2vec)
  &
  \small (d) Time Cost (t2vec)
  \\
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/dtw_ar}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/dtw_mr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/dtw_rr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/dtw_time}
  \end{minipage}
  \\
  \small (e) Approximation Ratio (DTW)
  &
  \small (f) Mean Rank (DTW)
  &
  \small (g) Relative Rank (DTW)
  &
  \small (h) Time Cost (DTW)
  \\
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/fre_ar}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/fre_mr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
  \includegraphics[width=4.5cm]{figures/fre_rr}
  \end{minipage}
  &
  \begin{minipage}{4.15cm}
    \includegraphics[width=4.5cm]{figures/fre_time}
  \end{minipage}
  \\
  \small (i) Approximation Ratio (Frechet)
  &
  \small (j) Mean Rank (Frechet)
  &
  \small (k) Relative Rank (Frechet)
  &
  \small (l) Time Cost (Frechet)
\end{tabular}
\caption{The influence of soft margin $\xi$ of FLS for t2vec, DTW and Frechet.}
\label{para_fls}
\vspace*{-2mm}
\end{figure*}

%\subsection{Problem Comparison}
\smallskip
\noindent\textbf{Comparison with trajectory similarity computation.}
The traditional Trajectory Similarity Computation (TSC) can be considered as a subproblem of Subtrajectory Similarity Computation (SSC) because the whole trajectory is actually only one of subtrajectories in the target trajectory.
%
This experiment is to evaluate the accuracy if we use the result of TSC to approximate the result of SSC.
  Similar to earlier experiments, we use the exact algorithm as the ground truth, and compare the average results of TSC and SSC  using 10,000 trajectory pairs from Porto and Harbin datasets, respectively. We use RLS for SSC.  As shown in Table~\ref{tscssc}, in terms of effectiveness, we can see that SSC performs much better than TSC: The mean rank and relative rank of TSC are around 10 times larger than those of SSC for t2vec and 20 times for DTW and Frechet.
  %
  This result shows that TSC is not a good approximation for SSC, although TSC runs faster.


%Regarding the efficiency, the time cost of SSC with RLS ia slightly larger than TSC. This is as expected and we explain as follows: (1) for point-matching based measures DTW and Frechet, we need to read trajectories from right to left to get suffix similarities, which is equivalent to a one time TSC; (2) we compute prefix similarities incrementally and it is also equivalent to a one time TSC; (3) we need to call the learning model to obtain a split decision at each time step; (4) note that in t2vec, we do not need to compute the suffix similarities as input, and thus t2vec (around $3\times$ TSC) is faster than DTW and Frechet (around $5\times$ TSC).

\begin{table*}
\hspace*{-.3cm}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Similarity Measure} & \multicolumn{4}{c|}{t2vec} & \multicolumn{4}{c|}{DTW} & \multicolumn{4}{c|}{Frechet} \\ \hline
Dataset                    & Problem    & AR  & MR  & RR  & Time (s) & AR  & MR & RR & Time (s) & AR   & MR  & RR  & Time (s)  \\ \hline
\multirow{2}{*}{Porto}     & TSC        &1.313     &156.153     &23.3\%     &285          &2.100     &752.831    &70.7\%    &181          &1.883      &559.462     &56.5\%     &192           \\ \cline{2-14}
                           & SSC        &1.098     &18.323     &3.0\%     &623          &1.028     &41.138    &3.5\%    &850          &1.034      &34.162     &3.6\%     &739           \\ \hline
\multirow{2}{*}{Harbin}    & TSC        &1.293     &678.311     &46.9\%     &317          &2.326     &1218.908    &72.2\%    & 283          &1.891      &854.042     &53.9\%     &152        \\ \cline{2-14}
                           & SSC        &1.025     &14.945     &1.3\%     &1024          &1.081     &75.324    &4.1\%    & 1346         &1.045      &64.729     &4.4\%     &887       \\ \hline
\end{tabular}
\caption{Comparison with Trajectory Similarity Computation and Subtrajectory Similarity Computation.}
\vspace*{-2mm}
\label{tscssc}
\end{table*}



==> v13 - technical/pfs.tex <==
\subsection{Prefix First Search (PFS)}
\label{ha:pfs}
In Lemma~\ref{lemma:subt}, we know any subtrajectory must correspond to a prefix of a suffix trajectory. Actually, the $\Psi_{S}$ of a suffix trajectory only provides some additional dissimilarity values during the search process, which means that we can ignore the $\Psi_{S}$ and only maintain $\Psi_{P}$ if the given trajectory can be exactly split. Based on this intuition, we design a new algorithm, called Prefix First Search (PFS). We illustrate the main idea using Example~\ref{example_idea_pfs}.

\begin{example}
\label{example_idea_pfs}
Consider a pair of candidate and query trajectory $C$, $Q$ in Figure~\ref{example:pfs}, where $t$ is the current time step.
\begin{itemize}[leftmargin=8pt]
  \item $t=1$, we initialize $sp$ as the current $t$, the initial dissimilarity value $\Psi$ as infinity, the initial intervals $\Lambda, \Gamma$ as empty sets, and the first hidden state as none. Compared with BSS and FSS, we only consider the prefix trajectory $C_{\Gamma=[1,1]}$. we split it because it is smaller than initial dissimilarity value $\Psi$, and then we update $sp$ as the next time step and have $C_{\Lambda=[1,1]}$.
  \item $t=2$, we delete the edge between 1 and 2 because a splitting operation happened in last time. We consider the prefix trajectory $C_{\Gamma=[2,2]}$ (Note that the interval update still follows the Equation~\ref{interval}), and decide to maintain it because it is smaller than current dissimilarity value. And then a splitting happens and $sp$ will be updated to next time step.
  \item $t=3$, we consider the prefix trajectory $C_{\Gamma=[3,3]}$, and do not split it because it is not smaller than current dissimilarity value~\footnote{The dissimilarity value computed by $t2vec$. Here, we only show an example to illustrate the current dissimilarity value is not smaller.}. Note that the current $sp$ is still 2 and not be updated at this time.
  \item $t=4$, we get a new prefix trajectory $C_{\Gamma=[3,4]}$, and maintain it because it is more similar than last $C_{\Lambda=[2,2]}$. A splitting happens at this time and $sp$ will be updated. Hence, the final returned result is the subtrajectory with interval $\Lambda = [3,4]$.
\end{itemize}
\end{example}

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/example_pfs}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{An example illustrating the PFS.}\label{example:pfs}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}

%\begin{algorithm}[t]
%	\caption{Prefix First Search}
%	\footnotesize{
%		\label{pfs}
%		\begin{algorithmic}[1]
%			\Require
%			Candidate trajectory $C$ and query trajectory $Q$;
%			\Ensure
%			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
%			\State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
%            \State get representation vector $h_{Q}$ for query trajectory $Q$;
%            \State initialize $\Psi \leftarrow \infty$, $\Lambda, \Gamma \leftarrow \emptyset$, $sp \leftarrow 1$ and $h_{0} \leftarrow None$;
%			\For{each time step $1 \leq t \leq |C|$}
%                \State $\Gamma \leftarrow [sp, t]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$, $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$;
%                \If {$\Psi_{P} < \Psi$}
%                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                    \State $sp \leftarrow t+1$, $h_{t} \leftarrow None$;
%                \EndIf
%			\EndFor
%	\end{algorithmic}}
%\end{algorithm}
% We present the algorithm details in Algorithm~\ref{pfs}.
\begin{lemma}
The total time complexity of PFS is $O(n)$.
\end{lemma}
\begin{proof}
\textcolor[rgb]{1.00,0.00,0.00}{The time cost of preprocessing is $O(n)$. In each time step, the update of $t2vec$ and Euclidean distance computation are $O(1)$. Hence, the overall time cost of PFS is $O(n)$.}
\end{proof}


==> v13 - technical/preliminary.tex <==
\subsection{Preliminary}
\label{pre:t2vec}
$t2vec$~\cite{li2018deep} is a state-of-the-art trajectory similarity measure based on deep representation learning. It adapts the sequence encoder-decoder framework to build learning model, as depicted in Figure~\ref{t2vec}.
It first considers locations $p$ as discrete tokens, and then maps each $p$ to a corresponding vector $x$ by a pretrained embedding layer, which is a simple forward neural network~\cite{bengio2003neural}. And $x$ can be considered as the representation of the current location $p$.

There are two main modules in the $t2vec$ - an encoder and a decoder. The encoder encodes the sequence $x$ into a fixed-dimensional vector $h$ by a kind of popular recurrent neural networks - GRU. Similarly, each $h$ in the encoder can be considered as the representation of each current prefix subtrajectory. For example in Figure~\ref{t2vec}, $h_1, h_2$ and $h_3$ are the representations of prefix $<p_1>, <p_1, p_2>$ and $<p_1, p_2, p_3>$. In $t2vec$, the representations of last encoder states can be used to compute trajectory similarity by the Euclidean distance between the vectors.

The decoder decodes out predicted location sequence $p^{pred}$ conditioned on the final output by the encoder. Also, $t2vec$ applies specific denoising mechanism and customized loss function, which makes it outperforms many popular similarity measures such as DTW~\cite{yi1998efficient}.

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/t2vec}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{\small{t2vec: representation learning-based trajectory similarity measure. The model reads
  the sequence $x$ and outputs the sequence of predicted location $p^{pred}$, where EOS is a special token indicating the end of a trajectory. Each $x$ is the representation of each $p$, and each hidden vector $h$ is the representation of each corresponding prefix subtrajectory in $<p_{1}, p_{2},...>$.}}\label{t2vec}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}


==> v13 - technical/problem.tex <==

\section{Problem Definition and Preliminaries}
\label{problem_and_preliminary}

%\subsection{Preliminaries}

The trace of a moving object such as a vehicle and a mobile user is usually captured by a trajectory. Specifically, a trajectory $T$ has its form as a sequence of time-stamped locations (called points), i.e., $T = <p_1, p_2, ..., p_n>$, where point $p_i = (x_i, y_i, t_i)$ means that the location is $(x_i, y_i)$ at time $t_i$. The size of trajectory $T$, denoted by $|T|$, corresponds to the number of points of $T$.

Given a trajectory $T=<p_1, p_2, ..., p_n>$ and $1\le i\le j\le n$, we denote by $T[i, j]$ the portion of $T$ that starts from the $i^{th}$ point and ends at the $j^{th}$ point, i.e., $T[i, j] = <p_i, p_{i+1}, ..., p_j>$. Besides, we say that $T[i, j]$ for any $1\le i \le j \le n$ is \emph{subtrajectory} of $T$. There are in total $\frac{n(n+1)}{2}$ subtrajectories of $T$. Note that any subtrajectory of a trajectory $T$ belongs to a trajectory itself.


\subsection{Problem Definition}
Suppose we have a database of many trajectories, which we call \emph{data trajectories}. As discussed in Section~\ref{intro}, one common application scenario would be that a user has a trajectory at hand, which we call a \emph{query trajectory} and would like to check what is the portion of the data trajectories that is the most similar to the one at his/her hand. Note that in some cases, by looking each data trajectory as whole, none is similar enough to the query trajectory, e.g., all data trajectories are relatively long while the query trajectory is relatively short.

We note that a more general query is to find the \emph{top-$k$} similar subtrajectories to a query trajectory, which reduces to the user's query as described above when $k = 1$. In this paper, we stick to the setting of $k=1$ since extending the techniques for the setting of $k=1$ to general settings of $k$ is straightforward. Specifically, the techniques for the setting $k=1$ in this paper are all based on a search process, which maintains the most similar subtrajectory found so far and updates it when a more similar subtrajectory is found during the process. These techniques could be adapted to general settings of $k$ by simply maintaining the $k$ most similar subtrajectories and updating them when a subtrajectory that is more similar than the $k^{th}$ most similar subtrajectory.

An intuitive solution to answer the user's query is to scan the data trajectories, and for each one, compute its subtrajectory that is the most similar to the query one based on some similarity measurement and update the most similar subtrajectory found so far if necessary. This solution could be further enhanced by employing indexing techniques such as the R-tree based index and the inverted-file based index for pruning~\cite{yao2019computing,wang2018torch}, e.g., the data trajectories that do not have any overlap with the query trajectory could usually be pruned. The key component of this solution (no matter whether indexing structures are used or not) is to compute for a given data trajectory, its subtrajectory that is the most similar to a query trajectory. We formally define the problem corresponding to this procedure as follows.
\begin{problem}[Similar Subtrajectory Search]
	Given a data trajectory $T = <p_1, p_2, ..., p_n>$ and a query trajectory $T_q=<q_1, q_2, ..., q_m>$,
	the \textbf{similar subtrajectory search (SimSub)} problem is to find a subtrajectory of $T$,
	denoted by $T[i^*, j^*]$ ($1\le i^* \le j^* \le n$), which is the most similar to $T_q$ according to a trajectory similarity measurement $\Theta(\cdot, \cdot)$,
	i.e., $[i^*, j^*] = \arg\max_{1\le i\le j\le n} \Theta(T[i, j], T_q)$.
	%\done
	\label{subtrajectory-search}
\end{problem}

%Given two trajectories $T$ and $T'$, we denote by $\Theta(T, T')$ the \emph{similarity} between $T$ and $T'$, which captures the extent to which $T$ and $T'$ are similar to each other. The larger the similarity $\Theta(T, T')$ is, the more similar $T$ and $T'$ are.
The SimSub problem relies on a similarity measurement $\Theta(T, T')$, which captures the extent to which two trajectories $T$ and $T'$ are similar to each other. The larger the similarity $\Theta(T, T')$ is, the more similar $T$ and $T'$ are. In the literature, several ``dissimilarity measurements'' have been proposed for $\Theta(\cdot, \cdot)$ such as DTW~\cite{yi1998efficient}, Frechet~\cite{alt1995computing}, LCSS~\cite{vlachos2002discovering}, ERP~\cite{chen2004marriage}, EDR~\cite{chen2005robust}, EDS~\cite{xie2014eds}, EDwP~\cite{ranu2015indexing}, and t2vec~\cite{li2018deep}. Different measurements have different merits and suit for different application scenarios. In this paper, we assume an abstract similarity measurement $\Theta(\cdot, \cdot)$, which could be instantiated with any of these existing measurements by applying some \emph{inverse operation} such as taking the ratio between 1 and a distance.


\if 0
Depending on whether we have indices on the data trajectories, we have two cases. Case 1: some indices such as a R-tree based index and a inverted file based index have been built on the data trajectories. In this case, the indices could be used to prune some data trajectories from being considered, e.g., they do not have any overlap with the query trajectory, and then
\fi
\if 0
We formalize this problem as the \emph{similar subtrajectory search} problem as follows.
\begin{problem}[Similar Subtrajectory Search (SimSub)]
	Let $\mathcal{D}$ be a database of data trajectories.
	Given a query trajectory $Q$,
	the \textbf{similar subtrajectory search} problem is to find a subtrajectory of a trajectory $T^*$, which is the most similar to the query trajectory according to a trajectory similarity measurement $\Theta(\cdot, \cdot)$,
	i.e., $T^* = \max_{T\in \mathcal{D}, 1\le i\le j\le e} \Theta(T[i, j], Q)$.
	%\done
	\label{subtrajectory-search}
\end{problem}
%
We note that a more general problem is one of finding the \emph{top-$k$} similar subtrajectories to a query trajectory, i.e., which reduces to the similar subtrajectory problem as defined above when $k = 1$. In this paper, we stick to the similar subtrajectory search problem since as could be verified later on, extending the techniques for the similar subtrajectory search problem (or the top-$1$ similar subtrajectory search problem) to the top-$k$ version is straightforward. Specifically, the techniques for the top-$1$ version are all based on a search process, which maintains the most similar subtrajectory found so ar and updates it when a more similar subtrajectory is found during the process. These techniques could be adapted to the top-$k$ version by simply maintaining the $k$ most similar subtrajectories and updating them when a subtrajectory that is more similar than the $k^{th}$ most similar subtrajectory.
\fi

\if 0
Let the data trajectory $T$ be $<p_1, p_2, ..., p_n>$ and the query trajectory $Q$ be $<q_1, q_2, ..., q_m>$. That is, $|T| = n$ and $|Q| = m$. Considering that in practice, a data trajectory is usually longer than a query one, we assume that $n \ge m$. We note that the techniques developed in this paper do not rely on this assumption - it is just that with this assumption, the expressions such as those of time complexities would look simpler for ease of presentation and in case that this assumption does not hold, the only consequence is that some expressions need to adjusted by replacing some $n$'s with $m$'s, which is quite straightforward and minor.
\fi



\subsection{Trajectory Similarity Measurements}

The SimSub problem assumes an abstract similarity measurement and the techniques developed could be applied to any existing measurements. Since the time complexity analysis of the algorithms proposed in this paper relies on the time complexities of computing a specific measurement in several different cases, in this part, we review three existing measurements, namely t2vec~\cite{li2018deep}, DTW~\cite{yi1998efficient}, and Frechet~\cite{alt1995computing}, and discuss their time complexities in different cases as background knowledge. The first two are the most widely used measurements and the last one is the most recently proposed one, which is a data-driven measurement.
%
%In this part, we discuss three instantiations of the abstract similarity measurement only, namely DTW, Frechet and t2vec, due to the page limit. The first two are the most widely used measurements and the last one is the most recently proposed one which is a data-driven measurement. Before we give the details of these measurements, we define the notations of three types of time complexity.
%

%Before we give the details of these measurements, we define some time complexity notations that would be used for the time complexity analysis on the algorithms proposed in this paper.
%
We denote by $\Phi$ the time complexity of computing the similarity between a general subtrajectory of $T$ and $T_q$ \emph{from scratch}, $\Phi_{inc}$ be the time complexity of computing $\Theta(T[i, j], T_q)$ ($1\le i < j \le n$) \emph{incrementally} assuming that $\Theta(T[i, j-1], T_q)$ has been computed already, and $\Phi_{ini}$ the time complexity of computing $\Theta(T[i, i], T_q)$ ($1\le i\le n$) from scratch since it cannot be computed incrementally. As will be discussed later, $\Phi_{inc}$ and $\Phi_{ini}$ are usually much smaller than $\Phi$ across different similarity measurements.
%

\smallskip\noindent\textbf{t2vec~\cite{li2018deep}.}
t2vec is a data-driven similarity measure based on deep representation learning. It adapts a sequence-to-sequence framework based on RNN~\cite{cho2014learning} and takes the final hidden vector of the encoder~\cite{rumelhart1988learning} to represent a trajectory. It computes the similarity between two trajectories based on the Euclidean distance between their representations as vectors.

Given $T$ and $T_q$, it takes $O(n)$ and $O(m)$ time to compute their hidden vectors, respectively and $O(1)$ to compute the Euclidean distance between two vectors~\cite{li2018deep}. Therefore, we know $\Phi = O(n + m + 1) = O(n + m)$. Since in the context studied in this paper, we need to compute the similarities between many subtrajectories and a query trajectory $T_q$, we assume that the representation of $T_q$ under t2vec is computed once and re-used many times, i.e., the cost of computing the representation of $T_q$, which is $O(m)$, could be amortized among all computations of similarity and then that for each one could be neglected. Because of the sequence-to-sequence nature of t2vec, given the representation of $T[i, j-1]$, it would take $O(1)$ to compute that of $T[i, j]$ ($1\le i < j\le n$). Therefore, we know $\Phi_{inc} = O(1)$. Besides, we know $\Phi_{ini} = O(1)$ since the subtrajectory involved in the computation of similarity, i.e., $T[i,i]$ ($1\le i\le n$), has its size equal to 1.


\smallskip\noindent\textbf{DTW~\cite{yi1998efficient}.} Given a data trajectory $T = <p_1, p_2,...,p_n>$ and a query trajectory $T_q = <q_1, q_2,...,q_m>$, the DTW distance is defined as below
\begin{equation}
\label{dtw_sm}
D_{i,j}=\left\{
\begin{aligned}
& \sum\nolimits_{h=1}^{i}d(p_h,q_1)&\text{if } j = 1\\
& \sum\nolimits_{k=1}^{j}d(p_1,q_k)&\text{if } i = 1\\
& d(p_i,q_j) + \\
& \min(D_{i-1,j-1}, D_{i-1,j},D_{i,j-1})&\text{otherwise}
\end{aligned}
\right.
\end{equation}
where $D_{i,j}$ denotes the DTW distance between $T[1,i]$ and $T_q[1, j]$ and $d(p_i,q_j)$ is the distance between $p_i$ and $q_j$ (typically the Euclidean distance, which could be computed in $O(1)$). Consider $\Phi$. It is clear that $\Phi = O(n\cdot m)$ since it needs to compute all pairwise distances between a point in a subtrajectory of $T$ and a point in $T_q$ and in general, the subtrajectory has its size of $O(n)$ and $T_q$ has its size of $m$.
%
Consider $\Phi_{inc}$. This should be the same as the time complexity of computing $D_{i,m}$ given that $D_{i-1,m}$ has been computed. Since $D_{i-1,m}$ has been computed, we can safely assume that $D_{i-1,1}$, $D_{i-1,2}$, ..., $D_{i-1,m}$ have been computed also according to Equation~\ref{dtw_sm} (note that we can always make this hold by enforcing that we compute $D_{i-1,m}$ or any other DTW distance in this way). Therefore, in order to compute $D_{i,m}$, we compute $D_{i,1}, D_{i,2}, ..., D_{i,m}$ sequentially, each of which would take $O(1)$ time with the information of $D_{i-1,k}$ ($1\le k\le m$) all available. That is, it takes $O(m)$ to compute $D_{i,m}$, and thus we know that $\Phi_{inc} = O(m)$.
%
Consider $\Phi_{ini}$. We know $\Phi_{ini} = O(m)$ since $T[i, i]$ ($1\le i \le n$) has its size always equal to 1 and $T_q$ has its size of $m$.



\smallskip\noindent\textbf{Frechet~\cite{alt1995computing}.} Given a data trajectory $T = <p_1, p_2,...,p_n>$ and a query trajectory $T_q = <q_1, q_2,...,q_m>$, the Frechet distance is defined as below
\begin{equation}
\label{fre_sm}
F_{i,j}=\left\{
\begin{aligned}
&\max\nolimits_{h=1}^{i}d(p_h,q_1)&\text{if }j = 1\\
&\max\nolimits_{k=1}^{j}d(p_1,q_k)&\text{if }i = 1\\
&\max(d(p_i,q_j),\\
& \min(F_{i-1,j-1},F_{i-1,j},F_{i,j-1}))&\text{otherwise}
\end{aligned}
\right.
\end{equation}
where $F_{i,j}$ denotes the Frechet distance between $T[1,i]$ and $T_q[1, j]$ and $d(p_i,q_j)$ is the distance between $p_i$ and $q_j$ (typically the Euclidean distance, which could be computed in $O(1)$).
%
When the Frechet distance is used, we have $\Phi = O(n\cdot m)$, $\Phi_{inc} = O(m)$, and $\Phi_{ini} = O(m)$, based on similar analysis as for the DTW distance.


The summary of $\Phi$, $\Phi_{inc}$ and $\Phi_{ini}$ for the similarity measurements corresponding to the distance measurements DTW, Frechet and t2vec is presented in Table~\ref{tab:similarity-complexities}.

\begin{table}[t!]
\centering
%	\hspace*{-.4cm}
	\caption{Time complexities of computing the similarity between a subtrajectory of $T$ and $T_q$ in three cases}
	\begin{tabular}{|l||c|c|c|}
		\hline
		{Time complexities}			&	t2vec 		&	DTW				&	Frechet			\\\hline
		$\Phi$ (general)			& 	$O(n + m)$	&	$O(n\cdot m)$	&	$O(n\cdot m)$	\\\hline
		$\Phi_{inc}$ (incremental)	& 	$O(1)$		&	$O(m)$			&	$O(m)$			\\\hline
		$\Phi_{ini}$ (initial)		& 	$O(1)$		&	$O(m)$			&	$O(m)$			\\\hline
	\end{tabular}
	%\vspace*{-2mm}
	\label{tab:similarity-complexities}
\end{table}







\if 0
Let $\Phi$ be the time complexity of computing the similarity between $T$ and $T_q$.

Depending on the similarity measurement, $\Phi$ could be different. For example, in cases that DTW and Frechet are used, $\Phi$ is $O(n\cdot m)$~\cite{yi1998efficient,alt1995computing} and in cases that t2vec is used, $\Phi$ is $O(n + m) $~\cite{li2018deep}.
%

Consider the time complexity of computing a subtrajectory $T[i, j]$ ($1\le i < j \le n$) and the query trajectory $T_q$, i.e., $\Theta(T[i, j], T_q)$. In general, it corresponds to $\Phi$ if the computation starts from scratch. It could be much lower than $\Phi$ if it is computed based on $\Theta(T[i, j-1], T_q)$ \emph{incrementally} and $\Theta(T[i, j-1], T_q)$ has been computed before.
%Specifically, when computing the similarity between a subtrajectory $T[i, j]$ ($1\le i < j \le n$) and the query trajectory $Q$, i.e., $\Theta(T[i, j], Q)$, we utilize the similarity between a smaller subtrajectory $T[i, j-1]$ and $Q$, i.e., $\Theta(T[i, j-1], Q)$, which would be faster than doing it from scratch.
Let $\Phi_{inc}$ be the time complexity of computing $\Theta(T[i, j], T_q)$ based on $\Theta(T[i, j-1], T_q)$.
%Usually, $\Phi_{inc}$ is much smaller than the time complexity of computing $\Theta(T[i, j], Q)$ from scratch, i.e., $\Phi$.

Again, depending on different similarity measurements being used, $\Phi_{inc}$ would be different. For example, as will be shown later (in Section~\ref{section:other}), when DTW or Frechet is used, $\Phi_{inc} = O(m)$ while $\Phi = O(n\cdot m)$ and when t2vec is used, $\Phi_{inc} = O(1)$ while $\Phi = O(n)$. That is, $\Phi_{inc}$ is much lower than $\Phi$, say, be a factor of $O(n)$ for many similarity measurements.
%Besides, by applying this idea recursively, we could compute $\Theta(T[i, j-1], Q)$ based on $\Theta(T[i, j-2], Q)$ and so on and this recursive process stops when we compute $\Theta(T[i, i], Q)$.

Besides, we let $\Phi_{ini}$ be the time complexity of computing $\Theta(T[i, i], T_q)$ (from scratch) since it cannot be computed incrementally.

Again, $\Phi_{ini}$ is much smaller than $\Phi$ since $T[i, i]$ has its size equal to 1. For example, as will be shown later (in Section~\ref{section:other}) when DTW or Frechet is used, $\Phi_{ini} = O(m)$ and when t2vec is used, $\Phi_{ini} = O(1)$. In summary, we present the time complexities of $\Phi$, $\Phi_{inc}$ and $\Phi_{ini}$ for three similarity measurements, DTW, Frechet and t2vec in Table~\ref{tab:similarity-complexities}.
\fi

\if 0
\subsection{Definition}
\label{problem}

\begin{definition}[Trajectory]
The movement of an object corresponds to a sequence of time-stamped locations, which is called a trajectory. Each trajectory $T = <p_1, p_2,...>$ has a sequence of tuples where $p_i = (\hat{x}_i, \hat{y}_i, t_i)$ is the $i^{th}$ location $(\hat{x}_i, \hat{y}_i)$ recorded by GPS with the time stamp $t_i$.
\end{definition}

\begin{definition}[Subtrajectory]
Let interval $\Lambda = [i, j]$ denote the subtrajectory $T_{\Lambda}$, which contains the locations between $p_i$ and $p_j$ of $T$. For any positive integers $i, j$, we have $1 \leq i \leq j \leq |T|$.
\end{definition}

\begin{definition}[Trajectory Similarity Measure]
For any two trajectories $T_i$ and $T_j$, the trajectory similarity measure is a function $f(T_i, T_j)$ that measures the dissimilarity value between $T_i$ and $T_j$.
\end{definition}

There are various types of trajectory similarity measures such as DTW distance and Frechet distance. In this paper, we apply the state-of-the-art trajectory similarity measure, namely $t2vec$~\cite{li2018deep}. It is the first deep learning-based approach to learning representations (vectors) of the underlying routes traveled by trajectories. Given two trajectories, it uses Euclidean distance between their route representations to measure the similarity of the two trajectories. More details are presented in Section~\ref{pre:t2vec}.
%Compared with some existing measures, $t2vec$ is robust to low data quality, and support accurate and efficient trajectory similarity computation and search.

\noindent
\textbf{Problem Statement}. Given a candidate trajectory $\Phi$ and a query trajectory $Q$, the goal of subtrajectory similarity computation is to find a subtrajectory $\Phi_{\Lambda}$ of $\Phi$, which has the minimum dissimilarity value $\Psi$ with $Q$.

Note that $t2vec$ captures trajectory similarity by the Euclidean distances in vector space. Thus, for any two trajectories, if they are similar, the dissimilarity value (or distance) between their vectors would be small.

The notations that are frequently used throughout the paper are given in Table~\ref{notation}.
\begin{table}
  \centering
  \small{
  \setlength{\belowcaptionskip}{1pt}
  \caption {Notations and meanings.}\label{notation}
  \begin{tabular}{c|c}
     \hline
          {\bf Notation}     & {\bf Meaning}\\
     \hline\hline
     $\mathcal{D}$ & Trajectory database\\
     \hline
          $C, Q$  & Candidate, query trajectory \\
     \hline
          $\overleftarrow{C}, \overleftarrow{Q}$ & Reverse candidate, reverse query trajectory \\
     \hline
          $x_{t}$  & Token vector at position $t$\\
     \hline
          $h_{t}, h'_{t}$ & Hidden state, backward hidden state at position $t$\\
     \hline
          $t2vec(h_{t-1},x_{t})$ &  t2vec learning model with input $h_{t-1}$ and $x_{t}$\\
     \hline $d(\cdot,\cdot)$ & Euclidean distance between two vectors\\
     \hline
          $\Phi_{\Lambda}$ & Results of subtrajectory with interval $\Lambda$\\
     \hline
          $\Psi$ & Results of subtrajectory dissimilarity value\\
     \hline
          $\Psi_{P}, \Psi_{S}$ & Prefix, suffix subtrajectory dissimilarity value\\
     \hline
          $\Gamma$ & Prefix interval\\
     \hline
          $\Delta$ & Suffix interval\\
     \hline
          $sp$ & Index of split point\\
     \hline
          $\widehat{t2vec}$ & t2vec model captured reverse trajectories\\
     \hline
          $K$ &  Delayed steps\\
     \hline
          $s,a,r$ & State, action, reward in reinforcement learning\\
     \hline
          $Q^*(s,a)$ & action-value function in reinforcement learning\\
     \hline
  \end{tabular}}
\end{table}
\fi


==> v13 - technical/proof.tex <==
\section{Theoretical Analysis}
For any given data trajectory $T$ with the length $n$, we denote $\Psi(\cdot) = \frac{rank_{T}(T_{\Lambda})}{\#subt_{T}}$ to measure the closeness of approximate approaches to the optimal result, where $\#subt_{T} = \frac{n(n+1)}{2}$ denotes the total number of candidate subtrajectories in $T$, and $rank_{T}(T_{\Lambda})$ denotes the rank of the returned subtrajectory $T_{\Lambda}$ by one of approximate approaches. Here, we default to rank all the subtrajectories in ascending order of their dissimilarity values with query, and thus a smaller $\Psi$ means that the result is closer to the optimal.

\begin{theorem}
$\Psi$(SizeS) has an upper bound $\frac{n^2-(4\xi+1)n+(4\xi+2)m-4\xi}{n^2+n}$.
\end{theorem}
\begin{proof}

Recall that in SizeS, we need to enumerate all subtrajectories with sizes within the range $[m-\xi, m+\xi]$, where $m$ is the length of query trajectory and $\xi \in [0, n-m]$ is a pre-defined parameter. During the search process, we will traverse $\Delta = (n-m+1)(2\xi+1)$ subtrajectories by SizeS and maintain the best one between them. We can assume that these subtrajectories are the worst of all $\#subt_{T}$ subtrajectories in $T$, because we cannot know one subtrajectory will definitely be better than another, that depends on the trajectory measurements (e.g. t2vec is a learning-based similarity.), and thus $\Delta$ is bounded by $\xi$ as $n-m+1 \leq \Delta \leq 2(n-m)^2+3(n-m)+1$, and we can further get an upper bound:
\begin{equation}
\begin{aligned}
\Psi(SizeS) & \leq \frac{\#subt_{T}-(n-m+1)+1}{\#subt_{T}}= \frac{n^2-n+2m}{n^2+n},
\end{aligned}
\end{equation}
and a lower bound:
\begin{equation}
\begin{aligned}
\Psi(SizeS) & \geq \frac{\#subt_{T}-(2(n-m)^2+3(n-m)+1)+1}{\#subt_{T}}\\
&= \frac{-3n^2-4m^2+8mn-5n+6m}{n^2+n}.
\end{aligned}
\end{equation}

\end{proof}

\begin{theorem}
The upper bound of $\Psi$(PSS) and $\Psi$(RLS) is $\frac{n^2-3n+2}{n^2+n}$.
\end{theorem}
\begin{proof}
Recall that in the splitting-based algorithms PSS or RLS, it needs to make a decision (split or not) at each time step, and we can always get two different subtrajectories (prefix and suffix), and thus we will traverse $2n$ subtrajectories during the search and maintain the best. Similarly, we can get an upper bound for PSS and RLS:
\begin{equation}
\begin{aligned}
\Psi(PSS), \Psi(RLS) \leq \frac{\#subt_{T}-2n+1}{\#subt_{T}} = \frac{n^2-3n+2}{n^2+n}.
\end{aligned}
\end{equation}
\end{proof}

\begin{theorem}
The upper bound of $\Psi$(POS) is $\frac{n^2-n+2}{n^2+n}$.
\end{theorem}
\begin{proof}
In POS, we only consider the prefix subtrajectories during the search, and the upper bound of $\Psi(POS)$ is $\frac{\#subt_{T}-n+1}{\#subt_{T}} = \frac{n^2-n+2}{n^2+n}$.
\end{proof}

\begin{theorem}
$\Psi$(POS-D) has an upper bound $\frac{n^2-n+2}{n^2+n}$, and a lower bound $\frac{n^2-(4K+1)n+2}{n^2+n}$.
\end{theorem}
\begin{proof}
POS-D is an improved version of POS, it waits for $K (K > 0)$ positions when a more similar prefix is found and then split at one of these positions, and scan $T$ again from the split. Thus, Let $ \Delta = n+\overline{K}\#split$ denote the number of subtrajectories traversed by POS-D, where $\overline{K}$ denotes the uncovered mean number of subtrajectories during the delay, which is bounded by $0 \leq \overline{K} \leq 2K$, and $\#delay$ means the number of delay, that is $0\leq \#delay \leq n$. Thus $n \leq \Delta \leq (2K+1)n$. Further. we have:
\begin{equation}
\begin{aligned}
\frac{\#subt_{T}-(2K+1)n+1}{\#subt_{T}} &\leq \Psi(POS-D) \leq \frac{\#subt_{T}-n+1}{\#subt_{T}}\\
\frac{n^2-(4K+1)n+2}{n^2+n} & \leq \Psi(POS-D) \leq \frac{n^2-n+2}{n^2+n}
\end{aligned}
\end{equation}
\end{proof}

The summary of theoretical analysis on achievable guarantees of approximate algorithms is presented in Table~\ref{tab:algorithm-theoretical}.
\begin{table}[t!]
	%	\hspace*{-.3cm}
	\caption{Theoretical analysis of approximate algorithms}
	\begin{tabular}{|l||c|c|c|c|}
		\hline
		Algorithms		&	lower bound &	upper bound							\\\hline
		SizeS			&	$\frac{-3n^2-4m^2+8mn-5n+6m}{n^2+n}$ &   $\frac{n^2-n+2m}{n^2+n}$  \\\hline
		PSS	            &   N/A &	$\frac{n^2-3n+2}{n^2+n}$		\\\hline
        POS	            &   N/A &   $\frac{n^2-n+2}{n^2+n}$  	\\\hline
        POS-D	        &   $\frac{n^2-(4K+1)n+2}{n^2+n}$ &	$\frac{n^2-n+2}{n^2+n}$   \\\hline
		RLS			    &   N/A &	$\frac{n^2-3n+2}{n^2+n}$  \\\hline
	\end{tabular}
	%	\vspace*{-2mm}
	\label{tab:algorithm-theoretical}
\end{table}


==> v13 - technical/related.tex <==
\section{RELATED WORK}
\label{related}
\textbf{Measuring Trajectory Similarity}.
Measuring the similarity between trajectories is a fundamental problem and has been studied extensively. Some classical solutions focus on indexing trajectories and performing similarity computation by the alignment of matching sample points. For example, DTW~\cite{yi1998efficient} is the first attempt at solving the local time shift issue for computing trajectory similarity. Frechet distance~\cite{alt1995computing} is a classical similarity measure that treats each trajectory as a spatial curve and takes into account the location and order of the sampling points. Further, ERP~\cite{chen2004marriage} and EDR~\cite{chen2005robust} are proposed to improve the ability to capture the spatial semantics in trajectories. However, these point-matching methods are inherently sensitive to noise and involved in quadratic time complexity, which exists commonly in trajectory-related problems. In recent years, some learning-based algorithms were proposed to speed up the similarity computation. Li et al.~\cite{li2018deep} propose to learn representations of trajectories in the form of vectors and then measure the similarity between two trajectories as the Euclidean distance between their corresponding vectors. Based on the deep representation learning, Wang et al.~\cite{wang2019effective} propose multiple trajectory similarity used in sports retrieval. Yao et al.~\cite{yao2019computing} employ deep metric learning to accelerate trajectory similarity computation. Nevertheless, all of the above-mentioned studies focus on measuring the whole trajectory similarity, which cannot be directly applied to measuring subtrajectory similarity. In particular, the efficiency of conventional similarity measures is challenged by a much larger candidate set, as a trajectory with length $n$ consists of $O(n^2)$ possible subtrajectories if we only simply enumerate each one.

\noindent
\textbf{Subtrajectory Similarity Related Problems}.
Measuring subtrajectory similarity is also a fundamental functionality in many tasks such as clustering~\cite{agarwal2018subtrajectory,lee2007trajectory,buchin2011detecting} and similarity join~\cite{tampakis2019distributed}. In~\cite{lee2007trajectory}, a general partition and group framework for subtrajectory clustering is proposed by Lee et al. Further, Buchin et al.~\cite{buchin2011detecting} show that the hardness of subtrajectory clustering based on Freechet distance, and Agarwal et al.~\cite{agarwal2018subtrajectory} apply the trajectory simplification technique to approximate discrete Frechet to reduce the time cost of clustering. Very recently, Tampakis et al.~\cite{tampakis2019distributed,tampakis2019scalable} proposed a distributed solution for subtrajectory join and clustering by utilizing the MapReduce programming model. Although these algorithms are related to subtrajectory similarity computation, they only focus on some specific problem settings and specific similarity measures such as Frechet distance. Additionally, in~\cite{van2007definition}, computation of subtrajectory similarity is proposed by considering the shape-dependent and time-dependent of trajectories. To improve the insufficiency of the existing point-matching trajectory measures, Xie et al.~\cite{xie2014eds} proposed a new segment-based distance EDS for subtrajectory similarity search. Although subtrajectory similarity computation is an important problem, it still lacks an efficient and general solution so far. For example, EDS is only a specially designed similarity measure and it also involves the $O(n^3)$ time complexity because of traversing all possible subtrajectories.

\noindent
\textbf{Index-based Trajectory Search}. Fast trajectory similarity search for large-scale database has attracted plenty of research interest as well. Classical trajectory works spend more effort on indexing DTW distance~\cite{yi1998efficient,keogh2005exact}. Subsequently, many studies proposed other advanced index structures for their respective similarity measures such as LCSS~\cite{vlachos2002discovering}, ERP~\cite{chen2004marriage} and EDR~\cite{chen2005robust}. In recent years, Ranu et al.~\cite{ranu2015indexing} formulate a robust distance function called EDwP and develop a new index TrajTree by borrowing the idea of TB-tree index~\cite{pfoser2000novel} and SETI~\cite{chakka2003indexing}. In addition, Yao et al.~\cite{yao2019computing} employ two spatial-based indexes (R-tree and Grid Inverted) for their trajectory similarity search based on metric learning.

\noindent
\textbf{Subsequence (Substring) Matching}. There is another related but different problem of subtrajectory similarity computation, called subsequence matching, which aims to obtain a subsequence that has the same length as the query in a given candidate sequence. In general, the candidate sequence is relatively long, containing for example millions or even trillions~\cite{rakthanmanon2012searching,rakthanmanon2013addressing} of elements. Several existing works ~\cite{gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked,moon2001duality,faloutsos1994fast} have proposed efficient pruning algorithms to obtain the matching. Compared with solutions of trajectory or subtrajectory similarity problems, there is no constraint for the length of query and candidate trajectories. In other words, the length of the target subtrajectory is not fixed. In addition, most of the subsequence studies proposed lower bounding pruning or early abandoning techniques based on some specific distance such as DTW~\cite{gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked} and Euclidean distance~\cite{faloutsos1994fast,moon2001duality}; however, our solution is general and distance independent. Similar to subsequence matching, substring matching wants to find exact occurrences of a short query string within a long candidate string, classical solutions such as KMP algorithm. To generalize from strings to continuous time series, chen et al.~\cite{chen2005robust} proposed EDR to handle strict equality of strings, it takes the real values
into account and relaxes equality to be within a certain tolerance. Further, they proposed a metric based similarity measure ERP~\cite{chen2004marriage} based on a similar idea of EDR.

\noindent
\textbf{Reinforcement Learning}. The goal of reinforcement learning is to guide agents on how to take actions to maximize a cumulative reward~\cite{sutton2018reinforcement} in an environment with unknown parameters, and the environment is generally modeled as a Markov decision process (MDP)~\cite{puterman2014markov}. In recent years, RL models are often utilized to solve some database related problems. For example, Zhang et al.~\cite{zhang2019end} use RL model for automatic DBMS tuning. Trummer et al.~\cite{trummer2018skinnerdb} use RL to learn optimal join orders in the SkinnerDB system. Wang et al.~\cite{wang2019adaptive} design an effective RL-based algorithm to the bipartite graph matching.
In this paper, we study subtrajectory similarity computation based on a popular reinforcement learning method - Deep Q Network (DQN), which is widely used to solve some problems with large state space such as Atari~\cite{mnih2013playing}. To the best of our knowledge, this is the first learning-based solution that supports measuring subtrajectory similarity.


==> v13 - technical/related_v2.tex <==
\section{RELATED WORK}
\label{related}

\noindent\textbf{(1) Trajectory Similarity Measurements.}
Measuring the similarity between trajectories is a fundamental problem and has been studied extensively. Some classical solutions focus on indexing trajectories and performing similarity computation by the alignment of matching sample points. For example, DTW~\cite{yi1998efficient} is the first attempt at solving the local time shift issue for computing trajectory similarity. Frechet distance~\cite{alt1995computing} is a classical similarity measure that treats each trajectory as a spatial curve and takes into account the location and order of the sampling points. Further, ERP~\cite{chen2004marriage} and EDR~\cite{chen2005robust} are proposed to improve the ability to capture the spatial semantics in trajectories. However, these point-matching methods are inherently sensitive to noise and suffer from quadratic time complexity. EDS~\cite{xie2014eds} and EDwP~\cite{ranu2015indexing} are two segment-matching methods, which operate on segments for matching two trajectories.
In recent years, some learning-based algorithms were proposed to speed up the similarity computation. Li et al.~\cite{li2018deep} propose to learn representations of trajectories in the form of vectors and then measure the similarity between two trajectories as the Euclidean distance between their corresponding vectors.
%
Some other studies~\cite{wang2018torch,yuan2019distributed,wang2019fast} define similarity measurements on trajectories based on road segments, to which the trajectories are matched.
%Based on the deep representation learning, Wang et al.~\cite{wang2019effective} propose multiple trajectory similarity used in sports retrieval.
Yao et al.~\cite{yao2019computing} employ deep metric learning to approximate and accelerate trajectory similarity computation.
%
In addition, Ma et al.~\cite{ma2012ksq} propose a similarity measurement called p-distance for uncertain trajectories and study the problem of searching for top-k similar trajectories to a given query trajectory based on p-distance.
%
Different specialized index techniques are developed for these similarity measures, such as DTW distance~\cite{yi1998efficient,keogh2005exact}, LCSS~\cite{vlachos2002discovering}, ERP~\cite{chen2004marriage}, EDR~\cite{chen2005robust}, and EDwP~\cite{ranu2015indexing}. However, these index techniques do not generalize to other similarity measures or subtrajectory similarity search.
%
%{\color{red}Some more detailed review of similarity measurements on trajectory data could be found in~\cite{su2020survey,wang2020survey}.}
%Following the work by Yao et al.~\cite{yao2019computing}, we also consider employing two spatial-based indexes (R-tree and Grid Inverted) for subtrajectory similarity search in our experiments.
%
In this paper, we assume an abstract trajectory similarity measurement, which could be instantiated with any of these existing similarity measurements and our techniques still apply.
\if 0
Nevertheless, all of the aforementioned studies focus on measuring the whole trajectory similarity and are not suitable for directly measuring subtrajectory similarity.
In this work, we develop a framework to use the existing trajectory similarity measures by numerating the subtrajectories and compute the similarity of each subtrajectory and the query trajectory. However, the complexity is high (to be discussed in Section~\ref{sec:non-learning}).
\fi
%
%In particular, the efficiency of conventional similarity measures is challenged by a much larger candidate set, as a trajectory with length $n$ consists of $O(n^2)$ possible subtrajectories if we only simply enumerate each one.

\smallskip
\noindent
\textbf{(2) Subtrajectory Similarity Related Problems.}
Measuring subtrajectory similarity is also a fundamental functionality in many tasks such as clustering~\cite{agarwal2018subtrajectory,lee2007trajectory,buchin2011detecting} and similarity join~\cite{tampakis2019distributed}. Lee et al~\cite{lee2007trajectory} propose a general partition and group framework for subtrajectory clustering. Further, Buchin et al.~\cite{buchin2011detecting} show the hardness of subtrajectory clustering based on Frechet distance, and Agarwal et al.~\cite{agarwal2018subtrajectory} apply the trajectory simplification technique to approximate discrete Frechet to reduce the time cost of subtrajectory clustering. Recently, Tampakis et al.~\cite{tampakis2019distributed,tampakis2019scalable} proposed a distributed solution for subtrajectory join and clustering by utilizing the MapReduce programming model. Although these algorithms need to consider subtrajectory similarity, similarity computation is not their focus and they usually first segment a trajectory into subtrajectories and employ an existing measure, such as Freechet distance.
%Additionally, in~\cite{van2007definition}, computation of subtrajectory similarity is proposed by considering the shape-dependent and time-dependent of trajectories.
%Xie et al.~\cite{xie2014eds} proposed a new segment-based distance EDS for subtrajectory similarity search, which takes $O(n^3)$ time complexity. Although subtrajectory similarity computation is an important problem, there exists no efficient solution.
%\noindent
%\textbf{Index-based Trajectory Search}. Different specialized index techniques are developed for these similarity measures, such as DTW distance~\cite{yi1998efficient,keogh2005exact}, LCSS~\cite{vlachos2002discovering}, ERP~\cite{chen2004marriage}, EDR~\cite{chen2005robust}, and EDwP~\cite{ranu2015indexing}. However, these index techniques do not generalize to other similarity measures or subtrajectory similarity search. Following the work by Yao et al.~\cite{yao2019computing}, we also consider employ two spatial-based indexes (R-tree and Grid Inverted) for trajectory similarity search in our experiments.

\smallskip
\noindent
\textbf{(3) Subsequence (Substring) Matching.} Subsequence matching is a related but different problem. It aims to find a subsequence that has the same length as the query in a given candidate sequence, which usually contains millions or even trillions~\cite{rakthanmanon2012searching,rakthanmanon2013addressing} of elements. Efficient pruning algorithms~\cite{gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked,moon2001duality,faloutsos1994fast} have been proposed for the matching, and these pruning algorithms are generally designed for a specific similarity measure, such as DTW~\cite{gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked,park2000efficient,kim2001index} and Euclidean distance~\cite{faloutsos1994fast,moon2001duality}, and cannot generalize to other measures.
%Similar to subsequence matching, substring matching~\cite{uno2008efficient,warren2006multi} wants to find exact occurrences of a short query string within a long candidate string. In contrast, in subtrajectory search the length of the target subtrajectory is not fixed and these solutions for subsequence matching or substring matching cannot be used to solve subtrajectory matching problem.
On the other hand, substring matching~\cite{kim2013efficient,zhang2010bed} often focuses on approximate matching based on the Edit distance. It aims to find a substring in a string to best match the query. Our problem differs from the substring matching problem mainly in two aspects. First, characters in a string have exact match (0 or 1) in the alphabet; however, the points of a trajectory are different. Second, substring matching techniques are usually designed based on the characteristics of strings. e.g.,
grammar structure patterns, or word concurrence patterns; however, a trajectory does not have such patterns.
%In terms of the idea of fuzzy matching inspired by substring (or subsequence) matching, we will compare it with our methods in experiments.

\smallskip
\noindent
\textbf{(4) Reinforcement Learning.} The goal of reinforcement learning is to guide agents on how to take actions to maximize a cumulative reward~\cite{sutton2018reinforcement} in an environment, and the environment is generally modeled as a Markov decision process (MDP)~\cite{puterman2014markov}. Recently, RL models have been utilized successfully to solve some database related problems. For example, Zhang et al.~\cite{zhang2019end} and Li et al.~\cite{li2019qtune} use RL model for automatic DBMS tuning. Trummer et al.~\cite{trummer2018skinnerdb} use RL to learn optimal join orders in the SkinnerDB system. Wang et al.~\cite{wang2019adaptive} design an effective RL-based algorithm for bipartite graph matching. Overall, there are two types of popular reinforcement learning methods: (1) model-based methods~\cite{brafman2002r,kearns2002near} that require to understand the environment and learn the parameters of the MDP in advance, and (2) model-free methods~\cite{watkins1992q,mnih2013playing} that make no efforts to learn a model and get feedback from the environment step by step. In this paper, we follow the model-free methods because they are more efficient. Specifically, we make use of a popular reinforcement learning method, namely Deep $Q$ Network (DQN)~\cite{mnih2013playing}, for splitting a trajectory into subtrajectories to be candidate solutions for similar subtrajectory search.
%, which is able to significantly reduce the complexity of subtrajectory similarity computation. Our solution is generic and is applicable to all the exiting trajectory similarity measures.


==> v13 - technical/response.tex <==

\newpage

\noindent
{\large
\textbf{Response to Review Report of Paper Titled with ``Efficient and Effective Similar Subtrajectory Search with Deep Reinforcement Learning'' (VLDB20 Paper ID = 1006)}}
%\label{sec:response}

\smallskip\noindent Dear PVLDB Meta-reviewer and Reviewers,

\smallskip
First, we would like to thank the reviewers for their constructive and inspiring comments. We have gone through these comments carefully and revised our draft accordingly.  Below we summarize the major changes that we have made in the revised paper.

%\section{Major Changes}
%\label{sec:majorChanges}

%We have the following major changes (marked in red of the current submission).
%\smallskip\noindent\textbf{Summary of Major Changes:}

\begin{enumerate}
  \item We have included some discussions on the approximation qualities of all approximate algorithms proposed in this paper. They could be found in the individual sections where the algorithms are proposed (Section~\ref{sec:non-learning} and Section~\ref{section:RLS}). Due to the page limit, we put their corresponding proofs in the appendix of the technical report version~\cite{TR}.
  \item We have included an example problem (shown in Figure~\ref{fig:input}) and use it for illustrating two representative algorithms PSS and RLS-Skip in Table~\ref{table:pss} and Table~\ref{table:rls_skip}, respectively.
  \item We have included two competitor algorithms, namely UCR and Random-S. UCR is adapted from the literature of time series as inspired by Reviewer 1's Comment 1 and Random-S is suggested by Reviewer 3. The descriptions of these algorithms could be found in Section~\ref{exper_setup} and the results of the comparisons between them and our RLS-Skip algorithm could be found in Figure~\ref{fig:UCR} and Figure~\ref{fig:random-s} of the revised paper. Overall, none of them are as competitive as RLS-Skip, e.g., UCR is dominated by RLS-Skip and works for DTW only, and Random-S provides trade-offs between efficiency and effectiveness not as good as those by RLS-Skip and is dominated by RLS-Skip in some cases.
  \item We have included a third trajectory dataset that is based on traces of humans, as suggested by Reviewer 1. The description of this dataset could be found in Section~\ref{exper_setup} and the results on this dataset are presented together with those on the two old datasets (due to the page limit, some results are presented in the technical report version). In general, the results on this newly-added dataset provide similar clues as those on the two old datasets.

  \item We have removed some experimental results from the revised paper, including the efficiency results on Harbin (some sub-figures of Figure 3 in the old version), the effectiveness results of varying query lengths in terms of AR and MR on Porto and in terms of AR, MR and RR on Harbin (some sub-figures of Figure 4 in the old version), and the effect of soft margin $\xi$ for SizeS in terms of AR and MR (some sub-figures in Figure 6 in the old version) and presented them in the technical report version~\cite{TR}. The reason is that they deliver similar clues as the results that remain in the revised paper and there is a page limit.
\end{enumerate}

These major changes are highlighted in blue in the revised paper.
Appended please find our detailed responses to both the reviewers' and meta-reviewer's comments.
Thank you for your time reading them.

\smallskip\noindent Yours sincerely\\
\smallskip\noindent Zheng, Cheng, Gao, and Yiding

%----------------
%\newpage
\section{Response to Reviewer 1's Report}
\label{subsec:reviewerOneReport}

\begin{comment1}
``R1W1. Although the framework is general, trajectory similarity metrics share some commons. For some of them, the ExactS approach can be optimized in the same way. So its performance can be better. But the paper does not talk about this potential of ExactS.''
\label{comment1:Optimization-ExactS}
\end{comment1}

\noindent\textbf{Response.}
Thank you for raising this very good point. First, we note that for some similarity measurements such as t2vec, it is hard to optimize ExactS further since ExactS has it time complexity of $O(n^2)$ for t2vec and it needs to traverse $O(n^2)$ subtrajectories.
For some other similarity measurements such as DTW and Frechet, since they were originally proposed for time series data and have been extensively studied for this data type, we searched the literature of time series more thoroughly, as inspired by this comment. We  found the UCR method~\cite{mueen2016extracting,rakthanmanon2012searching,rakthanmanon2013addressing}, which is a highly-cited tool for similar time series search and could be possibly adapted to our problem (though it works for DTW only).
%
A brief description of UCR is provided in the part of ``Compared Methods'' of Section~\ref{exper_setup}. We copy it here for easy reference.
%
\emph{``UCR was originally developed for searching subsequences of a time series, which are the most similar to a query time series and the similarity is based on the DTW distance. UCR enumerates all subsequences that are of the same length of the query time series and employs a rich set of techniques for pruning many of the subsequences.
%Spring is designed for the problem of finding a subsequence of a data time series, which is the most similar to a query time series.
%Spring corresponds to the dynamic programming process for computing the DTW or Frechet distance between the data time series and the query time series, where the latter is padded with a fictitious point that could be aligned with any point of the data time series with distance equal to 0.
We adapt UCR for our similar subtrajectory search problem (details of adaptions are provided in the appendix of the technical report version~\cite{TR}).''}
%
%We note that UCR only works for DTW, but not for Frechet or t2vec and Spring works for both DTW and Frechet, but not for t2vec.

We present the results of the comparison between UCR and RLS-Skip in Figure~\ref{fig:UCR}.
% and Figure~\ref{fig:spring}.
%
A detailed description of these results could be found in the part ``(9) Comparison with UCR'' of Section~\ref{effectiveness}. Here, we make a few notes: (1) UCR does not return exact solutions since it only considers those subtrajectories of the same size of the query trajectory;
%(2) UCR always run slower than RLS-Skip; (3) UCR returns worse solutions than RLS-Skip in most of the cases;
and
(2) UCR is dominated by RLS-Skip in terms of efficiency and effectiveness.
%(3) Spring can return exact solutions, in which cases, it runs faster than ExactS but much slower than RLS-Skip; and
%(4) In some cases, RLS-Skip dominates Spring in terms of both efficiency and effectiveness and in other cases, they provide different trade-offs, but not vice versa.

\begin{comment1}
``R1W2. The paper uses the taxi trajectory datasets in the experiments. But the taxi trip dataset has some uncommon characteristics that trajectories always follow the road network. So the trajectory is not as general as some other moving objects such as human beings. It would be better if some other datasets can be used besides the taxi trajectory dataset.''
\label{comment1:OtherDatasets}
\end{comment1}


\noindent\textbf{Response.} Thank you for your comment. In the revised paper, we include a third dataset called Sports, which involves trajectories of human beings, i.e., soccer players (Section~\ref{exper_setup}). We copy the description of the dataset here for easy reference. \emph{``The third dataset, denoted by Sports, involves around 0.2 million soccer player and ball trajectories collected from STATS Sports~\footnote{https://www.stats.com/artificial-intelligence (STATS, copyright 2019)} with a uniform sampling rate of 10 times per second and a mean length around 170.''}
%
We have conducted the sames experiments on this dataset as we did on the two old datasets. In general, the results on this newly-added dataset provide similar clues as those on the two old datasets.


\begin{comment1}
``R1D1. All splitting based and learning based algorithms have a trade-off between efficiency and effectiveness. The problem is that it does not discuss the maximum percentage of accuracy loss by various approximate algorithms. An algorithm without any guarantee on error bound is not reliable.''
\label{comment1:ApproximationRatio}
\end{comment1}

\noindent\textbf{Response.}
Thank you for your comment. In the revised paper, we include some discussion on the approximation quality for each of the approximate algorithms proposed in this paper. Unfortunately, neither the heuristic-based algorithms nor learning-based algorithms can provide a certain guarantee on the quality of the approximate solution. The proofs, which correspond to problem instances, could be found in the appendix in the technical report version~\cite{TR}. We note that while these results are negative in theory, these approximate algorithms, especially those learning-based ones such as RLS and RLS-Skip, work quite well in practice (e.g., all splitting-based algorithms have the approximation ratio smaller than 1.3 and RLS has the approximation ratio smaller than 1.1 for all similarity measurements and on all datasets (Figure~\ref{effect_result})). In addition, the problem instances that we constructed for proving the negative results in fact rarely happen in practice,
which are confirmed by the effectiveness results on real datasets.

In addition, we would like to note that machine learning has recently been used to develop algorithms for solving database problems and algorithm problems, which has been published in major DB conferences and algorithm conferences. Unfortunately, these algorithms usually have no guarantees, although they perform well empirically. For example, reinforcement learning can be successful used to solve combinatorial problems like TSP, Clique, Vertex Cover, etc., as well as database problems, such as knob tunning, view selection, join order selection, etc.  We appreciate the beauty of elegant algorithms with performance guarantees. However, we think heuristic algorithms with good empirical results also make good contributions.


\begin{comment1}
``R1D2. Approximate algorithms have a soft margin parameter which controls the trade-off between efficiency and effectiveness. This soft margin is the allowed gap between the query trajectory size and a subtrajectory size. The paper does not discuss the maximum allowed value of this soft margin in order to have sufficient reduction in search time while maintaining a good accuracy.''
\label{comment:soft-margin}
\end{comment1}

\noindent\textbf{Response.}
Thank you for your comment. The soft margin is a parameter of the SizeS algorithm. We studied the effects of this parameter on the effectiveness and efficiency of SizeS. The results are shown in Figure 6 in the old version (which now becomes Figure~\ref{para_fls} in the revised version). From the results, we notice that (1) when the soft margin is around 36, SizeS would become competitive in terms of effectiveness (i.e., its solution has similar RR as that of RLs-Skip); and (2) when the soft margin increases, the running time of SizeS increases, and for all settings of soft margin, SizeS runs slower than RLS-Skip (e.g., even when the soft margin is equal to 0, meaning only the subtrajectories of the same size as the query trajectory are considered, SizeS runs slower than RLS-Skip). In conclusion, when SizeS gives competitive effectiveness (e.g., when the soft margin is set to be 36), its running time becomes close to that of the exact algorithm ExactS (i.e., around 650ms v.s. 800ms), and when SizeS gives competitive efficiency (e.g., when the soft margin is set to be 0), its RR is above 50\%, which is far from being satisfactory.


\begin{comment1}
``R1D3. Although it is easily understandable why RLS-Skip takes less time compared to RLS algorithm, the paper does not discuss why RLS-Skip is better than splitting based algorithms in terms of accuracy and search time.''
\label{comment:explanation-RLS-Skip}
\end{comment1}

\noindent\textbf{Response.}
Thank you for your comment. In terms of accuracy, we include in Section~\ref{subsec:rls} a possible explanation on why RLS is better than non-learning splitting based algorithms. We copy it here for easy reference. \emph{``and the reason is possibly that RLS is based on a learned policy,
which makes decision more intelligent than simple heuristics that are human-crafted.''} Since RLS-Skip is a generalized version of RLS, this explanation applies to RLS-Skip as well. In terms of efficiency, the explanation was provided in the part of ``(2) Efficiency results'' of Section~\ref{effectiveness} in the old version. We copy it here for easy reference. \emph{``RLS-Skip runs the fastest since on those points that have been skipped, the cost of maintaining the states and making decisions is saved. In contrast, none of the other algorithms skip points.''}



\begin{comment1}
``R1D4. The paper also has grammatical error. For example, the first contribution discussed in Page-2, Column-1 has grammatical error. The sentence is The SimSub problem relies a trajectory similarity measurement.''
\label{comment:Typo}
\end{comment1}

\noindent\textbf{Response.} Thank you for your comment. We have fixed this grammatical error. We have also proof-read the draft and fixed all grammatical errors we found.


\section{Response to Reviewer 2's Report}
\label{subsec:reviewerTwoReport}


\begin{comment2}
``R2W1 and R2D1. The motivation could be improved. The motivation in page 1 is weak. It would be interesting to see some applications on top of spatiotemporal trajectories like those taxi traces used in the experiments.''
\label{comment2:Reviewer2-Motivation}
\end{comment2}


\noindent\textbf{Response.} Thank you for your comment. In the revised paper, we include an application of detour route detection (in Section~\ref{intro}), which is based on taxi traces. We copy the description here for easy reference. \emph{``Another potential application is detour route detection. 	It first collects those routes that have been reported by passengers to be detour routes and then searches for those subtrajectories of taxis' routes, which are similar to a detour route. The found subtrajectories are probably detour routes as well.''}
In addition, we note that technically it is possible to use the similarity between a part of a data trajectory $T$ and a query trajectory $T_q$ as a new type of similarity measurement between $T$ as a whole and $T_q$.
%Therefore, any applications of ``similar trajectory search'' could be those of ``similar subtrajectory search'' in this sense.
Therefore, ``similar subtrajectory search'' could be potentially used in those applications of ``similar trajectory search'', which are well-recognized and commonly-encountered in real life.


\begin{comment2}
``R2W2 and R2D2. The presentation of the algorithms is plain without illustrative examples. Sections 4 and 5 would benefit from a running example that explains how each algorithm works.''
	\label{comment2:Examples}
\end{comment2}


\noindent\textbf{Response.} Thank you for the suggestion. In the revised paper, we include an example problem (shown in Figure~\ref{fig:input}) and use it for illustrating two representative algorithms PSS and RLS-Skip in Table~\ref{table:pss} and Table~\ref{table:rls_skip}, respectively. Due to page limit, we do not illustrate the ExactS and SizeS algorithms (since they are easy enough), the POS and POS-D algorithms (since they are similar to PSS), or the RLS algorithm (since it is a special version of RLS-Skip).



\begin{comment2}
``R2W3 and R2D3. There is not analysis on the approximation ratios for the approximate algorithms. The paper would be more solid if it conducts analysis on the approximation ratios for those approximate algorithms.''
	\label{comment2:Approximation-Ratio}
\end{comment2}


\noindent\textbf{Response.} Thank you for your comment.
%Please refer to our response to Reviewer 1's Comment 3.
This comment is also mentioned by Reviewer 1 (Reviewer 1's Comment 3). Therefore, please refer to our response to Reviewer 1's Comment 3.


\begin{comment2}
``R2D4. The experiments for Figure 4: It's also interesting to see how the proposed algorithms handle very long query trajectories, e.g., with the same length as the data trajectories or even longer.''
	\label{comment2:LongQueryTrajectories}
\end{comment2}


\noindent\textbf{Response.} Thank you for your comment. This aspect has, in fact, been explored in the experiments of ``(5) The effect of query trajectory length'' in Section~\ref{effectiveness} of the old paper. We revised the experimental set-up for this part a bit in the revised paper to maker it clearer. We copy it here for easy reference.
\emph{``We prepare four groups of query trajectories from a dataset, namely $G1$, $G2$, $G3$, and $G4$, each with 10,000 trajectories, such that the lengths of the trajectories in a group are as follows: $G1=[30,45)$, $G2=[45,60)$, $G3=[60,75)$ and $G4=[75,90)$. Then, for each query trajectory, we prepare a data trajectory from the dataset. Note that for a query trajectory and a corresponding data trajectory, the latter may be longer than or shorter than the former. For each group, we report the average results.''}
%
We make a few notes here:
(1) based on how the query trajectories and data trajectories are prepared for this part of experiments, it could happen that the query trajectory has the length larger or equal to that of the data trajectory;
(2) from group $G1$ to $G4$, the lengths of query trajectories are increasing while the expected length of the data trajectories is unchanged, and thus the results from group $G1$ to $G4$ show a trend of how the algorithms would perform when the length of query trajectories increases; and
(3) based on the results, which are are shown in Figure~\ref{RR:querylength}, we notice that in terms of the effectiveness, the length of query trajectories does not have much effect except for SizeS, and in terms of efficiency, the length of query trajectories has some effect for DTW and Frechet but less for t2vec (since when using t2vec, all trajectories are mapped to vectors and then processed).

\begin{comment2}
``R2D5. The following paper should be cited and discussed in the trajectory similarity measurement part in Section	2. - KSQ: Top-k Similarity Query on Uncertain Trajectories. TKDE 25(9): 2049-2062 (2013)''
	\label{comment2:OneCitation}
\end{comment2}


\noindent\textbf{Response.} Thank you for referring this related study. We have cited this study in Section~\ref{related} of the revised paper. We copy it here for easy reference. \emph{``In addition, Ma et al.~\cite{ma2012ksq} propose a similarity measurement called p-distance for uncertain trajectories and study the problem of searching for top-k similar trajectories to a given query trajectory based on p-distance.''} In addition, we would like to note that this study targets uncertain trajectories and regards each trajectory as a whole for consideration, which are both different from our work.

\balance
\section{Response to Reviewer 3's Report}
\label{subsec:reviewerThreeReport}

\begin{comment3}
``R3W1. The proposed heuristic solutions (in Sections 4.2 and 4.3) and learning-based solutions (in Section 5) do not provide any theoretical guarantee on the rank of result. In Table 3, the mean rank of RLS-Skip is far from 1.''
\label{comment3:TheoreticalGuarantee}
\end{comment3}


\noindent\textbf{Response.}
Thank you for your comment.
This comment is also mentioned by Reviewer 1 (Reviewer 1's Comment 3). Therefore, please refer to our response to Reviewer 1's Comment 3.
%
We also note that in Table 3, the mean ranks, which are are far from 1 (e.g., from 40 to 100), should be acceptable if put in the context that there are a few thousands of subtrajetories, e.g., the corresponding relative ranks are not large (e.g., from 3.5\% to 8.9\%).

\begin{comment3}
``R3W2: The experimental study has not considered the following sampling algorithm as competitor method: "sample X random subtrajectories from the given trajectory, then compute the similarity of those subtrajectories to the query trajectory $T_q$". I speculate that this method can achieve an expected mean rank of 1\% by sampling only 100 random subtrajectories (regardless of the total number $O(n^2)$ of subtrajectories). As for comparison, in Table 3, the relative rank of RLS-Skip ranges from 3.5\% to 8.9\%.''
\label{comment3:Competitor}
\end{comment3}

\noindent\textbf{Response.} Thank you for raising this very good point. We call this method Random-S. With 100 sampled subtrajectories, the probability that Random-S returns a subtrajectory with RR at most 1\% (resp. 5\%) is equal to $(1-(1-1\%)^{100}) = 0.634$ (resp. $(1-(1-5\%)^{100}) = 0.994$), which look quite promising. Therefore, we consider Random-S as a competitor method in the revised paper and compare it against RLS-Skip. The results are shown in Figure~\ref{fig:random-s}. Indeed, when the sample size is around 100, the RR of Random-S approaches 1\% (Figure~\ref{fig:random-s} (a)), but meantime, its running time gets close to that of the exact algorithm ExactS (Figure~\ref{fig:random-s} (b)). In addition, for Random-S, the subtrajectories that are considered could be quite different, and thus it is not possible to compute their similarities \emph{incrementally} as it does for ExactS. As a result, even for a relatively small sample size, e.g., 100, the running time of Random-S is almost that of ExactS and significantly larger than that of RLS-Skip (25 times higher). Whereas when the sample size is small, e.g., below 20, Random-S has its effectiveness significantly degraded, which is clearly worse than that of RLS-Skip (Figure~\ref{fig:random-s}(a)), and meantime it still runs slower than RLS-Skip (Figure~\ref{fig:random-s}(b)).
%In conclusion, RLS-Skip dominates Random-S for some settings of sample size in terms of both efficiency and effectiveness and provides different trade-offs between them for other settings, but not vice versa.


\begin{comment3}
``R3W3. It is not easy to follow Sections 5.3 and 5.4. It'd be better if the authors could include some figures or examples to illustrate the techniques used in those subsections.''
\label{comment3:Examples}
\end{comment3}

\noindent\textbf{Response.} Thank you for the comment. In the revised paper, we include an example for illustrating RLS-Skip, where the input is shown in Figure~\ref{fig:input} and the process of RLS-Skip is illustrated in Table~\ref{table:rls_skip}. We do not illustrate the RLS algorithm since it is a special version of RLS-Skip and the space is limited.

\begin{comment3}
``R3D1. In Equation 2, there is an extra ')' in the "otherwise" case. In Table 2, a ')' is missing in the Big-O notation of the abstract similarity measurement of ExactS.''
\label{comment3:Typo}
\end{comment3}

\noindent\textbf{Response.} Thank you for the comments. We have fixed these typos in the revised paper.


\begin{comment3}
``R3D2. The experimental setup (Section 6.1) did not mention the parameter setting of SizeS.''
\label{comment3:ParameterSetting}
\end{comment3}

\noindent\textbf{Response.} Thank you for the comment. In the old version, the parameter setting of SizeS is mentioned when SizeS is specified in the part of ``Computed Methods'' in Section~\ref{exper_setup}. We copy it here for reference. \emph{``For SizeS, we use the setting $\xi = 5$ (with the results of its effect shown later on).''} In this revised paper, we have moved this description in the part of ``Parameter Setting'' in Section~\ref{exper_setup} since it looks natural to put there.

\begin{comment3}
``R3D3. Please report the learning time of RLS and RLS-skip in the experimental section. How much is the learning time compared to the "time without index" in Figure 3? How much is the learning time compared to the index construction time?''
\label{comment3:LearningTime}
\end{comment3}

\noindent\textbf{Response.} Thank you for the comment.
%
In the revised paper, we have presented the results of learning time of RLS and RLS-Skip in the part of ``(11) Training time'' in Section~\ref{effectiveness}. We copy the description here for easy reference. \emph{``The training times of the RLS and RLS-Skip models on different datasets are shown in Table~\ref{learntime}. It normally takes a couple of hours to train a reinforcement learning model for RLS and RLS-Skip. It takes less time to train RLS-Skip than RLS since we use the same number of trajectory pairs and epochs for training both algorithms and RLS-Skip runs faster.''}
For comparison with the time of query processing and index construction,
we consider the experiment of running queries over a database of 2 million points collected from the Porto dataset, whose results are shown in Figure~\ref{fig:efficiencyRLS}. It takes 4.4 hours to train RLS-Skip offline. Once it has been trained, it could be used for many queries online, e.g., for a query of finding top-50 similar subtrajectories from the database, the time is about 522s if no index structures are used and 23.08s if the Inverted index is used. Besides, on this database, the time of building the Inverted list is small, e.g., around 5.16s. The message is that the training time is still manageable, e.g., a couple of hours usually. In addition, the training is a one-time process, and after training, it can be used to serve the query processing of many queries.

\section{Response to Meta-Reviewer's Report}
%\subsection{Meta-Reviewer Comments and Response}

\begin{revision}
	``An analysis on the approximation ratios for those approximate algorithms needs to be provided.''
\end{revision}

\noindent\textbf{Response.}
Thank you for your comment.
We have finished this revision item.
Please refer to our response to Reviewer 1's Comment 3.

\begin{revision}
	``The presentation needs to be further improved significantly, including running examples, figures, etc.''
\end{revision}

\noindent\textbf{Response.}
Thank you for your comment.
We have finished this revision item.
Please refer to our response to Reviewer 2's Comment 2 and Reviewer 3's Comment 3.

\begin{revision}
	``More competitors need to be included in the comparison to justify the novelty.''
\end{revision}

\noindent\textbf{Response.}
Thank you for your comment.
We have finished this revision item.
Please refer to our responses to Reviewer 1's Comment 1 and Reviewer 3's Comment 2.

\begin{revision}
	``Additional trajectory datasets need to be tested.''
\end{revision}

\noindent\textbf{Response.}
Thank you for your comment.
We have finished this revision item.
Please refer to our responses to Reviewer 1's Comment 2.



==> v13 - technical/rl.tex <==
\section{RL-BASED SEARCH (RLS)}
\label{section:RLS}
Inspired by all the heuristic algorithms mentioned above, we further propose a data-driven method to guide trajectory splitting based on deep reinforcement learning, called RL-based Search (RLS).
\subsection{Trajectory Splitting in MDP Modeling}
From a high-level perspective, we first explain why we use the reinforcement learning.
The trajectory splitting process can be considered as a Markov decision process (MDP)~\cite{puterman2014markov} with unknown parameters. Recall that in each time step, we need to interact with the environment (i.e., the whole trajectory $C$) to make a decision (i.e., split or not), and then get a immediate reward (i.e., the dissimilarity value $\Psi$). In order to find an optimal strategy to split trajectories, we apply Reinforcement Learning (RL)~\cite{sutton2018reinforcement}, because it has been proven to be able to optimize the sequential decision-making problem in MDPs effectively. Next, we give the formal definitions for MDP in our problem.
\subsection{Definitions for MDP Modeling}
Given a candidate trajectory $C$ (environment), we define a Markov decision process in our problem is a 4-tuple $M = (\mathcal{S}, \mathcal{A}, \mathcal{T}, \mathcal{R})$.
\begin{definition}[State]
$\mathcal{S}$ is a state space for every state $s \in \mathcal{S}$.
\end{definition}
Recall that in heuristic algorithms, we have three candidate dissimilarity values in each time step, $\Psi$ denotes the dissimilarity value that we maintain currently. $\Psi_{P}$ denotes the prefix trajectory dissimilarity value, and $\Psi_{S}$ denotes the suffix trajectory dissimilarity value. We concatenate $\Psi$ and $\Psi_{P}$ to represent the current state $s = (\Psi, \Psi_{P})$. Here, we do not concatenate $\Psi_{S}$ because as discussed before, it is only a approximate value via encoding the trajectories in reverse, and thus may misguide the model's real decision.

\begin{definition}[Action]
$\mathcal{A} = \{0, 1\}$ is a action space for every action $a \in \mathcal{A}$.
\end{definition}
Action 0 means to make no splits and go to the next time step, and action 1 means to split at the current time step.

\begin{definition}[Transition Distribution]
$\mathcal{T}:(\mathcal{S} \times \mathcal{A} \times \mathcal{S'}) \rightarrow [0,1]$ is a transition distribution, which models the probability that action $a$ in state $s$ at time $t$ will lead to state $s'$ at next time $t+1$.
\end{definition}
We illustrate an example of state transition in Figure~\ref{state}. Note that the interval update still follows the Equation~\ref{interval} proposed in heuristic algorithms.
\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/state}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{\small{An example illustrating state transition $\mathcal{S} \times \mathcal{A} \times \mathcal{S'}$ for trajectory $T = <p_1, p_2, p_3>$.}}\label{state}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}

\begin{definition}[Reward]
$\mathcal{R}:(\mathcal{S} \times \mathcal{A}) \rightarrow \mathbb{R}^{+}$ is a reward function, the immediate reward $r$ is received after we conduct an action $a$ at state $s$.
\end{definition}
We define the reward $r$ in our problem as the difference between two adjacent dissimilarity values $\Psi$, that is $r_t = \Psi_{t-1} - \Psi_{t}$. We proof our definition is sound and RL can be used to solve the search problem using Lemma~\ref{lemma:opt}.
\begin{lemma}
\label{lemma:opt}
Finding the optimal subtrajectory is equivalent to maximizing the cumulative rewards at the initial state.
\end{lemma}

\begin{proof}
The goal of reinforcement learning is to find the optimal policy $\pi^*$ which can maximize expected cumulative reward.
\begin{equation}
\begin{aligned}
\label{eproof:given}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\pi^* = \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t= 0}^{|C|-1}\gamma^{t} r_{t+1}|\pi \bigg],
\end{aligned}
\end{equation}
where $\gamma$ is a discount rate and $\gamma \in [0,1)$. By our definition,
\begin{equation}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
r_{t+1} = \Psi_{t} - \Psi_{t+1} \geq 0.
\end{aligned}
\end{equation}
Thus, we have
\begin{equation}
\begin{aligned}
\label{eproof:rl}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\pi^* = \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t= 0}^{|C|-1}\gamma^{t} r_{t+1}|\pi \bigg] \Leftrightarrow \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}r_{t+1}|\pi \bigg].
%& = \max\limits_{\pi} \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}(\Psi_{t} - \Psi_{t+1})|\pi \bigg]
%= \max\limits_{\pi}(\Psi_{0} - \Psi_{|C|}) \Leftrightarrow \min\limits_{\pi}\Psi_{|C|}.
\end{aligned}
\end{equation}
We proof the Equation~\ref{eproof:rl} by contradiction. Suppose $\pi^*$ is not an optimal policy which can maximize the expected cumulative reward without discount rate $\gamma$. Thus, there exists a policy $\pi^0$ such that
\begin{equation}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}r_{t+1}|\pi^* \bigg] < \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}r_{t+1}|\pi^0 \bigg],
\end{aligned}
\end{equation}
and $\pi^* \neq \pi^0$. We know the reward $r_{t+1} \geq 0$ and $0 \leq \gamma^{t} \leq 1$ for $t \in \big[0, |C|-1\big]$. Further, we have
\begin{equation}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}\gamma^{t} r_{t+1}|\pi^* \bigg] < \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}\gamma^{t} r_{t+1}|\pi^0 \bigg],
\end{aligned}
\end{equation}
which contradicts our given Equation~\ref{eproof:given}, and thus Equation~\ref{eproof:rl} holds. Furthermore, we have
\begin{equation}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
\pi^* & \Leftrightarrow \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}r_{t+1}|\pi \bigg]
= \argmax\limits_{\pi} \mathbb{E}\bigg[ \sum_{t=0}^{|C|-1}(\Psi_{t} - \Psi_{t+1})|\pi \bigg]\\
& = \argmax\limits_{\pi}(\Psi_{0} - \Psi_{|C|}) \Leftrightarrow \argmin\limits_{\pi}\Psi_{|C|} \Leftrightarrow \arg\limits_{\pi}opt.
\end{aligned}
\end{equation}
$\Psi_{0}$ is a fixed initial value when given a pair of candidate
trajectory $C$ and query trajectory $Q$, and $\Psi_{|C|}$ is the final returned similarity. We know the $\min\Psi_{|C|}$ is equivalent to the optimal solution $opt$ because the optimal subtrajectory is a subtrajectory with the minimal dissimilarity value in all of the candidate subtrajectories. Hence, Lemma~\ref{lemma:opt} holds.
\end{proof}

\subsection{Deep Q Network (DQN)}
In this section, we give a brief preliminary of our reinforcement learning framework - Deep Q Network (DQN)~\cite{mnih2013playing}. DQN is a popular value-based RL method, whose core is the Q-value calculation defined as $Q^*(s, a)$, and furthermore, the iterative loss function is defined as follows.
\begin{equation}
\label{eq:rlobj}
\begin{aligned}
%\setlength{\abovedisplayskip}{1.5pt}
%\setlength{\belowdisplayskip}{1.5pt}
& Q^*(s_{t}, a_{t}) \leftarrow Q^*(s_{t}, a_{t}) + \\
& \alpha[r_{t+1}+\gamma\max \limits_{a} \underbrace{Q^*(s_{t+1}, a)}_{Target-NN} - \underbrace{Q^*(s_{t}, a_{t})}_{Current-NN}],
\end{aligned}
\end{equation}
where $\alpha$ is a learning rate, $s_t$ is the current state, $a_t$ is a chosen action, which depends on the current Q-value, $r_{t+1}$ is an obtained reward after taking action $a_t$, and $s_{t+1}$ is the next state. There are two main modules in DQN: $Current-NN$ and $Target-NN$, $Current-NN$ is used to calculate $Q^*(s_{t}, a_{t})$ and it interacts with the environment (the candidate trajectory $C$) to get transitions $(s_t,a_t,r_t,s_{t+1})$, which is stored in the replay memory $\mathcal{M}$, and $\mathcal{M}$ can be considered as a collection, we randomly sample transitions from $\mathcal{M}$ in the training process.
$Target-NN$ is used to calculate the next Q-value $Q^*(s_{t+1}, a_{t})$. Note that the parameters (weights) in the $Current-NN$ and $Target-NN$ will be updated during the training process. We illustrate the detailed DQN working process in Figure~\ref{rlmodel}.

\begin{figure}
  \centering
  % Requires \usepackage{graphicx}
  \includegraphics[width=8.5cm]{figures/rlmodel_v4}\\
  %\setlength{\abovecaptionskip}{1pt}
  \vspace{-2mm}
  \caption{\small{RLS model.}}\label{rlmodel}
  %\setlength{\belowcaptionskip}{0pt}
 \vspace{-3mm}
\end{figure}
\subsection{Algorithm Sketch}
\textcolor[rgb]{1.00,0.00,0.00}{In this section, we present the two main parts of RL-based Search (RLS): offline training (Algorithm~\ref{rlst_1}) and online search (Algorithm~\ref{rlst_3}). In Algorithm~\ref{rlst_1}, We first initialize the function $Q^*$ ($Current-NN$ and $Target-NN$) with some random weights and the size of the replay memory $\mathcal{M}$ (line 1). In the outer loop of iterating the episodes (lines 2-21), we first random a trajectory pair $C$ and $Q$ from trajectory database $\mathcal{D}$ (line 3), and then we need to get token sequences used to prefix trajectory similarity computation (line 4), representation vectors for query $Q$ (line 5). Note that here do not encode backward $h'$ for suffix trajectory similarity computation because we do not use $\Psi_{S}$ to define states as explained before.
Before the inner loop of iterating the time steps (lines 6-21), we need to initialize the trajectory dissimilarity values $\Psi, \Psi_{P}$, and concatenate them to get state $s$ (lines 6-7). In the training process (lines 8-20), we first get a greedy action at the current state with $\epsilon-$greedy strategy, which is a common approach in DQN, the main idea of this strategy is to select an action with an uniform
probability proportion $\epsilon$, and a typical parameter value for $\epsilon$ is generally set to 0.1 (line 9). If $a=1$, which means that we need to cut the trajectory (lines 10-12). And then we get a new state $s'$ (lines 13-14), maintain the current best $\Psi$ in order to calculate reward $r$ (line 15). Finally, we store the transition of this step $(s,a,r,s')$ in $\mathcal{M}$ and sample a minibatch for optimizing $Q^*$ according to Equation \ref{eq:rlobj} (lines 16-18). Note that the current $s$ is updated to the next $s'$ (line 19).}

\begin{algorithm}[t]
	\caption{RL-based Search: Offline Training}
	\footnotesize{
		\label{rlst_1}
		\begin{algorithmic}[1]
			\Require
			Trajectory database $\mathcal{D}$ and learning rate $\alpha$;
			\Ensure
			Learned action-value function $Q^*$;
            \State initialize $Q^*$ with random weights and replay memory $\mathcal{M}$;
            \For{$episode = 1, 2, 3,...$}
            \State sample candidate trajectory $C$ and query trajectory $Q$ from $\mathcal{D}$;
            \State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
            \State get representation vector $h_{Q}$ for $Q$;
            \State initialize $h_{0} \leftarrow None$, $h_{1} \leftarrow t2vec(h_{0}, x_{1})$;
            \State $\Psi_{P} \leftarrow d(h_{Q}, h_{1}), \Psi \leftarrow \Psi_{P}, s \leftarrow concat(\Psi, \Psi_{P})$;
            \For{each time step $2 \leq t \leq |C|$ in each $episode$}
            \State select $a = max_{a}Q^*(s,a;\theta)$ with $\epsilon-$greedy strategy;
            \If{$a = 1$}
            \State $h_{t-1} \leftarrow None$;
            \EndIf
            \State $h_{t} \leftarrow t2vec(h_{t-1}, x_{t}), \Psi_{P} \leftarrow d(h_{Q}, h_{t})$;
            %\State , $\Psi_{S} \leftarrow d(h_{\overleftarrow{Q}}, h'_{|C|-t})$;
            \State $s' \leftarrow concat(\Psi, \Psi_{P})$;%, \Psi_{S}
            \State $tmp \leftarrow \Psi$, $\Psi \leftarrow min(\Psi, \Psi_{P})$, $r \leftarrow tmp - \Psi$;%, \Psi_{S}
            \State store transition $(s,a,r,s')$ in $\mathcal{M}$;
            \State Sample random minibatch of transitions from $\mathcal{M}$;
            \State optimize $Q^*$ by gradient descent in Equation \ref{eq:rlobj};
            \State $s \leftarrow s'$;
            \EndFor
            \EndFor
	\end{algorithmic}}
\end{algorithm}
\textcolor[rgb]{1.00,0.00,0.00}{
The output of the offline training is the $Q^*$ of the $Current-NN$~\footnote{Note that the weights of $Target-NN$ is updated by $Current-NN$ during the training process as shown in Figure~\ref{rlmodel}, so finally, they have the same model structure and shared weights.}. In the online part, we first need to do the same preprocess as shown in offline (lines 1-2). Before the for-loop of iterating the time steps (lines 5-15), we need to initialize the index of splitting point $sp$, dissimilarity value $\Psi_{P}, \Psi$, and maintaining interval $\Lambda$ first (lines 3-4). After that, we select an action guided by $Q^*$ (line 6), if $a=1$, we cut the trajectory at this time step (lines 7-9). Next, we compute the $\Psi_{P}$ according to its interval $\Gamma$ (lines 10), and concatenate these two values as the state $s$, which is used to input to $Q^*$ (line 11). Finally, we update the target $\Lambda$ and $\Psi$ if there is a better result (line 12-14).} Overall, the online part shares a similar framework with the heuristic algorithms; however, the splitting strategy is determined by a data-driven model RLS.

%\begin{algorithm}[t]
%	\caption{RL-based Search: Update}
%	\footnotesize{
%		\label{rlst_2}
%		\begin{algorithmic}[1]
%			\Require
%			$\Psi, \Psi_{P}, \Psi_{S}, \Lambda, \Gamma, \Delta$;
%			\Ensure
%			Updated $\Lambda$, $\Psi$;
%            \If {$\Psi_{P} < \Psi$ or $\Psi_{S} < \Psi$}
%                \If {$\Psi_{P} < \Psi_{S}$}
%                    \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
%                \Else
%                    \State $\Lambda \leftarrow \Delta$, $\Psi \leftarrow \Psi_{S}$;
%                \EndIf
%            \EndIf
%	\end{algorithmic}}
%\end{algorithm}

\begin{algorithm}[t]
	\caption{RL-based Search: Online Search}
	\footnotesize{
		\label{rlst_3}
		\begin{algorithmic}[1]
			\Require
			Candidate trajectory $C$, query trajectory $Q$ and learned $Q^*$;
			\Ensure
			Subtrajectory $C_{\Lambda}$ and dissimilarity value $\Psi$;
            \State get token sequence $<x_{1},...,x_{|C|}>$ for candidate trajectory $C$;
            \State get representation vector $h_{Q}$ for $Q$;
            %\State set $h'_{0} \leftarrow None$ and get each backward hidden state $h'_{t}$ for $\overleftarrow{C}$;
            \State initialize $sp \leftarrow t$, $h_{0} \leftarrow None$, $h_{1} \leftarrow t2vec(h_{0}, x_{1})$;
            \State $\Psi_{P} \leftarrow d(h_{Q}, h_{1}), \Psi \leftarrow \Psi_{P}, s \leftarrow concat(\Psi, \Psi_{P}), \Lambda \leftarrow [1,1]$;
            \For{each time step $2 \leq t \leq |C|$}
            \State select $a = max_{a}Q^*(s,a;\theta)$ using $Q^*$;
            \If{$a = 1$}
            \State $sp \leftarrow t$, $h_{t-1} \leftarrow None$;
            \EndIf
            \State $\Gamma \leftarrow [sp, t]$, $h_{t} \leftarrow t2vec(h_{t-1}, x_{t})$, $\Psi_{P} \leftarrow d(h_{Q}, h_{t})$;
            \State $s \leftarrow concat(\Psi, \Psi_{P})$;
            \If{$\Psi_{P} < \Psi$}
            \State $\Lambda \leftarrow \Gamma$, $\Psi \leftarrow \Psi_{P}$;
            \EndIf
            \EndFor
	\end{algorithmic}}
\end{algorithm}

\begin{lemma}
The total time complexity of RLS is $O(n)$.
\end{lemma}
\begin{proof}
In Algorithm~\ref{rlst_3}, we explain the time complexity as follows: (1) it takes $O(n)$ to finish preprocessing (lines 1-2). (2) In each time step, the time cost of action selection by $Q^*$ is a constant (line 8) because the state $s$ is only a 2-dimensional vector and the neural network of $Q^*$ is only a simple forward neural network with 2-layers in our experimental evaluation. (3) The time cost of Euclidean distance computation, update and concatenation is a constant, which is obvious by observing the pseudocodes. Hence, the overall time complexity of RLS is $O(n)$.
\end{proof}


==> v13 - technical/rl_v2.tex <==

\section{Reinforcement Learning Based Algorithm}
\label{section:RLS}

A splitting-based algorithm has its effectiveness rely on the quality of the process of splitting a data trajectory. In order to find a solution of high quality, it requires to perform split operations at appropriate points such that some subtrajectories that are similar to a query trajectory are formed and then explored. The three splitting-based algorithms, namely PSS, POS and POS-D, mainly use some hand-crafted heuristics for making decisions on whether to perform a split operation at a specific point.
%For example, the PSS algorithm would choose to perform a split operation if one of the two subtrajectories including a prefix one and a suffix one that would be potentially formed if a split operation is performed is more similar to the query trajectory than the best subtrajectory found so far.
This process of splitting a trajectory into subtrajectories is a typical \emph{sequential decision making} process. Specifically, it scans the points sequentially and for each point, it makes a decision on whether or not to perform a split operation at the point.
In this paper, we propose to model this process as a \emph{Markov decision process} (MDP)~\cite{puterman2014markov} (Section~\ref{subsec:mdp-modelling}), adopt a \emph{deep-$Q$-network} (DQN)~\cite{mnih2013playing} for learning an optimal policy for the MDP (Section~\ref{subsec:dqn}), and then develop an algorithm called \emph{reinforcement learning based search} (RLS), which corresponds to a splitting-based algorithm that uses the learned policy for the process of splitting a data trajectory (Section~\ref{subsec:rls}) and an augmented version of RLS, called RLS-Skip, with better efficiency (Section~\ref{subsec:rls_skip})

\subsection{Trajectory Splitting as a MDP}
\label{subsec:mdp-modelling}
A MDP consists of four components, namely \emph{states}, \emph{actions}, \emph{transitions}, and \emph{rewards}, where (1) a state captures the \emph{environment} that is taken into account for decision making by an \emph{agent}; (2) an action is a possible decision that could be made by the agent; (3) a transition means that the state changes from one to another once an action is taken; and (4) a reward, which is associated with a transition, corresponds to some feedback indicating the quality of the action that causes the transition.
%
%We model the process of splitting a data trajectory as a MDP, which involves \emph{states}, \emph{actions}, \emph{transitions}, and \emph{rewards}, as follows.
We model the process of splitting a data trajectory as a MDP as follows.

\smallskip\noindent\textbf{(1) States.} We denote a state by $s$. Suppose it is currently scanning point $p_t$. $p_h$ denotes the point following the one, at which the last split operation happens if any and $p_1$ otherwise. We define the state of the current environment as a triplet $(\Theta_{best}, \Theta_{pre}, \Theta_{suf})$, where $\Theta_{best}$ is the largest similarity between a subtrajectory found so far and the query trajectory $T_q$, $\Theta_{pre}$ is $\Theta(T[h, t], T_q)$ and $\Theta_{suf}$ is $\Theta(T[t, n]^R, T_q^R)$. As could be noticed, a state captures the information about the query trajectory, the data trajectory, the point at which the last split happens, and the point that is being scanned, etc. Note that the state space is a three-dimensional continuous one.

\smallskip\noindent\textbf{(2) Actions.} We denote an action by $a$. We define two actions, namely $a = 1$ and $a = 0$. The former means to perform a split operation at the point that is being scanned and the latter means to move on to scan the next point.

\smallskip\noindent\textbf{(3) Transitions.}
%Suppose the current state is $s$ and we take an action $a$, and after that, we would observe a new environment captured by a new state $s'$.
In the process of splitting a trajectory, given a current state $s$ and an action $a$ to take, the probability that we would observe a specific state $s'$ is unknown. We note that the method that we use for solving the MDP in this paper is a \emph{model-free} one and could solve the MDP problem even with its transition information unknown.

\smallskip\noindent\textbf{(4) Rewards.}
We denote a reward by $r$.
%
We define the reward associated with the transition from state $s$ to state $s'$ after action $a$ is taken as $(s'.\Theta_{best} - s.\Theta_{best})$, where the $s'.\Theta_{best}$ is the first component of state $s'$ and $s.\Theta_{best}$ is the first component of state $s$. With this reward definition, the goal of the MDP problem, which is to maximize the accumulative rewards, is consistent with that of the process of splitting a data trajectory, which is to form a subtrajectory with the greatest possible similarity to the query trajectory. To see this, consider that the process goes through a sequence of states $s_1, s_2, ..., s_N$ and ends at $s_N$. Let $r_1, r_2, ..., r_{N-1}$ denote the rewards received at these states except for the termination state $s_N$. Then, when the future rewards are not discounted, we have $$\Sigma_{t}r_t = \Sigma_{t}(s_t.\Theta_{best} - s_{t-1}.\Theta_{best}) = s_N.\Theta_{best} - s_1.\Theta_{best}$$ where $s_N.\Theta_{best}$ corresponds to the similarity between the best subtrajectory found and the query trajectory $T_q$ and $s_1.\Theta_{best}$ corresponds to the best known similarity at the beginning, i.e., 0. Therefore, maximizing the accumulative rewards is equivalent to maximizing the similarity between the subtrajectory to be found and $T_q$ in this case.


\subsection{Deep-$Q$-Network (DQN) Learning}
\label{subsec:dqn}
%Deep Q Learning;
The core problem of a MDP is to find an optimal \emph{policy} for the agent, which corresponds to a function $\pi$ that specifies the action that the agent should choose when at a specific state so as to maximize the accumulative rewards.
One type of methods that are commonly used is those \emph{value-based} methods~\cite{sutton2018reinforcement,mnih2013playing}. The major idea is as follows. First, it defines an optimal action-value function $Q^*(s, a)$ (or $Q$ function), which represents the maximum amount of expected accumulative rewards it would receive by following any policy after seeing the state $s$ and taking the action $a$.
Second, it estimates $Q^*(s, a)$ using some methods such as $Q$-learning~\cite{watkins1992q} and deep-$Q$-network (DQN)~\cite{mnih2013playing}.
Third, it returns the policy, which always chooses for a given state $s$ the action $a$ that maximizes $Q^*(s, a)$.

\if 0
Different value-based methods differ in using different methods for estimating the $Q$ function.
For example, the $Q$-learning method~\cite{sutton2018reinforcement} estimates the function by using following Bellman Equation as an iterative update step:
\if 0
$$
Q^*(s, a) = E_{s'}[r + \gamma\cdot \max_{a'}Q^*(s', a')]
$$
$s'$ is a possible next state after action $a$ is taken for a given state $s$.
\fi
\begin{equation}
Q(s, a) \leftarrow Q(s, a) + \alpha\cdot [r + \gamma \cdot \max_{a'}Q(s', a') - Q(s, a)],
\end{equation}
where $s$ is the current state, $a$ is the action that is chosen based on some policy derived from $Q$, $r$ and $s'$ are the reward and the next state observed, respectively, $\alpha$ is the learning rate, and $\gamma$ is a discount factor.
%
The DQN method~\cite{mnih2013playing} parameterizes the $Q$ function as $Q(s, a; \theta)$ and then learns the parameters $\theta$.
%
$Q$-learning is suitable for cases where the state space is discrete and of small or moderate size while DQN is capable of handing cases where the state space is large and even continuous.
\fi

%\begin{algorithm}[t!]
%	\caption{Deep-$Q$-Network (DQN) Learning with Experience Replay}
%	\footnotesize{
%		\label{rlst_1}
%		\begin{algorithmic}[1]
%			\Require
%			A database $\mathcal{D}$ of data trajectories and a set of $\mathcal{D}_q$ of query trajectories;
%			\Ensure
%			Learned action-value function $Q(s,a;\theta)$;
%			\State initialize the reply memory $M$;
%			\State initialize the main network $Q(s, a; \theta)$ with random weights $\theta$;
%			\State initialize the target network $\hat{Q}(s, a; \theta^-)$ with weights $\theta^- = \theta$;
%			\For{$episode = 1, 2, 3,...$}
%			
%			\State sample a data trajectory $T$ and a query trajectory $T_q$;
%			\State $h \leftarrow 1$;
%			\State $\Theta_{best} \leftarrow 0$; $\Theta_{pre} \leftarrow \Theta(T[h,h], T_q)$; $\Theta_{suf} \leftarrow \Theta(T[h,n]^R, T_q^R)$;
%			\State observe the first state $s_1 = (\Theta_{best}, \Theta_{pre}, \Theta_{suf})$;
%			
%			\For{each time step $1 \leq t \leq |T|$}
%			
%			\State select a random action $a_t$ with probability $\epsilon$ and otherwise select action $a_t = \arg\max_{a}Q(s_t,a;\theta)$;
%			\If{$a_t = 1$}
%			\State $h\leftarrow t+1$;
%			\EndIf
%			\State $\Theta_{best} \leftarrow \max\{s_t.\Theta_{best}, s_t.\Theta_{pre}, s_t.\Theta_{suf}\}$;
%				\If{$t=|T|$}
%				%\State $\Theta_{pre} \leftarrow 0$; $\Theta_{suf} \leftarrow 0$;
%				\State \textbf{break};
%				\EndIf
%			\State $\Theta_{pre} \leftarrow \Theta(T[h,t+1], T_q)$; $\Theta_{suf} \leftarrow \Theta(T[t+1,n]^R, T_q^R)$;
%			\State observe the next state $s_{t+1} = (\Theta_{best}, \Theta_{pre}, \Theta_{suf})$;
%			\State observe the reward $r_t = s_{t+1}.\Theta_{best} - s_t.\Theta_{best}$;
%			\State store the experience $(s_t,a_t,r_t,s_{t+1})$ in the replay memory $\mathcal{M}$;
%			\State sample a random minibatch of experiences from $\mathcal{M}$ uniformly;
%			\State perform a gradient descent step on the loss as computed by Equatioin~(\ref{equ:dqn-loss}) wrt $\theta$;
%			\EndFor
%			\State copy the main network $Q(s,a;\theta)$ to $\hat{Q}(s, a; \theta^-)$;
%			%				\State reset $\theta^{-} \leftarrow \theta$;
%			\EndFor
%		\end{algorithmic}
%	}
%	\label{alg:dqn}
%\end{algorithm}

\begin{algorithm}[t]
	\caption{Deep-$Q$-Network (DQN) Learning with Experience Replay}\label{alg:dqn}
    \LinesNumbered
	\footnotesize{
		\KwIn{A database $\mathcal{D}$ of data trajectories and a set of $\mathcal{D}_q$ of query trajectories;}
        \KwOut{Learned action-value function $Q(s,a;\theta)$;}
		initialize the reply memory $M$;\\
		initialize the main network $Q(s, a; \theta)$ with random weights $\theta$;\\
		initialize the target network $\hat{Q}(s, a; \theta^-)$ with weights $\theta^- = \theta$;\\
			\For{$episode = 1, 2, 3,...$}{
			sample a data and query trajectory $T$, $T_q$;\\
			$h \leftarrow 1$;\\
			$\Theta_{best} \leftarrow 0$; $\Theta_{pre} \leftarrow \Theta(T[h,h], T_q)$; $\Theta_{suf} \leftarrow \Theta(T[h,n]^R, T_q^R)$;\\
			observe the first state $s_1 = (\Theta_{best}, \Theta_{pre}, \Theta_{suf})$;\\
			\For{each step $1 \leq t \leq |T|$}{
			select a random action $a_t$ with probability $\epsilon$ and select action $a_t = \arg\max_{a}Q(s_t,a;\theta)$ with probablity ($1-\epsilon$);\\
			\If{$a_t = 1$}{
			$h\leftarrow t+1$;}
			$\Theta_{best} \leftarrow \max\{s_t.\Theta_{best}, s_t.\Theta_{pre}, s_t.\Theta_{suf}\}$;\\
			\If{$t=|T|$}{
			\textbf{break};}
			$\Theta_{pre} \leftarrow \Theta(T[h,t+1], T_q)$; $\Theta_{suf} \leftarrow \Theta(T[t+1,n]^R, T_q^R)$;\\
			observe the next state $s_{t+1} = (\Theta_{best}, \Theta_{pre}, \Theta_{suf})$;\\
			observe the reward $r_t = s_{t+1}.\Theta_{best} - s_t.\Theta_{best}$;\\
			store the experience $(s_t,a_t,r_t,s_{t+1})$ in the replay memory $\mathcal{M}$;\\
			sample a random minibatch of experiences from $\mathcal{M}$ uniformly;\\
		    perform a gradient descent step on the loss as computed by Equatioin~(\ref{equ:dqn-loss}) wrt $\theta$;\\
			}
			copy the main network $Q(s,a;\theta)$ to $\hat{Q}(s, a; \theta^-)$;
}}
\end{algorithm}


In our MDP, the state space is a three dimensional continuous one, and thus we adopt the DQN method. Specifically, we use the \emph{deep $Q$ learning with replay memory}~\cite{mnih2015human} for learning the $Q$ functions. This method maintains two neural networks. One is called the \emph{main network} $Q(s,a;\theta)$, which is used to estimate the $Q$ function. The other is called the \emph{target network} $\hat{Q}(s,a;\theta^-)$, which is used to compute some form of loss for training the main network. Besides, it maintains a fixed-size pool called \emph{replay memory}, which contains the latest transitions that are sampled uniformly and used for training the main network. The intuition is to avoid the correlation among consecutive transitions. The detailed procedure of DQN for our MDP is presented in Algorithm~\ref{alg:dqn}, which we go through as follows. We maintain a database $\mathcal{D}$ of data trajectories and a set of $\mathcal{D}_q$ of query trajectories. It first initializes the reply memory $\mathcal{M}$ with some capacity, the main network $Q(s, a; \theta)$ with random weights, and the target network $\hat{Q}(s,a;\theta^-)$ by copying $Q(s,a;\theta)$ (Lines 1 - 3). Then, it involves a sequence of many episodes. For each episode, it samples a data trajectory $T$ from $\mathcal{D}$ and a query trajectory $T_q$ from $\mathcal{D}_q$, both uniformly (Lines 4 - 5). It initializes a variable $h$ such that $p_h$ corresponds to the point following the one, at which the last split operation is performed if any and $p_1$ otherwise (Line 6). It also initializes the state $s_1$ (Lines 7 - 8). Then, it proceeds with $|T|$ time steps. At the $t^{th}$ time step, it scans point $p_t$ and selects an action using the $\epsilon$-greedy strategy based on the main network, i.e., it performs a random action $a_t$ with the probability $\epsilon$ ($0 < \epsilon < 1$) and $a_t = \arg\max_{a}Q(s_t,a;\theta)$ with the probability $(1-\epsilon)$ (Lines 9 - 10).
If $a_t = 1$, it splits the trajectory at point $p_t$ and updates $h$ to be $t+1$ (Lines 11 - 13).
%For both cases of $a_t$, $\Theta_{best}$ to be the best one among the best known similarity and the similarities between the two newly formed subtrajectories and the query trajectory $T_q$, i.e., $\Theta_{best} \leftarrow \max\{s_t.\Theta_{best}, s_t.\Theta_{pre}, s_t.\Theta_{suf}\}$ (Line 14).
%The next state would be to scan the point $p_{t+1}$ and correspondingly it computes the similarities between those subtrajectories that would be formed, and we set a terminate value 0 for $\Theta_{pre}$ and $\Theta_{suf}$ when it scans the last point of $T$ (Lines 15-19).
It then updates $\Theta_{best}$ if possible (Line 14).
If the current point being scanned is the last point $p_n$, it terminates (Lines 15 - 17).
Otherwise, it observes a new state $s_{t+1}$ and the reward $r_t$ (Lines 18 - 20).
It then stores the experience $(s_t, a_t, r_t, s_{t+1})$ in the reply memory, samples a minibatch of experiences, and uses it to perform a gradient descent step for updating $\theta$ wrt a loss function (Lines 21 - 23). The loss function for one experience $(s, a, r, s')$ is as follows.
\begin{equation}
L(\theta) = (y - Q(s, a; \theta))^2
\label{equ:dqn-loss}
\end{equation}
where $y$ is equal to $r$ if $s'$ is a termination step and $r + \gamma\cdot \max_{a'}\hat{Q}(s', a'; \theta^-)$ otherwise.
%
Finally, it updates the target network $\hat{Q}(s, a;\theta^-)$ with the main network $Q(s,a;\theta)$ at the end of each episode (Line 25).
%
A graphical illustration of the method is shown in Figure~\ref{fig:dqn}.

\subsection{Reinforcement Learning based Search Algorithm (RLS)}
\label{subsec:rls}
%Algorithm part;
Once we have estimated the $Q$ functions $Q(s, a; \theta)$ via the deep $Q$ learning with experience replay, we use the policy, which always takes for a given state $s$ the action that maximizes $Q(s,a; \theta)$, for the process of splitting a data trajectory. Among all subtrajectories that are formed as a result of the process, we return the one with the greatest similarity to the query trajectory $T_q$. We call this algorithm \emph{reinforcement learning based search} (RLS). Essentially, it is the same as PSS except that it uses a policy learned via DQN instead of human-crafted heuristics for making decisions on how to split a data trajectory.

%Consider the time complexity of RLS.
%\smallskip\noindent\textbf{Time complexity.}
RLS has the same time complexity as PSS
since
%(1) RLS differs from PSS only in the way of making decisions on whether or not to split on a point; and (2)
both RLS and PSS make decisions based on the similarities of the subtrajectories that are being considered when scanning a point and the best-known similarity:
(1) RLS constructs a state involving them and goes through the main network of DQN with the state information, which is $O(1)$ given that the network is small-size (e.g., a few layers); and
(2) PSS simply conduct some comparisons among the similarities, which is also $O(1)$.
%(2) in RLS, the time cost of making a decision corresponds to that of going through the main network of DQN with some state information, which is $O(1)$ given that the network is small-size (e.g., a few layers); and
%(3) in PSS, the time cost is that of simply conducting two comparisons between the similarities of the subtrajectories that are being considered and that of the most similar subtrajectory found so far, which is clearly $O(1)$.
%but as will be shown empirically, RLS provides consistently better solutions than PSS and other splitting-based algorithms POS and POS-D.
In terms of effectiveness,
RLS provides consistently better solutions than PSS as well as POS and POS-D,
as will be shown in the empirical studies,
and the reason is possibly that RLS is based on a learned policy,
which makes decision more intelligent than simple heuristics that are human-crafted.

\begin{figure}[t]
	\centering
	% Requires \usepackage{graphicx}
	\includegraphics[width=8.5cm]{rlmodel_v5}\\
	%\setlength{\abovecaptionskip}{1pt}
	%\vspace{-2mm}
	\caption{Deep $Q$ learning with experience replay}%\label{rlmodel}
	%\setlength{\belowcaptionskip}{0pt}
	%\vspace{-3mm}
	\label{fig:dqn}
\end{figure}


\subsection{Reinforcement Learning based Search with Skipping (RLS-Skip)}
\label{subsec:rls_skip}

\begin{table*}[htb]
\centering
\scriptsize
\caption{Illustration of RLS-Skip with the DTW distance.}
%\vspace*{-4mm}
\label{table:rls_skip}
\begin{tabular}{|c|c|c|c|c|c|}
\hline
Initial      & \multicolumn{5}{c|}{$h = 1$, $T_{best} = \emptyset$ and  $\Theta_{best}=0$}                                                                       \\ \hline
Point   & State & Action & $h$ & $\Theta_{best}$ & $T_{best}$ \\ \hline
$p_1$           & $s_1=(\Theta_{best}=0, \Theta_{pre=T[1,1]}=0.124, \Theta_{suf=T[1,5]}=0.150)$     & $a_1 = \arg\max_{a}Q(s_1,a;\theta)=1: split$ & $2$ & $0.150$  & $T[1,5]$   \\ \hline
$p_2$           & $s_2=(\Theta_{best}=0.150, \Theta_{pre=T[2,2]}=0.236, \Theta_{suf=T[2,5]}=0.227)$ & $a_2 = \arg\max_{a}Q(s_2,a;\theta)=2: skip$ & $2$ & $0.236$  & $T[2,2]$   \\ \hline
$p_3$ (skipped) & -         & -        & -     & -  & -   \\ \hline
$p_4$           & $s_3=(\Theta_{best}=0.236, \Theta_{pre=T[2,4]}=0.333, \Theta_{suf=T[4,5]}=0.215)$ & $a_3 = \arg\max_{a}Q(s_3,a;\theta)=1: split$ & $5$ & $0.333$  & $T[2,4]$   \\ \hline
$p_5$           & $s_4=(\Theta_{best}=0.333, \Theta_{pre=T[5,5]}=0.152, \Theta_{suf=T[5,5]}=0.152)$ & $a_4 = \arg\max_{a}Q(s_4,a;\theta)=0: no-split$ & $5$ & $0.333$      & $T[2,4]$   \\ \hline
Output      & \multicolumn{5}{c|}{$T_{best} = T[2,4]$ with $\Theta_{best}=0.333$}                                                                       \\ \hline
\end{tabular}
%\vspace*{-2mm}
\end{table*}


In the RLS algorithm, each point is considered as a candidate for performing a split operation. While this helps to attain a reasonably large space of subtrajectories for exploration and hence achieving good effectiveness, it is somehow conservative and incurs some cost of decision marking for \emph{each} point. An alternative is to go a bit more optimistic and \emph{skip} some points from being considered as places for split operations. The benefit would be immediate, i.e., the cost of making decisions at these points is saved. Motivated by this, we propose to augment the MDP that is used by RLS by introducing $k$ more actions (apart from two existing ones: scanning the next point and performing a split operation), namely skipping $1$ point, skipping $2$ points, ..., skipping $k$ points. Here, $k$ is a hyperparameter, and by skipping $j$ points ($j = 1, 2, ..., k$), it means to skip points $p_{i+1}, p_{i+2}, ..., p_{i+j}$ and scan point $p_{i+j+1}$ next, where $p_i$ is the point that is being scanned. All other components of the MDP are kept the same as that for RLS. Note that when $k = 0$, this MDP reduces to the original one for RLS. We call the algorithm based on this augmented MDP \emph{RLS-Skip}.


To illustrate, consider again the example shown in Figure~\ref{fig:input}. Suppose that it has learned a policy using the DQN method, which is captured by the main network $Q(s, a; \theta)$. The process of RLS-Skip is depicted in Table~\ref{table:rls_skip}. Suppose the parameter $k$ is equal to 1, which implies that there are three possible actions 0 (no split), 1 (split), and 2 (no split and skip of 1 point).
%which implies that there are three possible actions: 0 meaning to continue to scan the next point, 1 meaning to perform a split operation, and 2 meaning to skip one point and then scan the point following the last point that has been skipped.
In addition, we write $\Theta_{pre} = \Theta(T[i,j], T_q)$ as $\Theta_{pre=T[i,j]}$ and
$\Theta_{suf} = \Theta(T[i,j], T_q)$ as $\Theta_{suf=T[i,j]}$ for simplicity. At the very beginning, it initializes $h$, $\Theta_{best}$ and $T_{best}$. It then scans point $p_1$, observes the first state $s_1$ as $(\Theta_{best} = 0, \Theta_{pre = T[1,1]} = 0.124, \Theta_{suf=T[1,5]} = 0.150)$ and finds the action $a_1 = \arg\max_{a}Q(s_1,a;\theta) = 1$, meaning to perform a split operation at $p_1$. It then updates $h$, $\Theta_{best}$, and $T_{best}$ as shown in the $3^{rd}$ row of the table. It continues to scan point $p_2$, observes the second state $s_2$ as $(\Theta_{best} = 0.150, \Theta_{pre = T[2,2]} = 0.236, \Theta_{suf=T[2,5]} = 0.227)$ and finds the action $a_2 = \arg\max_{a}Q(s_2,a;\theta) = 2$, meaning to skip the next 1 point, i.e., $p_3$. It keeps $h$ unchanged (since no splits are done) but updates $\Theta_{best}$ and $T_{best}$ to be $0.236$ and $T[2,2]$, respectively, since $T[2,2]$ is the subtrajectory with the largest similarity among all subtrajectories that have been considered. As a result of the skipping, it scans point $p_4$ next and proceeds similarly. It performs a split operation when scanning point $p_4$ and terminates after scanning point $p_5$. At the end, it returns $T[2,4]$, which has the similarity of $0.333$. 
%Note that $T[2,4]$ is the subtrajectory that is the most similar to the query trajectory among all possible subtrajectories.


%Consider the time complexity of RLS-skip.
While the cost of making decisions at those points that are skipped (i.e., that of going through the main network of the DQN) could be saved in RLS-Skip, the cost of constructing the states at those points that are not skipped would be more or less that of constructing the states at \emph{all} points since the state at a point involves some similarities, which are computed incrementally based on the similarities computed at those points before the point. Thus, by applying the skipping strategy alone would not help much in reducing the time cost since the cost of maintaining the states dominates that of making decisions. To fully unleash the power of the skipping strategy, we propose to ignore those points that have been skipped when maintaining the states. That is, to maintain the state $(\Theta_{best}, \Theta_{pre}, \Theta_{suf})$ at a point $p_i$, we compute $\Theta_{best}$ and $\Theta_{suf}$ in the same way as we do in RLS and $\Theta_{pre}$ as the similarity between the query trajectory and the subtrajectory consisting of those points that are before $p_i$ and \emph{have not been skipped}. Here, the prefix subtrajectory corresponds to a \emph{simplification} of that used in RLS~\cite{long2013direction}. While RLS-Skip has the same worse-case time complexity as RLS, e.g., it reduces to RLS when no skipping operations happen, the cost of maintaining the states for RLS-Skip would be much smaller. As shown in our empirical studies, RLS-Skip runs significantly faster than RLS as well as PSS, POS and POS-D.
In addition,
%since RLS-Skip (and RLS) are learning based,
%it is possible that the learned policy corresponds to that of PSS, POS, or POS-D. Therefore, the solution by RLS-Skip (and RLS) could be arbitrarily worse than the best one in the worst case.
RLS-Skip and RLS do not provide theoretical guarantees on the approximation quality due to their learning nature. The proofs can be found in the appendix of the technical report~\cite{TR}. Nevertheless, they work quite well in practice (e.g., RLS has the approximation ratio smaller than 1.1 for all similarity measurements and on all datasets (Figure~\ref{effect_result})). In addition, the problem instances that we constructed for proving the negative results in fact rarely happen in practice, which are confirmed by the effectiveness results on real datasets.



==> v13 - technical/setup.tex <==
\section{EXPERIMENTS}
\label{experiment}

\subsection{Experimental Setup}
\label{exper_setup}
\textbf{Dataset.} Our experiments are conducted on two real-world taxi trajectory datasets. The first dataset is collected from the city of Porto~\footnote{https://www.kaggle.com/c/pkdd-15-predict-taxi-service-trajectory-i/data}, Portugal around 18 months with a sampling interval of 15 seconds. %and each location sampled at 15 second intervals.
After filtering the trajectories with fewer than 30 sampling points, we obtain 1.2 million trajectories with a mean length around 60. The second dataset consists of trajectories collected from 13,000 taxis over 8 months in Harbin, China with non-uniform sampling rates. After removing the trajectories with fewer than 30 points, we get over 1 million trajectories with a mean length around 120.

\noindent\textbf{Parameter Setting.} For training t2vec model, we follow the original paper~\cite{li2018deep} for  parameter setting. We use a forward neural network with 2-layers to record Q-values in our RLS model. In the training process, the size of replay memory $\mathcal{M}$ is set at 2000. We train our model on 25k random trajectory pairs, using Adam stochastic gradient descent with an initial learning rate of 0.01. The minimal $\epsilon$ is set at 0.1 with decay 0.99 for $\epsilon$-greedy strategy, and the reward discount rate $\gamma$ is set at 0.95.

\noindent\textbf{Compared Methods.} We compare RL-based Search (RLS) and the proposed non-learning based algorithms (Section~\ref{sec:non-learning}), namely ExactS, SizeS, PSS, POS, and POS-D.
%Note that for DTW and Frechet distance we  modify GA by reading suffix trajectories from right to left, and thus do not need the BSS method. {\bf Gao not clear.. BCC is the same as GA for DTW?}
%
%In addition, inspired by the algorithms for approximate matching for substring and subsequence~\cite{kim2013efficient,zhang2010bed,gong2019fast,rakthanmanon2013addressing,rakthanmanon2012searching,athitsos2008approximate,han2007ranked,moon2001duality,faloutsos1994fast}, we further propose a baseline, called Fixed-Length Search (FLS) with soft margin $\xi$. Specifically, we search the subtrajectories with lengths from $|Q|-\xi$ to $|Q|+\xi$ in the candidate trajectory $C$, where $|Q|$ denotes the length of query trajectory and $\xi\in[0,|Q|)$. In case the fixed search lengths exceed the length of candidate trajectory $C$, we further limit the search bound from $min(|Q|-\xi,|C|)$ to $min(|Q|+\xi,|C|)$. Note that the result will get better as $\xi$ gets larger although the time cost will increase, and in extreme cases it may return the same result as the exact algorithm.
%
The default value of $\xi$ in PSS is set at 5 and we will report the effect of the parameter $\xi$ in our experiments.
For POS-D, we vary the delay positions $K$  from 4 to 7, and the results are similar. We set $K$ at 5 in our experiments. For RLS, when t2vec is adopted, we ignored the $\Theta_{suf}$ component of a state based on empirical findings.

\noindent\textbf{Evaluation Metrics.} We use three metrics to evaluate the effectiveness of the approximate algorithms using the results of the exact algorithm as the ground truth. (1) Approximate Ratio (AR). AR for the subtrajectory similarity computation is defined as $\frac{\Psi_{app}}{\Psi_{opt}}$, where $\Psi_{app}$ is the dissimilarity value returned by one of the approximate algorithms (e.g., SizeS, PSS, POS, POS-D, and RLS), and $\Psi_{opt}$ is the dissimilarity value of the exact algorithm.
%AR measures the performance of an online algorithm by the distance between the optimal solution, and thus
A smaller AR value indicates a better algorithm.
(2) Mean Rank (MR). %MR is a rank-based metric. Consider a trajectory pair $(C, Q)$,
We sort all the subtrajectories of the given candidate trajectory $C$ in ascending order of their dissimilarity values with query $Q$. %obtained by the exact algorithm, and
We denote by $rank_{C}(C_{\Lambda})$  the rank of the returned subtrajectory $C_{\Lambda}$ for a query trajectory $Q$ by an algorithm. We report the mean number of $rank_{C}(C_{\Lambda})$ as MR.
(3) Relative Rank (RR). %For the candidate trajectories $C$ with different lengths,
As the number of subtrajectories of a candidate trajectory $C$ varies a lot, we normalize the rank by the number of subtrajectories, i.e., $\frac{rank_{C}(C_{\Lambda})}{\#subt_{C}}$, where $\#subt_{C} = \frac{|C|(|C|+1)}{2}$. We call the matric by Relative Rank (RR).
Smaller MR or RR value indicates a better algorithm.

%is also different. Here, we denote the RR as the mean number of $\frac{rank_{C}(C_{\Lambda})}{\#subt_{C}}$, where $\#subt_{C}$ is the total number of subtrajectories of $C$, if the length of $C$ is $n$,  $\#subt_{C} = \frac{n(n+1)}{2}$.


\noindent\textbf{Evaluation Platform.} All the methods are implemented in Python 3.6. The implementation of RLS is based on Keras 2.2.0. The experiments are conducted on a server with 32-cores of Intel(R) Xeon(R) Gold 6150 CPU @ 2.70GHz 768.00GB RAM and one Nvidia Tesla V100-SXM2 GPU.


==> v13 - technical/theory.tex <==

\newpage
{\color{red}
\section{Quality Analysis of the SizeS Algorithm}
\label{sec:sizes-proof}
There usually exists a space, within which the objects move. Therefore, we assume the points of trajectories are all located in a $d_{max} \times d_{max}$ rectangle, where $d_{max}$ is a large number that captures the extent of the space. We use a coordinate system whose origin is at the middle of this rectangle.
%

\smallskip\noindent\textbf{Case 1: DTW.}
Consider a problem input with a query trajectory with $m$ points $T_q = <p_1', p_2', ..., p_m'>$ and a data trajectory with $n = m^2$ points $T = <p_{1,1}, p_{1,2}, ..., p_{1,m}, p_{2,1}, p_{2,2}, ..., p_{2,m}, ..., p_{m,1}, p_{m,2}, p_{m,m}>$. We assume that $m$ is an even number and $l = m / 2$. In addition, we let $d = d_{max} / m$.
The locations of the points in these trajectories are provided as follows.
\begin{itemize}
	\item $p_i' = ( - ( l - i + 1/2) \cdot d, 0)$ for $i = 1, 2, ..., l$;
	\item $p_i' = ( (i - l - 1/2) \cdot d, 0)$ for $i = l+1, l+2, ..., m$;
	\item $p_{i,j}$'s ($1\le j \le m$) are evenly located at the circle with its center at $p_i'$ and its radius equal to $\epsilon$, where $\epsilon$ is a very small real number for $i = 1, 2, ..., m$;
\end{itemize}

Consider the optimal solution. Its DTW distance, denoted by $D_o$, is at most the distance between $T$ and $T_q$, which is equal to $m^2\cdot \epsilon$ (points $p_{i,j}$ for $1\le j\le m$ are aligned with point $p_i'$ for $1\le i\le m$). That is, we have $D_o \le m^2 \cdot \epsilon$.

Consider the approximate solution returned by SizeS.  Suppose that $\xi = 0$. That is, we only consider subtrajectories with the length exactly equal to $m$. We further know that each such sub-trajectory consists of points, either all located at a circle with the center at one of the point of $T_q$ or some located at a circle with the center at a point $p_i'$ and others located at a circle with the center at a point $p_{i+1}'$ ($1\le i < m$). It could be verified that among these subtrajectories, the one with some located at the circle with the center at $p_l'$ and others at $p_{l+1}'$ has the smallest DTW distance from $T_q$ and would be returned. We denote its DTW distance to $T_q$ by $D_a$. It could be verified that $D_a > 2\times (\Sigma_{i=1}^{l-1} ((l-i)\cdot d - \epsilon) + \epsilon)$, where the lower bound of the Euclidean distance from a point of $T_q$ to its aligned point of the returned subtrajectory is (1) $((l-i)\cdot d - \epsilon)$ for $1\le i\le l-1$ and (2) $\epsilon$ for $i = l$; and (3) that of the point symmetric to $p_i'$ (w.r.t. the origin) for $l+1\le i\le m$ due to the symmetry. Therefore, we have
\begin{align*}
\frac{D_a}{D_o} 
& \ge \frac{2\times (\Sigma_{i=1}^{l-1} ((l-i)\cdot d - \epsilon) + \epsilon)}{m^2 \cdot \epsilon}\\
& = \frac{m^2/4\cdot d - m/2\cdot d - m\cdot \epsilon + 4\cdot\epsilon}{m^2\cdot \epsilon} \\
&= \frac{1/4\cdot d - 1/(2m)\cdot d - \epsilon/m + 4/m^2\cdot \epsilon}{\epsilon}
\end{align*}
which approaches infinity when m approaches infinity and $\epsilon$ approaches 0.
In summary, the solution returned by SizeS could be arbitrarily worse than the optimal one when DTW distance is used.

\smallskip\noindent\textbf{Case 2: Frechet and t2vec.}
Consider the case when Frechet distance is used. The optimal solution and the approximate solution returned would be the sames as the case when DTW distance is used, but the distances would be different. $D_o$ would be equal to $\epsilon$ and $D_a$ would be at least $((l-1)\cdot d - \epsilon)$. Therefore, we have
$$
\frac{D_a}{D_o} \ge \frac{(l-1)\cdot d - \epsilon}{\epsilon}
$$
which approaches infinity when $\epsilon$ approaches 0.

Consider the case when t2vec is used. Since it is a learning-based distance - in theory, it may reduce to any possible distance metric such as DTW and Frechet. Thus, the analysis for DTW or Frechet could be carried over for t2vec.

\if 0
We provide a theoretical guarantee on the rank for SizeS algorithm. SizeS enumerates all subtrajectories with the sizes within the range $[m-\xi, m+\xi]$, where $m$ is the length of query trajectory and $\xi$ is a controllable parameter. During the search process, we know SizeS will traverse $(n-m+1)(2\xi+1)$ subtrajectories and return the best one among them. We can safely assume the worst case is the subtrajectories tried by SizeS are the worst (i.e., smallest similarity) in all $\frac{n(n+1)}{2}$ subtrajectories in $T$. Thus, the rank is bounded by $\frac{n(n+1)}{2}-(n-m+1)(2\xi+1)+1$. The tightness of the bound is controllable by the parameter $\xi$.
\fi


\section{Quality Analysis of Spliting-based Algorithms}
\label{sec:splitting-proof}

\smallskip\noindent\textbf{Case 1: PSS with DTW.}
Consider a problem input with a data trajectory with $n+3$ points $T=<p_1', p_2', p_1, p_2, ..., p_n, p_3'>$ ($n$ is a positive integer) and a query trajectory $T_q = <p'>$. Let $d = d_{max}/2$. The locations of the points in these trajectories are provided as follows.
\begin{itemize}
	\item $p_1' = (-d/2, 0)$, $p_2' = (-d, 0)$;
	\item $p_i = (0, 0)$ for $i = 1, 2, ..., n$;
	\item $p_3' = (d, 0)$;
	\item $p' = (0, \epsilon)$, where $\epsilon$ is a very small non-negative real number;
\end{itemize}

Consider the optimal solution. It could be any subtrajectory $<p_i>$ ($1\le i \le n$) and the corresponding DTW distance is equal to $\epsilon$, which we denote by $D_o$.

Consider the approximate solution returned by PSS. It is the subtrajectory $<p_1'>$, which is explained as follows. When it scans the first point $p_1'$, it would split the trajectory at $p_1'$ and update the best-known subtrajectory to be $<p_1'>$ with the DTW distance equal to $\sqrt{d^2/4 + \epsilon^2}$. It then continues to scan the following points $p_2', p_1, ..., p_n, p_3'$ and would not perform any split operations at these points due to the fact that $p_2'$ and $p_3'$ are farther away from $p'$ than $p_1'$. As a result, $<p_1'>$ would be returned as a solution. We denote the DTW distance of this solution by $D_a$, i.e., $D_a = \sqrt{d^2/4 + \epsilon^2}$.

Consider the approximation ratio (AR). We have 
$$
\frac{D_a}{D_o} = \frac{\sqrt{d^2/4 + \epsilon^2}}{\epsilon} > \frac{d/2}{\epsilon}
$$
which approaches infinity when $\epsilon$ approaches zero.

Consider the mean rank (MR). We know that the rank of the approximate solution $<p_1'>$ is at least $\frac{n(n+1)}{2}+1$ since any subtrajectory of $<p_1, p_2, ..., p_n>$ has a smaller DTW distance than $<p_1'>$ (assuming $\epsilon = 0$). Therefore, the mean rank would approach infinity when $n$ approaches infinity.

Consider the relative rank (RR). Based on the analysis of mean rank, we know that the relative rank of the approximate solution $<p_1'>$ is at least $\frac{\frac{n(n+1)}{2}+1}{\frac{(n+3)(n+4)}{2}}$, which approaches 1 when $n$ approaches infinity.

In conclusion, the solution returned by PSS could be arbitrarily worse than the optimal one in terms of AR, MR, and RR, when the DTW distance is used.

\smallskip\noindent\textbf{Case 2: Other Algorithms and Similarity Measurements}
Consider the other algorithms, i.e., POS and POS-D. It could be verified that they would run exactly in the same way as PSS on the problem input provided in the Case 1. Therefore, the conclusion would be carried over. Consider the other measurements, namely, Frechet and t2vec. For Frechet, it could be verified that the optimal solution and the approximate solution returned by the algorithms are the same as those in the Case 1 and their Frechet distances and DTW distances to $T_q$ are equal since both solutions and $T_q$ involve one single point. As a result, the conclusion for DTW distance could be carried over for Frechet distance. For t2vec, since it is a learning-based distance - in theory, it may reduce to any possible distance metric such as DTW and Frechet. Thus, the analysis for DTW in the Case 1 could be carried over for t2vec.

}

\if 0
\section*{B. Arbitrary worse for splitting-based algorithms (PSS, POS and POS-D)}
\label{splitting-proof}
We prove the splitting-based algorithms are arbitrary worse by constructing the following cases for the approximation ratio and rank, respectively.
\subsection*{B.1 Approximation ratio analysis}
We consider two adjacent positions in a trajectory are bounded by a distance $d_{bound}$ and construct the case as follows:
\begin{equation*}
  \begin{aligned}
    &T=<p_1,p_2,\underbrace{...}_{k \text{ points}},p_*,\underbrace{...}_{k \text{ points}},p_n>, \text{and } T_q=<p_*>,
  \end{aligned}
\end{equation*}
where we instantiate the similarity with trajectory distance (e.g., DTW or Frechet by default) denoted by $D(\cdot,\cdot)$ and $dist(\cdot,\cdot)$ denotes the distance between the points (typically the Euclidean distance). Let $D(<p_1>, T_q) = d_1$, $dist(p_2, p_*) = d_2$ and $dist(p_n, p_*) = d_3$, we construct $d_1 < d_2$ and $d_1 < d_3$ and then we prove it is arbitrary worse for approximation ratio under the construction.

Run the splitting-based algorithms (PSS, POS and POS-D), we find a splitting is happened on $p_1$ due to the initial condition of these algorithms. Then, we choose to maintain the subtrajectory $<p_1>$ with the distance $d_1$ because it is smaller. We continue to scan the trajectory $T$, and we find no splitting will happen because we cannot find a smaller distance than $d_1$ from prefix $<p_2,...,p_i>$ and suffix $<p_i,...,p_n>$ for $2\leq i \leq n$ due to the boundary condition (recall the distance definition) of DTW or Frechet. Finally, these algorithms output subtrajectory $<p_1>$ with distance $d_1$ as results. Under the construction $d_1<d_2$, we can let the three points $p_1$, $p_2$ and $p_*$ form a triangle. Then, we have
\begin{equation*}
  \begin{aligned}
    &dist(p_1,p_*)+dist(p_1,p_2)>dist(p_2, p_*)\\
    &d_1>d_2-dist(p_1,p_2)>d_2-d_{bound}\\
  \end{aligned}
\end{equation*}
We know there is $k$ points between $p_2$ and $p_*$. we may assume $d_2=(k+1)*d_{bound}$, i.e., these points are collinear with the adjacent distance $d_{bound}$. Then, we further have
\begin{equation*}
  \begin{aligned}
    &d_1>(k+1)*d_{bound}-d_{bound}=k*d_{bound}\\
  \end{aligned}
\end{equation*}
We know $d_1$ increases as $k$ increases; however, the distance for the optimal solution is 0 because $T_q=<p_*>$ is a portion of $T$. Thus, the difference between the optimal distance and the approximate distance approaches arbitrary worse.

\subsection*{B.2 Rank analysis}
\label{splitting-proof-rank}
We construct the following case for rank analysis.
\begin{equation*}
  \begin{aligned}
    &T=<p_1,p_2,\underbrace{p_*,...,p_*}_{k \text{ points}},p_n>, \text{and } T_q=<p_*>.
  \end{aligned}
\end{equation*}
Here, we assume an object stays at position $p_*$ and GPS collects $k$ same points $p_*$ in the trajectory $T$. Similarly, we let $D(<p_1>, T_q) = d_1$, $dist(p_2, p_*) = d_2$ and $dist(p_n, p_*) = d_3$ and construct $d_1 < d_2$, $d_1 < d_3$. Based on the above analysis, we know splitting-based algorithms return the subtrajectory $<p_1>$ with the distance $d_1$, and there are $\frac{k(k+1)}{2}$ subtrajectories formed by the $k$ points with trajectory distance 0. Thus, the rank for these splitting-based algorithms is larger than $\frac{k(k+1)}{2}$ at least, and it increases as $k$ increases. The rank is also arbitrary worse.

\section*{C. Arbitrary worse for learning-based algorithms (RLS, RLS-Skip)}
We proof learning-based algorithms (RLS, RLS-Skip) is also arbitrary worse based on approximation ratio and rank analysis, respectively.
\subsection*{C.1 Approximation ratio analysis}
We construct the following case:
\begin{equation*}
  \begin{aligned}
    T=<p_1,\underbrace{...}_{k \text{ points}},p_*,\underbrace{...}_{k \text{ points}},p_n>, \text{and } T_q=<p_*>,
  \end{aligned}
\end{equation*}
We use the same notations as defined in the proof above. Let $dist(p_1, p_*) = d_1$ and $dist(p_n, p_*) = d_2$. We know learning-based algorithms can output arbitrary actions because it is a data-driven method. We consider the case of all actions are 0, which means no splitting will be happened during the MDP, and it will try $2*n$ subtrajectories that is prefix $<p_1, ... , p_i>$ and suffix $<p_i, ... , p_n>$ for $1 \leq i\leq n$. Similarly, we instantiate the trajectory similarity by DTW or Frechet distance, and we discuss the following two situations:
\begin{enumerate}
  \item If the returned subtrajectory from prefix $<p_1,..., p_i>$, we know $D(<p_1,..., p_i>, T_q) \geq dist(p_1, p_*)=d_1$ by DTW or Frechet definition. We know there are $k$ points between $p_1$ and $p_*$. We may assume $d_1 = (k + 1)*d_{bound}$ by constructing these points collinear with the adjacent distance $d_{bound}$. Then, $d_1$ will increase as $k$ increases; however, the distance outputted by the optimal solution is 0. Thus, the proof holds based on prefix analysis.
  \item Similarly, if the returned subtrajectory from suffix $<p_i,...,p_n>$, we know $D(<p_i,..., p_n>, T_q) \geq dist(p_n, p_*)=d_2$, and we can let the points between $p_*$ and $p_n$ collinear with the adjacent distance $d_{bound}$. Then, $d_2 = (k + 1)*d_{bound}$, and the distance difference between the optimal and the approximate is also arbitrary worse as $k$ increases.
\end{enumerate}
\subsection*{C.2 Rank analysis}
Similar to rank analysis above. We construct the following case and let all actions are 0 outputted by learning-based algorithms.
\begin{equation*}
  \begin{aligned}
    &T=<p_1,\underbrace{p_*,...,p_*}_{k \text{ points}},p_n>, \text{and } T_q=<p_*>.
  \end{aligned}
\end{equation*}
We know there are $\frac{k(k+1)}{2}$ subtrajectories formed by the $k$ same points $p_*$ with the trajectory distance 0. However, the returned distance of learning-based algorithms is either larger than $d_1$ or $d_2$ outputted by prefix or suffix, respectively. Thus, the rank of learning-based algorithms is larger than $\frac{k(k+1)}{2}$ at least, and it increases as $k$ increases. The proof for arbitrary worse based on rank holds.
\fi
